First Approximation for Uniform Lower and Upper Bounded Facility Location Problem avoiding violation in Lower Bounds

With growing emphasis on e-commerce marketplace platforms where we have a central platform mediating between the seller and the buyer, it becomes important to keep a check on the availability and profitability of the central store. A store serving too less clients can be non-profitable and a store getting too many orders can lead to bad service to the customers which can be detrimental for the business. In this paper, we study the facility location problem(FL) with upper and lower bounds on the number of clients an open facility serves. Constant factor approximations are known for the restricted variants of the problem with only the upper bounds or only the lower bounds. The only work that deals with bounds on both the sides violates both the bounds [8]. In this paper, we present the first (constant factor) approximation for the problem violating the upper bound by a factor of (5/2) without violating the lower bounds when both the lower and the upper bounds are uniform. We first give a tri-criteria (constant factor) approximation violating both the upper and the lower bounds and then get rid of violation in lower bounds by transforming the problem instance to an instance of capacitated facility location problem.

==> CopyofLBUBFLGeneralTree.tex <==
\section{Instance $I_1$ and $I_2$}
\label{instI1}

In this section, we first transform instance $I$ to instance $I_1$ ($\facilityset,~\clientset,~f^1,~c,~\B,~\capacityU$) of LBUBFL by moving the clients to the facilities serving them in the tri-criteria solution $S^t$ and then transform $I_1$ to an instance $I_2$ of LBFL by removing the facilities not opened in $S^t$.
%Let $\facilityset^t$ be the set of facilities opened by $S^t$. 
Recall that for a client $j$,  $\sigma^t(j)$ is the facility  in $\facilityset^t$ serving $j$. For $i \in \facilityset^t$, let $n_i$ be the number of clients served by $i$ in $S^t$, i.e., $n_i = |(\sigma^t)^{-1}(i)|$ and for $i \notin \facilityset^t$, $n_i = 0$. Move these clients to $i$ (see Fig.~\ref{Mapping1}). Thus, there are $n_i$ clients co-located with $i$. In $I_1$, our facility set is $\facilityset$ and the clients are at their new locations. Facility opening costs in $I_1$ are modified as follows: $f^1_i = 0$ for $i \in \facilityset^t$ and $=f_i$ for $i \notin \facilityset^t$.  


\begin{lemma}
Cost of optimal solution of $I_1$ is bounded by $Cost_I(S^t) + Cost_I(O)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_1$ of $I_1$: open $i$ in $S_1$ iff it is opened in $O$. Assign $j$ to $i$ in $S_1$ iff it is assigned to $i$ in $O$. $S_1$ satisfies both the lower bound as well as the upper bound as $O$ does so. For a client $j$, let $\sigma^*(j)$ be the facility serving $j$ in $O$. Then, the cost $\dist{ \sigma^t(j)}{\sigma^*(j))}$ of serving $j$ from its new location, $\sigma^t(j)$ is bounded by $\dist{j}{\sigma^t(j)} +\dist{j}{\sigma^*(j)}$ (see Fig. \ref{lemma1}). Summing over all $j \in \clientset$ and adding the facility opening costs, we get the desired claim.

\begin{figure}[t]
    \centering
    \includegraphics[width=4cm]{Figures/lemma 1.jpg}
    \caption{$c( \sigma^t(j), \sigma^*(j)) \leq c(j, \sigma^t(j)) + c(j, \sigma^*(j))$ }
    \label{lemma1}
\end{figure}
\end{proof}

\begin{figure}[t]
    \centering
    \includegraphics[width=9cm]{Figures/Mapping_0.jpg}
    \caption{Transforming instance $I$ to $I_1$ and  $I_1$ to $I_2$. Solid squares represent clients and circles represent facilities. Clients are moved to the facilities serving them in $S^t$ while transforming $I$ to $I_1$. Facilities not opened in $S^t$ are dropped while going from $I_1$ to $I_2$.}
    \label{Mapping1}
\end{figure} 

%section{Instance $I_2$} 
%\label{instI2}
    
   Next, we define an instance ~$I_2(\facilityset^t,~\clientset,~f^2,~c,~\B)$ of LBFL from $I_1$ by removing the facilities not in $\facilityset^t$ and ignoring the upper bounds. Instance $I_2$ is same as $I_1$ without the upper bounds, except that the facility set is $\facilityset^t$ now. Thus, $f^2_i = 0~\forall~i \in \facilityset^t$. % We will show that there exists a feasible solution $S_2$ of $I_2$ such that $Cost(S_2)$ is bounded by $2 Cost(O_1)$ where
  Let $O_1$ be an optimal solution of $I_1$. 
  For a client $j$, let $\sigma^1(j)$ be the facility serving $j$ in $O_1$.
 
 
 

\begin{lemma}
Cost of optimal solution of $I_2$ is bounded by $ 2Cost_{I_1}(O_1)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_2$ to $I_2$: for $i \in \facilityset^t$, open $i$ in $S_2$ if it is opened in $O_1$ and assign a client $j$ to it if it is assigned to $i$ in $O_1$. For a facility $i \notin \facilityset^t$, %the clients assigned to it need to be assigned to some other facility in $\facilityset^t$. Thus, for such $i$'s,
open its nearest facility $i'$ \textcolor{olive}{(if not already opened)} in $\facilityset^t$. Assign $j$ to $i'$ in $S_2$ if it is assigned to $i$ in $O_1$. $S_2$ satisfies the lower bound  as $O_1$ does so. Note that it need not satisfy the upper bounds. This is the reason we dropped upper bounds in $I_2$. The cost $c( \sigma^t(j), i')$
%$c( \sigma^t(j), \sigma^*(j))$ 
of serving $j$ from its new location is bounded by $c(\sigma^t(j), \sigma^1(j)) + c( \sigma^1(j), i') \le 2 c(\sigma^t(j), \sigma^1(j))$ (since $i'$ is closest in $\facilityset^t$ to $i =  \sigma^1(j)$). Summing over all $j \in \clientset$ we get the desired claim.
%$c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(i, \sigma^1(j)) \le c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(\sigma^t(j), \sigma^1(j))$ (since $i$ is closest in $\facilityset^t$, to $i' = \sigma^1(j)$) $\le 2(c(j, \sigma^t(j)) + c(j, \sigma^1(j)))$ (See Figure 1). Summing over all $j$'s, the claim follows.
%Same as Zoya etal
\end{proof}

%\textcolor{blue}{can be deleted now...I have added a line in the proof itself....Note that, while defining the instance $I_2$, we ignored the upper bounds on facilities because a facility $i' \in \facilityset^t$ might be nearest to many other facilities $\notin \facilityset^t$ thereby serving clients of all of them and hence violating upper bound.}


\section{Instance $I_{cap}$ of Capacitated Facility Location Problem}
\label{instIcap}

 
 In this section, we create an  instance $I_{cap}$ of capacitated facility location problem from $I_2$. 
 The main idea is to create  a demand of $\B - n_i$ units at locations where the number of clients served by the facility is less than $\B$ and a supply of $n_i - \B$ units at locations with surplus clients. For each facility $i \in \facilityset^t$, let $l(i)$ be the distance of $i$ from a nearest facility  $i' \in \facilityset^t$, $i' \neq i$ and let $\delta$ be a constant to be chosen appropriately. A facility $i$ is called {\em small} if $0< n_i \leq \B$ and  {\em big} otherwise. A big facility $i$ is split into two co-located facilities $i_1$ and $i_2$.
  We also split the set of clients at $i$ into two sets:  arbitrarily, $\B$ of these clients are placed at $i_1$ and the remaining $n_i - \B$ clients at $i_2$ (see Fig.~\ref{Mapping2}). 
   Instance $I_{cap}$ is then defined as follows:
A {\em small} facility $i$ needs additional $\B - n_{i}$ clients to satisfy its lower bound; hence a demand of $\B - n_{i}$ is created at $i$ in the $I_{cap}$ instance. A facility with capacity $\B$ and facility opening cost $\delta n_{i} l(i)$ is also created at $i$. 
For a {\em big} facility $i$, correspondingly two co-located facilities $i_1$ and $i_2$ are created with capacities $\B$ and $n_i - \B$ respectively. The facility opening cost of $i_1$ is $\delta \B l(i)$ whereas $i_2$ is free. Intuitively, since the lower bound of a big facility is satisfied, it has some extra ($n_i - \B$) clients, which can be used to satisfy the demand of clients in $I_{cap}$ for free. 
 %Thus, we define capacity of $i_1$ and $i_2$ to be $\B$ and $n_i - \B$ respectively. 
 The second type of big facilities are called {\em free}. 
 %The facility costs, capacities and demands are as shown in
 We use $i$ to refer to both the client (with demand) as well as the facility located at $i$. Let $\bar \facilityset^t$ be the set of facilities so obtained. The set of clients and the set of facilities are both $\bar \facilityset^t$. Table~\ref{tab:my_label} summarizes the instance. Also see Fig.~\ref{Mapping2}
 
 \begin{figure}
    \centering
    \includegraphics[width=8cm]{Figures/Mapping_1.jpg}
    \caption{Transforming instance $I_2$ to $I_{cap}$: $\B = 4$,
    %Solid squares represent clients and circles represent facilities. 
    $i'$ is small, $i$ is big.
    $i$ is split into $i_1$ and $i_2$ while transforming $I_2$ to $I_{cap}$, $i_2$ is free. Demand at the small facility $i'$ is $\B - n_{i'} = 1$ and at $i_1$, $i_2$, it is $0$. Capacities of $i'$ and $i_1$ are $\B = 4$ and it is $n_{i} - \B = 3$ of the free facility $i_2$.}
    \label{Mapping2}
\end{figure}
 
 \begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
       Type & $n_i$ & $u_i$ & $d_i$ & $f^t_i$ \\
        \hline
       {\em small} & $n_i \leq \B$ & $\B$ & $\B- n_i$& $\delta n_i l(i)$ \\
        \hline
       {\em big} & $n_i > \B$ & ($i_1$)$\B$ & $0$& $\delta \B l(i)$ \\
        & & ($i_2$) $n_i - \B$ & $0$& $0$ \\
       
        % &  &
          \hline 
       % $3$ & $0$ & $\B$ & $\B$& $\delta \B l(i)$ \\
        %\hline
    \end{tabular}
    \caption{Instance of $I_{cap}$: $d_i, u_i, f^t_i$ are demands, capacities and facility costs resp.}
    \label{tab:my_label}
\end{table}
 
 %Let $O_{cap}$ be an optimal solution to $I_{cap}$.
 
 %\textcolor{red}{define delta and l(i)}
 %The second type of big facilities are called {\em free}. %and the clients placed at them are also called {\em free}. 
 %Let $F_f$ denote the set of free facilities. 
 %and $Cf(i)$ denote the set of free clients at facility $i \in F_b$. i.e.$Cf(i)$ is the set of clients placed at $i_2 \in F_f$ (See Figure 2)....need to define $l(i)$.

 %In the next lemma, we show the existence of a feasible solution to $I_{cap}$ with cost no more than $(1+2\delta)Cost(O_2)$ where $O_2$ is an optimal solution of $I_2$. 




\begin{lemma}
%A feasible solution $S_{cap}$ for 
Let $O_2$ be an optimal solution of $I_2$. Then, cost of optimal solution to $I_{cap}$ is bounded by $(1+2\delta)Cost_{I_2}(O_2)$.
\end{lemma}

\begin{proof}
We will construct a feasible solution $S_{cap}$ to $I_{cap}$ of bounded cost from $O_2$.
 As $O_2$ satisfies the lower bound,  we can assume wlog that if $i$ is opened in $O_2$ then it serves all of its clients if $n_i \le \B$ (before taking more clients from outside) and it serves at least $\B$ of its clients before sending out its clients to other (small) facilities otherwise. 
Also, if two big facilities are opened in $O_2$, one does not serve the clients of the other. Let $\rho^2(j_i, i')$ denote the number of clients co-located at $i$ and assigned to $i'$ in $O_2$ and $\rho^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $S_{cap}$.
 \begin{figure}[t]
    \centering
    \includegraphics[width=10cm]{Figures/O2_Scap_assignments.jpg}
    \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ and $i'$ are closed in $O_2$. $\rho^2(j_{i_1}, t_1) = 2,~\rho^2(j_{i_1}, t_2) = 1,~\rho^2(j_{i_1}, t_3) = 1,~ \rho^2(j_{i_1}, t_4) = 0$ and $\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 1,~\rho^2(j_{i_2}, t_3) = 1,~ \rho^2(j_{i_2}, t_4) = 0$.  } %The middle figure shows how the assignments look like after splitting the big facilities. $\rho^2(j_{i_1}, i') = 2(/1/1)$ for $i'$ = top three facilities $t_1(/t_2/t_3)$ $\rho^2(j_{i_2}, i') = 1(/1/1) $ for the bottom three facilities $t_2(/t_3/t_4)$. Note that $t_1$ }
    \label{Mapping}
\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{Figures/O2_Scap assignments (2.1).jpg}
   \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ is open in $O_2$.   $\rho^c(j_{t_1}, i_2) = \rho^2(j_{i}, t_1) = 1, \rho^c(j_{t_2}, i_2) = \rho^2(j_{i}, t_2) = 2$,
  % $\rho^2(j_{i_1}, t_1) = 1,~\rho^2(j_{i_1}, t_2) = 1$ and %$\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 2$. 
   $i_2$ is open in $S_{cap}$. $t_1$ and $t_2$ must be small.}
    \label{O2_SCap2}
\end{figure}
    \begin{enumerate}
        \item   if $i$ is closed in $O_2$ then open $i$ if $i$ is small
        and open $(i_1 \& i_2)$ if it is big.
        
        Assignments are defined as follows (see Fig.~\ref{Mapping}):
        \begin{enumerate}
        
        \item If $i$ is small: Let $i$ serve its own demand. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. 
        \textcolor{green}{
        Note that the same cannot be done when $i'$ is big as there is no demand at $i'_1$ and $i'_2$. } Thus,  $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $ i' \ne i$ and $\rho^c(j_i, i) = d_i$. Also, $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). 
        Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = \B = u_i$. 
      
       % \item If $i$ is small: Let $i$ serve its own demand, \textcolor{blue}{i.e., $\rho^c(j_i, i) = d_i$}. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. \textcolor{blue}{Note that $i'$ must be small in this case. But y not big?????? I think it can be big as well, the only thing that will differ is $\rho^c(j_{i'}, i) = 0$ if $i'$ is big.} Thus, $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $i' \ne i$. Also, $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = \B = u_i$. \textcolor{blue}{Thus capacities are respected.}
        
       \item If $i$ is big: assign $\rho^2(j_{i_1}, i')$ (/$\rho^2(j_{i_2}, i')$) demand of $i'$ to $i_1$(/$i_2$) in our solution for small $i' \ne i$. Thus,
        $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_1) = \sum_{small~i' \ne i} \rho^2(j_{i_1}, i') \le \B = u_{i_1}$. Also,
         $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_2) \\ = \sum_{small~i' \ne i} \rho^2(j_{i_2}, i') \le n_i - \B = u_{i_2}$.
       %The second equality holds in each case as $i$ is closed in $O_2$.
        %\textcolor{green}{.....Is this the reason? Sapna...Pls see..}
        % Since there are no demands at $i_1$ and $i_2$, the capacities are respected.
     
       \end{enumerate}
     
     \item If $i$ is opened in $O_2$ and is big, open the free facility $i_2$ (see Fig.~\ref{O2_SCap2}): assign $\rho^2(j_{i}, i')$  demand of $i'$ to $i_2$ in our solution for small $i' \ne i$. Thus,
     %Thus,
      %  $\sigma^c(j_{i'}, i_2) = %\sigma^1(j_{i_2}, i'), i \ne i'$  
        $\sum_{i' \ne i}\rho^c(j_{i'}, i_2) = \sum_{i' \ne i} \rho^2(j_{i}, i') \le n_i - \B$ (the inequality holds by assumption on $O_2$) $= u_{i_2}$.
       % Thus the capacities are respected as there are no demands at $i_2$.
    \end{enumerate}
    
    Thus capacities are respected in each of the above cases. Next, we show that all the demands are satisfied. If a facility is opened in $S_{cap}$, it satisfies its own demand. 
Let $i$ be closed in $S_{cap}$. If $i$ is big ,we need not worry as $i_1$ and $i_2$ have no demand. So, let $i$ is small. Then, it must be opened in $O_2$. Then, 
$\sum_{i' \ne i}\rho^c(j_{i}, i') = $
$\sum_{small ~i' \ne i,  }\rho^c(j_{i}, i') + \sum_{i'_1: i' ~is ~big}\rho^c(j_{i}, i'_1) + 
\sum_{i'_2: i' ~is ~big}\rho^c(j_{i}, i'_2)= $
$\sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i'_1 : i' ~is ~big} \rho^2(j_{i'_1}, i)  + \\ \sum_{i'_2 : i' ~is ~big}\rho^2(j_{i'_2}, i)= \sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i' ~is ~big} \rho^2(j_{i'}, i) = \sum_{i' \ne i}\rho^2(j_{i'}, i)$
$\ge \B - n_i$  (since $O_2$ is a feasible solution of $I_2$) $= d_i$. 



Next, we bound the cost of the solution. The connection cost is \textcolor{olive}{at most that of $O_2$. } %same as 
\textcolor{green}{ or at most? we didn't bring back if anything went from i to i' in O2 where i' is big.}
%Next, we consider the facility opening costs. 
For facility costs, consider a facility $i$ that is opened in our solution and closed in $O_2$. Such a facility must have paid a cost of at least $n_i l(i)$ to get its clients served by other (opened) facilities in $O_2$. The facility cost paid by our solution is $ \delta min\{n_i, \B\} l(i) \le \delta n_i l(i)$. If $i$ is opened in $O_2$, then it must be serving at least $\B$ clients and hence paying a cost of at least $\B l(i)$ in $O_2$. In this case also, the facility cost paid by our solution is $ \delta min\{n_i, \B\} l(i) \le \delta \B l(i)$.  Summing over all $i$'s, we get %\textcolor{blue}{$FCost_{I_{cap}}(S_{cap}) \leq 2 \delta Cost_{I_2}(O_2)$, where $FCost_{\cdot}(\cdot)$ is the facility opening cost of a solution to $I_{cap}$ instance.} 
that the facility cost is bounded by $2 \delta Cost_{I_2}(O_2)$ and the total cost is bounded by $(1 + 2 \delta) Cost_{I_2}(O_2)$. Factor $2$ comes because we may have counted an edge $(i, i')$ twice, once as a client when $i$ was closed and once as a facility when $i'$ was opened in $O_2$.  
\end{proof}


% ****I am here - NG***** 

\section{Bi-criteria Solution $AS_1$ to $I_1$ from approximate solution $AS_{cap}$ to  $I_{cap}$} \label{bi-criteria}

In this section, we obtain a solution $AS_1$ to $I_1$ that violates the capacities/upper bounds by a factor of $(\beta + 2)$ without violating the lower bound. We first obtain an approximate solution $AS_{cap}$ to $I_{cap}$ using approximation algorithm \textcolor{olive}{of Bansal \etal} \cite{Bansal}.  $AS_{cap}$ is then used to construct $AS_1$.
Wlog assume that if a facility $i$ is opened in $AS_{cap}$ then it serves all its demand.\textcolor{green}{ May have to add a couple of lines here in view of the reviews of one of the reviewer: If this is not true, we can modify the $AS_{cap}$  and obtain another solution that satisfies this condition, of cost no more than that of $AS_{cap}$....will see if we can briefly say how we can modify $AS_{cap}$.}
This is always feasible as $d_i \le u_i$. $AS_1$ is obtained from $AS_{cap}$ by first defining the assignment of the clients and then opening the facilities that get at least $\B$ clients. Let $\rhobar^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $AS_{cap}$ and $\rhobar^1(j_i, i')$ denotes the number of clients co-located at $i$ and assigned to $i'$ in $AS_1$. 
%\textcolor{red}{ Initially each facility is assigned the clients co-located with it.}
Clients are assigned in three steps. In the first step, assign the clients co-located at a facility to itself. 
For small $i'$, additionally, we do the following  (type - $1$) re-assignments (see Fig. \ref{type1}): $(i)$ For small $i \ne i'$, assign $\rhobar^c(j_{i'}, i)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for small $i$. $(ii)$ For big $i$, assign $\rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ for big $i$. 
Claim~\ref{claim1} shows that these assignments are feasible and the capacities are violated only upto the extent to which they were violated by the tri-criteria solution $S^t$. 
\begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{Figures/Type 1 Assignments.jpg}
    \caption{($a$) $\B =5$, $t_1, t_2, t_3$ have demands $1$, $2$ and $1$ unit each respectively. In solution $AS_{cap}$, $1$ unit of demand of $t_1$ and $2$ units of demand of $t_2$ are assigned to $t_3$. (b) Solution $S_1$: initially, $n_i$ clients are initially assigned to facility $i$. (c) Type $1$ reassignments: $1$ and $2$ clients of $t_3$ reassigned to $t_1$ and $t_2$ respectively. After this reassignment, $t_3$ has only $1$ client.}
    \label{type1}
\end{figure}

\begin{claim}
\label{claim1}
    $(i)$ $\sum_{i' \ne i} \rhobar^1(j_i, i') \le n_i$, $\forall$ $i \in \bar \facilityset^t$.
    $(ii)$ $\sum_{i} \rhobar^1(j_i, i') \le max\{\B, n_{i'}\} \le \beta \capacityU$, for $\beta \ge 1$, $\forall$ $i' \in \bar \facilityset^t$.
 \end{claim}

\begin{proof}

    $(i)$ Since $\rhobar^c(j_{i}, i) = d_i$ therefore $\sum_{i' \ne i} \rhobar^1(j_i, i') = \sum_{i' \ne i} \rhobar^c(j_{i'}, i) \le u_i - d_i \le n_i$ in all the cases. $(ii)$ $\rhobar^1(j_{i'}, i') = n_{i'}$. For $ i \ne i'$, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$. Thus, $\sum_{i} \rhobar^1(j_i, i') = n_{i'} + \sum_{i \ne i'} \rhobar^c(j_{i'}, i) \le n_{i'} + d_{i'} \le max\{\B, n_{i'}\} \le \beta \capacityU$.
\end{proof}

Note that $AS_1$ so obtained may  still not satisfy the lower bound requirement. In fact, although each facility was assigned $n_i \ge  \alpha \B$  clients initially, they may be serving less clients now after type $1$ re-assignments. For example, in Fig. \ref{type1}, $t_3$ had $4$ clients initially which was reduced to $1$ after type $1$ reassignments. Let $P \subseteq  \facilityset^t$ be the set of facilities each of which is serving at least $\B$ clients after type-$1$ reassignments, and  $\bar P =  \facilityset^t \setminus P$ be the set of remaining facilities. 
 %That is, $ P= \{ i' \in \facilityset^t: \sum_{i}\rhobar^1(j_{i}, i') \ge \B$\}.
 We open all the facilities in $P$ and let them serve the clients assigned to them after type $1$ reassignments.
 
 \begin{observation}
    If a  small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge \B$. Similarly for a big facility $i'$, if $i'_1$ was closed in $AS_{cap}$ then $i'$ is in $P$.
     %\item If a small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge \B$.
    
     
    % \item If $i'$ is big then $\rhobar^1(j_{i'}, i') = n_{i'}  \ge \B$
 \end{observation}
 
 
 Thus, a small facility is in $\bar P$ only if it was open in $AS_{cap}$ and a big facility $i$ is in $\bar P$ only if $i_1$ was open in $AS_{cap}$. 
 %Also note that although each facility in $\bar P$ served at least $\alpha \B \ge \B/2$ clients in the tri-criteria solution $S^t$, they may be serving less clients now after step $1$ of assignment. \textcolor{red}{See Figure \ref{type1} for an example}.
 We now group these facilities so that each group serves at least $\B$ clients and open one facility in each group that serves all the clients in the group. For this we construct what we call as {\em facility trees}. We construct a graph $G$ with nodes corresponding to the facilities in \textcolor{olive}{$P \cup \bar P$.} For $i \in \bar P$, let $\eta(i)$ be the nearest other facility to $i$ in $\facilityset^t$. Then, $G$ consists of edges $(i, \eta(i))$ with edge costs $ \dist{i}{\eta(i)}$. Each component of $G$ is a tree except possibly a double-edge cycle at the root. In this case, we say that we have a root, called {\em root-pair} $<i_{r_1}, i_{r_2}>$ consisting of a pair of facilities $i_{r_1}$and $ i_{r_2}$. Also, a facility $i$ from $P$, if present, must be at the root of a tree. Clearly edge costs are non-increasing as we go up the tree. 

Now we are ready to define our second type of re-assignments.
\textcolor{violet}{
Let $x$ be a node in a tree $\mathcal T$. Let $children(x)$ denote the set of children of $x$ in $\mathcal T$. 
%if $x$ is not a root-pair. 
If $x$ is a root-pair $<r_1, r_2>$, then $children(x) = children(r_1) \cup children(r_2)$. %denote the union of children of $r_1$ and $r_2$ in $\mathcal T$.
Process the tree bottom-up using Algorithm~\ref{TreeProcessing} \textcolor{blue}{(Resolve refernce later- SAPNA)} to process a node $x$ of the tree. \textcolor{olive}{See Fig: (\ref{ProcessX})}.
\textcolor{violet}{ While processing a node $x$, its children are arranged and considered (left to right) in non- increasing distance from $x$.}
%till we reach the root node, which could be either a single facility in $P$ or a root-pair. 
}

 \begin{figure}[t]
    \centering
    \includegraphics[width=12cm]{Figures/ProcessX.jpg}
    \textcolor{red}{
     \caption{ Let $\B=5$, numbers inside a node represents the number of clients at the node. A dashed arrow from a node $u$ to node $v$ represents the movement of clients from $u$ to $v$; (A): A node $x$ along with its children in increasing order of their distances from $x$; (B): In steps $1$ to $7$, we open child $d$ and delete the edge $(d, x)$; (C): In steps $18 -20$, clients from $e$ are assigned to $c$ accumulating a total of $7$ clients at $c$. In the next iteration of the 'for' loop, in lines $14-16$, $c$ gets opened and the edge ($c, x$) is deleted; (D): In the next iteration, clients of $b$ are assigned to $a$; (E):  In the next iteration, clients of $a$ are assigned to $x$ in lines $27 - 28$;}
    }
   % \caption{ (A): A node $x$ along with its children. $\B=5$; Numbers inside each node represents the number of clients at those nodes; (B): Process($x$) - $1$ and $3$ clients from node $d$ and $e$ respectively, get assigned to node $c$, making its count to $8$. $c$ gets opened; (C): $2$ clients of node $b$ are assigned to node $a$, making its count $3$; (D):  $3$ clients of node $a$ are assigned to node $x$, making its count $6$;}
    \label{ProcessX}
\end{figure}

%\input{Gen-Algo.tex}
%\newpage 

\input{Gen-AlgoSG.tex}

\begin{algorithm}[H] 
    \footnotesize
    \setcounter{AlgoLine}{0}
	\SetAlgoLined
	%\scriptsize
    \DontPrintSemicolon  
    \SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
    \Input{$x ( x$ can be a root-pair node)}
    %\Output{}
    
	\For {$ y \in children(x)$} {
	 \If{$n_{y} \geq \B$}  {
	    Open facility $y$ \;
		 
		 Remove edge ($y, \eta(y)$) \textcolor{blue}{\tcp*{Remove the connection of $y$ from $x$}}
		 
		 Delete $y$ from $children(x)$;
	 }
	 }
	\If {$children(x) =  \phi$} {return;}
	
	Arrange $children(x)$ in the sequence $<y_1, \ldots y_k>$ such that $\dist{y_{i-1}}{\eta(y_{i-1})} \le \dist{y_{i}}{\eta(y_{i})} ~\forall ~i = 2 \ldots k$\;
	
%	Arrange $children(x)$ in the increasing order of their distances from $x$. Let $<y_1, \ldots y_k>$ be the sequence obtained.\;
	 
	%	 For $ y \in children(x), re-assigned(y) \gets false$ \textcolor{blue}{ \tcp*{boolean variable to indicate if clients of $rc_i$ are assigned to $lc_i$ or not; initially false}} 
		 
		 \For {$i = k$ down to $2$} {  
		 
		     \eIf{$n_{y_i} \geq \B$}  {
		 
		        Open facility $y_i$\;
		
		     Remove edge ($y_i, \eta(y_i)$) \textcolor{blue}{\tcp*{Remove the connection of $y_i$ from its parent}}
		 
		     Delete $y_i$ from $children(x)$;
		    }
		    {
		     $n_{y_{i-1}} = n_{y_{i-1}} + n_{y_{i}}$	 \tcp*{Send the clients of $y_i$ to $y_{i-1}$}
		 
		      Remove edge ($y_i, \eta(y_i)$) \textcolor{blue}{\tcp*{Remove the connection of $y_i$ from its parent}}
		 
		      Delete $y_i$ from $children(x)$\;
		    }
		 }
		 
		 \eIf {$n_{y_1} \geq \B$}  {
		 
		 Open facility $y_1$ \;
		 
		 %Remove edge ($y_1, \eta(y_1)$) \textcolor{blue}{\tcp*{Remove the connection of $y_1$ from its parent}}
		 
		 Delete $y_1$ from $children(x)$\;
		 }
		 {
		 $n_{\eta(y_1)} = n_{\eta(y_1)} + n_{y_{1}}$ \tcp*{Send the clients of $y_1$ to $\eta(y_1)$}
		 
		 %Remove edge ($y_1, \eta(y_1)$) \textcolor{blue}{\tcp*{Remove the connection of $y_1$ from its parent}}
		 
		 Delete $y_1$ from $children(x)$\;
		 }
		 
		 Return\;
	
	\label{TreeProcessing}
	\caption{Process($x$)}
\end{algorithm}

\newpage
 
There are two possibilities at the root: either we have a facility $i$ from $P$ or we have a root-pair.
%$<i_{r_1}, i_{r_2}>$. 
In the first case, we are done as $i$ is already open and has at least $\B$ clients. \textcolor{olive}{See Fig: (\ref{tree12})}. To handle the second case, we need to do a little more work. So, we define our assignments of third type as follows: 
($i$) If the total number of clients collected at  the root-pair node 
%$i_c, i_{r_1}$ and $i_{r_2}$ 
is at least $\B$ and at most $2\B$ then open any one of the two facilities in the root-pair and assign all the clients to it.\footnote{ we can open 
the facility with more number of clients and save $2$(to be seen again) factor in the connection cost.} \textcolor{olive}{See Fig: (\ref{tree3})}.
($ii$) If the total number of clients collected at  the root-pair node is more than $2\B$  then open both the facilities at the root node and distribute the clients  so that each one of them gets at least $\B$ clients. \textcolor{olive}{See Fig: (\ref{tree4})}.
($iii$) If the total number of clients collected at  the root-pair node  is less than $\B$, then let $i$ be the node in $P$ nearest to the root-pair, then $i$ is already open and has at least $\B$ clients. Send the clients collected at the root-pair to $i$. \textcolor{olive}{See Fig: (\ref{tree5})}.


\begin{figure}[t]
	\begin{tabular}{ccc}
		\includegraphics[width=12cm,scale=1.0]{Figures/Tree1.jpg}
		%& 
		%\includegraphics[width=6cm,scale=0.8]{Figures/Tree2.jpg}
		%\\
		%\textbf{(a)}& \ \ \textbf{(b)}& \ \ \textbf{(c)}
	\end{tabular}
	\textcolor{red}{
	\caption{ $\B=12$;(A) A tree $\mathcal{T}$;  Numbers inside each node represents the number of clients at those nodes.
	At any fixed level, nodes are processed in any arbitrary order (for the sake of example, we process them in left to right order). The tree does not change after the calls: Process($f$), Process($g$), Process($h$), Process($i$), Process($j$) and Process($k$). In each case, it returns at line no. $9$;  (B) Tree after Process($a$), Process($b$), Process($c$), Process($d$) and 
	Process($e$); (C) Tree after Process($x$) when $t \ge 3$ }.
	}
	
	%\caption{(A) A tree $\mathcal{T}$; $\B=12$; Numbers inside each node represents the number of clients at those nodes. (B) Algorithm Process() called in the following order: Process($a$) - $3$ and $6$ clients from node $g$ and $h$ respectively, get assigned to node $f$, making its count to $12$; Process($b$); Process($c$) - $9$ clients from $i$ are assigned to node $c$; Process($d$); Process($e$) - $3$ and $1$ clients from node $j$ and $k$ respectively, get assigned to it. Eventually, node $f$ and $c$ are opened; (C) Process($x$) - $2$, $1$ and $5$ clients from node $b$, $d$ and $e$ respectively, get assigned to node $x$, making its count to $t+8$; (D) $x\in P,~n_x = 12$ and $t=1$; All $9$ clients from children of $x$ are assigned to $x$. }
	\label{tree12}
\end{figure}


% \begin{figure}[t]
%    \centering
%    \includegraphics[width=7cm]{Figures/Tree1.jpg}
%    \caption{(A) A tree $\mathcal{T}$; $\B=12$; Numbers inside each node represents the number of clients at those nodes. (B) Algorithm Process() called in the following order: Process($a$) - $3$ and $6$ clients from node $g$ and $h$ respectively, get assigned to node $f$, making its count to $12$; Process($b$); Process($c$) - $9$ clients from $i$ are assigned to node $c$; Process($d$); Process($e$) - $3$ and $1$ clients from node $j$ and $k$ respectively, get assigned to it. Eventually, node $f$ and $c$ are opened; }
%    \label{tree1}
%\end{figure}

 %\begin{figure}[t]
  %  \centering
   % \includegraphics[width=7cm]{Figures/Tree2.jpg}
    %\caption{ $\B=12$; (C) Process($x$) - $2$, $1$ and $5$ clients from node $b$, $d$ and $e$ respectively, get assigned to node $x$, making its count to $t+8$; (D) $x\in P,~n_x = 12$ and $t=1$; All $9$ clients from children of $x$ are assigned to $x$. }
    %\label{tree2}
%\end{figure}


 \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{Figures/Tree3.jpg}
    \textcolor{red}{
    \caption{ $\B=12, t < 3$; (E)  $x = <i_{r_1}, i_{r_2}>$ is a root-pair node  with $\B \le n_{i_{r_1}} + n_{i_{r_2}} + t + 8 \le 2B$ (F) $t=2$ (give this in the figure and delete from here); open any of $i_{r_1}$ and $i_{r_2}$, say $i_{r_1}$ and assign all the clients to it.}
    }
    \label{tree3}
\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{Figures/Tree4.jpg}
    \textcolor{red}{
    \caption{ $\B=12, t < 3$; (E)  $x = <i_{r_1}, i_{r_2}>$ is a root-pair node  with $2\B \le n_{i_{r_1}} + n_{i_{r_2}} + t + 8 < 3B$ (F)  open both $i_{r_1}$ and $i_{r_2}$ and distribute the clients to them so that each of them gets at least $\B$ clients.}
    }
    %\caption{ $\B=12$; (G) $x = <i_{r_1}, i_{r_2}>$ is a root-pair node; $n_{i_{r_1}} = 8,~n_{i_{r_2}} = 9$ (F) $t=1$; All $9$ clients from children of $x$ are distributed between $i_{r_1}$ and $i_{r_2}$; both facilities in $x$ get opened. }
    \label{tree4}
\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{Figures/Tree5.jpg}
    \textcolor{red}{
    \caption{ $\B=12, t < 3$; (E)  $x = <i_{r_1}, i_{r_2}>$ is a root-pair node  with $ n_{i_{r_1}} + n_{i_{r_2}} + t + 8 < B$ (F)  open a facility $i \in P$ that is nearest to $\{i_{r_1}, i_{r_1}\}$ and assign all the clients to it.}
    }
   % \caption{ $\B=12$; (I) $x = <i_{r_1}, i_{r_2}>$ is a root-pair node; $n_{i_{r_1}} = n_{i_{r_2}} = 1$ (J) $t=1$; All $9$ clients from children of $x$ and, clients of $i_{r_1}$ and $i_{r_2}$ are assigned to $i \in P$.}
    \label{tree5}
\end{figure}

 
Clearly the opened facilities satisfy the lower bounds. Next, we bound the violation in the upper bound.
  
   \begin{lemma}
 Let $ i_c$ be the only child, if any,  of the root (/root-pair) of a tree. Let $i$ be the parent of $ i_c$ ($i$ is either in $P$ or it is one of $i_{r_1}$ and $i_{r_2}$ in case the root is a root-pair).
The number of clients collected in the second type of re assignments, at any node $x$ in the tree rooted at $i_c$ is at most $2\B$.
 \end{lemma}
 
 \begin{proof} 
 \textcolor{violet}{We will show that the number of clients collected at $x$ after Process($x$) is at most $2\B$. For this, note that $x$ receives $< \B$ clients from at most one of it's children. Hence, the claim follows.}
 \end{proof}
  
  If the number of clients collected at $i_c$ is $\ge \B$, it is opened and removed from further processing.
 Let $\pi_i$ be the number of clients assigned to the facility $i$ after first type of re-assignments. Then as shown earlier, $\pi_i \le \beta \capacityU$.  %Let $i$ be the parent of $ i_c$. In second and third types of assignments,  we never collect  more than $2\B$ clients at any node till we reach $i_c$.
 %Now we have the following scenarios: Suppose $ i_c$ has less than $\B$ clients,
 We have the following cases: ($i$) the root node $i$ is in $P$ and it gets additional at most $\B$ clients from $i_c$ making a total of at most $\pi_i + \B \le \beta \capacityU + \B \le (\beta + 1) \capacityU$ clients at $i$.
 ($ii$) the total number of clients collected at  the root-pair node 
%$i_c, i_{r_1}$ and $i_{r_2}$ 
is at least $\B$ and at most $2\B$.
 %($ii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at $i_c, i_{r_1}$ and $i_{r_2}$ is at least $\B$ and at most $2\B$. Thus, 
 The number of clients the opened facility gets is at most $2\B \le 2\capacityU$.
 ($iii$)  the total number of clients collected at the root-pair node  is more than $2\B$.  Note that the total number of clients collected at these facilities is at most $3\B$ and hence 
 ensuring that each of them gets at least $\B$ clients also ensures that none of them gets more than $2\B$ clients. Hence none of them gets more than $2\capacityU$ clients.
 %it is possible to distribute them to the two opened facilities so that each of them gets at most $2\B \le 2\capacityU$ clients.
 ($iv$) the total number of clients collected at the root-pair node is less than $\B$. 
 %Number of clients at $i_c$ and the root pair and, their nearest facility in $P$ are at most $\B$ and $\beta \capacityU$ respectively. 
 Thus, the number of clients the opened facility in $P$ gets is at most $\beta \capacityU + \B \le (\beta + 1) \capacityU$. 
 %The case when $i_c$ has at least $\B$ clients leads to the third scenario above and hence handled.
 
 
 We next bound the connection cost.  For any node $y$ in a tree, let $left-sibling(y)$ denote the left sibling of $y$ in step~\ref{} of the algorithm. Thus, $left-sibling(y_i) = y_{i-1}$. We will need the following lemma to bound the connection cost.
 
 \begin{lemma}
 For a node $y$ in a tree,
  $\dist{y}{left-sibling(y)} \le 3 \dist{y}{\eta(y)} = 3l(y)$. %.....This equality is correct, right? we have been assuming this....$P \cup \bar P = F^t$, right?
 \end{lemma}
 
 \begin{proof}
 \textcolor{violet}{
 If $\eta(\cone) = \eta(left-sibling(\cone))$  (i.e. $\cone$ and $left-sibling(\cone)$ are children of the same node), then it is easy to see that $\dist{\cone}{left-sibling(\cone)} \leq 2 \dist{\cone}{\eta(\cone)}$. Otherwise (which can be the case when root is a root-pair, see Figure~(\ref{3factorBound})), $\dist{\cone}{left-sibling(\cone)} \leq \dist{\cone}{\eta(\cone)} + \dist{\eta(\cone)}{\eta(left-sibling(\cone))} + \dist{\eta(left-sibling(\cone))}{left-sibling(\cone)} \le 3 \dist{\cone}{\eta(\cone)}$.
 }
 
  \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{Figures/3factorBound.jpg}
    \caption{$\dist{\cone}{left-sibling(\cone)}  \le 3 \dist{\cone}{\eta(\cone)}$}
    \label{3factorBound}
\end{figure}
 \end{proof}
 
 
 The cost of first type of re-assignments is \textcolor{olive}{at most the connection cost of $AS_{cap}$.} 
% \textcolor{red}{(or at most?Sapna/rajni) }
 To bound the connection cost of second type, observe that we never send more than $\B$ clients on any edge. 
 %In the second type of assignment, 
 Thus, a facility $i$ that sends its (at most $\B$ clients) to its parent or to its left sibling incurs a cost of at most $3\B l(i)$. Since the facility $i$ was opened in $AS_{cap}$, it pays facility opening cost of $\delta l(i) min \{n_i, \B\} \ge \delta l(i) \alpha \B$ in $AS_{cap}$. Summing over all $i \in \bar P$ for the second type of re-assignments, we see that the total connection cost in these re-assignments is bounded by 
 \textcolor{red}{
 $3 FCost_{I_{cap}}(AS_{cap})/\alpha \delta$ 
 } 
% \textcolor{olive}{D: $\sum_{i \in \bar P} \B l(i) \leq 6FCost_{I_{cap}}(AS_{cap})/\alpha \delta$  where factor 6 comes because sending clients to the left sibling incurs a cost of twice the cost to the node's parent and}
 where $FCost_{I_{cap}}(.)$ is the facility opening cost of a solution to the $I_{cap}$ instance.


 For the third type of re-assignments, we bound the cost as follows:
 %we bound the cost in two parts: ($a$) cost of sending ($< \B$) clients of $i_c$ to it's parent ($b$) Cost of sending ($< \B$) clients collected at the root pair $<i_{r_1}, i_{r_2}>$ to it's nearest facility in $P$. Cost of the first part is bounded by $\B l(i_c)$. 
 the cost of sending ($< \B$) clients by a facility $i$ in the root pair $<i_{r_1}, i_{r_2}>$ to the facility in $P$, nearest to the root-pair, is not bounded by $\B l(i)$ (where $l(i) = l(i_{r_1}) = l(i_{r_2})$). 
% we bound the cost as follows: 
 Note that the total number of clients, initially at $i_{r_1}$ and $i_{r_2}$ was $\ge 2 \alpha \B$. However, during re-assignments of type $1$, some of them got reassigned to other facilities. Note that these (other) facilities must have been closed in $AS_{cap}$ and hence do not belong to $\bar P$. Hence, each of these reassignments correspond to an assignment in $AS_{cap}$ whose cost was at least $l(i)$ and a total of at least $(2\alpha  - 1)\B l(i)$. Hence the cost of type $3$ re-assignments is bounded by \textcolor{blue}{$3 CCost_{I_{cap}}(AS_{cap})/ (2\alpha  - 1)$ where $CCost_{I_{cap}}(.)$ is the connection cost of a solution to the $I_{cap}$ instance}. 
 
 \textcolor{violet}{
 Hence the total cost of solution $S_1$  is $6\alpha/(2\alpha-1) \textcolor{blue}{Cost_{I_{cap}}(AS_{cap})}$ for $\delta= (2\alpha-1)/6\alpha^2 $. \textcolor{blue}{Why 6 times???}...Only this is left from my side.
 }
 

==> Gen-Algo.tex <==
\begin{algorithm}[H]
\footnotesize
    \SetAlgoLined
    %\KwData{$\clientset,~\facilityset$}
    %\KwResult{$\clientset',~\bundle{j'}~\forall~j'\in \clientset'$}
    \SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
    \Input{$x$}
    %\Output{}
		 
	% Process($lc_i$)\;
		 
	% Process($rc_i$)\;
	If $children(x) =  \phi$, return;
	
	For $ y \in children(x)$\\
	 \If{$n_{y} \geq \B$}  {
	 Open facility $y$ \;
		 
		 Remove edge ($y, \eta(y))$) \textcolor{blue}{\tcp*{Remove the connection of $lc_i$ from its parent}}
		 
		 Delete $y$ from $children(x)$;
	 }
	
	 Arrange $children(x)$ in the increasing order of their distances from $x$. Let $<y_1, \ldots y_k>$ be the sequence obtained.
	%	 For $ y \in children(x), re-assigned(y) \gets false$ \textcolor{blue}{ \tcp*{boolean variable to indicate if clients of $rc_i$ are assigned to $lc_i$ or not; initially false}} 
		 
		 For $i = k$ down to $2$ 
		 
		 \If{$n_{y_i} \geq \B$}  {
		 
		 Open facility $y_i$ \;
		 
		 Remove edge ($y_i, \eta(y_i))$) \textcolor{blue}{\tcp*{Remove the connection of $y_i$ from its parent}}
		 
		 Delete $y_i$ from $children(x)$;
		 
		 }
		 
		 else \\
		 
		\{\\
		$n_{y_{i-1}} = n_{y_{i-1}} + n_{y_{i}}$;
		 \tcp*{Send the clients of $y_i$ to $y_{i_1}$}
		 
		 Remove edge ($y_i, x)$)\; \textcolor{blue}{\tcp*{Remove the connection of $y_i$ from its parent $x$}}
		 
		 
		 Delete $y_i$ from $children(x)$\;\\
		 \}
		 
		 \If{$n_{y_1} \geq \B$}  {
		 
		 Open facility $y_1$ \;
		 
		 Remove edge ($y_1, x$) \textcolor{blue}{\tcp*{Remove the connection of $y_1$ from its parent}}
		 
		 Delete $y_1$ from $children(x)$;\;
		 
		 }
		 
		 else \\
		 
		\{\\
		$n_{x} = n_{x} + n_{y_{1}}$;
		 \tcp*{Send the clients of $y_1$ to $x$}
		 
		 Remove edge ($y_1, x)$)\; \textcolor{blue}{\tcp*{Remove the connection of $lc_i$ from its parent}}
		 
		 
		 Delete $y_1$ from $children(x)$\;\\
		 \}
	
	\label{Process_i}
	\caption{Process($x$)}
\end{algorithm}

==> LBFLO_ng.tex <==
\section{Instance $I_1$ and $I_2$}
\label{instI1}

We define an instance $I_1$ of LBFL.
Let $t \le B/4$.
Clients that were outliers in $S^t$ are removed in instance $I_1$.
Let $F^t$ be the set of facilities opened by $S^t$. For a client $j$, let $\sigma^t(j)$ be the facility to which $j$ is assigned in $S^t$. For $i \in F$, let $n_i$ be the number of clients served by $i$ in $S^t$. Move these clients to $i$ (see Fig.~\ref{Mapping1}). Thus, there are $n_i > B/2$ clients co-located with $i$. 
%For $i \in F^t$, $n_i = |(\sigma^t)^{-1}(i)|$ and for $i \notin F^t$, $n_i = 0$.   
In $I_1$, our facility set is $F$ and the clients are at their new locations. 
$f^1_i = 0$ for $i \in F^t$ and $=f_i$ for $i \notin F^t$.
%We will show that there exists a feasible solution $S_1$ of $I_1$ such that $Cost(S_1)$ is bounded by $Cost(S^t) + Cost(O)$. 
For a client $j$ served in $O$, let $\sigma^*(j)$ be the facility serving it. %$j$ in $O$. 

\begin{lemma}
There is a bi-criteria  solution $S_1$ of $I_1$ whose cost is bounded by $2 (Cost(S^t) + Cost(O))$.
\end{lemma}
\begin{proof}
We construct the solution $S_1$ of $I_1$ as follows: open $i$ in $S_1$ iff it is opened in $O$. Assign $j$ to $i$ in $S_1$ if it is assigned to $i$ in $O$. Let $O_o$ be the set of clients that are outliers in $O$. Let $O_i$ be the set of clients co-located with facility $i \in F^t$ and not served by $O$. Note that since $t \le B/4$ and $n_i > B/2$, at least $B/4$ clients at $i$ are served in $O$. Serve the clients in $O_i$ by the facilities serving the clients $(\sigma^t)^{-1} (i) \setminus O_i$ at a loss of factor $2$ in service cost.
%$j$ be a client co-located with facility $i= \sigma^t(j)$ and not served by $O$. 
$S_1$ violates the LB at most by a factor of $3/4$. LB is violated at a facility $i$ serving clients that were outliers in $S^t$ and are not present in $I_1$. Since this number is $\le B/4$, violation is at most $B - B/4 = 3B/4$.

%$S_1$ satisfies both the lower bound as well as the upper bound as $O$ does so. 
The cost $c( \sigma^t(j), \sigma^*(j))$ of serving $j$ from its new location is bounded by $c(j, \sigma^t(j)) + c(j, \sigma^*(j))$ if $j$ is not an outlier in $O$. Otherwise it can be charged to one of its co-located client that is served by $O$(see Fig. \ref{lemma1}). Thus, the claim follows.


\begin{figure}[t]
    \centering
    \includegraphics[width=9cm]{figures/mapping_0.jpg}
    \caption{Transforming instance $I$ to $I_1$ and  $I_1$ to $I_2$. Solid squares represent clients and circles represent facilities. Clients are moved to the facilities serving them in $S^t$ while transforming $I$ to $I_1$. Facilities not opened in $S^t$ are dropped while going from $I_1$ to $I_2$.}
    \label{Mapping1}
\end{figure} \end{proof}


\begin{figure}[t]
    \centering
    \includegraphics[width=4cm]{figures/lemma 1.jpg}
    \caption{$c( \sigma^t(j), \sigma^*(j)) \leq c(j, \sigma^t(j)) + c(j, \sigma^*(j))$ }
    \label{lemma1}
\end{figure}

  Next, we define an instance $I_2$ of LBFL.
  Instance $I_2$ is same as $I_1$ except that the facility set is $F^t$ now. $f^2_i = 0$ for all $i \in F^t$. 
 % We will show that there exists a feasible solution $S_2$ of $I_2$ such that $Cost(S_2)$ is bounded by $2 Cost(O_1)$ where
  Let $O_1$ be an optimal solution of $I_1$. 
  For a client $j$, let $\sigma^1(j)$ be the facility serving $j$ in $O_1$.

\begin{lemma}
There is a solution $S_2$ of $I_2$  that violates the LB by a factor of $3/4$ and whose cost is bounded by $ 2Cost(S_1)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_2$ of $I_2$: for $i$ \in $F^t$, open $i$ in $S_2$ if it is opened in $S_1$ and assign a client $j$ to it if it is assigned to $i$ in $S_1$. For $i$ \notin $F^t$, open its nearest facility $i'$ in $F^t$. Assign $j$ to $i'$ in $S_2$ if it is assigned to $i$ in $S_1$. $S_2$ violates the lower bound by $3/4$ as $S_1$ does so.  The cost $c( \sigma^t(j), i')$
%$c( \sigma^t(j), \sigma^*(j))$ 
of serving $j$ from its new location is bounded by $c(\sigma^t(j), \sigma^1(j)) + c( \sigma^1(j), i') \le 2 c(\sigma^t(j), \sigma^1(j))$ (since $i'$ is closest in $F^t$ to $i =  \sigma^1(j)$) where $\sigma^1(j)$ is the facility that serves $j$ in $S_1$. Summing over all $j$'s we get the desired claim.

%$c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(i, \sigma^1(j)) \le c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(\sigma^t(j), \sigma^1(j))$ (since $i$ is closest in $F^t$, to $i' = \sigma^1(j)$) $\le 2(c(j, \sigma^t(j)) + c(j, \sigma^1(j)))$ (See Figure 1). Summing over all $j$'s, the claim follows.
%Same as Zoya etal
\end{proof}




\section{Instance $I_{cap}$ for Capacitated Facility Location}
\label{instIcap}
For each facility $i \in F^t$, let $l(i)$ be the distance of $i$ from a nearest facility  $i' \in F^t$, $i' \neq i$ and let $\delta$ be a constant chosen appropriately. We say that a facility $i$ is {\em small} if $0< n_i < B$ and it is {\em big} otherwise. Every big facility $i$ is split into two co-located facilities $i_1$ and $i_2$ . We split the set of clients, at $i$, also into two sets.  $B$ of these clients are placed at $i_1$ and the remaining $n_i - B$ clients at $i_2$ (see Fig.~\ref{Mapping2}). The second type of big facilities are called {\em free}. 
 \begin{figure}
    \centering
    \includegraphics[width=8cm]{figures/mapping_1.jpg}
    \caption{Transforming instance $I_2$ to $I_{cap}$:
    %Solid squares represent clients and circles represent facilities. 
    $i'$ is small, $i$ is big.
    $i$ is split into $i_1$ and $i_2$ while transforming $I_2$ to $I_{cap}$, $i_2$ is free. Demand at the small facility $i'$ is $B - n_{i'} = 1$ and at $i_1$, $i_2$, it is $0$. Capacities of $i'$ and $i_1$ are $B = 4$ and it is $n_{i} - B = 3$ of the free facility $i_2$.}
    \label{Mapping2}
\end{figure}
%\textcolor{red}{ Let $F_f$ denote the set of free facilities (...will delete).} 
 Let $\bar F^t$ be the set of facilities so obtained. The set of clients and the set of facilities are both $\bar F^t$. %In the $I_{cap}$ instance, we place demands  at all of these facilities. 
 The facility costs, capacities and demands are as shown in Table~\ref{tab:my_label} (also see Fig.~\ref{Mapping2}).
 \begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
       Type & $n_i$ & $u_i$ & $d_i$ & $f^t_i$ \\
        \hline
       {\em small} & $n_i \leq B$ & $B$ & $B- n_i$& $\delta n_i l(i)$ \\
        \hline
       {\em big} & $n_i > B$ & ($i_1$)$B$ & $0$& $\delta B l(i)$ \\
        & & ($i_2$) $n_i - B$ & $0$& $0$ \\
       
        % &  &
          \hline 
       % $3$ & $0$ & $B$ & $B$& $\delta B l(i)$ \\
        %\hline
    \end{tabular}
    \caption{Instance of $I_{cap}$: $d_i, u_i, f^t_i$ are demands, capacities and facility costs resp.}
    \label{tab:my_label}
\end{table}
 
 %Let $O_{cap}$ be an optimal solution to $I_{cap}$.
 
 %\textcolor{red}{define delta and l(i)}
 %The second type of big facilities are called {\em free}. %and the clients placed at them are also called {\em free}. 
 %Let $F_f$ denote the set of free facilities. 
 %and $Cf(i)$ denote the set of free clients at facility $i \in F_b$. i.e.$Cf(i)$ is the set of clients placed at $i_2 \in F_f$ (See Figure 2)....need to define $l(i)$.





\begin{lemma}
%A feasible solution $S_{cap}$ for 
Cost of optimal solution to 
$I_{cap}$ is bounded by $(1+2\delta)Cost(O_2)$.
\end{lemma}

\begin{proof}
We will construct a feasible solution $S_{cap}$ to $I_{cap}$ of bounded cost.
Let $O_2$ be an optimal solution of $I_2$. As $O_2$ satisfies the lower bound,  we can assume wlog that if $i$ is opened in $O_2$ then it serves all of its clients if $n_i \le B$ (before taking more clients from outside) and it serves at least $B$ of its clients before sending out its clients to other (small) facilities otherwise. 
Also, if two big facilities are opened in $O_2$, one does not serve the clients of the other. Let $\rho^2(j_i, i')$ denote the number of clients co-located at $i$ and assigned to $i'$ in $O_2$ and $\rho^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $S_{cap}$ .
 \begin{figure}[t]
    \centering
    \includegraphics[width=10cm]{figures/O2_Scap assignments.jpg}
    \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ and $i'$ are closed in $O_2$. $\rho^2(j_{i_1}, t_1) = 2,~\rho^2(j_{i_1}, t_2) = 1,~\rho^2(j_{i_1}, t_3) = 1,~ \rho^2(j_{i_1}, t_4) = 0$ and $\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 1,~\rho^2(j_{i_2}, t_3) = 1,~ \rho^2(j_{i_2}, t_4) = 0$.  } %The middle figure shows how the assignments look like after splitting the big facilities. $\rho^2(j_{i_1}, i') = 2(/1/1)$ for $i'$ = top three facilities $t_1(/t_2/t_3)$ $\rho^2(j_{i_2}, i') = 1(/1/1) $ for the bottom three facilities $t_2(/t_3/t_4)$. Note that $t_1$ }
    \label{Mapping}
\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{figures/O2_Scap assignments (2.1).jpg}
   \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ is open in $O_2$.   $\rho^c(j_{t_1}, i_2) = \rho^2(j_{i}, t_1) = 1, \rho^c(j_{t_2}, i_2) = \rho^2(j_{i}, t_2) = 2$,
  % $\rho^2(j_{i_1}, t_1) = 1,~\rho^2(j_{i_1}, t_2) = 1$ and %$\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 2$. 
   $i_2$ is open in $S_{cap}$. $t_1$ and $t_2$ must be small.}
    \label{O2_SCap2}
\end{figure}
    \begin{enumerate}
        \item   if $i$ is closed in $O_2$ then open $i$ if $i$ is small
        and open $(i_1 \& i_2)$ if it is big.
        
        Assignments are defined as follows (see Fig.~\ref{Mapping}):
        \begin{enumerate}
            \item If $i$ is small: Let $i$ serve its own demand. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. Thus, 
        $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $ i' \ne i$ and $\rho^c(j_i, i) = d_i$. Also,
        $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). 
        Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = B = u_i$. %Thus capacities are respected.
      
         
        
       \item If $i$ is big: assign $\rho^2(j_{i_1}, i')$ (/$\rho^2(j_{i_2}, i')$) demand of $i'$ to $i_1$(/$i_2$) in our solution for small $i' \ne i$. Thus,
        $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_1) = \sum_{small~i' \ne i} \rho^2(j_{i_1}, i') \le B = u_{i_1}$.
         $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_2) = \sum_{small~i' \ne i} \rho^2(j_{i_2}, i') \le n_i - B = u_{i_2}$.
         The second equality holds in each case as $i$ is closed in $O_2$.
        % Since there are no demands at $i_1$ and $i_2$, the capacities are respected.
     
       \end{enumerate}
     
     \item Open free facility $i_2$ 
     %for $i_2 \in F_f$ (and 
     ($i$ is opened in $O_2$) (see Fig.~\ref{O2_SCap2}): assign $\rho^2(j_{i}, i')$  demand of $i'$ to $i_2$ in our solution for small $i' \ne i$. Thus,
     %Thus,
      %  $\sigma^c(j_{i'}, i_2) = %\sigma^1(j_{i_2}, i'), i \ne i'$  
        $\sum_{i' \ne i}\rho^c(j_{i'}, i_2) = \sum_{i' \ne i} \rho^2(j_{i}, i') \le n_i - B$ (the inequality holds by assumption on $O_2$) $= u_{i_2}$.
       % Thus the capacities are respected as there are no demands at $i_2$.
       
       \item \textcolor{red}{Open the special facility $i^*$ ($u_{i^*} = t, d_{i^*} = 0, f_{i^*} = 0 )$. If $i$ is closed in $S_{cap}$ and it is small, then it must be opened in $S_2$. Let $sp(i)$ be the set of clients in $Out(S^t)$ that are served by $i$ in $S/S_1/S_2)$. Assign $|sp(i)|$ demand of $i$ to the special facility $i^*$.}
    \end{enumerate}
    
    Next, we show that all the demands are satisfied. If a facility is opened in $S_{cap}$, it satisfies its own demand. 
Let $i$ be closed in $S_{cap}$. If $i$ is big ,we need not worry as $i_1$ and $i_2$ have no demand. So, let $i$ is small. Then, it must be opened in $O_2$. Then, 
\textcolor{red}{
$\sum_{i' \ne i}\rho^c(j_{i}, i') = $
$\sum_{small ~i' \ne i,  }\rho^c(j_{i}, i') + \sum_{i'_1: i' ~is ~big}\rho^c(j_{i}, i'_1) + 
\sum_{i'_2: i' ~is ~big}\rho^c(j_{i}, i'_2) + \rho^c(j_{i}, i^*)= $
$\sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i'_1 : i' ~is ~big} \rho^2(j_{i'_1}, i)  + \\ \sum_{i'_2 : i' ~is ~big}\rho^2(j_{i'_2}, i) + |sp(i)| = \sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i' ~is ~big}\rho^2(j_{i'}, i)  + |sp(i)| = \sum_{i' \ne i}\rho^2(j_{i'}, i)  + |sp(i)|$
$\ge B - n_i$  (since $O_2$ is a feasible solution of $I_2$) $= d_i$. 
}

Next, we bound the cost of the solution. The connection cost is same as that of $O_2$. %Next, we consider the facility opening costs. 
For facility costs, consider a facility $i$ that is opened in our solution and closed in $O_2$. Such a facility must have paid a cost of at least $n_i l(i)$ to get its clients served by other (opened) facilities. The facility cost paid by our solution is $ \delta min\{n_i, B\} l(i) \le \delta n_i l(i)$.  If $i$ is opened in $O_2$, then it must be serving at least $B$ clients and hence paying a cost of at least $B l(i)$. In this case also, the facility cost paid by our solution is $ \delta min\{n_i, B\} l(i) \le \delta B l(i)$. Thus the facility cost is bounded by $2\delta Cost(O_2)$ and the total cost is bounded by $(1 + 2 \delta) Cost(O_2)$. Factor $2$ comes because we may have counted an edge $(i, i')$ twice, once as client when $i$ was closed and once as a facility when $i'$ was opened in $O_2$.
\end{proof}



\section{Bi-criteria Solution $S_1$ to $I_1$ from approximate solution $AS_{cap}$ to  $I_{cap}$}
\label{bi-criteria}

Next we obtain a solution $\bar S_1$ to $I_1$ that violates the capacities/upper bounds by a factor of $(\beta + 1)$ without violating the lower bound. 
Wlog assume that if a facility $i$ is opened in $AS_{cap}$ then it serves all its demand. This is always feasible as $d_i \le u_i$. $S_1$ is obtained from $AS_{cap}$ by first defining the assignment of the clients and then opening the facilities that get at least $B$ clients. Let $\rhobar^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $AS_{cap}$ and $\rhobar^1(j_i, i')$ denotes the number of clients co-located at $i$ and assigned to $i'$ in $S_1$. 
%\textcolor{red}{ Initially each facility is assigned the clients co-located with it.}
Clients are assigned in three steps. In the first step, we define the assignments as follows:  For a big facility $i'$, assign all the clients co-located at $i'_1$ and $i'_2$ to $i$. For a small facility $i'$, assign the clients co-located at $i'$ to itself.  For small $i'$, additionally, we do the following  re-assignments (see Fig. \ref{type1}): $(i) $For small $i \ne i'$, assign $\rhobar^c(j_{i'}, i)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for small $i$. $(ii)$ For big $i$, assign $\rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ for big $i$.
\begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{figures/Type 1 Assignments.jpg}
    \caption{($a$) $B =5$, $t_1, t_2, t_3$ have demands $1$, $2$ and $1$ unit each respectively. In solution $AS_{cap}$, $1$ unit of demand of $t_1$ and $2$ units of demand of $t_2$ are assigned to $t_3$. (b) Solution $S_1$: initially, $n_i$ clients are initially assigned to facility $i$. (c) Type $1$ reassignments: $1$ and $2$ clients of $t_3$ reassigned to $t_1$ and $t_2$ respectively. After this reassignment, $t_3$ has only $1$ client.}
    \label{type1}
\end{figure}

\begin{claim}
    $(i)$ $\sum_{i' \ne i} \rhobar^1(j_i, i') \le n_i$, $\forall$ $i \in \bar F^t$.
    $(ii)$ $\sum_{i \ne i'} \rhobar^1(j_i, i') \le \beta U_{i'}$, $\forall$ $i' \in \bar F^t$.
 \end{claim}

\begin{proof}

    $(i)$ Since $\rhobar^c(j_{i}, i) = d_i$ therefore $\sum_{i' \ne i} \rhobar^c(j_{i'}, i) \le u_i - d_i \le n_i$ in all the cases. $(ii)$ $\rhobar^1(j_{i'}, i') = n_{i'}$.  
$\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for $ i' \ne i$. Thus,
 %   
    %\item $\rhobar^1(j_{i'}, i') =$ original $n_{i'}$ clients $ %\rhobar^c(j_{i'}, i')$.....(1) $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for $ i' \ne i$.....(2) Adding (1) and ((2) over all $i \ne i'$), we get
%
$\sum_{i} \rhobar^1(j_i, i') = n_{i'} + \sum_{i \ne i'} \rhobar^c(j_{i'}, i) \le n_{i'} + d_{i'} \le max\{B, n_{i'}\} \le \beta U_{i'}$
\end{proof}

Note that $S_1$ so obtained may not still satisfy the lower bound requirement. In fact, 
 although each facility was assigned $n_i \ge  \alpha B \ge B/2$ clients initially, they may be serving less clients now after type $1$ re-assignments. For example, in Fig. \ref{type1}, $t_3$ had $4$ clients initially which was reduced to $1$ after type $1$ reassignments. Let $P \subseteq  F^t$ be the set of facilities each of which is serving at least $B$ clients and  $\bar P =  F^t \setminus P$ be the set of remaining facilities. 
 %That is, $ P= \{ i' \in F^t: \sum_{i}\rhobar^1(j_{i}, i') \ge B$\}.
 We open all the facilities in $P$ and let them serve the clients assigned to them after type $1$ re-assignments.
 
 \begin{observation}
 If a  small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge B$.
     Similarly for a big facility $i'$, if $i'_1$ was closed in $AS_{cap}$ then $i'$ is in $P$.
     %\item If a small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge B$.
    
     
    % \item If $i'$ is big then $\rhobar^1(j_{i'}, i') = n_{i'}  \ge B$
 \end{observation}
 
 
 Thus, a small facility is in $\bar P$ only if it was open in $AS_{cap}$ and a big facility $i$ is in $\bar P$ only if $i_1$ was open in $AS_{cap}$. 
 %Also note that although each facility in $\bar P$ served at least $\alpha B \ge B/2$ clients in the tri-criteria solution $S^t$, they may be serving less clients now after step $1$ of assignment. \textcolor{red}{See Figure \ref{type1} for an example}.
 We now try to group these facilities so that each group serves at least $B$ clients and open one facility in each group that serves all the clients in the group. For this we construct what we call as {\em facility trees}. We construct a graph $G$ with nodes corresponding to the facilities in $\bar P$. For $i \in \bar P$, let $\eta(i)$ be the nearest other facility to $i$ in $F^t$. Then, $G$ consists of edges $(i, \eta(i))$. Each component of $G$ is a tree except possibly a double-edge cycle at the root. In this case, we say that we have a root, called {\em root-pair}, consisting of a pair of facilities say $i_i$ and  $i_2$ and denoted by $<i_{r_1}, i_{r_2}>$. Also, a facility $i$ from $P$, if present must be at the root of a tree. We try to process each tree bottom-up sending the clients of each facility to its parent. However doing so may result in too much violation in the capacities at the parent facility. 
 \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{figures/tree.jpg}
    \caption{Binary tree conversion process: (a) Tree $\mathcal{T}$ of unbounded degree: $a<b<c<g,~c<d$. (b) Binary routing tree (intermediate stage). (c) Final tree.}
    \label{tree}
\end{figure}

 To keep the capacity violation in check, we convert each tree into a binary tree
 %\textcolor{red}{
 (see Fig. \ref{tree}): first of all, we treat the double-edge cycle, if any, as a single node for this purpose. Then, at every node $x$, arrange the children of $x$ from left to right in non-decreasing order of distance from $x$.
  For each child $y$ (except for the nearest child) of $x$, add an edge to its left sibling %with weight $2\dist{ y}{\eta(y)}$ 
  and remove the edge $( y, x)$. There is no change in the outgoing edge of the leftmost child of $x$. 
Let $\sigmaone(y)$ be the parent of  $y$ in the so constructed tree. Its easy to see that $\dist{y}{\sigmaone(y)} \leq 3 \dist{y}{\eta(y)}$. Thus, we replace $\dist{y}{\sigmaone(y)}$ by $3 \dist{y}{\eta(y)}$ for all $y$. Henceforth, whenever we refer to distances, we mean the new edge weights. Now, every node has in-degree of at most $2$ with the in-degree of the root being at most $1$. 

Now we are ready to define our second type of re-assignments. Process the tree bottom-up as follows (see Fig. \ref{type2-3}): If $i$ has at least $B$ clients, open $i$ and disconnect $i$ from the tree by cutting the edge $(i, \sigmaone(i))$ else send its clients to its parent facility. The process is repeated till we reach the root. 



There are two possibilities at the root: either we have a facility $i$ from $P$ or we have a root-pair $<i_{r_1}, i_{r_2}>$. In the first case, we are done as $i$ is already open and has at least $B$ clients. To handle the second case, we need to do a little more work. So, we define our assignments of third type as follows (see Fig. \ref{type2-3}): ($i$) If the total number of clients at the root pair $<i_{r_1},i_{r_2}>$ is at least $B$ then open the facility with more number of clients, say $i_{r_1}$ and send the clients of $i_{r_2}$ to $i_{r_1}$. %(in our case, we cannot have a scenario in which both have at least B clients. If $i_2$ is the facility at which the rest of the tree hangs then the number of clients at $i_1$ cannot be more than $B$.....this is not true in Zoya's case because there a tree hangs at both the ends of the double-edge loop which we have eliminated....Since the number of clients at $i_1$ is less than B..the number of clients along any edge is still less than B ....only for our understanding...to be deleted later)..
($ii$) If the total number of clients at the root pair $<i_{r_1},i_{r_2}>$ is less than $B$, then let $i$ be the node in $P$ nearest to $\{i_{r_1}, i_{r_2}\}$. i.e., $i$ is already open and has at least $B$ clients. Send the clients of $i_{r_1}$ and $i_{r_2}$ to $i$.
\begin{figure}[t]
	\begin{tabular}{ccc}
		\includegraphics[width=40mm,scale=1.0]{figures/Type 2 Assignments.jpg}
		&& 
		\includegraphics[width=65mm,scale=1.0]{figures/Type 3 Assignments.jpg} 	
		\\
		\textbf{(A)}&&\ \ \textbf{(B)}& \ \
	\end{tabular}
	\caption{$B=4$ (A) Type 2 Assignments: (a) Before assignments. (b) After assignments.
	(B) Type 3 Assignments (i) Total clients at root pair $<i_{r_1},i_{r_2}>$ is at least $B$: (a) Before assignments. (b) After assignments: $i_{r_2}$ is open.  (ii) Total clients at root pair $<i_{r_1},i_{r_2}>$ is less than $B$: (a) Before assignments. (b) After assignments: $i_{r_1},i_{r_2}$ are both closed. 
	}
	\label{type2-3}
\end{figure}

%($i$) If both $i_1$ and $i_2$ have at least $B$ clients, open bot of them ($ii$) if one of them say $i_1$ has at least $B$ clients but $i_2$ doesn't then open $i_1$ and send the clients of $i_2$ to $i1$ ($iii$) If both of them have clients less than $B$ but in total they have at least $B$ clients, open any one of them, say $i_1$ and send the clients of the other to $i_1$.
 
 
 Next we bound the capacity violation: Let $\pi_i$ be the number of clients assigned to the facility $i$ after first type of re-assignments. Then as shown earlier, $\pi_i \le \beta U$. Let $ i_c$ be the only child of the root (/root pair). Let $i$ be the parent of $ i_c$. In second and third types of assignments,  we never collect more than $2B$ clients at any node till we reach $i_c$. Now we have the following scenarios: Suppose $ i_c$ has less than $B$ clients, we have the following cases: ($i$)  the root node $i$ is in $P$ and it gets additional at most $B$ clients from $i_c$ making a total of at most $\pi_i + B \le \beta U + B \le (\beta + 1) U$ clients at $i$.
 ($ii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at least $B$. Number of clients at $i_{r_1}$ and $i_{r_2}$ are at most $B$ and $2B$ respectively. Thus, the number of clients the opened facility gets is at most $3B \le 3 U$.
 ($iii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients less than $B$. Number of clients at the root pair and their nearest facility in $P$ are at most $B$ and $\beta U$ respectively. Thus, the number of clients the opened facility in $P$ gets is at most $\beta U + B \le (\beta + 1) U$. 
 %The case when $i_c$ has at least $B$ clients leads to the third scenario above and hence handled.
 
 We next bound the connection cost: the cost of first type of re-assignments is same as that of $AS_{cap}$.
 To bound the connection cost of second type, observe that we never send more than $B$ clients on any edge. 
 %In the second type of assignment, 
 Let a facility $i$ sends its (at most $B$ clients) to its parent. Since the facility $i$ was opened in $AS_{cap}$, it pays facility cost of $\delta l(i) min \{n_i, B\} \ge \delta l(i) \alpha B$. Summing over all $i \in \bar P$ for the second type of re-assignments, we see that the total connection cost in these re-assignments is bounded by $3 Cost_f(AS_{cap})/\alpha \delta$ where $Cost_f(.)$ is the facility opening cost of a solution to the $I_{cap}$ instance. For the third type of re-assignments, the cost of sending (at most $B$) clients by a facility $i$ in the root pair $<i_{r_1}, i_{r_2}>$ is not bounded by $B l(i)$. We bound the cost as follows: the total number of clients, initially at $i_{r_1}$ and $i_{r_2}$ was $\ge 2 \alpha B$. However, during re-assignments of type $1$, some of them got reassigned to other facilities. Note that these (other) facilities must have been closed in $AS_{cap}$ and hence do not belong to $\bar P$. Hence, each of these reassignments correspond to an assignment in $AS_{cap}$ whose cost was at least $l(i)$ and a total of at least $(2\alpha  - 1)B l(i)$. Hence the cost of type $3$ re-assignments is bounded by $3 Cost_c(AS_{cap})/ (2\alpha  - 1)$ where $Cost_c(.)$ is the connection cost of a solution to the $I_{cap}$ instance. Hence the total cost of solution $S_1$  is $6\alpha/(2\alpha-1)$ for $\delta= (2\alpha-1)/6\alpha^2$.
 


==> LBUFL.tex <==
\section{Instance $I_1$ and $I_2$}
\label{instI1}

In this section, we first transform instance $I$ to instance $I_1$ ($\facilityset,~\clientset,~f^1,~c,~\B,~\capacityU$) of LBUBFL by moving the clients to the facilities serving them in the tri-criteria solution $S^t$ and then transform $I_1$ to an instance $I_2$ of LBFL by removing the facilities not opened in $S^t$.
%Let $\facilityset^t$ be the set of facilities opened by $S^t$. 
Recall that for a client $j$,  $\sigma^t(j)$ is the facility  in $\facilityset^t$ serving $j$. For $i \in \facilityset^t$, let $n_i$ be the number of clients served by $i$ in $S^t$, i.e., $n_i = |(\sigma^t)^{-1}(i)|$ and for $i \notin \facilityset^t$, $n_i = 0$. Move these clients to $i$ (see Fig.~\ref{Mapping1}). Thus, there are $n_i$ clients co-located with $i$. In $I_1$, our facility set is $\facilityset$ and the clients are at their new locations. Facility opening costs in $I_1$ are modified as follows: $f^1_i = 0$ for $i \in \facilityset^t$ and $=f_i$ for $i \notin \facilityset^t$.  


\begin{lemma}
Cost of optimal solution of $I_1$ is bounded by $Cost_I(S^t) + Cost_I(O)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_1$ of $I_1$: open $i$ in $S_1$ iff it is opened in $O$. Assign $j$ to $i$ in $S_1$ iff it is assigned to $i$ in $O$. $S_1$ satisfies both the lower bound as well as the upper bound as $O$ does so. For a client $j$, let $\sigma^*(j)$ be the facility serving $j$ in $O$. Then, the cost $\dist{ \sigma^t(j)}{\sigma^*(j))}$ of serving $j$ from its new location, $\sigma^t(j)$ is bounded by $\dist{j}{\sigma^t(j)} +\dist{j}{\sigma^*(j)}$ (see Fig. \ref{lemma1}). Summing over all $j \in \clientset$ and adding the facility opening costs, we get the desired claim.

\begin{figure}[t]
    \centering
    \includegraphics[width=4cm]{Figures/lemma 1.jpg}
    \caption{$c( \sigma^t(j), \sigma^*(j)) \leq c(j, \sigma^t(j)) + c(j, \sigma^*(j))$ }
    \label{lemma1}
\end{figure}
\end{proof}

\begin{figure}[t]
    \centering
    \includegraphics[width=9cm]{Figures/Mapping_0.jpg}
    \caption{Transforming instance $I$ to $I_1$ and  $I_1$ to $I_2$. Solid squares represent clients and circles represent facilities. Clients are moved to the facilities serving them in $S^t$ while transforming $I$ to $I_1$. Facilities not opened in $S^t$ are dropped while going from $I_1$ to $I_2$.}
    \label{Mapping1}
\end{figure} 

%section{Instance $I_2$} 
%\label{instI2}
    
   Next, we define an instance ~$I_2(\facilityset^t,~\clientset,~f^2,~c,~\B)$ of LBFL from $I_1$ by removing the facilities not in $\facilityset^t$ and ignoring the upper bounds. Instance $I_2$ is same as $I_1$ without the upper bounds, except that the facility set is $\facilityset^t$ now. Thus, $f^2_i = 0~\forall~i \in \facilityset^t$. % We will show that there exists a feasible solution $S_2$ of $I_2$ such that $Cost(S_2)$ is bounded by $2 Cost(O_1)$ where
  Let $O_1$ be an optimal solution of $I_1$. 
  For a client $j$, let $\sigma^1(j)$ be the facility serving $j$ in $O_1$.
 
 
 

\begin{lemma}
Cost of optimal solution of $I_2$ is bounded by $ 2Cost_{I_1}(O_1)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_2$ to $I_2$: for $i \in \facilityset^t$, open $i$ in $S_2$ if it is opened in $O_1$ and assign a client $j$ to it if it is assigned to $i$ in $O_1$. For a facility $i \notin \facilityset^t$, %the clients assigned to it need to be assigned to some other facility in $\facilityset^t$. Thus, for such $i$'s,
open its nearest facility $i'$ \textcolor{olive}{(if not already opened)} in $\facilityset^t$. Assign $j$ to $i'$ in $S_2$ if it is assigned to $i$ in $O_1$. $S_2$ satisfies the lower bound  as $O_1$ does so. Note that it need not satisfy the upper bounds. This is the reason we dropped upper bounds in $I_2$. The cost $c( \sigma^t(j), i')$
%$c( \sigma^t(j), \sigma^*(j))$ 
of serving $j$ from its new location is bounded by $c(\sigma^t(j), \sigma^1(j)) + c( \sigma^1(j), i') \le 2 c(\sigma^t(j), \sigma^1(j))$ (since $i'$ is closest in $\facilityset^t$ to $i =  \sigma^1(j)$). Summing over all $j \in \clientset$ we get the desired claim.
%$c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(i, \sigma^1(j)) \le c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(\sigma^t(j), \sigma^1(j))$ (since $i$ is closest in $\facilityset^t$, to $i' = \sigma^1(j)$) $\le 2(c(j, \sigma^t(j)) + c(j, \sigma^1(j)))$ (See Figure 1). Summing over all $j$'s, the claim follows.
%Same as Zoya etal
\end{proof}

%\textcolor{blue}{can be deleted now...I have added a line in the proof itself....Note that, while defining the instance $I_2$, we ignored the upper bounds on facilities because a facility $i' \in \facilityset^t$ might be nearest to many other facilities $\notin \facilityset^t$ thereby serving clients of all of them and hence violating upper bound.}


\section{Instance $I_{cap}$ of Capacitated Facility Location Problem}
\label{instIcap}

 
 In this section, we create an  instance $I_{cap}$ of capacitated facility location problem from $I_2$. 
 The main idea is to create  a demand of $\B - n_i$ units at locations where the number of clients served by the facility is less than $\B$ and a supply of $n_i - \B$ units at locations with surplus clients. For each facility $i \in \facilityset^t$, let $l(i)$ be the distance of $i$ from a nearest facility  $i' \in \facilityset^t$, $i' \neq i$ and let $\delta$ be a constant to be chosen appropriately. A facility $i$ is called {\em small} if $0< n_i \leq \B$ and  {\em big} otherwise. A big facility $i$ is split into two co-located facilities $i_1$ and $i_2$.
  We also split the set of clients at $i$ into two sets:  arbitrarily, $\B$ of these clients are placed at $i_1$ and the remaining $n_i - \B$ clients at $i_2$ (see Fig.~\ref{Mapping2}). 
   Instance $I_{cap}$ is then defined as follows:
A {\em small} facility $i$ needs additional $\B - n_{i}$ clients to satisfy its lower bound; hence a demand of $\B - n_{i}$ is created at $i$ in the $I_{cap}$ instance. A facility with capacity $\B$ and facility opening cost $\delta n_{i} l(i)$ is also created at $i$. 
For a {\em big} facility $i$, correspondingly two co-located facilities $i_1$ and $i_2$ are created with capacities $\B$ and $n_i - \B$ respectively. The facility opening cost of $i_1$ is $\delta \B l(i)$ whereas $i_2$ is free. Intuitively, since the lower bound of a big facility is satisfied, it has some extra ($n_i - \B$) clients , which can be used to satisfy the demand of clients in $I_{cap}$ for free. 
 %Thus, we define capacity of $i_1$ and $i_2$ to be $\B$ and $n_i - \B$ respectively. 
 The second type of big facilities are called {\em free}. 
 %The facility costs, capacities and demands are as shown in
 We use $i$ to refer to both the client (with demand) as well as the facility located at $i$. Let $\bar \facilityset^t$ be the set of facilities so obtained. The set of clients and the set of facilities are both $\bar \facilityset^t$. Table~\ref{tab:my_label} summarizes the instance. Also see Fig.~\ref{Mapping2}
 
 \begin{figure}
    \centering
    \includegraphics[width=8cm]{Figures/Mapping_1.jpg}
    \caption{Transforming instance $I_2$ to $I_{cap}$: $\B = 4$,
    %Solid squares represent clients and circles represent facilities. 
    $i'$ is small, $i$ is big.
    $i$ is split into $i_1$ and $i_2$ while transforming $I_2$ to $I_{cap}$, $i_2$ is free. Demand at the small facility $i'$ is $\B - n_{i'} = 1$ and at $i_1$, $i_2$, it is $0$. Capacities of $i'$ and $i_1$ are $\B = 4$ and it is $n_{i} - \B = 3$ of the free facility $i_2$.}
    \label{Mapping2}
\end{figure}
 
 \begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
       Type & $n_i$ & $u_i$ & $d_i$ & $f^t_i$ \\
        \hline
       {\em small} & $n_i \leq \B$ & $\B$ & $\B- n_i$& $\delta n_i l(i)$ \\
        \hline
       {\em big} & $n_i > \B$ & ($i_1$)$\B$ & $0$& $\delta \B l(i)$ \\
        & & ($i_2$) $n_i - \B$ & $0$& $0$ \\
       
        % &  &
          \hline 
       % $3$ & $0$ & $\B$ & $\B$& $\delta \B l(i)$ \\
        %\hline
    \end{tabular}
    \caption{Instance of $I_{cap}$: $d_i, u_i, f^t_i$ are demands, capacities and facility costs resp.}
    \label{tab:my_label}
\end{table}
 
 %Let $O_{cap}$ be an optimal solution to $I_{cap}$.
 
 %\textcolor{red}{define delta and l(i)}
 %The second type of big facilities are called {\em free}. %and the clients placed at them are also called {\em free}. 
 %Let $F_f$ denote the set of free facilities. 
 %and $Cf(i)$ denote the set of free clients at facility $i \in F_b$. i.e.$Cf(i)$ is the set of clients placed at $i_2 \in F_f$ (See Figure 2)....need to define $l(i)$.

 %In the next lemma, we show the existence of a feasible solution to $I_{cap}$ with cost no more than $(1+2\delta)Cost(O_2)$ where $O_2$ is an optimal solution of $I_2$. 




\begin{lemma}
%A feasible solution $S_{cap}$ for 
Let $O_2$ be an optimal solution of $I_2$. Then, cost of optimal solution to $I_{cap}$ is bounded by $(1+2\delta)Cost_{I_2}(O_2)$.
\end{lemma}

\begin{proof}
We will construct a feasible solution $S_{cap}$ to $I_{cap}$ of bounded cost from $O_2$.
 As $O_2$ satisfies the lower bound,  we can assume wlog that if $i$ is opened in $O_2$ then it serves all of its clients if $n_i \le \B$ (before taking more clients from outside) and it serves at least $\B$ of its clients before sending out its clients to other (small) facilities otherwise. 
Also, if two big facilities are opened in $O_2$, one does not serve the clients of the other. Let $\rho^2(j_i, i')$ denote the number of clients co-located at $i$ and assigned to $i'$ in $O_2$ and $\rho^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $S_{cap}$.
 \begin{figure}[t]
    \centering
    \includegraphics[width=10cm]{Figures/O2_Scap_assignments.jpg}
    \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ and $i'$ are closed in $O_2$. $\rho^2(j_{i_1}, t_1) = 2,~\rho^2(j_{i_1}, t_2) = 1,~\rho^2(j_{i_1}, t_3) = 1,~ \rho^2(j_{i_1}, t_4) = 0$ and $\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 1,~\rho^2(j_{i_2}, t_3) = 1,~ \rho^2(j_{i_2}, t_4) = 0$.  } %The middle figure shows how the assignments look like after splitting the big facilities. $\rho^2(j_{i_1}, i') = 2(/1/1)$ for $i'$ = top three facilities $t_1(/t_2/t_3)$ $\rho^2(j_{i_2}, i') = 1(/1/1) $ for the bottom three facilities $t_2(/t_3/t_4)$. Note that $t_1$ }
    \label{Mapping}
\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{Figures/O2_Scap assignments (2.1).jpg}
   \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ is open in $O_2$.   $\rho^c(j_{t_1}, i_2) = \rho^2(j_{i}, t_1) = 1, \rho^c(j_{t_2}, i_2) = \rho^2(j_{i}, t_2) = 2$,
  % $\rho^2(j_{i_1}, t_1) = 1,~\rho^2(j_{i_1}, t_2) = 1$ and %$\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 2$. 
   $i_2$ is open in $S_{cap}$. $t_1$ and $t_2$ must be small.}
    \label{O2_SCap2}
\end{figure}
    \begin{enumerate}
        \item   if $i$ is closed in $O_2$ then open $i$ if $i$ is small
        and open $(i_1 \& i_2)$ if it is big.
        
        Assignments are defined as follows (see Fig.~\ref{Mapping}):
        \begin{enumerate}
        
        \item If $i$ is small: Let $i$ serve its own demand. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. 
        \textcolor{green}{
        Note that the same cannot be done when $i'$ is big as there is no demand at $i'_1$ and $i'_2$. } Thus,  $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $ i' \ne i$ and $\rho^c(j_i, i) = d_i$. Also, $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). 
        Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = \B = u_i$. 
      
       % \item If $i$ is small: Let $i$ serve its own demand, \textcolor{blue}{i.e., $\rho^c(j_i, i) = d_i$}. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. \textcolor{blue}{Note that $i'$ must be small in this case. But y not big?????? I think it can be big as well, the only thing that will differ is $\rho^c(j_{i'}, i) = 0$ if $i'$ is big.} Thus, $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $i' \ne i$. Also, $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = \B = u_i$. \textcolor{blue}{Thus capacities are respected.}
        
       \item If $i$ is big: assign $\rho^2(j_{i_1}, i')$ (/$\rho^2(j_{i_2}, i')$) demand of $i'$ to $i_1$(/$i_2$) in our solution for small $i' \ne i$. Thus,
        $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_1) = \sum_{small~i' \ne i} \rho^2(j_{i_1}, i') \le \B = u_{i_1}$. Also,
         $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_2) \\ = \sum_{small~i' \ne i} \rho^2(j_{i_2}, i') \le n_i - \B = u_{i_2}$.
       %The second equality holds in each case as $i$ is closed in $O_2$.
        %\textcolor{green}{.....Is this the reason? Sapna...Pls see..}
        % Since there are no demands at $i_1$ and $i_2$, the capacities are respected.
     
       \end{enumerate}
     
     \item If $i$ is opened in $O_2$ and is big, open the free facility $i_2$ (see Fig.~\ref{O2_SCap2}): assign $\rho^2(j_{i}, i')$  demand of $i'$ to $i_2$ in our solution for small $i' \ne i$. Thus,
     %Thus,
      %  $\sigma^c(j_{i'}, i_2) = %\sigma^1(j_{i_2}, i'), i \ne i'$  
        $\sum_{i' \ne i}\rho^c(j_{i'}, i_2) = \sum_{i' \ne i} \rho^2(j_{i}, i') \le n_i - \B$ (the inequality holds by assumption on $O_2$) $= u_{i_2}$.
       % Thus the capacities are respected as there are no demands at $i_2$.
    \end{enumerate}
    
    Thus capacities are respected in each of the above cases. Next, we show that all the demands are satisfied. If a facility is opened in $S_{cap}$, it satisfies its own demand. 
Let $i$ be closed in $S_{cap}$. If $i$ is big ,we need not worry as $i_1$ and $i_2$ have no demand. So, let $i$ is small. Then, it must be opened in $O_2$. Then, 
$\sum_{i' \ne i}\rho^c(j_{i}, i') = $
$\sum_{small ~i' \ne i,  }\rho^c(j_{i}, i') + \sum_{i'_1: i' ~is ~big}\rho^c(j_{i}, i'_1) + 
\sum_{i'_2: i' ~is ~big}\rho^c(j_{i}, i'_2)= $
$\sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i'_1 : i' ~is ~big} \rho^2(j_{i'_1}, i)  + \\ \sum_{i'_2 : i' ~is ~big}\rho^2(j_{i'_2}, i)= \sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i' ~is ~big} \rho^2(j_{i'}, i) = \sum_{i' \ne i}\rho^2(j_{i'}, i)$
$\ge \B - n_i$  (since $O_2$ is a feasible solution of $I_2$) $= d_i$. 



Next, we bound the cost of the solution. The connection cost is \textcolor{olive}{at most that of $O_2$. } %same as 
\textcolor{green}{ or at most? we didn't bring back if anything went from i to i' in O2 where i' is big.}
%Next, we consider the facility opening costs. 
For facility costs, consider a facility $i$ that is opened in our solution and closed in $O_2$. Such a facility must have paid a cost of at least $n_i l(i)$ to get its clients served by other (opened) facilities in $O_2$. The facility cost paid by our solution is $ \delta min\{n_i, \B\} l(i) \le \delta n_i l(i)$. If $i$ is opened in $O_2$, then it must be serving at least $\B$ clients and hence paying a cost of at least $\B l(i)$ in $O_2$. In this case also, the facility cost paid by our solution is $ \delta min\{n_i, \B\} l(i) \le \delta \B l(i)$.  Summing over all $i$'s, we get %\textcolor{blue}{$FCost_{I_{cap}}(S_{cap}) \leq 2 \delta Cost_{I_2}(O_2)$, where $FCost_{\cdot}(\cdot)$ is the facility opening cost of a solution to $I_{cap}$ instance.} 
that the facility cost is bounded by $2 \delta Cost_{I_2}(O_2)$ and the total cost is bounded by $(1 + 2 \delta) Cost_{I_2}(O_2)$. Factor $2$ comes because we may have counted an edge $(i, i')$ twice, once as a client when $i$ was closed and once as a facility when $i'$ was opened in $O_2$.  
\end{proof}


% ****I am here - NG***** 

\section{Bi-criteria Solution $S_1$ to $I_1$ from approximate solution $AS_{cap}$ to  $I_{cap}$} \label{bi-criteria}

In this section, we obtain a solution $S_1$ to $I_1$ that violates the capacities/upper bounds by a factor of $(\beta + 2)$ without violating the lower bound. We first obtain an approximate solution $AS_{cap}$ to $I_{cap}$ using any approximation algorithm \cite{Bansal}.  $AS_{cap}$ is then used to construct $S_1$.
Wlog assume that if a facility $i$ is opened in $AS_{cap}$ then it serves all its demand.\textcolor{green}{ May have to add a couple of lines here in view of the reviews of one of the reviewer: If this is not true, we can modify the $AS_{cap}$  and obtain another solution that satisfies this condition, of cost no more than that of $AS_{cap}$....will see if we can briefly say how we can modify $AS_{cap}$.}
This is always feasible as $d_i \le u_i$. $S_1$ is obtained from $AS_{cap}$ by first defining the assignment of the clients and then opening the facilities that get at least $\B$ clients. Let $\rhobar^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $AS_{cap}$ and $\rhobar^1(j_i, i')$ denotes the number of clients co-located at $i$ and assigned to $i'$ in $S_1$. 
%\textcolor{red}{ Initially each facility is assigned the clients co-located with it.}
Clients are assigned in three steps. In the first step, assign the clients co-located at a facility to itself. 
For small $i'$, additionally, we do the following  (type - $1$) re-assignments (see Fig. \ref{type1}): $(i)$ For small $i \ne i'$, assign $\rhobar^c(j_{i'}, i)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for small $i$. $(ii)$ For big $i$, assign $\rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ for big $i$. 
Claim ~\ref{claim1} shows that these assignments are feasible and the capacities are violated only upto the extent to which they were violated by the tri-criteria solution $S^t$. 
\begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{Figures/Type 1 Assignments.jpg}
    \caption{($a$) $\B =5$, $t_1, t_2, t_3$ have demands $1$, $2$ and $1$ unit each respectively. In solution $AS_{cap}$, $1$ unit of demand of $t_1$ and $2$ units of demand of $t_2$ are assigned to $t_3$. (b) Solution $S_1$: initially, $n_i$ clients are initially assigned to facility $i$. (c) Type $1$ reassignments: $1$ and $2$ clients of $t_3$ reassigned to $t_1$ and $t_2$ respectively. After this reassignment, $t_3$ has only $1$ client.}
    \label{type1}
\end{figure}

\begin{claim}
\label{claim1}
    $(i)$ $\sum_{i' \ne i} \rhobar^1(j_i, i') \le n_i$, $\forall$ $i \in \bar \facilityset^t$.
    $(ii)$ $\sum_{i} \rhobar^1(j_i, i') \le max\{\B, n_{i'}\} \le \beta \capacityU$, for $\beta \ge 1$, $\forall$ $i' \in \bar \facilityset^t$.
 \end{claim}

\begin{proof}

    $(i)$ Since $\rhobar^c(j_{i}, i) = d_i$ therefore $\sum_{i' \ne i} \rhobar^1(j_i, i') = \sum_{i' \ne i} \rhobar^c(j_{i'}, i) \le u_i - d_i \le n_i$ in all the cases. $(ii)$ $\rhobar^1(j_{i'}, i') = n_{i'}$. For $ i \ne i'$, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$. Thus, $\sum_{i} \rhobar^1(j_i, i') = n_{i'} + \sum_{i \ne i'} \rhobar^c(j_{i'}, i) \le n_{i'} + d_{i'} \le max\{\B, n_{i'}\} \le \beta \capacityU$.
\end{proof}

Note that $S_1$ so obtained may  still not satisfy the lower bound requirement. In fact, although each facility was assigned $n_i \ge  \alpha \B$  clients initially, they may be serving less clients now after type $1$ re-assignments. For example, in Fig. \ref{type1}, $t_3$ had $4$ clients initially which was reduced to $1$ after type $1$ reassignments. Let $P \subseteq  \facilityset^t$ be the set of facilities each of which is serving at least $\B$ clients after type-$1$ reassignments, and  $\bar P =  \facilityset^t \setminus P$ be the set of remaining facilities. 
 %That is, $ P= \{ i' \in \facilityset^t: \sum_{i}\rhobar^1(j_{i}, i') \ge \B$\}.
 We open all the facilities in $P$ and let them serve the clients assigned to them after type $1$ reassignments.
 
 \begin{observation}
    If a  small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge \B$. Similarly for a big facility $i'$, if $i'_1$ was closed in $AS_{cap}$ then $i'$ is in $P$.
     %\item If a small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge \B$.
    
     
    % \item If $i'$ is big then $\rhobar^1(j_{i'}, i') = n_{i'}  \ge \B$
 \end{observation}
 
 
 Thus, a small facility is in $\bar P$ only if it was open in $AS_{cap}$ and a big facility $i$ is in $\bar P$ only if $i_1$ was open in $AS_{cap}$. 
 %Also note that although each facility in $\bar P$ served at least $\alpha \B \ge \B/2$ clients in the tri-criteria solution $S^t$, they may be serving less clients now after step $1$ of assignment. \textcolor{red}{See Figure \ref{type1} for an example}.
 We now group these facilities so that each group serves at least $\B$ clients and open one facility in each group that serves all the clients in the group. For this we construct what we call as {\em facility trees}. We construct a graph $G$ with nodes corresponding to the facilities in \textcolor{olive}{$P \cup \bar P$.} For $i \in \bar P$, let $\eta(i)$ be the nearest other facility to $i$ in $\facilityset^t$. Then, $G$ consists of edges $(i, \eta(i))$. Each component of $G$ is a tree except possibly a double-edge cycle at the root. In this case, we say that we have a root, called {\em root-pair} $<i_{r_1}, i_{r_2}>$ consisting of a pair of facilities $i_{r_1}$and $ i_{r_2}$. Also, a facility $i$ from $P$, if present, must be at the root of a tree. 
 \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{Figures/tree.jpg}
    \caption{Binary tree conversion process: (a) Tree $\mathcal{T}$ of unbounded degree: $a<b<c<g,~c<d$. (b) Binary routing tree (intermediate stage). (c) Final tree.}
    \label{tree}
\end{figure}

We process each tree bottom-up sending the clients of each facility to its parent. However doing so may result in too much violation in the capacities at the parent facility. To keep the capacity violation in check, we convert each tree into a binary tree (see Fig. \ref{tree}): first of all, we treat the double-edge cycle, if any, as a single node for this purpose. Then, at every node $x$, arrange the children of $x$ from left to right in non-decreasing order of distance from $x$. For each child $y$ (except for the nearest child) of $x$, add an edge to its left sibling %with weight $2\dist{ y}{\eta(y)}$ 
and remove the edge $( y, x)$. There is no change in the outgoing edge of the leftmost child of $x$. Let $\sigmaone(y)$ be the parent of $y$ in the so constructed tree.  

\begin{lemma}
For any node $y$ in the binary tree, $\dist{y}{\sigmaone(y)} \leq 3 \dist{y}{\eta(y)}$. 
\end{lemma} 
\begin{proof}
Let $\mathcal{T}$ be a tree.
For any node $x$ that is not a root pair, it is easy to see that $\dist{y}{\sigmaone(y)} \leq 2 \dist{y}{\eta(y)}$ for all children $y$ of $x$. Next consider a root pair $<r_1, r_2>$. Let 
$\cone_1 \ldots \cone_k$ 
be the children of $r_1/r_2$ in the increasing order of
$\dist{\cone_i}{\eta(\cone_i)}$. Then $\psi(\cone_i) = \cone_{i-1}$ for $i = 2 \ldots k$ and $\psi(\cone_1) = \eta(\cone_1)$. If,  for $i = 2 \ldots k$, $\eta(\cone_i) = \eta(\psi(\cone_i)) (= r_1/r_2)$ (i.e. $\cone_i$ and $\psi(\cone_i)$ are children of the same node ($r_1/r_2$)), then  $\dist{\cone_i}{\sigmaone(\cone_i)} \leq 2 \dist{\cone_i}{\eta(\cone_i)}$. Otherwise (see Figure~\ref{}), $\dist{\cone_i}{\sigmaone(\cone_i)} \leq \dist{\cone_i}{\eta(\cone_i)} + \dist{\eta(\cone_i)}{\eta(\cone_{i-1})} + \dist{\eta(\cone_{i-1})}{\cone_{i-1}} \le 3 \dist{\cone_i}{\eta(\cone_i)}$. \end{proof}





%Its easy to see that $\dist{y}{\sigmaone(y)} \leq 3 \dist{y}{\eta(y)}$. 
Thus, we replace $\dist{y}{\sigmaone(y)}$ by $3 \dist{y}{\eta(y)}$ for all $y$. Henceforth, whenever we refer to distances, we mean the new edge weights. Now, every node has in-degree of at most $2$ with the in-degree of the root being at most $1$. 

Now we are ready to define our second type of re-assignments.
\textcolor{violet}{Process the tree bottom-up using Algorithm~\ref{} until we reach the root node, which could be either a single facility in $P$ or a root-pair. Processing of the root-pair node is slightly different and is explained in Algorithm~\ref{}
}
 Let $ i_c$ be the only child, if any,  of the root (/root pair) of a tree. Let $i$ be the parent of $ i_c$ ($i$ is either in $P$ or it is one of $i_{r_1}$ and $i_{r_2}$ in case the root is a root pair).
Process the tree bottom-up, til we reach $i_c$, as follows (see Fig. \ref{type2-3} \textcolor{blue}{($A$)}): \\
\textcolor{green}{
Process(i)\\
Process($L_i$), Process($R_i$) \\
If $L_i$ has at least $\B$ clients, open $L_i$ and disconnect $L_i$ from the tree by cutting the edge $(L_i, \sigmaone(L_i))$ and setting $L_i$ to NULL.\\
If $R_i$ has at least $\B$ clients, open $R_i$ and disconnect $R_i$ from the tree by cutting the edge $(R_i, \sigmaone(R_i))$ and setting $R_i$ to NULL.\\
If none of $L_i$ and $R_i$ is NULL, send the clients of $R_i$ to $L_i$. \\
If $L_i(/R_i)$ is non-NULL, send it's clients to $i$.\\
}


\begin{algorithm}[H] 
    \SetAlgoLined
    %\KwData{$\clientset,~\facilityset$}
    %\KwResult{$\clientset',~\bundle{j'}~\forall~j'\in \clientset'$}
    \SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
    \Input{$i$}
    %\Output{}
		 
	% Process($lc_i$)\;
		 
	% Process($rc_i$)\;
		 
		 \textcolor{blue}{$re-assigned(rc_i) = false$ \tcp*{boolean variable to indicate if clients of $rc_i$ are assigned to $lc_i$ or not; initially false}} 
		 
		 
		 
		 \If{$n_{rc_i} \geq \B$}  {
		 
		 Open facility $rc_i$\;
		 
		 Remove edge ($rc_i, \psi(rc_i)$)  \textcolor{blue}{\tcp*{Remove the connection of $rc_i$ from its parent}}
		 
		 $rc_i \gets$ NULL\;
		 
		 }
		 
		 \If{$lc_i \ne $ NULL AND $rc_i \ne $ NULL}  {
		 
		   $n_{lc_i} \gets  n_{lc_i} + n_{rc_i}$
		   
		   	   $re-assigned(rc_i) \gets true$
		   
		    \If{$n_{lc_i} \geq \B$}  {
		 
		 Open facility $lc_i$\;
		 
		 Remove edge ($lc_i, \psi(lc_i)$)\;
		 
		 $lc_i \gets$ NULL\;
		 
		 }
		 }
		 
   	\If{$lc_i \ne $ NULL AND ($re-assigned(rc_i) = true$ OR $rc_i =$ NULL) \textcolor{blue}{Isnt the part after AND condition redundant?? Its not required,I think}} {
		 
		   $n_i \gets  n_i + n_{lc_i}$
		  
		 } 
		 
		 \If{$rc_i \ne $ NULL AND   ($re-assigned(rc_i) \ne true$)}  {
		   $n_i \gets  n_i + n_{rc_i}$ \textcolor{blue}{\tcp*{ $lc_i$ must be NULL in this case.}}
		 }
		
		
	\label{Process_i}
	\caption{Process($i$)}
\end{algorithm}
 
 



(D later: Process the tree bottom-up as follows (see Fig. \ref{type2-3} \textcolor{blue}{($A$)}): 
If $i$ has at least $\B$ clients, open $i$ and disconnect $i$ from the tree by cutting the edge $(i, \sigmaone(i))$ else send its clients to its parent facility. The process is repeated till we reach the root. 

 \begin{lemma}
 \textcolor{red}{
(I think D: Repetition: Let $ i_c$ be the only child, if any,  of the root (/root pair)of a tree. Let $i$ be the parent of $ i_c$ ($i$ is either in $P$ or it is one of $i_{r_1}$ and $i_{r_2}$ in case the root is a root pair).
}
The number of clients collected in the second type of re assignments, at any node $x$  in the subtree rooted at $i_c$, is at most $2\B$.
 \end{lemma}
 
 \begin{proof} 
 \textcolor{violet}{We will show that the number of clients collected at $x$ after Process($x$) is at most $2\B$. For this, note that $x$ receives $< \B$ clients from at most one of it's children. Hence, the claim follows.}
 (to be seen again after finalising the algorithm)
 We will show that the number of clients collected at $i$ after Process($i$) is at most $2\B$. For this, note that if the number of clients collected at both $L_i$ as well as $R_i$ are individually $< \B$, then $R_i$ sends its clients to $L_i$. Thus, $i$ receives clients from at most one of its children in case the child has collected $< \B$ clients. Since all nodes except possibly the root are in $\bar P$, $i$ has at most $\B$ clients of its own. Hence, the claim follows.
 
 \end{proof}


There are two possibilities at the root: either we have a facility $i$ from $P$ or we have a root-pair $<i_{r_1}, i_{r_2}>$. In the first case, we are done as $i$ is already open and has at least $\B$ clients. To handle the second case, we need to do a little more work. So, we define our assignments of third type as follows (see Fig. \ref{type2-3} \textcolor{blue}{($\B$)}): 
($i$) If the total number of clients at   $i_c, i_{r_1}$ and $i_{r_2}$ is at least $\B$ and at most $2\B$ then open the facility with more number of clients from $i_{r_1}$ and $i_{r_2}$, say $i_{r_1}$ and send the clients of $i_c$ and $i_{r_2}$ to $i_{r_1}$.
($ii$) If the total number of clients at $i_c, i_{r_1}$ and $i_{r_2}$ is more than $2\B$  then open both $i_{r_1}$ and $i_{r_2}$, and distribute the clients of $i_c$ so that each one of them gets at least $\B$ clients.
($iii$) If the total number of clients at $i_c, i_{r_1}$ and $i_{r_2}$ is less than $\B$, then let $i$ be the node in $P$ nearest to $\{i_{r_1}, i_{r_2}\}$, then $i$ is already open and has at least $\B$ clients. Send the clients of $i_c, i_{r_1}$ and $i_{r_2}$ to $i$.

($i$) If the total number of clients at the root pair $<i_{r_1},i_{r_2}>$ is at least $\B$ then open the facility with more number of clients, say $i_{r_1}$ and send the clients of $i_{r_2}$ to $i_{r_1}$. %(in our case, we cannot have a scenario in which both have at least \B clients. If $i_2$ is the facility at which the rest of the tree hangs then the number of clients at $i_1$ cannot be more than $\B$.....this is not true in Zoya's case because there a tree hangs at both the ends of the double-edge loop which we have eliminated....Since the number of clients at $i_1$ is less than \B..the number of clients along any edge is still less than \B ....only for our understanding...to be deleted later)..
($ii$) If the total number of clients at the root pair $<i_{r_1},i_{r_2}>$ is less than $\B$, then let $i$ be the node in $P$ nearest to $\{i_{r_1}, i_{r_2}\}$, i.e., $i$ is already open and has at least $\B$ clients. Send the clients of $i_{r_1}$ and $i_{r_2}$ to $i$.
\begin{figure}[t]
	\begin{tabular}{ccc}
		\includegraphics[width=40mm,scale=1.0]{Figures/Type 2 Assignments.jpg}
		&& 
		\includegraphics[width=65mm,scale=1.0]{Figures/Type 3 Assignments.jpg} 	
		\\
		\textbf{(A)}&&\ \ \textbf{(B)}& \ \
	\end{tabular}
	\caption{$\B=4$ (A) Type 2 Assignments: (a) Before assignments. (b) After assignments.
	(B) Type 3 Assignments (i) Total clients at root pair $<i_{r_1},i_{r_2}>$ is at least $\B$: (a) Before assignments. (b) After assignments: $i_{r_2}$ is open.  (ii) Total clients at root pair $<i_{r_1},i_{r_2}>$ is less than $\B$: (a) Before assignments. (b) After assignments: $i_{r_1},i_{r_2}$ are both closed. 
	}
	\label{type2-3}
\end{figure}

%($i$) If both $i_1$ and $i_2$ have at least $\B$ clients, open bot of them ($ii$) if one of them say $i_1$ has at least $\B$ clients but $i_2$ doesn't then open $i_1$ and send the clients of $i_2$ to $i1$ ($iii$) If both of them have clients less than $\B$ but in total they have at least $\B$ clients, open any one of them, say $i_1$ and send the clients of the other to $i_1$.
 
 
% \textcolor{red}{need to see this part again}
 %Next we bound the capacity violation:  Let $\pi_i$ be the number of clients assigned to the facility $i$ after first type of re-assignments. Then as shown earlier, $\pi_i \le \beta \capacityU$. (Reptn:D: Let $ i_c$ be the only child of the root (/root pair). Let $i$ be the parent of $ i_c$. In second and third types of assignments,  we never collect more than $2\B$  \textcolor{red}{additional $2\B$, no?}  clients at any node till we reach $i_c$ \textcolor{blue}{Can we shift this statement to case ii where it is used??}. )
% Now we have the following scenarios: Suppose $ i_c$ has less than $\B$ clients, we have the following cases: ($i$)  the root node $i$ is in $P$ and it gets additional at most $\B$ clients from $i_c$ making a total of at most $\pi_i + \B \le \beta \capacityU + \B \le (\beta + 1) \capacityU$ clients at $i$. ($ii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at least $\B$. Number of clients at $i_{r_1}$ and $i_{r_2}$ are at most $\B$ and $2\B$ respectively. Thus, the number of clients the opened facility gets is at most $3\B \le 3 \capacityU$. ($iii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients less than $\B$. Number of clients at the root pair and their nearest facility in $P$ are at most $\B$ and $\beta \capacityU$ respectively. Thus, the number of clients the opened facility in $P$ gets is at most $\beta \capacityU + \B \le (\beta + 1) \capacityU$. 
 
  Next, we bound the capacity violation: 
 Let $\pi_i$ be the number of clients assigned to the facility $i$ after first type of re-assignments. Then as shown earlier, $\pi_i \le \beta \capacityU$.  Let $i$ be the parent of $ i_c$. In second and third types of assignments,  we never collect  more than $2\B$ clients at any node till we reach $i_c$.
 Now we have the following scenarios: Suppose $ i_c$ has less than $\B$ clients, we have the following cases: ($i$) the root node $i$ is in $P$ and it gets additional at most $\B$ clients from $i_c$ making a total of at most $\pi_i + \B \le \beta \capacityU + \B \le (\beta + 1) \capacityU$ clients at $i$.
 ($ii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at $i_c, i_{r_1}$ and $i_{r_2}$ is at least $\B$ and at most $2\B$. Thus, the number of clients the opened facility gets is at most $2\B \le 2\capacityU$.
 ($iii$)  the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at $i_c, i_{r_1}$ and $i_{r_2}$ is more than $2\B$.  Note that the total number of clients at these facilities is at most $3\B$ and hence it is possible to distribute them to the two opened facilities $i_{r_1}$ and $i_{r_2}$ so that each of them gets at most $2\B \le 2\capacityU$ clients. ($iv$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at $i_c, i_{r_1}$ and $i_{r_2}$ is less than $\B$. 
 %Number of clients at $i_c$ and the root pair and, their nearest facility in $P$ are at most $\B$ and $\beta \capacityU$ respectively. 
 Thus, the number of clients the opened facility in $P$ gets is at most $\beta \capacityU + \B \le (\beta + 1) \capacityU$. 
 %The case when $i_c$ has at least $\B$ clients leads to the third scenario above and hence handled.
 
 
 We next bound the connection cost: the cost of first type of re-assignments is \textcolor{olive}{at most the connection cost of $AS_{cap}$.} 
% \textcolor{red}{(or at most?Sapna/rajni) }
 To bound the connection cost of second type, observe that we never send more than $\B$ clients on any edge. 
 %In the second type of assignment, 
 Let a facility $i$ sends its (at most $\B$ clients) to its parent or to its left sibling. Since the facility $i$ was opened in $AS_{cap}$, it pays facility opening cost of $\delta l(i) min \{n_i, \B\} \ge \delta l(i) \alpha \B$. Summing over all $i \in \bar P$ for the second type of re-assignments, we see that the total connection cost in these re-assignments is bounded by 
 \textcolor{red}{
 $3 FCost_{I_{cap}}(AS_{cap})/\alpha \delta$ (Sapna...to be seen)
 } \textcolor{olive}{$\sum_{i \in \bar P} \B l(i) \leq 6FCost_{I_{cap}}(AS_{cap})/\alpha \delta$  where factor 6 comes because sending clients to the left sibling incurs a cost of twice the cost to the node's parent and $FCost_{I_{cap}}(AS_{cap})$ is the facility opening cost of a solution to $I_{cap}$ instance.}
% \textcolor{red}{define FCost}
  %of edge weights being thrice of their original weight during the formation of binary tree.
 %\textcolor{blue}{ \st {where $Cost_f(.)$ is the facility opening cost of a solution to the $I_{cap}$ instance }}


 For the third type of re-assignments, we bound the cost in two parts: ($a$) cost of sending ($< \B$) clients of $i_c$ to it's parent ($b$) Cost of sending ($< \B$) clients collected at the root pair $<i_{r_1}, i_{r_2}>$ to it's nearest facility in $P$. Cost of the first part is bounded by $\B l(i_c)$. The cost of sending ($< \B$) clients by a facility $i$ in the root pair $<i_{r_1}, i_{r_2}>$ is not bounded by $\B l(i)$ (where $l(i) = l(i_{r_1}) = l(i_{r_2})$). We bound the cost as follows: the total number of clients, initially at $i_{r_1}$ and $i_{r_2}$ was $\ge 2 \alpha \B$. However, during re-assignments of type $1$, some of them got reassigned to other facilities. Note that these (other) facilities must have been closed in $AS_{cap}$ and hence do not belong to $\bar P$. Hence, each of these reassignments correspond to an assignment in $AS_{cap}$ whose cost was at least $l(i)$ and a total of at least $(2\alpha  - 1)\B l(i)$. Hence the cost of type $3$ re-assignments is bounded by \textcolor{blue}{$3 CCost_{I_{cap}}(AS_{cap})/ (2\alpha  - 1)$ where $CCost_{I_{cap}}(AS_{cap})$ is the connection cost of $AS_{cap}$ solution.} Hence the total cost of solution $S_1$  is $6\alpha/(2\alpha-1) \textcolor{blue}{Cost_{I_{cap}}(AS_{cap})}$ for $\delta= (2\alpha-1)/6\alpha^2 $. \textcolor{blue}{Why 6 times???}
 

==> NEW Journal version WADS 2021 (LBUBFL)/Conclusion.tex <==

\section{Conclusion and Future Work}
In this paper, we presented 
the first (constant) approximation algorithm for facility location problem with uniform lower and upper bounds without violating the lower bounds.
Upper bounds are violated by ($5/2$)-factor. 
%at constant factor loss in cost. %Our algorithm can be modified to work for general (splittable) demands...discuss (for journal version, you will ahve to write it for general demands...you can't simply write it like that). 
%Once we write in terms of $\tau$, we can add this: 
Violation in the upper bound is less when the gap between the lower and the upper bound is large. For example, if $\B \le \capacityU/2$ then 
%$\tau \le 1/2$ and hence 
the upper bound violation is at most $\beta + \frac{1}{2} \le 2$.


%Also, our (large) factor 
%Though our factor is large but it
%can be significantly improved by extending the ideas of Ahmadian and Swamy \cite{Ahmadian_LBFL}, i.e., instead of reducing the problem to CFL, we reduce it to Discounted Capacitated Facility Location to improve the approximation ratio....Sapna, I think we had discussed and concluded that it was not possible.

In future, if one can obtain a tri-criteria solution (with $\alpha > 1/2$) when one of the bounds is uniform and the other is non-uniform, then it can be simply plugged into our technique to obtain similar result for the problem. When the upper bounds are non-uniform and %$\tau (\le 1)$ is the largest value such that $ \B \le \tau \capacityU_i$,
$\tau = \frac{1}{\max_i \{\capacityU_i/\B \}}$ then $ \B \le \tau \capacityU_i$ for all $i$ and $\tau \le 1$. Also, violation in the upper bounds, then, is $\le \beta + \tau \le \beta + 1$. When the lower bounds are non-uniform and $\tau = \frac{1}{\max_i \{\capacityU/\B_i \}}$ then $ \B_i \le \tau \capacityU$ for all $i$ and $\tau \le 1$. As before, violation in the upper bounds is $\le \beta + \tau \le \beta + 1$.
%$\tau$ is largest value such that $ \B_i \le \tau \capacityU$, $\tau$ is still at most $1$. 
Note that, for this case, we can not use the tri-criteria solution of Friggstad \etal~\cite{friggstad_et_al_LBUFL} as $\alpha < 1/2$ in their solution. 
%It will be interesting to see if their solution can be modified to obtain a solution with $\alpha> 1/2$.


%In future, it will be interesting to obtain a bi-criteria solution for the problem when one of the bounds are non-uniform. For non-uniform capacities and uniform lower bounds, if one can obtain a tri-criteria solution then it can be simply plugged into our technique to obtain bi-criteria solution for the problem.



%\textcolor{cyan}{Although we have considered only uniform bounds in this paper, it will be interesting and challenging to get a bi-criteria solution for the problem when upper bounds are non-uniform or when both lower and upper bounds are non-uniform. Our algorithm works for non-uniform upper bounds and uniform lower bounds if we can get a tri-criteria solution for the problem. Moreover, Shi Li \cite{Li_NonUnifLBFL}, use some more involved reductions to handle non-uniform lower bounds. It will be challenging to first get a tri-criteria
%for FL with non-uniform lower and upper bounds and then extend the ideas of Shi Li to get rid of violations.}


%$k$-median and Knapsack median problem are problems that are closely related to facility location problem. In literature we have seen how algorithms for facility location problems are extended to work for knapsack median and $k$-median problem. Therefore, extending the results in this paper to $k$-median/knapsack median with lower and upper bounds is well motivated and interesting and we leave it for future work.

==> NEW Journal version WADS 2021 (LBUBFL)/CopyofLBUBFLGeneralTree.tex <==
\section{Instance $I_1$ and $I_2$}
\label{instI1}

In this section, we first transform instance $I$ to instance $I_1$ ($\facilityset,~\clientset,~f^1,~c,~\B,~\capacityU$) of LBUBFL by moving the clients to the facilities serving them in the tri-criteria solution $S^t$ and then transform $I_1$ to an instance $I_2$ of LBFL by removing the facilities not opened in $S^t$.
%Let $\facilityset^t$ be the set of facilities opened by $S^t$. 
Recall that for a client $j$,  $\sigma^t(j)$ is the facility  in $\facilityset^t$ serving $j$. For $i \in \facilityset^t$, let $n_i$ be the number of clients served by $i$ in $S^t$, i.e., $n_i = |(\sigma^t)^{-1}(i)|$ and for $i \notin \facilityset^t$, $n_i = 0$. Move these clients to $i$ (see Fig.~\ref{Mapping1}). Thus, there are $n_i$ clients co-located with $i$. In $I_1$, our facility set is $\facilityset$ and the clients are at their new locations. Facility opening costs in $I_1$ are modified as follows: $f^1_i = 0$ for $i \in \facilityset^t$ and $=f_i$ for $i \notin \facilityset^t$.  


\begin{lemma}
Cost of optimal solution of $I_1$ is bounded by $Cost_I(S^t) + Cost_I(O)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_1$ of $I_1$: open $i$ in $S_1$ iff it is opened in $O$. Assign $j$ to $i$ in $S_1$ iff it is assigned to $i$ in $O$. $S_1$ satisfies both the lower bound as well as the upper bound as $O$ does so. For a client $j$, let $\sigma^*(j)$ be the facility serving $j$ in $O$. Then, the cost $\dist{ \sigma^t(j)}{\sigma^*(j))}$ of serving $j$ from its new location, $\sigma^t(j)$ is bounded by $\dist{j}{\sigma^t(j)} +\dist{j}{\sigma^*(j)}$ (see Fig. \ref{lemma1}). Summing over all $j \in \clientset$ and adding the facility opening costs, we get the desired claim.

\begin{figure}[t]
    \centering
    \includegraphics[width=4cm]{Figures/lemma 1.jpg}
    \caption{$c( \sigma^t(j), \sigma^*(j)) \leq c(j, \sigma^t(j)) + c(j, \sigma^*(j))$ }
    \label{lemma1}
\end{figure}
\end{proof}

\begin{figure}[t]
    \centering
    \includegraphics[width=9cm]{Figures/Mapping_0.jpg}
    \caption{Transforming instance $I$ to $I_1$ and  $I_1$ to $I_2$. Solid squares represent clients and circles represent facilities. Clients are moved to the facilities serving them in $S^t$ while transforming $I$ to $I_1$. Facilities not opened in $S^t$ are dropped while going from $I_1$ to $I_2$.}
    \label{Mapping1}
\end{figure} 

%section{Instance $I_2$} 
%\label{instI2}
    
   Next, we define an instance ~$I_2(\facilityset^t,~\clientset,~f^2,~c,~\B)$ of LBFL from $I_1$ by removing the facilities not in $\facilityset^t$ and ignoring the upper bounds. Instance $I_2$ is same as $I_1$ without the upper bounds, except that the facility set is $\facilityset^t$ now. Thus, $f^2_i = 0~\forall~i \in \facilityset^t$. % We will show that there exists a feasible solution $S_2$ of $I_2$ such that $Cost(S_2)$ is bounded by $2 Cost(O_1)$ where
  Let $O_1$ be an optimal solution of $I_1$. 
  For a client $j$, let $\sigma^1(j)$ be the facility serving $j$ in $O_1$.
 
 
 

\begin{lemma}
Cost of optimal solution of $I_2$ is bounded by $ 2Cost_{I_1}(O_1)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_2$ to $I_2$: for $i \in \facilityset^t$, open $i$ in $S_2$ if it is opened in $O_1$ and assign a client $j$ to it if it is assigned to $i$ in $O_1$. For a facility $i \notin \facilityset^t$, %the clients assigned to it need to be assigned to some other facility in $\facilityset^t$. Thus, for such $i$'s,
open its nearest facility $i'$ \textcolor{olive}{(if not already opened)} in $\facilityset^t$. Assign $j$ to $i'$ in $S_2$ if it is assigned to $i$ in $O_1$. $S_2$ satisfies the lower bound  as $O_1$ does so. Note that it need not satisfy the upper bounds. This is the reason we dropped upper bounds in $I_2$. The cost $c( \sigma^t(j), i')$
%$c( \sigma^t(j), \sigma^*(j))$ 
of serving $j$ from its new location is bounded by $c(\sigma^t(j), \sigma^1(j)) + c( \sigma^1(j), i') \le 2 c(\sigma^t(j), \sigma^1(j))$ (since $i'$ is closest in $\facilityset^t$ to $i =  \sigma^1(j)$). Summing over all $j \in \clientset$ we get the desired claim.
%$c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(i, \sigma^1(j)) \le c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(\sigma^t(j), \sigma^1(j))$ (since $i$ is closest in $\facilityset^t$, to $i' = \sigma^1(j)$) $\le 2(c(j, \sigma^t(j)) + c(j, \sigma^1(j)))$ (See Figure 1). Summing over all $j$'s, the claim follows.
%Same as Zoya etal
\end{proof}

%\textcolor{blue}{can be deleted now...I have added a line in the proof itself....Note that, while defining the instance $I_2$, we ignored the upper bounds on facilities because a facility $i' \in \facilityset^t$ might be nearest to many other facilities $\notin \facilityset^t$ thereby serving clients of all of them and hence violating upper bound.}


\section{Instance $I_{cap}$ of Capacitated Facility Location Problem}
\label{instIcap}

 
 In this section, we create an  instance $I_{cap}$ of capacitated facility location problem from $I_2$. 
 The main idea is to create  a demand of $\B - n_i$ units at locations where the number of clients served by the facility is less than $\B$ and a supply of $n_i - \B$ units at locations with surplus clients. For each facility $i \in \facilityset^t$, let $l(i)$ be the distance of $i$ from a nearest facility  $i' \in \facilityset^t$, $i' \neq i$ and let $\delta$ be a constant to be chosen appropriately. A facility $i$ is called {\em small} if $0< n_i \leq \B$ and  {\em big} otherwise. A big facility $i$ is split into two co-located facilities $i_1$ and $i_2$.
  We also split the set of clients at $i$ into two sets:  arbitrarily, $\B$ of these clients are placed at $i_1$ and the remaining $n_i - \B$ clients at $i_2$ (see Fig.~\ref{Mapping2}). 
   Instance $I_{cap}$ is then defined as follows:
A {\em small} facility $i$ needs additional $\B - n_{i}$ clients to satisfy its lower bound; hence a demand of $\B - n_{i}$ is created at $i$ in the $I_{cap}$ instance. A facility with capacity $\B$ and facility opening cost $\delta n_{i} l(i)$ is also created at $i$. 
For a {\em big} facility $i$, correspondingly two co-located facilities $i_1$ and $i_2$ are created with capacities $\B$ and $n_i - \B$ respectively. The facility opening cost of $i_1$ is $\delta \B l(i)$ whereas $i_2$ is free. Intuitively, since the lower bound of a big facility is satisfied, it has some extra ($n_i - \B$) clients, which can be used to satisfy the demand of clients in $I_{cap}$ for free. 
 %Thus, we define capacity of $i_1$ and $i_2$ to be $\B$ and $n_i - \B$ respectively. 
 The second type of big facilities are called {\em free}. 
 %The facility costs, capacities and demands are as shown in
 We use $i$ to refer to both the client (with demand) as well as the facility located at $i$. Let $\bar \facilityset^t$ be the set of facilities so obtained. The set of clients and the set of facilities are both $\bar \facilityset^t$. Table~\ref{tab:my_label} summarizes the instance. Also see Fig.~\ref{Mapping2}
 
 \begin{figure}
    \centering
    \includegraphics[width=8cm]{Figures/Mapping_1.jpg}
    \caption{Transforming instance $I_2$ to $I_{cap}$: $\B = 4$,
    %Solid squares represent clients and circles represent facilities. 
    $i'$ is small, $i$ is big.
    $i$ is split into $i_1$ and $i_2$ while transforming $I_2$ to $I_{cap}$, $i_2$ is free. Demand at the small facility $i'$ is $\B - n_{i'} = 1$ and at $i_1$, $i_2$, it is $0$. Capacities of $i'$ and $i_1$ are $\B = 4$ and it is $n_{i} - \B = 3$ of the free facility $i_2$.}
    \label{Mapping2}
\end{figure}
 
 \begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
       Type & $n_i$ & $u_i$ & $d_i$ & $f^t_i$ \\
        \hline
       {\em small} & $n_i \leq \B$ & $\B$ & $\B- n_i$& $\delta n_i l(i)$ \\
        \hline
       {\em big} & $n_i > \B$ & ($i_1$)$\B$ & $0$& $\delta \B l(i)$ \\
        & & ($i_2$) $n_i - \B$ & $0$& $0$ \\
       
        % &  &
          \hline 
       % $3$ & $0$ & $\B$ & $\B$& $\delta \B l(i)$ \\
        %\hline
    \end{tabular}
    \caption{Instance of $I_{cap}$: $d_i, u_i, f^t_i$ are demands, capacities and facility costs resp.}
    \label{tab:my_label}
\end{table}
 
 %Let $O_{cap}$ be an optimal solution to $I_{cap}$.
 
 %\textcolor{red}{define delta and l(i)}
 %The second type of big facilities are called {\em free}. %and the clients placed at them are also called {\em free}. 
 %Let $F_f$ denote the set of free facilities. 
 %and $Cf(i)$ denote the set of free clients at facility $i \in F_b$. i.e.$Cf(i)$ is the set of clients placed at $i_2 \in F_f$ (See Figure 2)....need to define $l(i)$.

 %In the next lemma, we show the existence of a feasible solution to $I_{cap}$ with cost no more than $(1+2\delta)Cost(O_2)$ where $O_2$ is an optimal solution of $I_2$. 




\begin{lemma}
%A feasible solution $S_{cap}$ for 
Let $O_2$ be an optimal solution of $I_2$. Then, cost of optimal solution to $I_{cap}$ is bounded by $(1+2\delta)Cost_{I_2}(O_2)$.
\end{lemma}

\begin{proof}
We will construct a feasible solution $S_{cap}$ to $I_{cap}$ of bounded cost from $O_2$.
 As $O_2$ satisfies the lower bound,  we can assume wlog that if $i$ is opened in $O_2$ then it serves all of its clients if $n_i \le \B$ (before taking more clients from outside) and it serves at least $\B$ of its clients before sending out its clients to other (small) facilities otherwise. 
Also, if two big facilities are opened in $O_2$, one does not serve the clients of the other. Let $\rho^2(j_i, i')$ denote the number of clients co-located at $i$ and assigned to $i'$ in $O_2$ and $\rho^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $S_{cap}$.
 \begin{figure}[t]
    \centering
    \includegraphics[width=10cm]{Figures/O2_Scap_assignments.jpg}
    \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ and $i'$ are closed in $O_2$. $\rho^2(j_{i_1}, t_1) = 2,~\rho^2(j_{i_1}, t_2) = 1,~\rho^2(j_{i_1}, t_3) = 1,~ \rho^2(j_{i_1}, t_4) = 0$ and $\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 1,~\rho^2(j_{i_2}, t_3) = 1,~ \rho^2(j_{i_2}, t_4) = 0$.  } %The middle figure shows how the assignments look like after splitting the big facilities. $\rho^2(j_{i_1}, i') = 2(/1/1)$ for $i'$ = top three facilities $t_1(/t_2/t_3)$ $\rho^2(j_{i_2}, i') = 1(/1/1) $ for the bottom three facilities $t_2(/t_3/t_4)$. Note that $t_1$ }
    \label{Mapping}
\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{Figures/O2_Scap assignments (2.1).jpg}
   \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ is open in $O_2$.   $\rho^c(j_{t_1}, i_2) = \rho^2(j_{i}, t_1) = 1, \rho^c(j_{t_2}, i_2) = \rho^2(j_{i}, t_2) = 2$,
  % $\rho^2(j_{i_1}, t_1) = 1,~\rho^2(j_{i_1}, t_2) = 1$ and %$\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 2$. 
   $i_2$ is open in $S_{cap}$. $t_1$ and $t_2$ must be small.}
    \label{O2_SCap2}
\end{figure}
    \begin{enumerate}
        \item   if $i$ is closed in $O_2$ then open $i$ if $i$ is small
        and open $(i_1 \& i_2)$ if it is big.
        
        Assignments are defined as follows (see Fig.~\ref{Mapping}):
        \begin{enumerate}
        
        \item If $i$ is small: Let $i$ serve its own demand. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. 
        \textcolor{green}{
        Note that the same cannot be done when $i'$ is big as there is no demand at $i'_1$ and $i'_2$. } Thus,  $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $ i' \ne i$ and $\rho^c(j_i, i) = d_i$. Also, $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). 
        Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = \B = u_i$. 
      
       % \item If $i$ is small: Let $i$ serve its own demand, \textcolor{blue}{i.e., $\rho^c(j_i, i) = d_i$}. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. \textcolor{blue}{Note that $i'$ must be small in this case. But y not big?????? I think it can be big as well, the only thing that will differ is $\rho^c(j_{i'}, i) = 0$ if $i'$ is big.} Thus, $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $i' \ne i$. Also, $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = \B = u_i$. \textcolor{blue}{Thus capacities are respected.}
        
       \item If $i$ is big: assign $\rho^2(j_{i_1}, i')$ (/$\rho^2(j_{i_2}, i')$) demand of $i'$ to $i_1$(/$i_2$) in our solution for small $i' \ne i$. Thus,
        $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_1) = \sum_{small~i' \ne i} \rho^2(j_{i_1}, i') \le \B = u_{i_1}$. Also,
         $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_2) \\ = \sum_{small~i' \ne i} \rho^2(j_{i_2}, i') \le n_i - \B = u_{i_2}$.
       %The second equality holds in each case as $i$ is closed in $O_2$.
        %\textcolor{green}{.....Is this the reason? Sapna...Pls see..}
        % Since there are no demands at $i_1$ and $i_2$, the capacities are respected.
     
       \end{enumerate}
     
     \item If $i$ is opened in $O_2$ and is big, open the free facility $i_2$ (see Fig.~\ref{O2_SCap2}): assign $\rho^2(j_{i}, i')$  demand of $i'$ to $i_2$ in our solution for small $i' \ne i$. Thus,
     %Thus,
      %  $\sigma^c(j_{i'}, i_2) = %\sigma^1(j_{i_2}, i'), i \ne i'$  
        $\sum_{i' \ne i}\rho^c(j_{i'}, i_2) = \sum_{i' \ne i} \rho^2(j_{i}, i') \le n_i - \B$ (the inequality holds by assumption on $O_2$) $= u_{i_2}$.
       % Thus the capacities are respected as there are no demands at $i_2$.
    \end{enumerate}
    
    Thus capacities are respected in each of the above cases. Next, we show that all the demands are satisfied. If a facility is opened in $S_{cap}$, it satisfies its own demand. 
Let $i$ be closed in $S_{cap}$. If $i$ is big ,we need not worry as $i_1$ and $i_2$ have no demand. So, let $i$ is small. Then, it must be opened in $O_2$. Then, 
$\sum_{i' \ne i}\rho^c(j_{i}, i') = $
$\sum_{small ~i' \ne i,  }\rho^c(j_{i}, i') + \sum_{i'_1: i' ~is ~big}\rho^c(j_{i}, i'_1) + 
\sum_{i'_2: i' ~is ~big}\rho^c(j_{i}, i'_2)= $
$\sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i'_1 : i' ~is ~big} \rho^2(j_{i'_1}, i)  + \\ \sum_{i'_2 : i' ~is ~big}\rho^2(j_{i'_2}, i)= \sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i' ~is ~big} \rho^2(j_{i'}, i) = \sum_{i' \ne i}\rho^2(j_{i'}, i)$
$\ge \B - n_i$  (since $O_2$ is a feasible solution of $I_2$) $= d_i$. 



Next, we bound the cost of the solution. The connection cost is \textcolor{olive}{at most that of $O_2$. } %same as 
\textcolor{green}{ or at most? we didn't bring back if anything went from i to i' in O2 where i' is big.}
%Next, we consider the facility opening costs. 
For facility costs, consider a facility $i$ that is opened in our solution and closed in $O_2$. Such a facility must have paid a cost of at least $n_i l(i)$ to get its clients served by other (opened) facilities in $O_2$. The facility cost paid by our solution is $ \delta min\{n_i, \B\} l(i) \le \delta n_i l(i)$. If $i$ is opened in $O_2$, then it must be serving at least $\B$ clients and hence paying a cost of at least $\B l(i)$ in $O_2$. In this case also, the facility cost paid by our solution is $ \delta min\{n_i, \B\} l(i) \le \delta \B l(i)$.  Summing over all $i$'s, we get %\textcolor{blue}{$FCost_{I_{cap}}(S_{cap}) \leq 2 \delta Cost_{I_2}(O_2)$, where $FCost_{\cdot}(\cdot)$ is the facility opening cost of a solution to $I_{cap}$ instance.} 
that the facility cost is bounded by $2 \delta Cost_{I_2}(O_2)$ and the total cost is bounded by $(1 + 2 \delta) Cost_{I_2}(O_2)$. Factor $2$ comes because we may have counted an edge $(i, i')$ twice, once as a client when $i$ was closed and once as a facility when $i'$ was opened in $O_2$.  
\end{proof}


% ****I am here - NG***** 

\section{Bi-criteria Solution $AS_1$ to $I_1$ from approximate solution $AS_{cap}$ to  $I_{cap}$} \label{bi-criteria}

In this section, we obtain a solution $AS_1$ to $I_1$ that violates the capacities/upper bounds by a factor of $(\beta + 2)$ without violating the lower bound. We first obtain an approximate solution $AS_{cap}$ to $I_{cap}$ using approximation algorithm \textcolor{olive}{of Bansal \etal} \cite{Bansal}.  $AS_{cap}$ is then used to construct $AS_1$.
Wlog assume that if a facility $i$ is opened in $AS_{cap}$ then it serves all its demand.\textcolor{green}{ May have to add a couple of lines here in view of the reviews of one of the reviewer: If this is not true, we can modify the $AS_{cap}$  and obtain another solution that satisfies this condition, of cost no more than that of $AS_{cap}$....will see if we can briefly say how we can modify $AS_{cap}$.}
This is always feasible as $d_i \le u_i$. $AS_1$ is obtained from $AS_{cap}$ by first defining the assignment of the clients and then opening the facilities that get at least $\B$ clients. Let $\rhobar^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $AS_{cap}$ and $\rhobar^1(j_i, i')$ denotes the number of clients co-located at $i$ and assigned to $i'$ in $AS_1$. 
%\textcolor{red}{ Initially each facility is assigned the clients co-located with it.}
Clients are assigned in three steps. In the first step, assign the clients co-located at a facility to itself. 
For small $i'$, additionally, we do the following  (type - $1$) re-assignments (see Fig. \ref{type1}): $(i)$ For small $i \ne i'$, assign $\rhobar^c(j_{i'}, i)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for small $i$. $(ii)$ For big $i$, assign $\rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ for big $i$. 
Claim~\ref{claim1} shows that these assignments are feasible and the capacities are violated only upto the extent to which they were violated by the tri-criteria solution $S^t$. 
\begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{Figures/Type 1 Assignments.jpg}
    \caption{($a$) $\B =5$, $t_1, t_2, t_3$ have demands $1$, $2$ and $1$ unit each respectively. In solution $AS_{cap}$, $1$ unit of demand of $t_1$ and $2$ units of demand of $t_2$ are assigned to $t_3$. (b) Solution $S_1$: initially, $n_i$ clients are initially assigned to facility $i$. (c) Type $1$ reassignments: $1$ and $2$ clients of $t_3$ reassigned to $t_1$ and $t_2$ respectively. After this reassignment, $t_3$ has only $1$ client.}
    \label{type1}
\end{figure}

\begin{claim}
\label{claim1}
    $(i)$ $\sum_{i' \ne i} \rhobar^1(j_i, i') \le n_i$, $\forall$ $i \in \bar \facilityset^t$.
    $(ii)$ $\sum_{i} \rhobar^1(j_i, i') \le max\{\B, n_{i'}\} \le \beta \capacityU$, for $\beta \ge 1$, $\forall$ $i' \in \bar \facilityset^t$.
 \end{claim}

\begin{proof}

    $(i)$ Since $\rhobar^c(j_{i}, i) = d_i$ therefore $\sum_{i' \ne i} \rhobar^1(j_i, i') = \sum_{i' \ne i} \rhobar^c(j_{i'}, i) \le u_i - d_i \le n_i$ in all the cases. $(ii)$ $\rhobar^1(j_{i'}, i') = n_{i'}$. For $ i \ne i'$, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$. Thus, $\sum_{i} \rhobar^1(j_i, i') = n_{i'} + \sum_{i \ne i'} \rhobar^c(j_{i'}, i) \le n_{i'} + d_{i'} \le max\{\B, n_{i'}\} \le \beta \capacityU$.
\end{proof}

Note that $AS_1$ so obtained may  still not satisfy the lower bound requirement. In fact, although each facility was assigned $n_i \ge  \alpha \B$  clients initially, they may be serving less clients now after type $1$ re-assignments. For example, in Fig. \ref{type1}, $t_3$ had $4$ clients initially which was reduced to $1$ after type $1$ reassignments. Let $P \subseteq  \facilityset^t$ be the set of facilities each of which is serving at least $\B$ clients after type-$1$ reassignments, and  $\bar P =  \facilityset^t \setminus P$ be the set of remaining facilities. 
 %That is, $ P= \{ i' \in \facilityset^t: \sum_{i}\rhobar^1(j_{i}, i') \ge \B$\}.
 We open all the facilities in $P$ and let them serve the clients assigned to them after type $1$ reassignments.
 
 \begin{observation}
    If a  small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge \B$. Similarly for a big facility $i'$, if $i'_1$ was closed in $AS_{cap}$ then $i'$ is in $P$.
     %\item If a small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge \B$.
    
     
    % \item If $i'$ is big then $\rhobar^1(j_{i'}, i') = n_{i'}  \ge \B$
 \end{observation}
 
 
 Thus, a small facility is in $\bar P$ only if it was open in $AS_{cap}$ and a big facility $i$ is in $\bar P$ only if $i_1$ was open in $AS_{cap}$. 
 %Also note that although each facility in $\bar P$ served at least $\alpha \B \ge \B/2$ clients in the tri-criteria solution $S^t$, they may be serving less clients now after step $1$ of assignment. \textcolor{red}{See Figure \ref{type1} for an example}.
 We now group these facilities so that each group serves at least $\B$ clients and open one facility in each group that serves all the clients in the group. For this we construct what we call as {\em facility trees}. We construct a graph $G$ with nodes corresponding to the facilities in \textcolor{olive}{$P \cup \bar P$.} For $i \in \bar P$, let $\eta(i)$ be the nearest other facility to $i$ in $\facilityset^t$. Then, $G$ consists of edges $(i, \eta(i))$ with edge costs $ \dist{i}{\eta(i)}$. Each component of $G$ is a tree except possibly a double-edge cycle at the root. In this case, we say that we have a root, called {\em root-pair} $<i_{r_1}, i_{r_2}>$ consisting of a pair of facilities $i_{r_1}$and $ i_{r_2}$. Also, a facility $i$ from $P$, if present, must be at the root of a tree. Clearly edge costs are non-increasing as we go up the tree. 

Now we are ready to define our second type of re-assignments.
\textcolor{violet}{
Let $x$ be a node in a tree $\mathcal T$. Let $children(x)$ denote the set of children of $x$ in $\mathcal T$. 
%if $x$ is not a root-pair. 
If $x$ is a root-pair $<r_1, r_2>$, then $children(x) = children(r_1) \cup children(r_2)$. %denote the union of children of $r_1$ and $r_2$ in $\mathcal T$.
Process the tree bottom-up using Algorithm~\ref{TreeProcessing} \textcolor{blue}{(Resolve refernce later- SAPNA)} to process a node $x$ of the tree. \textcolor{olive}{See Fig: (\ref{ProcessX})}.
\textcolor{violet}{ While processing a node $x$, its children are arranged and considered (left to right) in non- increasing distance from $x$.}
%till we reach the root node, which could be either a single facility in $P$ or a root-pair. 
}

 \begin{figure}[t]
    \centering
    \includegraphics[width=12cm]{Figures/ProcessX.jpg}
    \textcolor{red}{
     \caption{ Let $\B=5$, numbers inside a node represents the number of clients at the node. A dashed arrow from a node $u$ to node $v$ represents the movement of clients from $u$ to $v$; (A): A node $x$ along with its children in increasing order of their distances from $x$; (B): In steps $1$ to $7$, we open child $d$ and delete the edge $(d, x)$; (C): In steps $18 -20$, clients from $e$ are assigned to $c$ accumulating a total of $7$ clients at $c$. In the next iteration of the 'for' loop, in lines $14-16$, $c$ gets opened and the edge ($c, x$) is deleted; (D): In the next iteration, clients of $b$ are assigned to $a$; (E):  In the next iteration, clients of $a$ are assigned to $x$ in lines $27 - 28$;}
    }
   % \caption{ (A): A node $x$ along with its children. $\B=5$; Numbers inside each node represents the number of clients at those nodes; (B): Process($x$) - $1$ and $3$ clients from node $d$ and $e$ respectively, get assigned to node $c$, making its count to $8$. $c$ gets opened; (C): $2$ clients of node $b$ are assigned to node $a$, making its count $3$; (D):  $3$ clients of node $a$ are assigned to node $x$, making its count $6$;}
    \label{ProcessX}
\end{figure}

%\input{Gen-Algo.tex}
%\newpage 

\input{Gen-AlgoSG.tex}

\begin{algorithm}[H] 
    \footnotesize
    \setcounter{AlgoLine}{0}
	\SetAlgoLined
	%\scriptsize
    \DontPrintSemicolon  
    \SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
    \Input{$x ( x$ can be a root-pair node)}
    %\Output{}
    
	\For {$ y \in children(x)$} {
	 \If{$n_{y} \geq \B$}  {
	    Open facility $y$ \;
		 
		 Remove edge ($y, \eta(y)$) \textcolor{blue}{\tcp*{Remove the connection of $y$ from $x$}}
		 
		 Delete $y$ from $children(x)$;
	 }
	 }
	\If {$children(x) =  \phi$} {return;}
	
	Arrange $children(x)$ in the sequence $<y_1, \ldots y_k>$ such that $\dist{y_{i-1}}{\eta(y_{i-1})} \le \dist{y_{i}}{\eta(y_{i})} ~\forall ~i = 2 \ldots k$\;
	
%	Arrange $children(x)$ in the increasing order of their distances from $x$. Let $<y_1, \ldots y_k>$ be the sequence obtained.\;
	 
	%	 For $ y \in children(x), re-assigned(y) \gets false$ \textcolor{blue}{ \tcp*{boolean variable to indicate if clients of $rc_i$ are assigned to $lc_i$ or not; initially false}} 
		 
		 \For {$i = k$ down to $2$} {  
		 
		     \eIf{$n_{y_i} \geq \B$}  {
		 
		        Open facility $y_i$\;
		
		     Remove edge ($y_i, \eta(y_i)$) \textcolor{blue}{\tcp*{Remove the connection of $y_i$ from its parent}}
		 
		     Delete $y_i$ from $children(x)$;
		    }
		    {
		     $n_{y_{i-1}} = n_{y_{i-1}} + n_{y_{i}}$	 \tcp*{Send the clients of $y_i$ to $y_{i-1}$}
		 
		      Remove edge ($y_i, \eta(y_i)$) \textcolor{blue}{\tcp*{Remove the connection of $y_i$ from its parent}}
		 
		      Delete $y_i$ from $children(x)$\;
		    }
		 }
		 
		 \eIf {$n_{y_1} \geq \B$}  {
		 
		 Open facility $y_1$ \;
		 
		 %Remove edge ($y_1, \eta(y_1)$) \textcolor{blue}{\tcp*{Remove the connection of $y_1$ from its parent}}
		 
		 Delete $y_1$ from $children(x)$\;
		 }
		 {
		 $n_{\eta(y_1)} = n_{\eta(y_1)} + n_{y_{1}}$ \tcp*{Send the clients of $y_1$ to $\eta(y_1)$}
		 
		 %Remove edge ($y_1, \eta(y_1)$) \textcolor{blue}{\tcp*{Remove the connection of $y_1$ from its parent}}
		 
		 Delete $y_1$ from $children(x)$\;
		 }
		 
		 Return\;
	
	\label{TreeProcessing}
	\caption{Process($x$)}
\end{algorithm}

\newpage
 
There are two possibilities at the root: either we have a facility $i$ from $P$ or we have a root-pair.
%$<i_{r_1}, i_{r_2}>$. 
In the first case, we are done as $i$ is already open and has at least $\B$ clients. \textcolor{olive}{See Fig: (\ref{tree12})}. To handle the second case, we need to do a little more work. So, we define our assignments of third type as follows: 
($i$) If the total number of clients collected at  the root-pair node 
%$i_c, i_{r_1}$ and $i_{r_2}$ 
is at least $\B$ and at most $2\B$ then open any one of the two facilities in the root-pair and assign all the clients to it.\footnote{ we can open 
the facility with more number of clients and save $2$(to be seen again) factor in the connection cost.} \textcolor{olive}{See Fig: (\ref{tree3})}.
($ii$) If the total number of clients collected at  the root-pair node is more than $2\B$  then open both the facilities at the root node and distribute the clients  so that each one of them gets at least $\B$ clients. \textcolor{olive}{See Fig: (\ref{tree4})}.
($iii$) If the total number of clients collected at  the root-pair node  is less than $\B$, then let $i$ be the node in $P$ nearest to the root-pair, then $i$ is already open and has at least $\B$ clients. Send the clients collected at the root-pair to $i$. \textcolor{olive}{See Fig: (\ref{tree5})}.


\begin{figure}[t]
	\begin{tabular}{ccc}
		\includegraphics[width=12cm,scale=1.0]{Figures/Tree1.jpg}
		%& 
		%\includegraphics[width=6cm,scale=0.8]{Figures/Tree2.jpg}
		%\\
		%\textbf{(a)}& \ \ \textbf{(b)}& \ \ \textbf{(c)}
	\end{tabular}
	\textcolor{red}{
	\caption{ $\B=12$;(A) A tree $\mathcal{T}$;  Numbers inside each node represents the number of clients at those nodes.
	At any fixed level, nodes are processed in any arbitrary order (for the sake of example, we process them in left to right order). The tree does not change after the calls: Process($f$), Process($g$), Process($h$), Process($i$), Process($j$) and Process($k$). In each case, it returns at line no. $9$;  (B) Tree after Process($a$), Process($b$), Process($c$), Process($d$) and 
	Process($e$); (C) Tree after Process($x$) when $t \ge 3$ }.
	}
	
	%\caption{(A) A tree $\mathcal{T}$; $\B=12$; Numbers inside each node represents the number of clients at those nodes. (B) Algorithm Process() called in the following order: Process($a$) - $3$ and $6$ clients from node $g$ and $h$ respectively, get assigned to node $f$, making its count to $12$; Process($b$); Process($c$) - $9$ clients from $i$ are assigned to node $c$; Process($d$); Process($e$) - $3$ and $1$ clients from node $j$ and $k$ respectively, get assigned to it. Eventually, node $f$ and $c$ are opened; (C) Process($x$) - $2$, $1$ and $5$ clients from node $b$, $d$ and $e$ respectively, get assigned to node $x$, making its count to $t+8$; (D) $x\in P,~n_x = 12$ and $t=1$; All $9$ clients from children of $x$ are assigned to $x$. }
	\label{tree12}
\end{figure}


% \begin{figure}[t]
%    \centering
%    \includegraphics[width=7cm]{Figures/Tree1.jpg}
%    \caption{(A) A tree $\mathcal{T}$; $\B=12$; Numbers inside each node represents the number of clients at those nodes. (B) Algorithm Process() called in the following order: Process($a$) - $3$ and $6$ clients from node $g$ and $h$ respectively, get assigned to node $f$, making its count to $12$; Process($b$); Process($c$) - $9$ clients from $i$ are assigned to node $c$; Process($d$); Process($e$) - $3$ and $1$ clients from node $j$ and $k$ respectively, get assigned to it. Eventually, node $f$ and $c$ are opened; }
%    \label{tree1}
%\end{figure}

 %\begin{figure}[t]
  %  \centering
   % \includegraphics[width=7cm]{Figures/Tree2.jpg}
    %\caption{ $\B=12$; (C) Process($x$) - $2$, $1$ and $5$ clients from node $b$, $d$ and $e$ respectively, get assigned to node $x$, making its count to $t+8$; (D) $x\in P,~n_x = 12$ and $t=1$; All $9$ clients from children of $x$ are assigned to $x$. }
    %\label{tree2}
%\end{figure}


 \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{Figures/Tree3.jpg}
    \textcolor{red}{
    \caption{ $\B=12, t < 3$; (E)  $x = <i_{r_1}, i_{r_2}>$ is a root-pair node  with $\B \le n_{i_{r_1}} + n_{i_{r_2}} + t + 8 \le 2B$ (F) $t=2$ (give this in the figure and delete from here); open any of $i_{r_1}$ and $i_{r_2}$, say $i_{r_1}$ and assign all the clients to it.}
    }
    \label{tree3}
\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{Figures/Tree4.jpg}
    \textcolor{red}{
    \caption{ $\B=12, t < 3$; (E)  $x = <i_{r_1}, i_{r_2}>$ is a root-pair node  with $2\B \le n_{i_{r_1}} + n_{i_{r_2}} + t + 8 < 3B$ (F)  open both $i_{r_1}$ and $i_{r_2}$ and distribute the clients to them so that each of them gets at least $\B$ clients.}
    }
    %\caption{ $\B=12$; (G) $x = <i_{r_1}, i_{r_2}>$ is a root-pair node; $n_{i_{r_1}} = 8,~n_{i_{r_2}} = 9$ (F) $t=1$; All $9$ clients from children of $x$ are distributed between $i_{r_1}$ and $i_{r_2}$; both facilities in $x$ get opened. }
    \label{tree4}
\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{Figures/Tree5.jpg}
    \textcolor{red}{
    \caption{ $\B=12, t < 3$; (E)  $x = <i_{r_1}, i_{r_2}>$ is a root-pair node  with $ n_{i_{r_1}} + n_{i_{r_2}} + t + 8 < B$ (F)  open a facility $i \in P$ that is nearest to $\{i_{r_1}, i_{r_1}\}$ and assign all the clients to it.}
    }
   % \caption{ $\B=12$; (I) $x = <i_{r_1}, i_{r_2}>$ is a root-pair node; $n_{i_{r_1}} = n_{i_{r_2}} = 1$ (J) $t=1$; All $9$ clients from children of $x$ and, clients of $i_{r_1}$ and $i_{r_2}$ are assigned to $i \in P$.}
    \label{tree5}
\end{figure}

 
Clearly the opened facilities satisfy the lower bounds. Next, we bound the violation in the upper bound.
  
   \begin{lemma}
 Let $ i_c$ be the only child, if any,  of the root (/root-pair) of a tree. Let $i$ be the parent of $ i_c$ ($i$ is either in $P$ or it is one of $i_{r_1}$ and $i_{r_2}$ in case the root is a root-pair).
The number of clients collected in the second type of re assignments, at any node $x$ in the tree rooted at $i_c$ is at most $2\B$.
 \end{lemma}
 
 \begin{proof} 
 \textcolor{violet}{We will show that the number of clients collected at $x$ after Process($x$) is at most $2\B$. For this, note that $x$ receives $< \B$ clients from at most one of it's children. Hence, the claim follows.}
 \end{proof}
  
  If the number of clients collected at $i_c$ is $\ge \B$, it is opened and removed from further processing.
 Let $\pi_i$ be the number of clients assigned to the facility $i$ after first type of re-assignments. Then as shown earlier, $\pi_i \le \beta \capacityU$.  %Let $i$ be the parent of $ i_c$. In second and third types of assignments,  we never collect  more than $2\B$ clients at any node till we reach $i_c$.
 %Now we have the following scenarios: Suppose $ i_c$ has less than $\B$ clients,
 We have the following cases: ($i$) the root node $i$ is in $P$ and it gets additional at most $\B$ clients from $i_c$ making a total of at most $\pi_i + \B \le \beta \capacityU + \B \le (\beta + 1) \capacityU$ clients at $i$.
 ($ii$) the total number of clients collected at  the root-pair node 
%$i_c, i_{r_1}$ and $i_{r_2}$ 
is at least $\B$ and at most $2\B$.
 %($ii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at $i_c, i_{r_1}$ and $i_{r_2}$ is at least $\B$ and at most $2\B$. Thus, 
 The number of clients the opened facility gets is at most $2\B \le 2\capacityU$.
 ($iii$)  the total number of clients collected at the root-pair node  is more than $2\B$.  Note that the total number of clients collected at these facilities is at most $3\B$ and hence 
 ensuring that each of them gets at least $\B$ clients also ensures that none of them gets more than $2\B$ clients. Hence none of them gets more than $2\capacityU$ clients.
 %it is possible to distribute them to the two opened facilities so that each of them gets at most $2\B \le 2\capacityU$ clients.
 ($iv$) the total number of clients collected at the root-pair node is less than $\B$. 
 %Number of clients at $i_c$ and the root pair and, their nearest facility in $P$ are at most $\B$ and $\beta \capacityU$ respectively. 
 Thus, the number of clients the opened facility in $P$ gets is at most $\beta \capacityU + \B \le (\beta + 1) \capacityU$. 
 %The case when $i_c$ has at least $\B$ clients leads to the third scenario above and hence handled.
 
 
 We next bound the connection cost.  For any node $y$ in a tree, let $left-sibling(y)$ denote the left sibling of $y$ in step~\ref{} of the algorithm. Thus, $left-sibling(y_i) = y_{i-1}$. We will need the following lemma to bound the connection cost.
 
 \begin{lemma}
 For a node $y$ in a tree,
  $\dist{y}{left-sibling(y)} \le 3 \dist{y}{\eta(y)} = 3l(y)$. %.....This equality is correct, right? we have been assuming this....$P \cup \bar P = F^t$, right?
 \end{lemma}
 
 \begin{proof}
 \textcolor{violet}{
 If $\eta(\cone) = \eta(left-sibling(\cone))$  (i.e. $\cone$ and $left-sibling(\cone)$ are children of the same node), then it is easy to see that $\dist{\cone}{left-sibling(\cone)} \leq 2 \dist{\cone}{\eta(\cone)}$. Otherwise (which can be the case when root is a root-pair, see Figure~(\ref{3factorBound})), $\dist{\cone}{left-sibling(\cone)} \leq \dist{\cone}{\eta(\cone)} + \dist{\eta(\cone)}{\eta(left-sibling(\cone))} + \dist{\eta(left-sibling(\cone))}{left-sibling(\cone)} \le 3 \dist{\cone}{\eta(\cone)}$.
 }
 
  \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{Figures/3factorBound.jpg}
    \caption{$\dist{\cone}{left-sibling(\cone)}  \le 3 \dist{\cone}{\eta(\cone)}$}
    \label{3factorBound}
\end{figure}
 \end{proof}
 
 
 The cost of first type of re-assignments is \textcolor{olive}{at most the connection cost of $AS_{cap}$.} 
% \textcolor{red}{(or at most?Sapna/rajni) }
 To bound the connection cost of second type, observe that we never send more than $\B$ clients on any edge. 
 %In the second type of assignment, 
 Thus, a facility $i$ that sends its (at most $\B$ clients) to its parent or to its left sibling incurs a cost of at most $3\B l(i)$. Since the facility $i$ was opened in $AS_{cap}$, it pays facility opening cost of $\delta l(i) min \{n_i, \B\} \ge \delta l(i) \alpha \B$ in $AS_{cap}$. Summing over all $i \in \bar P$ for the second type of re-assignments, we see that the total connection cost in these re-assignments is bounded by 
 \textcolor{red}{
 $3 FCost_{I_{cap}}(AS_{cap})/\alpha \delta$ 
 } 
% \textcolor{olive}{D: $\sum_{i \in \bar P} \B l(i) \leq 6FCost_{I_{cap}}(AS_{cap})/\alpha \delta$  where factor 6 comes because sending clients to the left sibling incurs a cost of twice the cost to the node's parent and}
 where $FCost_{I_{cap}}(.)$ is the facility opening cost of a solution to the $I_{cap}$ instance.


 For the third type of re-assignments, we bound the cost as follows:
 %we bound the cost in two parts: ($a$) cost of sending ($< \B$) clients of $i_c$ to it's parent ($b$) Cost of sending ($< \B$) clients collected at the root pair $<i_{r_1}, i_{r_2}>$ to it's nearest facility in $P$. Cost of the first part is bounded by $\B l(i_c)$. 
 the cost of sending ($< \B$) clients by a facility $i$ in the root pair $<i_{r_1}, i_{r_2}>$ to the facility in $P$, nearest to the root-pair, is not bounded by $\B l(i)$ (where $l(i) = l(i_{r_1}) = l(i_{r_2})$). 
% we bound the cost as follows: 
 Note that the total number of clients, initially at $i_{r_1}$ and $i_{r_2}$ was $\ge 2 \alpha \B$. However, during re-assignments of type $1$, some of them got reassigned to other facilities. Note that these (other) facilities must have been closed in $AS_{cap}$ and hence do not belong to $\bar P$. Hence, each of these reassignments correspond to an assignment in $AS_{cap}$ whose cost was at least $l(i)$ and a total of at least $(2\alpha  - 1)\B l(i)$. Hence the cost of type $3$ re-assignments is bounded by \textcolor{blue}{$3 CCost_{I_{cap}}(AS_{cap})/ (2\alpha  - 1)$ where $CCost_{I_{cap}}(.)$ is the connection cost of a solution to the $I_{cap}$ instance}. 
 
 \textcolor{violet}{
 Hence the total cost of solution $S_1$  is $6\alpha/(2\alpha-1) \textcolor{blue}{Cost_{I_{cap}}(AS_{cap})}$ for $\delta= (2\alpha-1)/6\alpha^2 $. \textcolor{blue}{Why 6 times???}...Only this is left from my side.
 }
 

==> NEW Journal version WADS 2021 (LBUBFL)/Gen-Algo.tex <==
\begin{algorithm}[H]
\footnotesize
    \SetAlgoLined
    %\KwData{$\clientset,~\facilityset$}
    %\KwResult{$\clientset',~\bundle{j'}~\forall~j'\in \clientset'$}
    \SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
    \Input{$x$}
    %\Output{}
		 
	% Process($lc_i$)\;
		 
	% Process($rc_i$)\;
	If $children(x) =  \phi$, return;
	
	For $ y \in children(x)$\\
	 \If{$n_{y} \geq \B$}  {
	 Open facility $y$ \;
		 
		 Remove edge ($y, \eta(y))$) \textcolor{blue}{\tcp*{Remove the connection of $lc_i$ from its parent}}
		 
		 Delete $y$ from $children(x)$;
	 }
	
	 Arrange $children(x)$ in the increasing order of their distances from $x$. Let $<y_1, \ldots y_k>$ be the sequence obtained.
	%	 For $ y \in children(x), re-assigned(y) \gets false$ \textcolor{blue}{ \tcp*{boolean variable to indicate if clients of $rc_i$ are assigned to $lc_i$ or not; initially false}} 
		 
		 For $i = k$ down to $2$ 
		 
		 \If{$n_{y_i} \geq \B$}  {
		 
		 Open facility $y_i$ \;
		 
		 Remove edge ($y_i, \eta(y_i))$) \textcolor{blue}{\tcp*{Remove the connection of $y_i$ from its parent}}
		 
		 Delete $y_i$ from $children(x)$;
		 
		 }
		 
		 else \\
		 
		\{\\
		$n_{y_{i-1}} = n_{y_{i-1}} + n_{y_{i}}$;
		 \tcp*{Send the clients of $y_i$ to $y_{i_1}$}
		 
		 Remove edge ($y_i, x)$)\; \textcolor{blue}{\tcp*{Remove the connection of $y_i$ from its parent $x$}}
		 
		 
		 Delete $y_i$ from $children(x)$\;\\
		 \}
		 
		 \If{$n_{y_1} \geq \B$}  {
		 
		 Open facility $y_1$ \;
		 
		 Remove edge ($y_1, x$) \textcolor{blue}{\tcp*{Remove the connection of $y_1$ from its parent}}
		 
		 Delete $y_1$ from $children(x)$;\;
		 
		 }
		 
		 else \\
		 
		\{\\
		$n_{x} = n_{x} + n_{y_{1}}$;
		 \tcp*{Send the clients of $y_1$ to $x$}
		 
		 Remove edge ($y_1, x)$)\; \textcolor{blue}{\tcp*{Remove the connection of $lc_i$ from its parent}}
		 
		 
		 Delete $y_1$ from $children(x)$\;\\
		 \}
	
	\label{Process_i}
	\caption{Process($x$)}
\end{algorithm}

==> NEW Journal version WADS 2021 (LBUBFL)/Gen-AlgoSG.tex <==
\begin{algorithm}[H] 
    \footnotesize
    \setcounter{AlgoLine}{0}
	\SetAlgoLined
	%\scriptsize
    \DontPrintSemicolon  
    \SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
    \Input{$x ( x$ can be a root-pair node)}
    %\Output{}
    
	\For {$ y \in children(x)$} {
	 \If{$n_{y} \geq \B$}  {
	    Open facility $y$ \;
		 
		 Remove edge ($y, \eta(y)$) \tcp*{Remove the connection of $y$ from its parent}
		 
		 Delete $y$ from $children(x)$;
	 }
	 }
	\If {$children(x) =  \phi$} {return;}
	
	Arrange $children(x)$ in the sequence $<y_1, \ldots y_k>$ such that $\dist{y_{i}}{\eta(y_{i})} \geq \dist{y_{i + 1}}{\eta(y_{i + 1})} ~\forall ~i = 1 \ldots k - 1$\;
	
%	Arrange $children(x)$ in the increasing order of their distances from $x$. Let $<y_1, \ldots y_k>$ be the sequence obtained.\;
	 
	%	 For $ y \in children(x), re-assigned(y) \gets false$ \textcolor{blue}{ \tcp*{boolean variable to indicate if clients of $rc_i$ are assigned to $lc_i$ or not; initially false}} 
		 
		 \For {$i = 1$ to $k-1$} {  
		 
		     \eIf{$n_{y_i} \geq \B$}  {
		 
		        Open facility $y_i$\;
		
		     Remove edge ($y_i, \eta(y_i)$) \tcp*{Remove the connection of $y_i$ from its parent}
		 
		     Delete $y_i$ from $children(x)$;
		    }
		    {
		     $n_{y_{i+1}} = n_{y_{i + 1}} + n_{y_{i}}$	 \tcp*{Send the clients of $y_i$ to $y_{i+1}$}
		 
		      Remove edge ($y_{i}, \eta(y_{i})$) \tcp*{Remove the connection of $y_i$ from its parent}
		 
		      Delete $y_{i}$ from $children(x)$\;
		    }
		 }
		 
		 \eIf {$n_{y_k} \geq \B$}  {
		 
		 Open facility $y_k$ \;
		 
		 %Remove edge ($y_1, \eta(y_1)$) \textcolor{blue}{\tcp*{Remove the connection of $y_1$ from its parent}}
		 
		 Delete $y_k$ from $children(x)$\;
		 }
		 {
		 $n_{\eta(y_k)} = n_{\eta(y_k)} + n_{y_{k}}$ \tcp*{Send the clients of $y_k$ to $\eta(y_k)$}
		 
		 %Remove edge ($y_1, \eta(y_1)$) \textcolor{blue}{\tcp*{Remove the connection of $y_1$ from its parent}}
		 
		 Delete $y_k$ from $children(x)$\;
		 }
		 
		 Return\;
	
	\label{TreeProcessing}
	\caption{Process($x$)}
\end{algorithm}

==> NEW Journal version WADS 2021 (LBUBFL)/Intro_rd.tex <==
\section{Introduction}
Facility location problem (FL) is a well motivated and extensively studied problem. Given a set of facilities with facility opening costs and a set of clients with a metric specifying the connection costs between facilities and clients, the goal is to select a subset of facilities such that the total cost of opening the selected facilities and connecting clients to the opened facilities is minimized. 



With growing emphasis on e-commerce marketplace platforms where we have a central platform mediating between the seller and the buyer, it becomes important to keep a check on the availability and profitability of the central store. A store serving too less clients can be non-profitable and a store getting too many orders can lead to bad service to the customers. This scenario leads to what we call as the lower- and upper- bounded facility location (LBUBFL) problem.
%\textcolor{blue}{
There are several other applications requiring both the lower as well as the upper bound on the number of clients assigned to the selected facilities. In a real world transportation problem presented by Lim et al.~\cite{Lim_transportation}, there are a set of carriers and a set of customers who wish to ship a certain number of cargoes through these carriers. There is a transportation cost associated to ship a cargo through a particular carrier. The goal of the company is to ship cargoes in these carriers such that the total transportation cost is minimized. There is a natural upper bound on the number of cargoes a carrier can carry imposed by the capacity of the carrier.  In addition, the shipping companies are required to engage their carriers with a \textquotedblleft minimum quantity commitment\textquotedblright~when shipping cargoes to United States. 
Another scenario in which the problem can be useful is in the applications requiring balancing of load 
on the facilities along with maintaining capacity constraints.

In this paper, we study the facility location problem with lower and upper bounds. We are given a set $ \clientset$ of clients and a set $\facilityset$ of facilities with lower bounds $\B_i$ and upper bounds $\capacityU_i$ on the minimum and the maximum number of clients a facility $i$ can serve, respectively. Setting up a facility at location $i$ incurs cost $f_i$(called the {\em facility opening cost}) and servicing a client $j$ by a facility $i$ incurs cost $\dist{i}{j}$ (called the {\em service cost}). We assume that the costs are metric, i.e., they satisfy the triangle inequality. Our goal is to open a subset $\facilityset' \subseteq \facilityset$ and compute an assignment function $\sigma : \clientset \rightarrow \facilityset'  $ (where $\sigma(j)$ denotes the facility that serves $j$ in the solution)
%serve the clients from the opened facilities such that every facility satisfies the lower and the upper bound 
such that $ \B_i \leq |\sigma^{-1}(i)| \leq  \capacityU_i ~\forall i \in \facilityset'$
and, the total cost of setting up the facilities and servicing the clients is minimised. The problem is known to be NP-Hard.  We present the first (constant factor) approximation for the problem with uniform lower and uniform upper bounds, i.e., $\B_i=\B$ and $\capacityU_i=\capacityU~\forall i \in \facilityset$ without violating the lower bounds, as stated in Theorem \ref{mainThm}.
%violating the upper bounds by a factor of $(3 + \epsilon)$ when both the lower and the upper bounds are uniform. 

\begin{definition}
A tri-criteria $ (\alpha, \beta, \gamma)$- approximation for LBUBFL problem is a solution $S= (\facilityset',\sigma$)
%in polynomial time 
satisfying $\alpha \B \leq~|\sigma^{-1}(i)| \leq \beta \capacityU ~\forall i \in \facilityset' , \alpha \le 1, \beta \ge 1$, with cost no more than  $\gamma OPT$, where $OPT$ denotes the cost of an optimal solution of the problem. 
\end{definition}

\begin{theorem} \label{mainThm}
  %( $\textcolor{magenta}{O(\ell^2), 1, 1+1/\ell}$) 
 A $(1, 5/2, O(1))$- 
 approximation can be obtained for LBUBFL in polynomial time.
\end{theorem}


Constant factor approximations are known for the problem with upper bounds only (popularly known as Capacitated Facility Location (CFL)) with~\cite{Shmoys,capkmByrkaFRS2013,GroverGKP18} and without~\cite{KPR,ChudakW99,mathp,paltree,mahdian_universal,zhangchenye,Bansal,Anfocs2014} violating the capacities using local search / LP rounding techniques. Constant factor approximations are also known for the problem with lower bounds only with~\cite{Minkoff_LBFL,Guha_LBFL,Han_LBkM} and without~\cite{Zoya_LBFL,Ahmadian_LBFL,Li_NonUnifLBFL} violating the lower bounds. The only work that deals with the bounds on both the sides is due to Friggstad et al. \cite{friggstad_et_al_LBUFL},
%To the best of our knowledge, the only known result for the problem is by friggstad et al. \cite{friggstad_et_al_LBUFL}, they have considered
which deals with the problem with non-uniform lower bounds and uniform upper bounds.  They gave a constant factor approximation for the problem using LP-rounding,  violating both the upper and the lower bound by a constant factor. The technique cannot be used to get rid of the violation in the lower bounds even if they are uniform as the authors show an unbounded integrality gap for the problem. Thus, our result is an improvement over them when the lower bounds are uniform in the sense that they violate both the bounds whereas we do not violate the lower bounds.


%\begin{theorem}
 %There is a polynomial time algorithm that approximates uniform-lower and uniform-upper bounded facility location problem within a constant factor violating the upper bounds by a factor of $3 + \epsilon$.
%\end{theorem}

\subsection{Related Work}
For capacitated facility location with  uniform capacities, Shmoys et al.~\cite{Shmoys} gave the first constant factor($7$) algorithm with a capacity blow-up of $7/2$ using LP rounding techniques.   An $O(1/\epsilon^2)$ factor approximation, with $(2 + \epsilon)$ violation in capacities, follows as a special case of C$k$FLP by Byrka et al.~\cite{capkmByrkaFRS2013}. Grover et al.~\cite{GroverGKP18} reduced the capacity violation to $(1 + \epsilon)$. For non-uniform capacities, Levi et al. \cite{LeviSS12} gave a 5-factor approximation algorithm using LP-rounding for a restricted version of the problem in which the facility opening costs are uniform. Later, An et al.~\cite{Anfocs2014} gave the first LP-based constant factor approximation algorithm without violating the capacities, by strengthening the natural LP. 
 
 The local search technique has been particularly useful to deal with capacities. Korupolu et al.~\cite{KPR} gave the first constant factor ($8+\epsilon$) approximation for  uniform capacities, which was further improved by Chudak and Williamson  \cite{ChudakW99} to ($6+\epsilon$). % followed by Chudak and Shmoys \cite{} to ($5.83+\epsilon$). 
 The factor was subsequently reduced to $3$ by Aggarwal et al.~\cite{mathp}, which is also the best known result for the problem. For non-uniform capacities, Pal et al.~\cite{paltree} gave the first constant factor $(8.53 + \epsilon)$ approximation algorithm which was subsequently improved to $(7.88 +\epsilon)$ by Mahdian and Pal~\cite{mahdian_universal} and to  $(5.83+\epsilon)$ by Zhang et al.~\cite{zhangchenye} with the current best being $(5 + \epsilon)$ due to Bansal et al.~\cite{Bansal}. 

Lower-Bounded Facility Location (LBFL) problem was introduced by Karger and Minkoff \cite{Minkoff_LBFL} and Guha et al.~\cite{Guha_LBFL} independently in 2000. Both of them gave a bi-criteria algorithm, that is a constant-factor approximation with constant factor violation in lower bounds. Zoya Svitkina \cite{Zoya_LBFL} presented the first true constant factor($448$) approximation for the problem with uniform lower bounds by reducing the problem to CFL. This was later improved to $82.6$ by Ahmadian and Swamy \cite{Ahmadian_LBFL} using reduction to a special case of CFL called  Capacitated Discounted Facility Location. Later Shi Li \cite{Li_NonUnifLBFL} gave the first true constant ($4000$) factor approximation for the problem with non uniform lower bounds. Li obtained the result by reducing the problem  to CFL via two intermediate problems called, LBFL-P(Lower bounded facility location with penalties) and TCSD(Transportation with configurable supplies and demands).
Han et al. \cite{Han_LBkM} gave a bi-criteria solution for the problem as a particular case of lower bounded $k$-FL problem when the lower bounds are non-uniform.

Another variant of LBFL, called Lower bounded $k$-Median problem(LB$k$M) was considered by Guo et al. \cite{Guo_LBkM} and Arutyunova and Schmidt \cite{arutyunova_LBkM} with uniform lower bounds, where they gave constant factor approximations for the problems by reducing them to CFL and LBFL respectively. For Lower bounded $k$-Facility Location problem LB$k$FL problem with non-uniform lower bounds, Han et al. \cite{Han_LBkM} presented a bi-criteria algorithm giving $\alpha$ factor violaton in lower bounds and $\frac{1+\alpha}{1-\alpha}\rho$-approximation where $\rho$ is the approximation ratio for $k$FL problem and $\alpha$ is a constant. They also extend these results to LB$k$M and lower bounded knapsack median problem.

Friggstad et al.~\cite{friggstad_et_al_LBUFL} is the only work that deals with the problem with bounds on both the sides. The paper considers non-uniform lower bounds and uniform upper bounds. They gave a constant factor approximation, using LP rounding techniques, violating both the lower and the upper bounds. %$(\rho = max \{ \frac{(2\zeta+1)(2\eta+1)+\zeta}{\zeta} +4(\eta+1), \frac{2\eta}{\eta-1} \frac{\zeta+1}{\zeta}\})$ 
%for . They use LP rounding techniques to give violations in both upper and lower bounds.
%$\alpha= max\{\zeta, \frac{2\eta}{\eta-1}\}$  and $\beta = \frac{\zeta+1}{\zeta}$ violations in lower and upper bound respectively.

\subsection{High Level Idea}
Let $I$ be an input instance of the LBUBFL problem. We first present a tri-criteria solution $(> 1/2, 3/2, O(1))$ violating both the lower as well as the upper bound and then 
%extend the ideas of Zoya et al.~\cite{Zoya_LBFL}to 
get rid of the violation in the lower bound by reducing the problem instance $I$ to an instance $I_{cap}$ of CFL via a series of reductions ($I \rightarrow I_1 \rightarrow I_2 \rightarrow I_{cap}$).
%
As we will see that maintaining  $\alpha > 1/2$ is crucial in getting rid of the violation in the lower bound and hence the tri-criteria solution of Friggstad et. al.~\cite{friggstad_et_al_LBUFL} cannot be used here as $\alpha < 1/2$ in their work. Also, when the lower bounds are uniform, our approach is comparatively simpler and straightforward.
%
%\textcolor{cyan}{Note that  the tri-criteria solution of Friggstad et. al.~\cite{friggstad_et_al_LBUFL} cannot be used as $\alpha < 1/2$ in their work. }
%and to keep check on the violations in the upper bounds.
%in a similar manner.
%\cite{Zoya_LBFL} to get rid of the violations in the lower bound.
%Capacities/upper bounds are violated at two places in \cite{Zoya_LBFL}: one while constructing a feasible solution for the $I_2$ instance; second while collecting at least $B$ clients at a facility in the facility trees. As the violation in $I_2$ cannot be handled, we defer the capacities to be handled later and ignore them while constructing $I_2$. 
%We control the violation in the capacities while processing the facility trees by converting them into binary trees.
Let $Cost_\mathcal{I}(\mathcal{S})$ denotes the cost of a solution $\mathcal{S}$ to an instance $\mathcal{I}$. We work in the following steps:
\begin{enumerate}
    \item 
    %We first compute a tri-criteria solution %$\textcolor{magenta}{((2\ell^2 + 3\ell +2), 1-1/\ell, 1+1/\ell})$ 
    %$\textcolor{cyan}{(O(1),(1 - \frac{1}{\ell}), (2 - \frac{1}{\ell}))}$ - approximation $S^t = (\facilityset^t, \sigma^t $)  to $I$ where $\ell > 2$ is a tuneable parameter via clustering and filtering techniques. The violations in the lower and the upper bounds are denoted by $\alpha$ and $\beta$ respectively. Thus, $\alpha = 1-1/\ell$ and $\beta = (2 - \frac{1}{\ell})$.

    We first compute a tri-criteria solution 
    $(> 1/2, 3/2, O(1))$ - approximation
    $S^t = (\facilityset^t, \sigma^t $) to $I$ via clustering and filtering techniques. 
   % The violations in the lower and the upper bounds are denoted by $\alpha$ and $\beta$ respectively.
    Thus, $\alpha >1/2$ and $\beta = 3/2$.
    
   \item We transform the instance $I$ into another instance $I_1$ of LBUBFL by moving the clients assigned to a facility $i$ in the  tri-criteria solution $S^t$ to $i$.  Let $O$ denote the optimal solution of $I$.
   To construct a solution of $I_1$, a client $j$ is assigned to a facility $i$ if it was assigned to $i$ in $O$. The connection cost is bounded by the sum of the cost $j$ pays in $S^t$ and in $O$. Thus, $Cost_{I_1}(O_1) \le  Cost_I(S^t) + Cost_I(O)$ where $O_1$ denotes the optimal solution of $I_1$.
   %$\le  (6\ell+ 7) Cost(O)$.
   
   
    
    \item The instance $I_1$ is transformed into another instance $I_2$ of LBFL, ignoring the upper bounds. The facility set is reduced to $\facilityset^t$ and the facilities in $\facilityset^t$ are assumed to be available free of cost. If a client $j$ is assigned, in $O_1$, to a facility $i$ not in $\facilityset^t$ then it is assigned to the facility $i'\in \facilityset^t$ nearest to $i$ (assume that the distances are distinct) and we open $i'$. The connection cost is bounded by twice the cost $j$ pays in $O_1$ by a simple triangle inequality. Let $O_2$ denote the optimal solution of $I_2$. Then,  $Cost_{I_2}(O_2) \le 2Cost_{I_1}(O_1)$.

    \item Finally, we create an instance $I_{cap}$ of CFL from $I_2$. The key idea in the reduction is: let $n_i$ be the number of clients assigned to a facility $i$ in $\facilityset^t$. If $i$ violates the lower bound, we create a demand of $\B - n_i$ at $i$ in the CFL instance otherwise we create a supply of $n_i - \B$ at $i$. The solution of the CFL instance then guides us to increase the assignments at some of the violating facilities until it gets $\B$ clients or decides to shut them.
   % shut some of these open facilities and increase the assignments at others so as to respect the lower bounds. 
    The process results in an increased violation in the capacities by plus $1$. 
    
    Let $O_{cap}$ be an optimal solution of $I_{cap}$. We show that  $Cost_{I_{cap}}(O_{cap}) \le (1+2\delta) Cost_{I_2}(O_2)$ for an appropriately chosen constant $\delta$.
    %$\le (1+2\delta)(12\ell+14)Cost(O)$.
    
    \item We obtain an $(5 + \epsilon)$-approximate solution $ AS_{cap}$ for $I_{cap}$ by using the algorithm of Bansal \etal~\cite{Bansal} for CFL.
    Thus, $Cost_{I_{cap}}(AS_{cap}) \le (5 + \epsilon) Cost_{I_{cap}}(O_{cap})$.
    
    %$ \le (5 + \epsilon) \cdot (1+2\delta) \cdot (12\ell+14) Cost(O)$.
    
     \item From $ AS_{cap}$, we obtain an approximate solution $AS_1$ to $I_1$ 
     %\textcolor{red}{do we obtain solution for $I_1$ or $I_2$?}
     such that the upper bounds are violated by a factor of $(\beta + 1)$ with no violation in lower bounds and $Cost_{I_1}(S_1) \le \frac{2(\alpha+1)}{(2\alpha-1)} Cost_{I_{cap}}(AS_{cap})$. Facility trees are constructed and processed bottom-up. Clients are either moved up in the tree to the parent or to a sibling until we collect  at least $\B$ clients at a facility. Whenever $\B$ clients are assigned to a facility $i$, $i$ is opened and the subtree rooted at $i$ is chopped off the tree and the process is repeated with the remaining tree. 
     %To keep the violation in the upper bounds low, we create binary facility trees.
     
  
   \item From $AS_1$, we obtain a solution $S$ to $I$ by paying the facility cost and moving the clients back to their original location. Thus, $ Cost_I(S) \le  Cost_I(S^t) + Cost_{I_1}(AS_1)$.
   
  
\end{enumerate}

Our main contributions are in Steps $1$ and $6$. 

\subsection{Organisation of the Paper}
In Section \ref{tri-criteria}, we present a tri-criteria algorithm for LBUBFL using LP rounding techniques. In Section \ref{instI1}, we reduce instance $I$ to $I_1$ and then $I_1$ to $I_2$, followed by reduction to  $I_{cap}$ in Section \ref{instIcap}. Finally, a bi-criteria solution, that does not violate the lower bounds, is obtained in Section \ref{bi-criteria}.

==> NEW Journal version WADS 2021 (LBUBFL)/LBFLO_ng.tex <==
\section{Instance $I_1$ and $I_2$}
\label{instI1}

We define an instance $I_1$ of LBFL.
Let $t \le B/4$.
Clients that were outliers in $S^t$ are removed in instance $I_1$.
Let $F^t$ be the set of facilities opened by $S^t$. For a client $j$, let $\sigma^t(j)$ be the facility to which $j$ is assigned in $S^t$. For $i \in F$, let $n_i$ be the number of clients served by $i$ in $S^t$. Move these clients to $i$ (see Fig.~\ref{Mapping1}). Thus, there are $n_i > B/2$ clients co-located with $i$. 
%For $i \in F^t$, $n_i = |(\sigma^t)^{-1}(i)|$ and for $i \notin F^t$, $n_i = 0$.   
In $I_1$, our facility set is $F$ and the clients are at their new locations. 
$f^1_i = 0$ for $i \in F^t$ and $=f_i$ for $i \notin F^t$.
%We will show that there exists a feasible solution $S_1$ of $I_1$ such that $Cost(S_1)$ is bounded by $Cost(S^t) + Cost(O)$. 
For a client $j$ served in $O$, let $\sigma^*(j)$ be the facility serving it. %$j$ in $O$. 

\begin{lemma}
There is a bi-criteria  solution $S_1$ of $I_1$ whose cost is bounded by $2 (Cost(S^t) + Cost(O))$.
\end{lemma}
\begin{proof}
We construct the solution $S_1$ of $I_1$ as follows: open $i$ in $S_1$ iff it is opened in $O$. Assign $j$ to $i$ in $S_1$ if it is assigned to $i$ in $O$. Let $O_o$ be the set of clients that are outliers in $O$. Let $O_i$ be the set of clients co-located with facility $i \in F^t$ and not served by $O$. Note that since $t \le B/4$ and $n_i > B/2$, at least $B/4$ clients at $i$ are served in $O$. Serve the clients in $O_i$ by the facilities serving the clients $(\sigma^t)^{-1} (i) \setminus O_i$ at a loss of factor $2$ in service cost.
%$j$ be a client co-located with facility $i= \sigma^t(j)$ and not served by $O$. 
$S_1$ violates the LB at most by a factor of $3/4$. LB is violated at a facility $i$ serving clients that were outliers in $S^t$ and are not present in $I_1$. Since this number is $\le B/4$, violation is at most $B - B/4 = 3B/4$.

%$S_1$ satisfies both the lower bound as well as the upper bound as $O$ does so. 
The cost $c( \sigma^t(j), \sigma^*(j))$ of serving $j$ from its new location is bounded by $c(j, \sigma^t(j)) + c(j, \sigma^*(j))$ if $j$ is not an outlier in $O$. Otherwise it can be charged to one of its co-located client that is served by $O$(see Fig. \ref{lemma1}). Thus, the claim follows.


\begin{figure}[t]
    \centering
    \includegraphics[width=9cm]{figures/mapping_0.jpg}
    \caption{Transforming instance $I$ to $I_1$ and  $I_1$ to $I_2$. Solid squares represent clients and circles represent facilities. Clients are moved to the facilities serving them in $S^t$ while transforming $I$ to $I_1$. Facilities not opened in $S^t$ are dropped while going from $I_1$ to $I_2$.}
    \label{Mapping1}
\end{figure} \end{proof}


\begin{figure}[t]
    \centering
    \includegraphics[width=4cm]{figures/lemma 1.jpg}
    \caption{$c( \sigma^t(j), \sigma^*(j)) \leq c(j, \sigma^t(j)) + c(j, \sigma^*(j))$ }
    \label{lemma1}
\end{figure}

  Next, we define an instance $I_2$ of LBFL.
  Instance $I_2$ is same as $I_1$ except that the facility set is $F^t$ now. $f^2_i = 0$ for all $i \in F^t$. 
 % We will show that there exists a feasible solution $S_2$ of $I_2$ such that $Cost(S_2)$ is bounded by $2 Cost(O_1)$ where
  Let $O_1$ be an optimal solution of $I_1$. 
  For a client $j$, let $\sigma^1(j)$ be the facility serving $j$ in $O_1$.

\begin{lemma}
There is a solution $S_2$ of $I_2$  that violates the LB by a factor of $3/4$ and whose cost is bounded by $ 2Cost(S_1)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_2$ of $I_2$: for $i$ \in $F^t$, open $i$ in $S_2$ if it is opened in $S_1$ and assign a client $j$ to it if it is assigned to $i$ in $S_1$. For $i$ \notin $F^t$, open its nearest facility $i'$ in $F^t$. Assign $j$ to $i'$ in $S_2$ if it is assigned to $i$ in $S_1$. $S_2$ violates the lower bound by $3/4$ as $S_1$ does so.  The cost $c( \sigma^t(j), i')$
%$c( \sigma^t(j), \sigma^*(j))$ 
of serving $j$ from its new location is bounded by $c(\sigma^t(j), \sigma^1(j)) + c( \sigma^1(j), i') \le 2 c(\sigma^t(j), \sigma^1(j))$ (since $i'$ is closest in $F^t$ to $i =  \sigma^1(j)$) where $\sigma^1(j)$ is the facility that serves $j$ in $S_1$. Summing over all $j$'s we get the desired claim.

%$c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(i, \sigma^1(j)) \le c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(\sigma^t(j), \sigma^1(j))$ (since $i$ is closest in $F^t$, to $i' = \sigma^1(j)$) $\le 2(c(j, \sigma^t(j)) + c(j, \sigma^1(j)))$ (See Figure 1). Summing over all $j$'s, the claim follows.
%Same as Zoya etal
\end{proof}




\section{Instance $I_{cap}$ for Capacitated Facility Location}
\label{instIcap}
For each facility $i \in F^t$, let $l(i)$ be the distance of $i$ from a nearest facility  $i' \in F^t$, $i' \neq i$ and let $\delta$ be a constant chosen appropriately. We say that a facility $i$ is {\em small} if $0< n_i < B$ and it is {\em big} otherwise. Every big facility $i$ is split into two co-located facilities $i_1$ and $i_2$ . We split the set of clients, at $i$, also into two sets.  $B$ of these clients are placed at $i_1$ and the remaining $n_i - B$ clients at $i_2$ (see Fig.~\ref{Mapping2}). The second type of big facilities are called {\em free}. 
 \begin{figure}
    \centering
    \includegraphics[width=8cm]{figures/mapping_1.jpg}
    \caption{Transforming instance $I_2$ to $I_{cap}$:
    %Solid squares represent clients and circles represent facilities. 
    $i'$ is small, $i$ is big.
    $i$ is split into $i_1$ and $i_2$ while transforming $I_2$ to $I_{cap}$, $i_2$ is free. Demand at the small facility $i'$ is $B - n_{i'} = 1$ and at $i_1$, $i_2$, it is $0$. Capacities of $i'$ and $i_1$ are $B = 4$ and it is $n_{i} - B = 3$ of the free facility $i_2$.}
    \label{Mapping2}
\end{figure}
%\textcolor{red}{ Let $F_f$ denote the set of free facilities (...will delete).} 
 Let $\bar F^t$ be the set of facilities so obtained. The set of clients and the set of facilities are both $\bar F^t$. %In the $I_{cap}$ instance, we place demands  at all of these facilities. 
 The facility costs, capacities and demands are as shown in Table~\ref{tab:my_label} (also see Fig.~\ref{Mapping2}).
 \begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
       Type & $n_i$ & $u_i$ & $d_i$ & $f^t_i$ \\
        \hline
       {\em small} & $n_i \leq B$ & $B$ & $B- n_i$& $\delta n_i l(i)$ \\
        \hline
       {\em big} & $n_i > B$ & ($i_1$)$B$ & $0$& $\delta B l(i)$ \\
        & & ($i_2$) $n_i - B$ & $0$& $0$ \\
       
        % &  &
          \hline 
       % $3$ & $0$ & $B$ & $B$& $\delta B l(i)$ \\
        %\hline
    \end{tabular}
    \caption{Instance of $I_{cap}$: $d_i, u_i, f^t_i$ are demands, capacities and facility costs resp.}
    \label{tab:my_label}
\end{table}
 
 %Let $O_{cap}$ be an optimal solution to $I_{cap}$.
 
 %\textcolor{red}{define delta and l(i)}
 %The second type of big facilities are called {\em free}. %and the clients placed at them are also called {\em free}. 
 %Let $F_f$ denote the set of free facilities. 
 %and $Cf(i)$ denote the set of free clients at facility $i \in F_b$. i.e.$Cf(i)$ is the set of clients placed at $i_2 \in F_f$ (See Figure 2)....need to define $l(i)$.





\begin{lemma}
%A feasible solution $S_{cap}$ for 
Cost of optimal solution to 
$I_{cap}$ is bounded by $(1+2\delta)Cost(O_2)$.
\end{lemma}

\begin{proof}
We will construct a feasible solution $S_{cap}$ to $I_{cap}$ of bounded cost.
Let $O_2$ be an optimal solution of $I_2$. As $O_2$ satisfies the lower bound,  we can assume wlog that if $i$ is opened in $O_2$ then it serves all of its clients if $n_i \le B$ (before taking more clients from outside) and it serves at least $B$ of its clients before sending out its clients to other (small) facilities otherwise. 
Also, if two big facilities are opened in $O_2$, one does not serve the clients of the other. Let $\rho^2(j_i, i')$ denote the number of clients co-located at $i$ and assigned to $i'$ in $O_2$ and $\rho^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $S_{cap}$ .
 \begin{figure}[t]
    \centering
    \includegraphics[width=10cm]{figures/O2_Scap assignments.jpg}
    \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ and $i'$ are closed in $O_2$. $\rho^2(j_{i_1}, t_1) = 2,~\rho^2(j_{i_1}, t_2) = 1,~\rho^2(j_{i_1}, t_3) = 1,~ \rho^2(j_{i_1}, t_4) = 0$ and $\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 1,~\rho^2(j_{i_2}, t_3) = 1,~ \rho^2(j_{i_2}, t_4) = 0$.  } %The middle figure shows how the assignments look like after splitting the big facilities. $\rho^2(j_{i_1}, i') = 2(/1/1)$ for $i'$ = top three facilities $t_1(/t_2/t_3)$ $\rho^2(j_{i_2}, i') = 1(/1/1) $ for the bottom three facilities $t_2(/t_3/t_4)$. Note that $t_1$ }
    \label{Mapping}
\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{figures/O2_Scap assignments (2.1).jpg}
   \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ is open in $O_2$.   $\rho^c(j_{t_1}, i_2) = \rho^2(j_{i}, t_1) = 1, \rho^c(j_{t_2}, i_2) = \rho^2(j_{i}, t_2) = 2$,
  % $\rho^2(j_{i_1}, t_1) = 1,~\rho^2(j_{i_1}, t_2) = 1$ and %$\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 2$. 
   $i_2$ is open in $S_{cap}$. $t_1$ and $t_2$ must be small.}
    \label{O2_SCap2}
\end{figure}
    \begin{enumerate}
        \item   if $i$ is closed in $O_2$ then open $i$ if $i$ is small
        and open $(i_1 \& i_2)$ if it is big.
        
        Assignments are defined as follows (see Fig.~\ref{Mapping}):
        \begin{enumerate}
            \item If $i$ is small: Let $i$ serve its own demand. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. Thus, 
        $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $ i' \ne i$ and $\rho^c(j_i, i) = d_i$. Also,
        $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). 
        Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = B = u_i$. %Thus capacities are respected.
      
         
        
       \item If $i$ is big: assign $\rho^2(j_{i_1}, i')$ (/$\rho^2(j_{i_2}, i')$) demand of $i'$ to $i_1$(/$i_2$) in our solution for small $i' \ne i$. Thus,
        $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_1) = \sum_{small~i' \ne i} \rho^2(j_{i_1}, i') \le B = u_{i_1}$.
         $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_2) = \sum_{small~i' \ne i} \rho^2(j_{i_2}, i') \le n_i - B = u_{i_2}$.
         The second equality holds in each case as $i$ is closed in $O_2$.
        % Since there are no demands at $i_1$ and $i_2$, the capacities are respected.
     
       \end{enumerate}
     
     \item Open free facility $i_2$ 
     %for $i_2 \in F_f$ (and 
     ($i$ is opened in $O_2$) (see Fig.~\ref{O2_SCap2}): assign $\rho^2(j_{i}, i')$  demand of $i'$ to $i_2$ in our solution for small $i' \ne i$. Thus,
     %Thus,
      %  $\sigma^c(j_{i'}, i_2) = %\sigma^1(j_{i_2}, i'), i \ne i'$  
        $\sum_{i' \ne i}\rho^c(j_{i'}, i_2) = \sum_{i' \ne i} \rho^2(j_{i}, i') \le n_i - B$ (the inequality holds by assumption on $O_2$) $= u_{i_2}$.
       % Thus the capacities are respected as there are no demands at $i_2$.
       
       \item \textcolor{red}{Open the special facility $i^*$ ($u_{i^*} = t, d_{i^*} = 0, f_{i^*} = 0 )$. If $i$ is closed in $S_{cap}$ and it is small, then it must be opened in $S_2$. Let $sp(i)$ be the set of clients in $Out(S^t)$ that are served by $i$ in $S/S_1/S_2)$. Assign $|sp(i)|$ demand of $i$ to the special facility $i^*$.}
    \end{enumerate}
    
    Next, we show that all the demands are satisfied. If a facility is opened in $S_{cap}$, it satisfies its own demand. 
Let $i$ be closed in $S_{cap}$. If $i$ is big ,we need not worry as $i_1$ and $i_2$ have no demand. So, let $i$ is small. Then, it must be opened in $O_2$. Then, 
\textcolor{red}{
$\sum_{i' \ne i}\rho^c(j_{i}, i') = $
$\sum_{small ~i' \ne i,  }\rho^c(j_{i}, i') + \sum_{i'_1: i' ~is ~big}\rho^c(j_{i}, i'_1) + 
\sum_{i'_2: i' ~is ~big}\rho^c(j_{i}, i'_2) + \rho^c(j_{i}, i^*)= $
$\sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i'_1 : i' ~is ~big} \rho^2(j_{i'_1}, i)  + \\ \sum_{i'_2 : i' ~is ~big}\rho^2(j_{i'_2}, i) + |sp(i)| = \sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i' ~is ~big}\rho^2(j_{i'}, i)  + |sp(i)| = \sum_{i' \ne i}\rho^2(j_{i'}, i)  + |sp(i)|$
$\ge B - n_i$  (since $O_2$ is a feasible solution of $I_2$) $= d_i$. 
}

Next, we bound the cost of the solution. The connection cost is same as that of $O_2$. %Next, we consider the facility opening costs. 
For facility costs, consider a facility $i$ that is opened in our solution and closed in $O_2$. Such a facility must have paid a cost of at least $n_i l(i)$ to get its clients served by other (opened) facilities. The facility cost paid by our solution is $ \delta min\{n_i, B\} l(i) \le \delta n_i l(i)$.  If $i$ is opened in $O_2$, then it must be serving at least $B$ clients and hence paying a cost of at least $B l(i)$. In this case also, the facility cost paid by our solution is $ \delta min\{n_i, B\} l(i) \le \delta B l(i)$. Thus the facility cost is bounded by $2\delta Cost(O_2)$ and the total cost is bounded by $(1 + 2 \delta) Cost(O_2)$. Factor $2$ comes because we may have counted an edge $(i, i')$ twice, once as client when $i$ was closed and once as a facility when $i'$ was opened in $O_2$.
\end{proof}



\section{Bi-criteria Solution $S_1$ to $I_1$ from approximate solution $AS_{cap}$ to  $I_{cap}$}
\label{bi-criteria}

Next we obtain a solution $\bar S_1$ to $I_1$ that violates the capacities/upper bounds by a factor of $(\beta + 1)$ without violating the lower bound. 
Wlog assume that if a facility $i$ is opened in $AS_{cap}$ then it serves all its demand. This is always feasible as $d_i \le u_i$. $S_1$ is obtained from $AS_{cap}$ by first defining the assignment of the clients and then opening the facilities that get at least $B$ clients. Let $\rhobar^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $AS_{cap}$ and $\rhobar^1(j_i, i')$ denotes the number of clients co-located at $i$ and assigned to $i'$ in $S_1$. 
%\textcolor{red}{ Initially each facility is assigned the clients co-located with it.}
Clients are assigned in three steps. In the first step, we define the assignments as follows:  For a big facility $i'$, assign all the clients co-located at $i'_1$ and $i'_2$ to $i$. For a small facility $i'$, assign the clients co-located at $i'$ to itself.  For small $i'$, additionally, we do the following  re-assignments (see Fig. \ref{type1}): $(i) $For small $i \ne i'$, assign $\rhobar^c(j_{i'}, i)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for small $i$. $(ii)$ For big $i$, assign $\rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ for big $i$.
\begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{figures/Type 1 Assignments.jpg}
    \caption{($a$) $B =5$, $t_1, t_2, t_3$ have demands $1$, $2$ and $1$ unit each respectively. In solution $AS_{cap}$, $1$ unit of demand of $t_1$ and $2$ units of demand of $t_2$ are assigned to $t_3$. (b) Solution $S_1$: initially, $n_i$ clients are initially assigned to facility $i$. (c) Type $1$ reassignments: $1$ and $2$ clients of $t_3$ reassigned to $t_1$ and $t_2$ respectively. After this reassignment, $t_3$ has only $1$ client.}
    \label{type1}
\end{figure}

\begin{claim}
    $(i)$ $\sum_{i' \ne i} \rhobar^1(j_i, i') \le n_i$, $\forall$ $i \in \bar F^t$.
    $(ii)$ $\sum_{i \ne i'} \rhobar^1(j_i, i') \le \beta U_{i'}$, $\forall$ $i' \in \bar F^t$.
 \end{claim}

\begin{proof}

    $(i)$ Since $\rhobar^c(j_{i}, i) = d_i$ therefore $\sum_{i' \ne i} \rhobar^c(j_{i'}, i) \le u_i - d_i \le n_i$ in all the cases. $(ii)$ $\rhobar^1(j_{i'}, i') = n_{i'}$.  
$\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for $ i' \ne i$. Thus,
 %   
    %\item $\rhobar^1(j_{i'}, i') =$ original $n_{i'}$ clients $ %\rhobar^c(j_{i'}, i')$.....(1) $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for $ i' \ne i$.....(2) Adding (1) and ((2) over all $i \ne i'$), we get
%
$\sum_{i} \rhobar^1(j_i, i') = n_{i'} + \sum_{i \ne i'} \rhobar^c(j_{i'}, i) \le n_{i'} + d_{i'} \le max\{B, n_{i'}\} \le \beta U_{i'}$
\end{proof}

Note that $S_1$ so obtained may not still satisfy the lower bound requirement. In fact, 
 although each facility was assigned $n_i \ge  \alpha B \ge B/2$ clients initially, they may be serving less clients now after type $1$ re-assignments. For example, in Fig. \ref{type1}, $t_3$ had $4$ clients initially which was reduced to $1$ after type $1$ reassignments. Let $P \subseteq  F^t$ be the set of facilities each of which is serving at least $B$ clients and  $\bar P =  F^t \setminus P$ be the set of remaining facilities. 
 %That is, $ P= \{ i' \in F^t: \sum_{i}\rhobar^1(j_{i}, i') \ge B$\}.
 We open all the facilities in $P$ and let them serve the clients assigned to them after type $1$ re-assignments.
 
 \begin{observation}
 If a  small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge B$.
     Similarly for a big facility $i'$, if $i'_1$ was closed in $AS_{cap}$ then $i'$ is in $P$.
     %\item If a small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge B$.
    
     
    % \item If $i'$ is big then $\rhobar^1(j_{i'}, i') = n_{i'}  \ge B$
 \end{observation}
 
 
 Thus, a small facility is in $\bar P$ only if it was open in $AS_{cap}$ and a big facility $i$ is in $\bar P$ only if $i_1$ was open in $AS_{cap}$. 
 %Also note that although each facility in $\bar P$ served at least $\alpha B \ge B/2$ clients in the tri-criteria solution $S^t$, they may be serving less clients now after step $1$ of assignment. \textcolor{red}{See Figure \ref{type1} for an example}.
 We now try to group these facilities so that each group serves at least $B$ clients and open one facility in each group that serves all the clients in the group. For this we construct what we call as {\em facility trees}. We construct a graph $G$ with nodes corresponding to the facilities in $\bar P$. For $i \in \bar P$, let $\eta(i)$ be the nearest other facility to $i$ in $F^t$. Then, $G$ consists of edges $(i, \eta(i))$. Each component of $G$ is a tree except possibly a double-edge cycle at the root. In this case, we say that we have a root, called {\em root-pair}, consisting of a pair of facilities say $i_i$ and  $i_2$ and denoted by $<i_{r_1}, i_{r_2}>$. Also, a facility $i$ from $P$, if present must be at the root of a tree. We try to process each tree bottom-up sending the clients of each facility to its parent. However doing so may result in too much violation in the capacities at the parent facility. 
 \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{figures/tree.jpg}
    \caption{Binary tree conversion process: (a) Tree $\mathcal{T}$ of unbounded degree: $a<b<c<g,~c<d$. (b) Binary routing tree (intermediate stage). (c) Final tree.}
    \label{tree}
\end{figure}

 To keep the capacity violation in check, we convert each tree into a binary tree
 %\textcolor{red}{
 (see Fig. \ref{tree}): first of all, we treat the double-edge cycle, if any, as a single node for this purpose. Then, at every node $x$, arrange the children of $x$ from left to right in non-decreasing order of distance from $x$.
  For each child $y$ (except for the nearest child) of $x$, add an edge to its left sibling %with weight $2\dist{ y}{\eta(y)}$ 
  and remove the edge $( y, x)$. There is no change in the outgoing edge of the leftmost child of $x$. 
Let $\sigmaone(y)$ be the parent of  $y$ in the so constructed tree. Its easy to see that $\dist{y}{\sigmaone(y)} \leq 3 \dist{y}{\eta(y)}$. Thus, we replace $\dist{y}{\sigmaone(y)}$ by $3 \dist{y}{\eta(y)}$ for all $y$. Henceforth, whenever we refer to distances, we mean the new edge weights. Now, every node has in-degree of at most $2$ with the in-degree of the root being at most $1$. 

Now we are ready to define our second type of re-assignments. Process the tree bottom-up as follows (see Fig. \ref{type2-3}): If $i$ has at least $B$ clients, open $i$ and disconnect $i$ from the tree by cutting the edge $(i, \sigmaone(i))$ else send its clients to its parent facility. The process is repeated till we reach the root. 



There are two possibilities at the root: either we have a facility $i$ from $P$ or we have a root-pair $<i_{r_1}, i_{r_2}>$. In the first case, we are done as $i$ is already open and has at least $B$ clients. To handle the second case, we need to do a little more work. So, we define our assignments of third type as follows (see Fig. \ref{type2-3}): ($i$) If the total number of clients at the root pair $<i_{r_1},i_{r_2}>$ is at least $B$ then open the facility with more number of clients, say $i_{r_1}$ and send the clients of $i_{r_2}$ to $i_{r_1}$. %(in our case, we cannot have a scenario in which both have at least B clients. If $i_2$ is the facility at which the rest of the tree hangs then the number of clients at $i_1$ cannot be more than $B$.....this is not true in Zoya's case because there a tree hangs at both the ends of the double-edge loop which we have eliminated....Since the number of clients at $i_1$ is less than B..the number of clients along any edge is still less than B ....only for our understanding...to be deleted later)..
($ii$) If the total number of clients at the root pair $<i_{r_1},i_{r_2}>$ is less than $B$, then let $i$ be the node in $P$ nearest to $\{i_{r_1}, i_{r_2}\}$. i.e., $i$ is already open and has at least $B$ clients. Send the clients of $i_{r_1}$ and $i_{r_2}$ to $i$.
\begin{figure}[t]
	\begin{tabular}{ccc}
		\includegraphics[width=40mm,scale=1.0]{figures/Type 2 Assignments.jpg}
		&& 
		\includegraphics[width=65mm,scale=1.0]{figures/Type 3 Assignments.jpg} 	
		\\
		\textbf{(A)}&&\ \ \textbf{(B)}& \ \
	\end{tabular}
	\caption{$B=4$ (A) Type 2 Assignments: (a) Before assignments. (b) After assignments.
	(B) Type 3 Assignments (i) Total clients at root pair $<i_{r_1},i_{r_2}>$ is at least $B$: (a) Before assignments. (b) After assignments: $i_{r_2}$ is open.  (ii) Total clients at root pair $<i_{r_1},i_{r_2}>$ is less than $B$: (a) Before assignments. (b) After assignments: $i_{r_1},i_{r_2}$ are both closed. 
	}
	\label{type2-3}
\end{figure}

%($i$) If both $i_1$ and $i_2$ have at least $B$ clients, open bot of them ($ii$) if one of them say $i_1$ has at least $B$ clients but $i_2$ doesn't then open $i_1$ and send the clients of $i_2$ to $i1$ ($iii$) If both of them have clients less than $B$ but in total they have at least $B$ clients, open any one of them, say $i_1$ and send the clients of the other to $i_1$.
 
 
 Next we bound the capacity violation: Let $\pi_i$ be the number of clients assigned to the facility $i$ after first type of re-assignments. Then as shown earlier, $\pi_i \le \beta U$. Let $ i_c$ be the only child of the root (/root pair). Let $i$ be the parent of $ i_c$. In second and third types of assignments,  we never collect more than $2B$ clients at any node till we reach $i_c$. Now we have the following scenarios: Suppose $ i_c$ has less than $B$ clients, we have the following cases: ($i$)  the root node $i$ is in $P$ and it gets additional at most $B$ clients from $i_c$ making a total of at most $\pi_i + B \le \beta U + B \le (\beta + 1) U$ clients at $i$.
 ($ii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at least $B$. Number of clients at $i_{r_1}$ and $i_{r_2}$ are at most $B$ and $2B$ respectively. Thus, the number of clients the opened facility gets is at most $3B \le 3 U$.
 ($iii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients less than $B$. Number of clients at the root pair and their nearest facility in $P$ are at most $B$ and $\beta U$ respectively. Thus, the number of clients the opened facility in $P$ gets is at most $\beta U + B \le (\beta + 1) U$. 
 %The case when $i_c$ has at least $B$ clients leads to the third scenario above and hence handled.
 
 We next bound the connection cost: the cost of first type of re-assignments is same as that of $AS_{cap}$.
 To bound the connection cost of second type, observe that we never send more than $B$ clients on any edge. 
 %In the second type of assignment, 
 Let a facility $i$ sends its (at most $B$ clients) to its parent. Since the facility $i$ was opened in $AS_{cap}$, it pays facility cost of $\delta l(i) min \{n_i, B\} \ge \delta l(i) \alpha B$. Summing over all $i \in \bar P$ for the second type of re-assignments, we see that the total connection cost in these re-assignments is bounded by $3 Cost_f(AS_{cap})/\alpha \delta$ where $Cost_f(.)$ is the facility opening cost of a solution to the $I_{cap}$ instance. For the third type of re-assignments, the cost of sending (at most $B$) clients by a facility $i$ in the root pair $<i_{r_1}, i_{r_2}>$ is not bounded by $B l(i)$. We bound the cost as follows: the total number of clients, initially at $i_{r_1}$ and $i_{r_2}$ was $\ge 2 \alpha B$. However, during re-assignments of type $1$, some of them got reassigned to other facilities. Note that these (other) facilities must have been closed in $AS_{cap}$ and hence do not belong to $\bar P$. Hence, each of these reassignments correspond to an assignment in $AS_{cap}$ whose cost was at least $l(i)$ and a total of at least $(2\alpha  - 1)B l(i)$. Hence the cost of type $3$ re-assignments is bounded by $3 Cost_c(AS_{cap})/ (2\alpha  - 1)$ where $Cost_c(.)$ is the connection cost of a solution to the $I_{cap}$ instance. Hence the total cost of solution $S_1$  is $6\alpha/(2\alpha-1)$ for $\delta= (2\alpha-1)/6\alpha^2$.
 


==> NEW Journal version WADS 2021 (LBUBFL)/LBUBFLGeneralTree.tex <==
\section{Instance $I_1$ and $I_2$}
\label{instI1}

In this section, we first transform instance $I$ to instance $I_1$ ($\facilityset,~\clientset,~f^1,~c,~\B,~\capacityU$) of LBUBFL by moving the clients to the facilities serving them in the tri-criteria solution $S^t$ and then transform $I_1$ to an instance $I_2$ of LBFL by removing the facilities not opened in $S^t$.
%Let $\facilityset^t$ be the set of facilities opened by $S^t$. 
Recall that for a client $j$,  $\sigma^t(j)$ is the facility  in $\facilityset^t$ serving $j$. For $i \in \facilityset^t$, let $n_i$ be the number of clients served by $i$ in $S^t$, i.e., $n_i = |(\sigma^t)^{-1}(i)|$ and for $i \notin \facilityset^t$, $n_i = 0$. Move these clients to $i$ (see Fig.~\ref{Mapping1}). Thus, there are $n_i$ clients co-located with $i$. In $I_1$, our facility set is $\facilityset$ and the clients are at their new locations. Facility opening costs in $I_1$ are modified as follows: $f^1_i = 0$ for $i \in \facilityset^t$ and $=f_i$ for $i \notin \facilityset^t$.  


\begin{lemma}
Cost of optimal solution of $I_1$ is bounded by $Cost_I(S^t) + Cost_I(O)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_1$ of $I_1$: open $i$ in $S_1$ iff it is opened in $O$. Assign $j$ to $i$ in $S_1$ iff it is assigned to $i$ in $O$. $S_1$ satisfies both the lower bound as well as the upper bound as $O$ does so. For a client $j$, let $\sigma^*(j)$ be the facility serving $j$ in $O$. Then, the cost $\dist{ \sigma^t(j)}{\sigma^*(j))}$ of serving $j$ from its new location, $\sigma^t(j)$ is bounded by $\dist{j}{\sigma^t(j)} +\dist{j}{\sigma^*(j)}$ (see Fig. \ref{lemma1}). Summing over all $j \in \clientset$ and adding the facility opening costs, we get the desired claim.

\begin{figure}[t]
    \centering
    \includegraphics[width=9cm]{ Mapping_0.jpg}
    \caption{Transforming instance $I$ to $I_1$ and  $I_1$ to $I_2$. Solid squares represent clients and circles represent facilities. Clients are moved to the facilities serving them in $S^t$ while transforming $I$ to $I_1$. Facilities not opened in $S^t$ are dropped while going from $I_1$ to $I_2$.}
    \label{Mapping1}
\end{figure} 


\begin{figure}[t]
    \centering
    \includegraphics[width=4cm]{ lemma_1.jpg}
    \caption{$c( \sigma^t(j), \sigma^*(j)) \leq c(j, \sigma^t(j)) + c(j, \sigma^*(j))$ }
    \label{lemma1}
\end{figure}
\end{proof}



%section{Instance $I_2$} 
%\label{instI2}
    
   Next, we define an instance ~$I_2(\facilityset^t,~\clientset,~f^2,~c,~\B)$ of LBFL from $I_1$ by removing the facilities not in $\facilityset^t$ and ignoring the upper bounds. Instance $I_2$ is same as $I_1$ without the upper bounds, except that the facility set is $\facilityset^t$ now. Thus, $f^2_i = 0~\forall~i \in \facilityset^t$. % We will show that there exists a feasible solution $S_2$ of $I_2$ such that $Cost(S_2)$ is bounded by $2 Cost(O_1)$ where
  Let $O_1$ be an optimal solution of $I_1$. 
  For a client $j$, let $\sigma^1(j)$ be the facility serving $j$ in $O_1$.
 
 
 

\begin{lemma}
Cost of optimal solution of $I_2$ is bounded by $ 2Cost_{I_1}(O_1)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_2$ to $I_2$: for $i \in \facilityset^t$, open $i$ in $S_2$ if it is opened in $O_1$ and assign a client $j$ to it if it is assigned to $i$ in $O_1$. For a facility $i \notin \facilityset^t$, %the clients assigned to it need to be assigned to some other facility in $\facilityset^t$. Thus, for such $i$'s,
open its nearest facility $i'$ (if not already opened) in $\facilityset^t$. Assign $j$ to $i'$ in $S_2$ if it is assigned to $i$ in $O_1$. $S_2$ satisfies the lower bound  as $O_1$ does so. Note that it need not satisfy the upper bounds. This is the reason we dropped upper bounds in $I_2$. The cost $c( \sigma^t(j), i')$
%$c( \sigma^t(j), \sigma^*(j))$ 
of serving $j$ from its new location is bounded by $c(\sigma^t(j), \sigma^1(j)) + c( \sigma^1(j), i') \le 2 c(\sigma^t(j), \sigma^1(j))$ (since $i'$ is closest in $\facilityset^t$ to $i =  \sigma^1(j)$). Summing over all $j \in \clientset$ we get the desired claim.
%$c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(i, \sigma^1(j)) \le c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(\sigma^t(j), \sigma^1(j))$ (since $i$ is closest in $\facilityset^t$, to $i' = \sigma^1(j)$) $\le 2(c(j, \sigma^t(j)) + c(j, \sigma^1(j)))$ (See Figure 1). Summing over all $j$'s, the claim follows.
%Same as Zoya etal
\end{proof}

%\textcolor{blue}{can be deleted now...I have added a line in the proof itself....Note that, while defining the instance $I_2$, we ignored the upper bounds on facilities because a facility $i' \in \facilityset^t$ might be nearest to many other facilities $\notin \facilityset^t$ thereby serving clients of all of them and hence violating upper bound.}


\section{Instance $I_{cap}$ of Capacitated Facility Location Problem}
\label{instIcap}

 
 In this section, we create an  instance $I_{cap}$ of capacitated facility location problem from $I_2$. 
 The main idea is to create  a demand of $\B - n_i$ units at locations where the number of clients served by the facility is less than $\B$ and a supply of $n_i - \B$ units at locations with surplus clients. For each facility $i \in \facilityset^t$, let $l(i)$ be the distance of $i$ from a nearest facility  $i' \in \facilityset^t$, $i' \neq i$ and let $\delta$ be a constant to be chosen appropriately. A facility $i$ is called {\em small} if $0< n_i \leq \B$ and  {\em big} otherwise. A big facility $i$ is split into two co-located facilities $i_1$ and $i_2$.
  We also split the set of clients at $i$ into two sets:  arbitrarily, $\B$ of these clients are placed at $i_1$ and the remaining $n_i - \B$ clients at $i_2$ (see Fig.~\ref{Mapping2}). 
   Instance $I_{cap}$ is then defined as follows:
A {\em small} facility $i$ needs additional $\B - n_{i}$ clients to satisfy its lower bound; hence a demand of $\B - n_{i}$ is created at $i$ in the $I_{cap}$ instance. A facility with capacity $\B$ and facility opening cost $\delta n_{i} l(i)$ is also created at $i$. 
For a {\em big} facility $i$, correspondingly two co-located facilities $i_1$ and $i_2$ are created with capacities $\B$ and $n_i - \B$ respectively. The facility opening cost of $i_1$ is $\delta \B l(i)$ whereas $i_2$ is free. Intuitively, since the lower bound of a big facility is satisfied, it has some extra ($n_i - \B$) clients, which can be used to satisfy the demand of clients in $I_{cap}$ for free. 
 %Thus, we define capacity of $i_1$ and $i_2$ to be $\B$ and $n_i - \B$ respectively. 
 The second type of big facilities are called {\em free}. 
 %The facility costs, capacities and demands are as shown in
 We use $i$ to refer to both the client (with demand) as well as the facility located at $i$. Let $\bar \facilityset^t$ be the set of facilities so obtained. The set of clients and the set of facilities are both $\bar \facilityset^t$. Table~\ref{tab:my_label} summarizes the instance. Also see Fig.~\ref{Mapping2}
 
 \begin{figure}
    \centering
    \includegraphics[width=8cm]{ Mapping_1.jpg}
    \caption{Transforming instance $I_2$ to $I_{cap}$: $\B = 4$,
    %Solid squares represent clients and circles represent facilities. 
    $i'$ is small, $i$ is big.
    $i$ is split into $i_1$ and $i_2$ while transforming $I_2$ to $I_{cap}$, $i_2$ is free. Demand at the small facility $i'$ is $\B - n_{i'} = 1$ and at $i_1$, $i_2$, it is $0$. Capacities of $i'$ and $i_1$ are $\B = 4$ and it is $n_{i} - \B = 3$ of the free facility $i_2$.}
    \label{Mapping2}
\end{figure}
 
 \begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
       Type & $n_i$ & $u_i$ & $d_i$ & $f^t_i$ \\
        \hline
       {\em small} & $n_i \leq \B$ & $\B$ & $\B- n_i$& $\delta n_i l(i)$ \\
        \hline
       {\em big} & $n_i > \B$ & ($i_1$)$\B$ & $0$& $\delta \B l(i)$ \\
        & & ($i_2$) $n_i - \B$ & $0$& $0$ \\
       
        % &  &
          \hline 
       % $3$ & $0$ & $\B$ & $\B$& $\delta \B l(i)$ \\
        %\hline
    \end{tabular}
    \caption{Instance of $I_{cap}$: $d_i, u_i, f^t_i$ are demands, capacities and facility costs resp.}
    \label{tab:my_label}
\end{table}
 
 %Let $O_{cap}$ be an optimal solution to $I_{cap}$.
 
 %\textcolor{red}{define delta and l(i)}
 %The second type of big facilities are called {\em free}. %and the clients placed at them are also called {\em free}. 
 %Let $F_f$ denote the set of free facilities. 
 %and $Cf(i)$ denote the set of free clients at facility $i \in F_b$. i.e.$Cf(i)$ is the set of clients placed at $i_2 \in F_f$ (See Figure 2)....need to define $l(i)$.

 %In the next lemma, we show the existence of a feasible solution to $I_{cap}$ with cost no more than $(1+2\delta)Cost(O_2)$ where $O_2$ is an optimal solution of $I_2$. 




\begin{lemma}
%A feasible solution $S_{cap}$ for 
Let $O_2$ be an optimal solution of $I_2$. Then, cost of optimal solution to $I_{cap}$ is bounded by $(1+2\delta)Cost_{I_2}(O_2)$.
\end{lemma}

\begin{proof}
We will construct a feasible solution $S_{cap}$ to $I_{cap}$ of bounded cost from $O_2$.
 As $O_2$ satisfies the lower bound,  we can assume wlog that if $i$ is opened in $O_2$ then it serves all of its clients if $n_i \le \B$ (before taking more clients from outside) and it serves at least $\B$ of its clients before sending out its clients to other (small) facilities otherwise. 
Also, if two big facilities are opened in $O_2$, one does not serve the clients of the other. Let $\rho^2(j_i, i')$ denote the number of clients co-located at $i$ and assigned to $i'$ in $O_2$ and $\rho^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $S_{cap}$.
 \begin{figure}[t]
    \centering
    \includegraphics[width=10cm]{ O2_Scap_assignments.jpg}
    \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ and $i'$ are closed in $O_2$. $\rho^2(j_{i_1}, t_1) = 2,~\rho^2(j_{i_1}, t_2) = 1,~\rho^2(j_{i_1}, t_3) = 1,~ \rho^2(j_{i_1}, t_4) = 0$ and $\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 1,~\rho^2(j_{i_2}, t_3) = 1,~ \rho^2(j_{i_2}, t_4) = 0$.  } %The middle figure shows how the assignments look like after splitting the big facilities. $\rho^2(j_{i_1}, i') = 2(/1/1)$ for $i'$ = top three facilities $t_1(/t_2/t_3)$ $\rho^2(j_{i_2}, i') = 1(/1/1) $ for the bottom three facilities $t_2(/t_3/t_4)$. Note that $t_1$ }
    \label{Mapping}
\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{ O2_Scap_assignments_2.jpg}
   \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ is open in $O_2$.   $\rho^c(j_{t_1}, i_2) = \rho^2(j_{i}, t_1) = 1, \rho^c(j_{t_2}, i_2) = \rho^2(j_{i}, t_2) = 2$,
  % $\rho^2(j_{i_1}, t_1) = 1,~\rho^2(j_{i_1}, t_2) = 1$ and %$\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 2$. 
   $i_2$ is open in $S_{cap}$. $t_1$ and $t_2$ must be small.}
    \label{O2_SCap2}
\end{figure}
    \begin{enumerate}
        \item   if $i$ is closed in $O_2$ then open $i$ if $i$ is small
        and open $(i_1 \& i_2)$ if it is big.
        
        Assignments are defined as follows (see Fig.~\ref{Mapping}):
        \begin{enumerate}
        
        \item If $i$ is small: Let $i$ serve its own demand. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. Note that the same cannot be done when $i'$ is big as there is no demand at $i'_1$ and $i'_2$. Thus,  $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $ i' \ne i$ and $\rho^c(j_i, i) = d_i$. Also, $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). 
        Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = \B = u_i$. 
      
       % \item If $i$ is small: Let $i$ serve its own demand, \textcolor{blue}{i.e., $\rho^c(j_i, i) = d_i$}. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. \textcolor{blue}{Note that $i'$ must be small in this case. But y not big?????? I think it can be big as well, the only thing that will differ is $\rho^c(j_{i'}, i) = 0$ if $i'$ is big.} Thus, $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $i' \ne i$. Also, $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = \B = u_i$. \textcolor{blue}{Thus capacities are respected.}
        
       \item If $i$ is big: assign $\rho^2(j_{i_1}, i')$ (/$\rho^2(j_{i_2}, i')$) demand of $i'$ to $i_1$(/$i_2$) in our solution for small $i' \ne i$. Thus,
        $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_1) = \sum_{small~i' \ne i} \rho^2(j_{i_1}, i') \le \B = u_{i_1}$. Also,
         $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_2) \\ = \sum_{small~i' \ne i} \rho^2(j_{i_2}, i') \le n_i - \B = u_{i_2}$.
       %The second equality holds in each case as $i$ is closed in $O_2$.
        %\textcolor{green}{.....Is this the reason? Sapna...Pls see..}
        % Since there are no demands at $i_1$ and $i_2$, the capacities are respected.
     
       \end{enumerate}
     
     \item If $i$ is opened in $O_2$ and is big, open the free facility $i_2$ (see Fig.~\ref{O2_SCap2}): assign $\rho^2(j_{i}, i')$  demand of $i'$ to $i_2$ in our solution for small $i' \ne i$. Thus,
     %Thus,
      %  $\sigma^c(j_{i'}, i_2) = %\sigma^1(j_{i_2}, i'), i \ne i'$  
        $\sum_{i' \ne i}\rho^c(j_{i'}, i_2) = \sum_{i' \ne i} \rho^2(j_{i}, i') \le n_i - \B$ (the inequality holds by assumption on $O_2$) $= u_{i_2}$.
       % Thus the capacities are respected as there are no demands at $i_2$.
    \end{enumerate}
    
    Thus capacities are respected in each of the above cases. Next, we show that all the demands are satisfied. If a facility is opened in $S_{cap}$, it satisfies its own demand. 
Let $i$ be closed in $S_{cap}$. If $i$ is big ,we need not worry as $i_1$ and $i_2$ have no demand. So, let $i$ is small. Then, it must be opened in $O_2$. Then, 
$\sum_{i' \ne i}\rho^c(j_{i}, i') = $
$\sum_{small ~i' \ne i,  }\rho^c(j_{i}, i') + \sum_{i'_1: i' ~is ~big}\rho^c(j_{i}, i'_1) + 
\sum_{i'_2: i' ~is ~big}\rho^c(j_{i}, i'_2)= $
$\sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i'_1 : i' ~is ~big} \rho^2(j_{i'_1}, i)  + \\ \sum_{i'_2 : i' ~is ~big}\rho^2(j_{i'_2}, i)= \sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i' ~is ~big} \rho^2(j_{i'}, i) = \sum_{i' \ne i}\rho^2(j_{i'}, i)$
$\ge \B - n_i$  (since $O_2$ is a feasible solution of $I_2$) $= d_i$. 



Next, we bound the cost of the solution. The connection cost is at most that of $O_2$. %same as 
%\textcolor{green}{ or at most? we didn't bring back if anything went from i to i' in O2 where i' is big.}
%Next, we consider the facility opening costs. 
For facility costs, consider a facility $i$ that is opened in our solution and closed in $O_2$. Such a facility must have paid a cost of at least $n_i l(i)$ to get its clients served by other (opened) facilities in $O_2$. The facility cost paid by our solution is $ \delta min\{n_i, \B\} l(i) \le \delta n_i l(i)$. If $i$ is opened in $O_2$, then it must be serving at least $\B$ clients and hence paying a cost of at least $\B l(i)$ in $O_2$. In this case also, the facility cost paid by our solution is $ \delta min\{n_i, \B\} l(i) \le \delta \B l(i)$.  Summing over all $i$'s, we get %\textcolor{blue}{$FCost_{I_{cap}}(S_{cap}) \leq 2 \delta Cost_{I_2}(O_2)$, where $FCost_{\cdot}(\cdot)$ is the facility opening cost of a solution to $I_{cap}$ instance.} 
that the facility cost is bounded by $2 \delta Cost_{I_2}(O_2)$ and the total cost is bounded by $(1 + 2 \delta) Cost_{I_2}(O_2)$. Factor $2$ comes because we may have counted an edge $(i, i')$ twice, once as a client when $i$ was closed and once as a facility when $i'$ was opened in $O_2$.  
\end{proof}


% ****I am here - NG***** 

\section{Approximate Solution $AS_1$ to $I_1$ from approximate solution $AS_{cap}$ to  $I_{cap}$} \label{bi-criteria}

In this section,  we obtain
 a solution $AS_1$ to $I_1$ that violates the upper bounds by a factor of $(\beta + 1)$ without violating the lower bounds. This is the second major contribution of our work. We first obtain a ($5+\epsilon$)-approximate solution $AS_{cap}$ to $I_{cap}$ using approximation algorithm of Bansal \etal~\cite{Bansal}.  $AS_{cap}$ is then used to construct $AS_1$. Wlog assume that if a facility $i$ is opened in $AS_{cap}$ then it serves all its demand. (This is always feasible as $d_i \le u_i$.)  If this is not true, we can modify $AS_{cap}$  and obtain another solution, that satisfies the condition, of cost no more than that of $AS_{cap}$.
 $AS_1$ is obtained from $AS_{cap}$ by first defining the assignment of the clients and then opening the facilities that get at least $\B$ clients. Let $\rhobar^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $AS_{cap}$ and $\rhobar^1(j_i, i')$ denotes the number of clients co-located at $i$ and assigned to $i'$ in $AS_1$. 
%\textcolor{red}{ Initially each facility is assigned the clients co-located with it.}
Clients are assigned in three steps. In the first step, assign the clients co-located at a facility to itself. 
For small $i'$, additionally, we do the following  (type - $1$) re-assignments (see Fig. \ref{type1}): $(i)$ For small $i \ne i'$, assign $\rhobar^c(j_{i'}, i)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for small $i$. $(ii)$ For big $i$, assign $\rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ for big $i$. 
Claim~\ref{claim1} shows that these assignments are feasible and the capacities are violated only upto the extent to which they were violated by the tri-criteria solution $S^t$. 
\begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{ Type_1_Assignments.jpg}
    \caption{($a$) $\B =5$, $t_1, t_2, t_3$ have demands $1$, $2$ and $1$ unit each respectively. In solution $AS_{cap}$, $1$ unit of demand of $t_1$ and $2$ units of demand of $t_2$ are assigned to $t_3$. (b) Solution $S_1$: initially, $n_i$ clients are initially assigned to facility $i$. (c) Type $1$ reassignments: $1$ and $2$ clients of $t_3$ reassigned to $t_1$ and $t_2$ respectively. After this reassignment, $t_3$ has only $1$ client.}
    \label{type1}
\end{figure}

\begin{claim}
\label{claim1}
    $(i)$ $\sum_{i' \ne i} \rhobar^1(j_i, i') \le n_i$, $\forall$ $i \in \bar \facilityset^t$.
    $(ii)$ $\sum_{i} \rhobar^1(j_i, i') \le max\{\B, n_{i'}\} \le \beta \capacityU$, %\textcolor{magenta}{for $\beta \ge 1$, }  
    $\forall$ $i' \in \bar \facilityset^t$.
 \end{claim}

\begin{proof}

    $(i)$ Since $\rhobar^c(j_{i}, i) = d_i$ therefore $\sum_{i' \ne i} \rhobar^1(j_i, i') = \sum_{i' \ne i} \rhobar^c(j_{i'}, i) \le u_i - d_i \le n_i$ in all the cases. $(ii)$ $\rhobar^1(j_{i'}, i') = n_{i'}$. For $ i \ne i'$, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$. Thus, $\sum_{i} \rhobar^1(j_i, i') = n_{i'} + \sum_{i \ne i'} \rhobar^c(j_{i'}, i) \le n_{i'} + d_{i'} \le max\{\B, n_{i'}\} \le \beta \capacityU$.
\end{proof}

Note that $AS_1$ so obtained may  still not satisfy the lower bound requirement. In fact, although each facility was assigned $n_i \ge \alpha \B$  clients initially, they may be serving less clients now after type $1$ re-assignments. For example, in Fig. \ref{type1}, $t_3$ had $4$ clients initially which was reduced to $1$ after type $1$ reassignments. Let $P \subseteq  \facilityset^t$ be the set of facilities each of which is serving at least $\B$ clients after type-$1$ reassignments, and  $\bar P =  \facilityset^t \setminus P$ be the set of remaining facilities. 
 %That is, $ P= \{ i' \in \facilityset^t: \sum_{i}\rhobar^1(j_{i}, i') \ge \B$\}.
 We open all the facilities in $P$ and let them serve the clients assigned to them after type $1$ reassignments.
 
 \begin{observation}
    If a  small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge \B$. Similarly for a big facility $i'$, if $i'_1$ was closed in $AS_{cap}$ then $i'$ is in $P$.
     %\item If a small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge \B$.
    
     
    % \item If $i'$ is big then $\rhobar^1(j_{i'}, i') = n_{i'}  \ge \B$
 \end{observation}
 
 
 Thus, a small facility is in $\bar P$ only if it was open in $AS_{cap}$ and a big facility $i$ is in $\bar P$ only if $i_1$ was open in $AS_{cap}$. 
 %Also note that although each facility in $\bar P$ served at least $\alpha \B \ge \B/2$ clients in the tri-criteria solution $S^t$, they may be serving less clients now after step $1$ of assignment. \textcolor{red}{See Figure \ref{type1} for an example}.
 We now group these facilities so that each group serves at least $\B$ clients and open one facility in each group that serves all the clients in the group. For this we construct what we call as {\em facility trees}. We construct a graph $G$ with nodes corresponding to the facilities in $P \cup \bar P$. For $i \in \bar P$, let $\eta(i)$ be the nearest other facility to $i$ in $\facilityset^t$. Then, $G$ consists of edges $(i, \eta(i))$ with edge costs $ \dist{i}{\eta(i)}$. Each component of $G$ is a tree except possibly a double-edge cycle at the root. In this case, we say that we have a root, called {\em root-pair} $\rootpair$ consisting of a pair of facilities $i_{r_1}$and $ i_{r_2}$. Also, a facility $i$ from $P$, if present, must be at the root of a tree. Clearly edge costs are non-increasing as we go up the tree. 

Now we are ready to define our second type of re-assignments.
Let $x$ be a node in a tree $\mathcal T$. Let $children(x)$ denote the set of children of $x$ in $\mathcal T$. 
%if $x$ is not a root-pair. 
If $x$ is a root-pair $\rootpair$, then $children(x) = children(r_1) \cup children(r_2)$. %denote the union of children of $r_1$ and $r_2$ in $\mathcal T$.
Process the tree bottom-up (level by level) where processing of a node $x$ is explained in  Algorithm $1$, %\textcolor{olive}{(Resolve reference - SAPNA)} 
see Fig: (\ref{Process-X}). 
 While processing a node $x$, we first open (in lines $2-6$) and remove all its children with at least $\B$ clients; remaining children of $x$ are arranged and considered (left to right) in non-increasing order of distance from $x$.
%till we reach the root node, which could be either a single facility in $P$ or a root-pair. 
 For any child $y \in children(x)$, let $right-sibling(y)$ denote the adjacent right sibling of $y$ in the arrangement; thus, $right-sibling(y_i) = y_{i+1}$.



%\input{Gen-Algo.tex}
%\newpage 
\newpage

\input{Gen-AlgoSG.tex}
%\newpage
  \begin{figure}[t]
    \centering
    \includegraphics[width=12cm]{ ProcessX.jpg}
     \caption{   Let $\B=5$, numbers inside a node represents the number of clients at the node. A dashed arrow from a node $u$ to node $v$ represents the movement of clients from $u$ to $v$; (A): A node $x$ along with its children in decreasing order of their distances from $x$; (B): In steps $1$ to $7$, we open child $b$ and delete the edge $(b, x)$; (C): In steps $18 -20$, clients from $a$ are assigned to $c$ accumulating a total of $7$ clients at $c$. In the next iteration of the 'for' loop, in lines $14-16$, $c$ gets opened and the edge ($c, x$) is deleted; (D): In the next iteration, clients of $d$ are assigned to $e$; (E(i)): $t=1$.  In the next iteration, clients of $e$ are assigned to $x$ in lines $27 - 28$; (E(ii)): $t=3$. $e$ gets opened in lines $23 - 25$;} 
    \label{Process-X}
\end{figure}

There are two possibilities at the root: either we have a facility $i$ from $P$ or we have a root-pair $\rootpair$.
In the first case, we are done as $i$ is already open and has at least $\B$ clients. See Fig: (\ref{tree12}) and (\ref{tree2}). To handle the second case, we need to do a little more work. So, we define our assignments of third type as follows: 
($i$) If the total number of clients collected at  the root-pair node 
%$i_c, i_{r_1}$ and $i_{r_2}$ 
is at least $\B$ and at most $2\B$ then open any one of the two facilities in the root-pair and assign all the clients to it.\footnote{ we can open the facility with more number of clients and save $2$(to be seen again) factor in the connection cost.} See Fig: (\ref{tree3}-(A)).
($ii$) If the total number of clients collected at  the root-pair node is more than $2\B$  then open both the facilities at the root node and distribute the clients  so that each one of them gets at least $\B$ clients. See Fig: (\ref{tree3}-(B)).
($iii$) If the total number of clients collected at  the root-pair node  is less than $\B$, then let $i$ be the node in $P$ nearest to the root-pair i.e. $i =  argmin_{i' \in P} \min \{ \dist{i'}{r_1}, \dist{i'}{r_2}\}$, then $i$ is already open and has at least $\B$ clients. Send the clients collected at the root-pair to $i$. See Fig: (\ref{tree4}).


\begin{figure}[t]
	\begin{tabular}{ccc}
		\includegraphics[width=9cm,scale=0.8]{ Tree1.0.jpg}
		& 
		\includegraphics[width=4cm,scale=0.8]{ Tree1.1.jpg}
		\\
		%\textbf{(a)}& \ \ \textbf{(b)}& \ \ \textbf{(c)}
	\end{tabular}
	\caption{$\B=12$. (A) A tree $\mathcal{T}$;  Numbers inside each node represents the number of clients at those nodes.
	%At any fixed level, nodes are processed in left to right order. 
	The tree does not change after the calls: Process($f$), Process($g$), Process($h$), Process($i$), Process($j$) and Process($k$). In each case, it returns at line no. $9$;  (B) Tree after Process($a$), Process($b$), Process($c$), Process($d$) and Process($e$); (C) Tree after line $22$ of Process($x$).
	%when $t \leq 3$ 
	}
	
	\label{tree12}
\end{figure}


% \begin{figure}[t]
%    \centering
%    \includegraphics[width=7cm]{ Tree1.jpg}
%    \caption{(A) A tree $\mathcal{T}$; $\B=12$; Numbers inside each node represents the number of clients at those nodes. (B) Algorithm Process() called in the following order: Process($a$) - $3$ and $6$ clients from node $g$ and $h$ respectively, get assigned to node $f$, making its count to $12$; Process($b$); Process($c$) - $9$ clients from $i$ are assigned to node $c$; Process($d$); Process($e$) - $3$ and $1$ clients from node $j$ and $k$ respectively, get assigned to it. Eventually, node $f$ and $c$ are opened; }
%    \label{tree1}
%\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=4cm]{ Tree2.jpg}
    \caption{ $\B=12,~t=1$. Before Process($x$): $n_x = 13$. Tree after Process($x$) when root node $x \in P$.  }
    \label{tree2}
\end{figure}


 \begin{figure}[t]
    \centering
    \includegraphics[width=10cm]{ Tree3.jpg}
    \caption{    $\B=12$, $x = <i_{r_1}, i_{r_2}>$ is a root-pair node with $n_{i_{r_1}} = 8,~n_{i_{r_2}} = 6$. (A) $t =1$. Before Process($x$): $\B \le n_{i_{r_1}} + n_{i_{r_2}} + 9 \le 2\B$. Tree after Process($x$): any one of $i_{r_1}$ and $i_{r_2}$, say $i_{r_1}$, is opened and all the clients are assigned to it; (B)$t =3$. Before Process($x$): $2\B \le n_{i_{r_1}} + n_{i_{r_2}} + 11 \le 3\B$. Tree after Process($x$): $i_{r_1}$ and $i_{r_2}$ are both opened and clients are distributed among them.}
    
    \label{tree3}
\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=5cm]{ Tree4.jpg}
    \caption{$\B=12, t =1$. $x = <i_{r_1}, i_{r_2}>$ is a root-pair node with $ n_{i_{r_1}} + n_{i_{r_2}} + 9 < \B$. Tree after Process($x$).}
    
    \label{tree4}
\end{figure}


 
Clearly the opened facilities satisfy the lower bounds. Next, we bound the violation in the upper bound.
  
\begin{lemma}
%Let $ i_c$ be the rightmost child, if any,  of the root (/root-pair) $r$ of a tree after line $11$ when Process($r$) is invoked. Let $i$ be the parent of $ i_c$ ($i$ is either $r$ and is in $P$ or it is one of ${r_1}$ and ${r_2}$ in case $r =\rootpair$ is a root-pair). The number of clients collected in the second type of re-assignments, at any node $x$ in the tree rooted at $i_c$ is at most $2\B$.

The number of clients collected in the second type of re-assignments, at any non-root node $x$ is at most $2\B$.
 \end{lemma}
 
 \begin{proof} 
 Note that a node $x$ receives clients either from one of its children (at line $27$) when Process($x$) is invoked  or from one of its siblings (at line $18$) when Process($\eta(x)$) is invoked. In either case, it has $< \B$ clients of its own and it receives $<\B$ clients from its child/sibling.  Hence, the claim follows.
 \end{proof}
  
  If the number of clients collected at $i_c$ is $\ge \B$, it is opened (at line $24$) and removed from further processing when Process($\eta(i_c)$) is invoked. 
  %So, let the number of clients collected at $i_c$ is $< \B$.
 Let $\pi_i$ be the number of clients assigned to the facility $i$ after first type of re-assignments. Then as shown earlier, $\pi_i \le \beta \capacityU$.  %Let $i$ be the parent of $ i_c$. In second and third types of assignments,  we never collect  more than $2\B$ clients at any node till we reach $i_c$.
 %Now we have the following scenarios: Suppose $ i_c$ has less than $\B$ clients,
 We have the following cases: ($i$) the root node $i$ is in $P$ and it gets additional  $< \B$ clients from $i_c$ making a total of at most $\pi_i + \B \le \beta \capacityU + \B \le (\beta + 1) \capacityU$ clients at $i$.
 ($ii$) the total number of clients collected at  the root-pair node 
%$i_c, i_{r_1}$ and $i_{r_2}$ 
is at least $\B$ and at most $2\B $.
 %($ii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at $i_c, i_{r_1}$ and $i_{r_2}$ is at least $\B$ and at most $2\B$. Thus, 
 The number of clients the opened facility gets is at most $2\B \le 2\capacityU \le (\beta + 1) \capacityU$.
 ($iii$)  the total number of clients collected at the root-pair node  is more than $2\B$.  Note that the total number of clients collected at these facilities is at most $3\B$ and hence 
 ensuring that each of them gets at least $\B$ clients also ensures that none of them gets more than $2\B$ clients. Hence none of them gets more than $2\capacityU \le (\beta + 1) \capacityU$ clients.
 %it is possible to distribute them to the two opened facilities so that each of them gets at most $2\B \le 2\capacityU$ clients.
 ($iv$) the total number of clients collected at the root-pair node is less than $\B$. 
 %Number of clients at $i_c$ and the root pair and, their nearest facility in $P$ are at most $\B$ and $\beta \capacityU$ respectively. 
 Thus, the number of clients the opened facility in $P$ gets is at most $\beta \capacityU + \B \le (\beta + 1) \capacityU$. 
 %The case when $i_c$ has at least $\B$ clients leads to the third scenario above and hence handled.
 
 
 We next bound the connection cost.  
 %For any node $y$ in a tree, let \textcolor{blue}{$right-sibling(y)$} denote the \textcolor{blue}{right sibling} of $y$ in step~\ref{} of the algorithm. Thus, \textcolor{blue}{$left-sibling(y_i) = y_{i+1}$}.
 We will need the following lemma to bound the connection cost.

 
 
\begin{lemma}
 For a node $y$ in a tree,
  $\dist{y}{right-sibling(y)} \le 3 \dist{y}{\eta(y)} = 3l(y)$. %.....This equality is correct, right? we have been assuming this....$P \cup \bar P = F^t$, right?
 \end{lemma}
 \begin{proof}
 If $\eta(\cone) = \eta(right-sibling(\cone))$  (i.e. $\cone$ and $right-sibling(\cone)$ are children of the same node), then it is easy to see that $\dist{\cone}{right-sibling(\cone)} \leq 2 \dist{\cone}{\eta(\cone)}$. Otherwise (which can be the case when root is a root-pair, see Figure~(\ref{3factorBound})), $\dist{\cone}{right-sibling(\cone)} \leq \dist{\cone}{\eta(\cone)} + \dist{\eta(\cone)}{\eta(right-sibling(\cone))} + \dist{\eta(right-sibling(\cone))}{right-sibling(\cone)} \le 3 \dist{\cone}{\eta(\cone)}$.
 \end{proof}
 
  \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{ 3factorBound.jpg}
    \caption{$\dist{\cone}{right-sibling(\cone)}  \le 3 \dist{\cone}{\eta(\cone)}$}
    \label{3factorBound}
\end{figure}

 
 
 The cost of first type of re-assignments is at most the connection cost of $AS_{cap}$.
% \textcolor{red}{(or at most?Sapna/rajni) }
 To bound the connection cost of second type, observe that we never send more than $\B$ clients on any edge. 
 %In the second type of assignment, 
 Thus, a facility $i$ that sends its (at most $\B$ clients) to its parent or to its right sibling incurs a cost of at most $3\B l(i)$. Since the facility $i$ was opened in $AS_{cap}$, it pays facility opening cost of $\delta l(i) min \{n_i, \B\} \ge \delta l(i) \alpha \B$ in $AS_{cap}$. Summing over all $i \in \bar P$ for the second type of re-assignments, we see that the total connection cost in these re-assignments is bounded by  $3 FCost_{I_{cap}}(AS_{cap})/\alpha \delta$ 
% \textcolor{olive}{D: $\sum_{i \in \bar P} \B l(i) \leq 6FCost_{I_{cap}}(AS_{cap})/\alpha \delta$  where factor 6 comes because sending clients to the left sibling incurs a cost of twice the cost to the node's parent and}
 where $FCost_{I_{cap}}(.)$ is the facility opening cost of a solution to the $I_{cap}$ instance.


 For the third type of re-assignments, we bound the cost as follows:
 %we bound the cost in two parts: ($a$) cost of sending ($< \B$) clients of $i_c$ to it's parent ($b$) Cost of sending ($< \B$) clients collected at the root pair $<i_{r_1}, i_{r_2}>$ to it's nearest facility in $P$. Cost of the first part is bounded by $\B l(i_c)$. 
 the cost of sending ($< \B$) clients by a facility $i$ in the root pair $\rootpair$ to the facility in $P$, nearest to the root-pair, is not bounded by $\B l(i)$ (where $l(i) = l(i_{r_1}) = l(i_{r_2})$). 
% we bound the cost as follows: 
 Note that the total number of clients, initially at $i_{r_1}$ and $i_{r_2}$ was $\ge 2 \alpha \B$. However, during re-assignments of type $1$, some of them got reassigned to other facilities. Note that these (other) facilities must have been closed in $AS_{cap}$ and hence do not belong to $\bar P$. Hence, each of these reassignments correspond to an assignment in $AS_{cap}$ whose cost was at least $l(i)$ and a total of at least $(2\alpha  - 1)\B l(i)$. Hence the cost of type $3$ re-assignments is bounded by $3 CCost_{I_{cap}}(AS_{cap})/ (2\alpha  - 1)$ where $CCost_{I_{cap}}(.)$ is the connection cost of a solution to the $I_{cap}$ instance. Hence, the total cost of solution $AS_1$  is $max\{1+\frac{3}{(2\alpha-1)},\frac{3}{\alpha\delta}\}Cost_{I_{cap}}(AS_{cap}) = max\{\frac{2(\alpha+1)}{(2\alpha-1)},\frac{3}{\alpha\delta}\} Cost_{I_{cap}}(AS_{cap}) = \frac{2(\alpha+1)}{(2\alpha-1)} Cost_{I_{cap}}(AS_{cap}) $ for $\delta= \frac{3(2\alpha-1)}{2\alpha(\alpha+1)} $.
 
 
Thus, the total cost of the solution is,\\ $ Cost_I(S) \le  Cost_I(S^t) + Cost_{I_1}(AS_1)$\\
   $\leq O(1) Cost_I(O) + \frac{2(\alpha+1)}{(2\alpha-1)} Cost_{I_{cap}}(AS_{cap}) $\\
    $\leq O(1) Cost_I(O) +  \frac{2(\alpha+1)(5+\epsilon)}{(2\alpha-1)} Cost_{I_{cap}}(O_{cap})$\\
   $\leq O(1) Cost_I(O) +  \frac{12(\alpha+1)}{(2\alpha-1)} Cost_{I_{cap}}(O_{cap})$\\
   $ \leq O(1) Cost_I(O) + \frac{12(\alpha+1)(1 + 2\delta)}{(2\alpha-1)}  Cost_{I_2}(O_2) $\\
   $\leq O(1) Cost_I(O) + \frac{12(\alpha^2 + 7 \alpha -3)}{\alpha (2\alpha-1)}  Cost_{I_2}(O_2)$\\
   $= O(1) Cost_I(O) +  \frac{24(\alpha^2 + 7 \alpha -3)}{\alpha (2\alpha-1)}  Cost_{I_1}(O_1)$\\
    $= O(1) Cost_I(O) +  \frac{24(\alpha^2 + 7 \alpha -3)}{\alpha (2\alpha-1)} (Cost_I(S^t) + Cost_I(O))$\\
   $= O(1) Cost_I(O) +  \frac{24(\alpha^2 + 7 \alpha -3)}{\alpha (2\alpha-1)} (O(1) Cost_I(O))$\\
   %$= O(1) Cost_I(O) +  \frac{432(\alpha^2 + 7 \alpha -3)}{\alpha (2\alpha-1)} Cost_I(O)$\\
   $=O(1) Cost_I(O)$
   
 %  \textcolor{magenta}{Thus, the total cost of the solution is,\\ $ Cost_I(S) \le  Cost_I(S^t) + Cost_{I_1}(AS_1)$\\
  % $\leq (2\ell^2 + 3\ell+2) Cost_I(O) + \frac{2(\alpha+1)}{(2\alpha-1)} Cost_{I_{cap}}(AS_{cap}) $\\
  % $= (2\ell^2 + 3\ell+2) Cost_I(O) + \frac{2(2\ell-1)}{(\ell -2)} Cost_{I_{cap}}(AS_{cap})$\\
   %$\leq (2\ell^2 + 3\ell+2) Cost_I(O) + \frac{2(2\ell-1) (5+\epsilon)}{(\ell-2)} Cost_{I_{cap}}(O_{cap})$\\
   %$ \leq (2\ell^2 + 3\ell+2) Cost_I(O) + \frac{2(2\ell-1) (5+\epsilon)  (1 + 2\delta) }{(\ell-2)}  Cost_{I_2}(O_2) $\\
   %$\leq (2\ell^2 + 3\ell+2) Cost_I(O) + \frac{4(2\ell-1) (5+\epsilon) (1 + 2\delta) }{(\ell-2)} Cost_{I_1}(O_1)$\\
   %$= (2\ell^2 + 3\ell+2) Cost_I(O) +  \frac{4(5\ell^2 - 9 \ell + 1) (5+\epsilon) }{(\ell-1)(\ell-2)} Cost_{I_1}(O_1)$\\
    %$= (2\ell^2 + 3\ell+2) Cost_I(O) +  \frac{4(5\ell^2 - 9 \ell + 1) (5+\epsilon) }{(\ell-1)(\ell-2)} (Cost_I(S^t) + Cost_I(O))$\\
   %$= (2\ell^2 + 3\ell+2) Cost_I(O) +   \frac{4(5\ell^2 - 9 \ell + 1) (5+\epsilon) }{(\ell-1)(\ell-2)} ((2\ell^2 + 3\ell+3) Cost_I(O))$\\
   %$=O(\ell^2) Cost_I(O)$}
  
  
 %\textcolor{magenta}{Choosing $\ell=O(1/\epsilon)$ and $\ell >2$, we get cost bound of $O(1/\epsilon^2)$.}
 
%\textcolor{violet}{ Hence the total cost of solution $AS_1$  is $6\alpha/(2\alpha-1) \textcolor{blue}{Cost_{I_{cap}}(AS_{cap})}$ for $\delta= (2\alpha-1)/6\alpha^2 $. \textcolor{blue}{Why 6 times???}...Only this is left from my side. }

==> NEW Journal version WADS 2021 (LBUBFL)/LBUFL.tex <==
\section{Instance $I_1$ and $I_2$}
\label{instI1}

In this section, we first transform instance $I$ to instance $I_1$ ($\facilityset,~\clientset,~f^1,~c,~\B,~\capacityU$) of LBUBFL by moving the clients to the facilities serving them in the tri-criteria solution $S^t$ and then transform $I_1$ to an instance $I_2$ of LBFL by removing the facilities not opened in $S^t$.
%Let $\facilityset^t$ be the set of facilities opened by $S^t$. 
Recall that for a client $j$,  $\sigma^t(j)$ is the facility  in $\facilityset^t$ serving $j$. For $i \in \facilityset^t$, let $n_i$ be the number of clients served by $i$ in $S^t$, i.e., $n_i = |(\sigma^t)^{-1}(i)|$ and for $i \notin \facilityset^t$, $n_i = 0$. Move these clients to $i$ (see Fig.~\ref{Mapping1}). Thus, there are $n_i$ clients co-located with $i$. In $I_1$, our facility set is $\facilityset$ and the clients are at their new locations. Facility opening costs in $I_1$ are modified as follows: $f^1_i = 0$ for $i \in \facilityset^t$ and $=f_i$ for $i \notin \facilityset^t$.  


\begin{lemma}
Cost of optimal solution of $I_1$ is bounded by $Cost_I(S^t) + Cost_I(O)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_1$ of $I_1$: open $i$ in $S_1$ iff it is opened in $O$. Assign $j$ to $i$ in $S_1$ iff it is assigned to $i$ in $O$. $S_1$ satisfies both the lower bound as well as the upper bound as $O$ does so. For a client $j$, let $\sigma^*(j)$ be the facility serving $j$ in $O$. Then, the cost $\dist{ \sigma^t(j)}{\sigma^*(j))}$ of serving $j$ from its new location, $\sigma^t(j)$ is bounded by $\dist{j}{\sigma^t(j)} +\dist{j}{\sigma^*(j)}$ (see Fig. \ref{lemma1}). Summing over all $j \in \clientset$ and adding the facility opening costs, we get the desired claim.

\begin{figure}[t]
    \centering
    \includegraphics[width=4cm]{Figures/lemma 1.jpg}
    \caption{$c( \sigma^t(j), \sigma^*(j)) \leq c(j, \sigma^t(j)) + c(j, \sigma^*(j))$ }
    \label{lemma1}
\end{figure}
\end{proof}

\begin{figure}[t]
    \centering
    \includegraphics[width=9cm]{Figures/Mapping_0.jpg}
    \caption{Transforming instance $I$ to $I_1$ and  $I_1$ to $I_2$. Solid squares represent clients and circles represent facilities. Clients are moved to the facilities serving them in $S^t$ while transforming $I$ to $I_1$. Facilities not opened in $S^t$ are dropped while going from $I_1$ to $I_2$.}
    \label{Mapping1}
\end{figure} 

%section{Instance $I_2$} 
%\label{instI2}
    
   Next, we define an instance ~$I_2(\facilityset^t,~\clientset,~f^2,~c,~\B)$ of LBFL from $I_1$ by removing the facilities not in $\facilityset^t$ and ignoring the upper bounds. Instance $I_2$ is same as $I_1$ without the upper bounds, except that the facility set is $\facilityset^t$ now. Thus, $f^2_i = 0~\forall~i \in \facilityset^t$. % We will show that there exists a feasible solution $S_2$ of $I_2$ such that $Cost(S_2)$ is bounded by $2 Cost(O_1)$ where
  Let $O_1$ be an optimal solution of $I_1$. 
  For a client $j$, let $\sigma^1(j)$ be the facility serving $j$ in $O_1$.
 
 
 

\begin{lemma}
Cost of optimal solution of $I_2$ is bounded by $ 2Cost_{I_1}(O_1)$.
\end{lemma}
\begin{proof}
We construct a feasible solution $S_2$ to $I_2$: for $i \in \facilityset^t$, open $i$ in $S_2$ if it is opened in $O_1$ and assign a client $j$ to it if it is assigned to $i$ in $O_1$. For a facility $i \notin \facilityset^t$, %the clients assigned to it need to be assigned to some other facility in $\facilityset^t$. Thus, for such $i$'s,
open its nearest facility $i'$ \textcolor{olive}{(if not already opened)} in $\facilityset^t$. Assign $j$ to $i'$ in $S_2$ if it is assigned to $i$ in $O_1$. $S_2$ satisfies the lower bound  as $O_1$ does so. Note that it need not satisfy the upper bounds. This is the reason we dropped upper bounds in $I_2$. The cost $c( \sigma^t(j), i')$
%$c( \sigma^t(j), \sigma^*(j))$ 
of serving $j$ from its new location is bounded by $c(\sigma^t(j), \sigma^1(j)) + c( \sigma^1(j), i') \le 2 c(\sigma^t(j), \sigma^1(j))$ (since $i'$ is closest in $\facilityset^t$ to $i =  \sigma^1(j)$). Summing over all $j \in \clientset$ we get the desired claim.
%$c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(i, \sigma^1(j)) \le c(j, \sigma^t(j)) + c(j, \sigma^1(j)) + c(\sigma^t(j), \sigma^1(j))$ (since $i$ is closest in $\facilityset^t$, to $i' = \sigma^1(j)$) $\le 2(c(j, \sigma^t(j)) + c(j, \sigma^1(j)))$ (See Figure 1). Summing over all $j$'s, the claim follows.
%Same as Zoya etal
\end{proof}

%\textcolor{blue}{can be deleted now...I have added a line in the proof itself....Note that, while defining the instance $I_2$, we ignored the upper bounds on facilities because a facility $i' \in \facilityset^t$ might be nearest to many other facilities $\notin \facilityset^t$ thereby serving clients of all of them and hence violating upper bound.}


\section{Instance $I_{cap}$ of Capacitated Facility Location Problem}
\label{instIcap}

 
 In this section, we create an  instance $I_{cap}$ of capacitated facility location problem from $I_2$. 
 The main idea is to create  a demand of $\B - n_i$ units at locations where the number of clients served by the facility is less than $\B$ and a supply of $n_i - \B$ units at locations with surplus clients. For each facility $i \in \facilityset^t$, let $l(i)$ be the distance of $i$ from a nearest facility  $i' \in \facilityset^t$, $i' \neq i$ and let $\delta$ be a constant to be chosen appropriately. A facility $i$ is called {\em small} if $0< n_i \leq \B$ and  {\em big} otherwise. A big facility $i$ is split into two co-located facilities $i_1$ and $i_2$.
  We also split the set of clients at $i$ into two sets:  arbitrarily, $\B$ of these clients are placed at $i_1$ and the remaining $n_i - \B$ clients at $i_2$ (see Fig.~\ref{Mapping2}). 
   Instance $I_{cap}$ is then defined as follows:
A {\em small} facility $i$ needs additional $\B - n_{i}$ clients to satisfy its lower bound; hence a demand of $\B - n_{i}$ is created at $i$ in the $I_{cap}$ instance. A facility with capacity $\B$ and facility opening cost $\delta n_{i} l(i)$ is also created at $i$. 
For a {\em big} facility $i$, correspondingly two co-located facilities $i_1$ and $i_2$ are created with capacities $\B$ and $n_i - \B$ respectively. The facility opening cost of $i_1$ is $\delta \B l(i)$ whereas $i_2$ is free. Intuitively, since the lower bound of a big facility is satisfied, it has some extra ($n_i - \B$) clients , which can be used to satisfy the demand of clients in $I_{cap}$ for free. 
 %Thus, we define capacity of $i_1$ and $i_2$ to be $\B$ and $n_i - \B$ respectively. 
 The second type of big facilities are called {\em free}. 
 %The facility costs, capacities and demands are as shown in
 We use $i$ to refer to both the client (with demand) as well as the facility located at $i$. Let $\bar \facilityset^t$ be the set of facilities so obtained. The set of clients and the set of facilities are both $\bar \facilityset^t$. Table~\ref{tab:my_label} summarizes the instance. Also see Fig.~\ref{Mapping2}
 
 \begin{figure}
    \centering
    \includegraphics[width=8cm]{Figures/Mapping_1.jpg}
    \caption{Transforming instance $I_2$ to $I_{cap}$: $\B = 4$,
    %Solid squares represent clients and circles represent facilities. 
    $i'$ is small, $i$ is big.
    $i$ is split into $i_1$ and $i_2$ while transforming $I_2$ to $I_{cap}$, $i_2$ is free. Demand at the small facility $i'$ is $\B - n_{i'} = 1$ and at $i_1$, $i_2$, it is $0$. Capacities of $i'$ and $i_1$ are $\B = 4$ and it is $n_{i} - \B = 3$ of the free facility $i_2$.}
    \label{Mapping2}
\end{figure}
 
 \begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
       Type & $n_i$ & $u_i$ & $d_i$ & $f^t_i$ \\
        \hline
       {\em small} & $n_i \leq \B$ & $\B$ & $\B- n_i$& $\delta n_i l(i)$ \\
        \hline
       {\em big} & $n_i > \B$ & ($i_1$)$\B$ & $0$& $\delta \B l(i)$ \\
        & & ($i_2$) $n_i - \B$ & $0$& $0$ \\
       
        % &  &
          \hline 
       % $3$ & $0$ & $\B$ & $\B$& $\delta \B l(i)$ \\
        %\hline
    \end{tabular}
    \caption{Instance of $I_{cap}$: $d_i, u_i, f^t_i$ are demands, capacities and facility costs resp.}
    \label{tab:my_label}
\end{table}
 
 %Let $O_{cap}$ be an optimal solution to $I_{cap}$.
 
 %\textcolor{red}{define delta and l(i)}
 %The second type of big facilities are called {\em free}. %and the clients placed at them are also called {\em free}. 
 %Let $F_f$ denote the set of free facilities. 
 %and $Cf(i)$ denote the set of free clients at facility $i \in F_b$. i.e.$Cf(i)$ is the set of clients placed at $i_2 \in F_f$ (See Figure 2)....need to define $l(i)$.

 %In the next lemma, we show the existence of a feasible solution to $I_{cap}$ with cost no more than $(1+2\delta)Cost(O_2)$ where $O_2$ is an optimal solution of $I_2$. 




\begin{lemma}
%A feasible solution $S_{cap}$ for 
Let $O_2$ be an optimal solution of $I_2$. Then, cost of optimal solution to $I_{cap}$ is bounded by $(1+2\delta)Cost_{I_2}(O_2)$.
\end{lemma}

\begin{proof}
We will construct a feasible solution $S_{cap}$ to $I_{cap}$ of bounded cost from $O_2$.
 As $O_2$ satisfies the lower bound,  we can assume wlog that if $i$ is opened in $O_2$ then it serves all of its clients if $n_i \le \B$ (before taking more clients from outside) and it serves at least $\B$ of its clients before sending out its clients to other (small) facilities otherwise. 
Also, if two big facilities are opened in $O_2$, one does not serve the clients of the other. Let $\rho^2(j_i, i')$ denote the number of clients co-located at $i$ and assigned to $i'$ in $O_2$ and $\rho^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $S_{cap}$.
 \begin{figure}[t]
    \centering
    \includegraphics[width=10cm]{Figures/O2_Scap_assignments.jpg}
    \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ and $i'$ are closed in $O_2$. $\rho^2(j_{i_1}, t_1) = 2,~\rho^2(j_{i_1}, t_2) = 1,~\rho^2(j_{i_1}, t_3) = 1,~ \rho^2(j_{i_1}, t_4) = 0$ and $\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 1,~\rho^2(j_{i_2}, t_3) = 1,~ \rho^2(j_{i_2}, t_4) = 0$.  } %The middle figure shows how the assignments look like after splitting the big facilities. $\rho^2(j_{i_1}, i') = 2(/1/1)$ for $i'$ = top three facilities $t_1(/t_2/t_3)$ $\rho^2(j_{i_2}, i') = 1(/1/1) $ for the bottom three facilities $t_2(/t_3/t_4)$. Note that $t_1$ }
    \label{Mapping}
\end{figure}

 \begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{Figures/O2_Scap assignments (2.1).jpg}
   \caption{Feasible solution $S_{cap}$ to $I_{cap}$ from $O_2$: $i$ is open in $O_2$.   $\rho^c(j_{t_1}, i_2) = \rho^2(j_{i}, t_1) = 1, \rho^c(j_{t_2}, i_2) = \rho^2(j_{i}, t_2) = 2$,
  % $\rho^2(j_{i_1}, t_1) = 1,~\rho^2(j_{i_1}, t_2) = 1$ and %$\rho^2(j_{i_2}, t_1) = 0,~\rho^2(j_{i_2}, t_2) = 2$. 
   $i_2$ is open in $S_{cap}$. $t_1$ and $t_2$ must be small.}
    \label{O2_SCap2}
\end{figure}
    \begin{enumerate}
        \item   if $i$ is closed in $O_2$ then open $i$ if $i$ is small
        and open $(i_1 \& i_2)$ if it is big.
        
        Assignments are defined as follows (see Fig.~\ref{Mapping}):
        \begin{enumerate}
        
        \item If $i$ is small: Let $i$ serve its own demand. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. 
        \textcolor{green}{
        Note that the same cannot be done when $i'$ is big as there is no demand at $i'_1$ and $i'_2$. } Thus,  $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $ i' \ne i$ and $\rho^c(j_i, i) = d_i$. Also, $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). 
        Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = \B = u_i$. 
      
       % \item If $i$ is small: Let $i$ serve its own demand, \textcolor{blue}{i.e., $\rho^c(j_i, i) = d_i$}. In addition, assign $\rho^2(j_i, i')$ demand of $i'$ to $i$ in our solution for small $i' \ne i$. \textcolor{blue}{Note that $i'$ must be small in this case. But y not big?????? I think it can be big as well, the only thing that will differ is $\rho^c(j_{i'}, i) = 0$ if $i'$ is big.} Thus, $\rho^c(j_{i'}, i) = \rho^2(j_i, i')$, for small $i' \ne i$. Also, $\sum_{small~i' \ne i}\rho^c(j_{i'}, i) = \sum_{small~i' \ne i} \rho^2(j_i, i') \le n_i$.
        %(second equality holds as $i$ is closed in $O_1$). Hence, $\sum_{i'}\rho^c(j_{i'}, i) \le n_i + d_i = \B = u_i$. \textcolor{blue}{Thus capacities are respected.}
        
       \item If $i$ is big: assign $\rho^2(j_{i_1}, i')$ (/$\rho^2(j_{i_2}, i')$) demand of $i'$ to $i_1$(/$i_2$) in our solution for small $i' \ne i$. Thus,
        $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_1) = \sum_{small~i' \ne i} \rho^2(j_{i_1}, i') \le \B = u_{i_1}$. Also,
         $\sum_{small~i' \ne i}\rho^c(j_{i'}, i_2) \\ = \sum_{small~i' \ne i} \rho^2(j_{i_2}, i') \le n_i - \B = u_{i_2}$.
       %The second equality holds in each case as $i$ is closed in $O_2$.
        %\textcolor{green}{.....Is this the reason? Sapna...Pls see..}
        % Since there are no demands at $i_1$ and $i_2$, the capacities are respected.
     
       \end{enumerate}
     
     \item If $i$ is opened in $O_2$ and is big, open the free facility $i_2$ (see Fig.~\ref{O2_SCap2}): assign $\rho^2(j_{i}, i')$  demand of $i'$ to $i_2$ in our solution for small $i' \ne i$. Thus,
     %Thus,
      %  $\sigma^c(j_{i'}, i_2) = %\sigma^1(j_{i_2}, i'), i \ne i'$  
        $\sum_{i' \ne i}\rho^c(j_{i'}, i_2) = \sum_{i' \ne i} \rho^2(j_{i}, i') \le n_i - \B$ (the inequality holds by assumption on $O_2$) $= u_{i_2}$.
       % Thus the capacities are respected as there are no demands at $i_2$.
    \end{enumerate}
    
    Thus capacities are respected in each of the above cases. Next, we show that all the demands are satisfied. If a facility is opened in $S_{cap}$, it satisfies its own demand. 
Let $i$ be closed in $S_{cap}$. If $i$ is big ,we need not worry as $i_1$ and $i_2$ have no demand. So, let $i$ is small. Then, it must be opened in $O_2$. Then, 
$\sum_{i' \ne i}\rho^c(j_{i}, i') = $
$\sum_{small ~i' \ne i,  }\rho^c(j_{i}, i') + \sum_{i'_1: i' ~is ~big}\rho^c(j_{i}, i'_1) + 
\sum_{i'_2: i' ~is ~big}\rho^c(j_{i}, i'_2)= $
$\sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i'_1 : i' ~is ~big} \rho^2(j_{i'_1}, i)  + \\ \sum_{i'_2 : i' ~is ~big}\rho^2(j_{i'_2}, i)= \sum_{small ~i' \ne i,  }\rho^2(j_{i'}, i) + \sum_{i' ~is ~big} \rho^2(j_{i'}, i) = \sum_{i' \ne i}\rho^2(j_{i'}, i)$
$\ge \B - n_i$  (since $O_2$ is a feasible solution of $I_2$) $= d_i$. 



Next, we bound the cost of the solution. The connection cost is \textcolor{olive}{at most that of $O_2$. } %same as 
\textcolor{green}{ or at most? we didn't bring back if anything went from i to i' in O2 where i' is big.}
%Next, we consider the facility opening costs. 
For facility costs, consider a facility $i$ that is opened in our solution and closed in $O_2$. Such a facility must have paid a cost of at least $n_i l(i)$ to get its clients served by other (opened) facilities in $O_2$. The facility cost paid by our solution is $ \delta min\{n_i, \B\} l(i) \le \delta n_i l(i)$. If $i$ is opened in $O_2$, then it must be serving at least $\B$ clients and hence paying a cost of at least $\B l(i)$ in $O_2$. In this case also, the facility cost paid by our solution is $ \delta min\{n_i, \B\} l(i) \le \delta \B l(i)$.  Summing over all $i$'s, we get %\textcolor{blue}{$FCost_{I_{cap}}(S_{cap}) \leq 2 \delta Cost_{I_2}(O_2)$, where $FCost_{\cdot}(\cdot)$ is the facility opening cost of a solution to $I_{cap}$ instance.} 
that the facility cost is bounded by $2 \delta Cost_{I_2}(O_2)$ and the total cost is bounded by $(1 + 2 \delta) Cost_{I_2}(O_2)$. Factor $2$ comes because we may have counted an edge $(i, i')$ twice, once as a client when $i$ was closed and once as a facility when $i'$ was opened in $O_2$.  
\end{proof}


% ****I am here - NG***** 

\section{Bi-criteria Solution $S_1$ to $I_1$ from approximate solution $AS_{cap}$ to  $I_{cap}$} \label{bi-criteria}

In this section, we obtain a solution $S_1$ to $I_1$ that violates the capacities/upper bounds by a factor of $(\beta + 2)$ without violating the lower bound. We first obtain an approximate solution $AS_{cap}$ to $I_{cap}$ using any approximation algorithm \cite{Bansal}.  $AS_{cap}$ is then used to construct $S_1$.
Wlog assume that if a facility $i$ is opened in $AS_{cap}$ then it serves all its demand.\textcolor{green}{ May have to add a couple of lines here in view of the reviews of one of the reviewer: If this is not true, we can modify the $AS_{cap}$  and obtain another solution that satisfies this condition, of cost no more than that of $AS_{cap}$....will see if we can briefly say how we can modify $AS_{cap}$.}
This is always feasible as $d_i \le u_i$. $S_1$ is obtained from $AS_{cap}$ by first defining the assignment of the clients and then opening the facilities that get at least $\B$ clients. Let $\rhobar^c(j_{i'}, i)$ denotes the amount of demand of $i'$ assigned to $i$ in $AS_{cap}$ and $\rhobar^1(j_i, i')$ denotes the number of clients co-located at $i$ and assigned to $i'$ in $S_1$. 
%\textcolor{red}{ Initially each facility is assigned the clients co-located with it.}
Clients are assigned in three steps. In the first step, assign the clients co-located at a facility to itself. 
For small $i'$, additionally, we do the following  (type - $1$) re-assignments (see Fig. \ref{type1}): $(i)$ For small $i \ne i'$, assign $\rhobar^c(j_{i'}, i)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$ for small $i$. $(ii)$ For big $i$, assign $\rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ clients co-located at $i$ to $i'$. Thus, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i_1) + \rhobar^c(j_{i'}, i_2)$ for big $i$. 
Claim ~\ref{claim1} shows that these assignments are feasible and the capacities are violated only upto the extent to which they were violated by the tri-criteria solution $S^t$. 
\begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{Figures/Type 1 Assignments.jpg}
    \caption{($a$) $\B =5$, $t_1, t_2, t_3$ have demands $1$, $2$ and $1$ unit each respectively. In solution $AS_{cap}$, $1$ unit of demand of $t_1$ and $2$ units of demand of $t_2$ are assigned to $t_3$. (b) Solution $S_1$: initially, $n_i$ clients are initially assigned to facility $i$. (c) Type $1$ reassignments: $1$ and $2$ clients of $t_3$ reassigned to $t_1$ and $t_2$ respectively. After this reassignment, $t_3$ has only $1$ client.}
    \label{type1}
\end{figure}

\begin{claim}
\label{claim1}
    $(i)$ $\sum_{i' \ne i} \rhobar^1(j_i, i') \le n_i$, $\forall$ $i \in \bar \facilityset^t$.
    $(ii)$ $\sum_{i} \rhobar^1(j_i, i') \le max\{\B, n_{i'}\} \le \beta \capacityU$, for $\beta \ge 1$, $\forall$ $i' \in \bar \facilityset^t$.
 \end{claim}

\begin{proof}

    $(i)$ Since $\rhobar^c(j_{i}, i) = d_i$ therefore $\sum_{i' \ne i} \rhobar^1(j_i, i') = \sum_{i' \ne i} \rhobar^c(j_{i'}, i) \le u_i - d_i \le n_i$ in all the cases. $(ii)$ $\rhobar^1(j_{i'}, i') = n_{i'}$. For $ i \ne i'$, $\rhobar^1(j_i, i') = \rhobar^c(j_{i'}, i)$. Thus, $\sum_{i} \rhobar^1(j_i, i') = n_{i'} + \sum_{i \ne i'} \rhobar^c(j_{i'}, i) \le n_{i'} + d_{i'} \le max\{\B, n_{i'}\} \le \beta \capacityU$.
\end{proof}

Note that $S_1$ so obtained may  still not satisfy the lower bound requirement. In fact, although each facility was assigned $n_i \ge  \alpha \B$  clients initially, they may be serving less clients now after type $1$ re-assignments. For example, in Fig. \ref{type1}, $t_3$ had $4$ clients initially which was reduced to $1$ after type $1$ reassignments. Let $P \subseteq  \facilityset^t$ be the set of facilities each of which is serving at least $\B$ clients after type-$1$ reassignments, and  $\bar P =  \facilityset^t \setminus P$ be the set of remaining facilities. 
 %That is, $ P= \{ i' \in \facilityset^t: \sum_{i}\rhobar^1(j_{i}, i') \ge \B$\}.
 We open all the facilities in $P$ and let them serve the clients assigned to them after type $1$ reassignments.
 
 \begin{observation}
    If a  small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge \B$. Similarly for a big facility $i'$, if $i'_1$ was closed in $AS_{cap}$ then $i'$ is in $P$.
     %\item If a small facility $i'$ was closed in $AS_{cap}$ then $i'$ is in $P$: $\rhobar^1(j_{i'}, i') +  \sum_{i \ne i'} \rhobar^1(j_i, i')=$ $n_{i'} +  \sum_{i \ne i'} \rhobar^c(j_{i'}, i) = n_{i'} + d_{i'} \ge \B$.
    
     
    % \item If $i'$ is big then $\rhobar^1(j_{i'}, i') = n_{i'}  \ge \B$
 \end{observation}
 
 
 Thus, a small facility is in $\bar P$ only if it was open in $AS_{cap}$ and a big facility $i$ is in $\bar P$ only if $i_1$ was open in $AS_{cap}$. 
 %Also note that although each facility in $\bar P$ served at least $\alpha \B \ge \B/2$ clients in the tri-criteria solution $S^t$, they may be serving less clients now after step $1$ of assignment. \textcolor{red}{See Figure \ref{type1} for an example}.
 We now group these facilities so that each group serves at least $\B$ clients and open one facility in each group that serves all the clients in the group. For this we construct what we call as {\em facility trees}. We construct a graph $G$ with nodes corresponding to the facilities in \textcolor{olive}{$P \cup \bar P$.} For $i \in \bar P$, let $\eta(i)$ be the nearest other facility to $i$ in $\facilityset^t$. Then, $G$ consists of edges $(i, \eta(i))$. Each component of $G$ is a tree except possibly a double-edge cycle at the root. In this case, we say that we have a root, called {\em root-pair} $<i_{r_1}, i_{r_2}>$ consisting of a pair of facilities $i_{r_1}$and $ i_{r_2}$. Also, a facility $i$ from $P$, if present, must be at the root of a tree. 
 \begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{Figures/tree.jpg}
    \caption{Binary tree conversion process: (a) Tree $\mathcal{T}$ of unbounded degree: $a<b<c<g,~c<d$. (b) Binary routing tree (intermediate stage). (c) Final tree.}
    \label{tree}
\end{figure}

We process each tree bottom-up sending the clients of each facility to its parent. However doing so may result in too much violation in the capacities at the parent facility. To keep the capacity violation in check, we convert each tree into a binary tree (see Fig. \ref{tree}): first of all, we treat the double-edge cycle, if any, as a single node for this purpose. Then, at every node $x$, arrange the children of $x$ from left to right in non-decreasing order of distance from $x$. For each child $y$ (except for the nearest child) of $x$, add an edge to its left sibling %with weight $2\dist{ y}{\eta(y)}$ 
and remove the edge $( y, x)$. There is no change in the outgoing edge of the leftmost child of $x$. Let $\sigmaone(y)$ be the parent of $y$ in the so constructed tree.  

\begin{lemma}
For any node $y$ in the binary tree, $\dist{y}{\sigmaone(y)} \leq 3 \dist{y}{\eta(y)}$. 
\end{lemma} 
\begin{proof}
Let $\mathcal{T}$ be a tree.
For any node $x$ that is not a root pair, it is easy to see that $\dist{y}{\sigmaone(y)} \leq 2 \dist{y}{\eta(y)}$ for all children $y$ of $x$. Next consider a root pair $<r_1, r_2>$. Let 
$\cone_1 \ldots \cone_k$ 
be the children of $r_1/r_2$ in the increasing order of
$\dist{\cone_i}{\eta(\cone_i)}$. Then $\psi(\cone_i) = \cone_{i-1}$ for $i = 2 \ldots k$ and $\psi(\cone_1) = \eta(\cone_1)$. If,  for $i = 2 \ldots k$, $\eta(\cone_i) = \eta(\psi(\cone_i)) (= r_1/r_2)$ (i.e. $\cone_i$ and $\psi(\cone_i)$ are children of the same node ($r_1/r_2$)), then  $\dist{\cone_i}{\sigmaone(\cone_i)} \leq 2 \dist{\cone_i}{\eta(\cone_i)}$. Otherwise (see Figure~\ref{}), $\dist{\cone_i}{\sigmaone(\cone_i)} \leq \dist{\cone_i}{\eta(\cone_i)} + \dist{\eta(\cone_i)}{\eta(\cone_{i-1})} + \dist{\eta(\cone_{i-1})}{\cone_{i-1}} \le 3 \dist{\cone_i}{\eta(\cone_i)}$. \end{proof}





%Its easy to see that $\dist{y}{\sigmaone(y)} \leq 3 \dist{y}{\eta(y)}$. 
Thus, we replace $\dist{y}{\sigmaone(y)}$ by $3 \dist{y}{\eta(y)}$ for all $y$. Henceforth, whenever we refer to distances, we mean the new edge weights. Now, every node has in-degree of at most $2$ with the in-degree of the root being at most $1$. 

Now we are ready to define our second type of re-assignments.
\textcolor{violet}{Process the tree bottom-up using Algorithm~\ref{} until we reach the root node, which could be either a single facility in $P$ or a root-pair. Processing of the root-pair node is slightly different and is explained in Algorithm~\ref{}
}
 Let $ i_c$ be the only child, if any,  of the root (/root pair) of a tree. Let $i$ be the parent of $ i_c$ ($i$ is either in $P$ or it is one of $i_{r_1}$ and $i_{r_2}$ in case the root is a root pair).
Process the tree bottom-up, til we reach $i_c$, as follows (see Fig. \ref{type2-3} \textcolor{blue}{($A$)}): \\
\textcolor{green}{
Process(i)\\
Process($L_i$), Process($R_i$) \\
If $L_i$ has at least $\B$ clients, open $L_i$ and disconnect $L_i$ from the tree by cutting the edge $(L_i, \sigmaone(L_i))$ and setting $L_i$ to NULL.\\
If $R_i$ has at least $\B$ clients, open $R_i$ and disconnect $R_i$ from the tree by cutting the edge $(R_i, \sigmaone(R_i))$ and setting $R_i$ to NULL.\\
If none of $L_i$ and $R_i$ is NULL, send the clients of $R_i$ to $L_i$. \\
If $L_i(/R_i)$ is non-NULL, send it's clients to $i$.\\
}


\begin{algorithm}[H] 
    \SetAlgoLined
    %\KwData{$\clientset,~\facilityset$}
    %\KwResult{$\clientset',~\bundle{j'}~\forall~j'\in \clientset'$}
    \SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
    \Input{$i$}
    %\Output{}
		 
	% Process($lc_i$)\;
		 
	% Process($rc_i$)\;
		 
		 \textcolor{blue}{$re-assigned(rc_i) = false$ \tcp*{boolean variable to indicate if clients of $rc_i$ are assigned to $lc_i$ or not; initially false}} 
		 
		 
		 
		 \If{$n_{rc_i} \geq \B$}  {
		 
		 Open facility $rc_i$\;
		 
		 Remove edge ($rc_i, \psi(rc_i)$)  \textcolor{blue}{\tcp*{Remove the connection of $rc_i$ from its parent}}
		 
		 $rc_i \gets$ NULL\;
		 
		 }
		 
		 \If{$lc_i \ne $ NULL AND $rc_i \ne $ NULL}  {
		 
		   $n_{lc_i} \gets  n_{lc_i} + n_{rc_i}$
		   
		   	   $re-assigned(rc_i) \gets true$
		   
		    \If{$n_{lc_i} \geq \B$}  {
		 
		 Open facility $lc_i$\;
		 
		 Remove edge ($lc_i, \psi(lc_i)$)\;
		 
		 $lc_i \gets$ NULL\;
		 
		 }
		 }
		 
   	\If{$lc_i \ne $ NULL AND ($re-assigned(rc_i) = true$ OR $rc_i =$ NULL) \textcolor{blue}{Isnt the part after AND condition redundant?? Its not required,I think}} {
		 
		   $n_i \gets  n_i + n_{lc_i}$
		  
		 } 
		 
		 \If{$rc_i \ne $ NULL AND   ($re-assigned(rc_i) \ne true$)}  {
		   $n_i \gets  n_i + n_{rc_i}$ \textcolor{blue}{\tcp*{ $lc_i$ must be NULL in this case.}}
		 }
		
		
	\label{Process_i}
	\caption{Process($i$)}
\end{algorithm}
 
 



(D later: Process the tree bottom-up as follows (see Fig. \ref{type2-3} \textcolor{blue}{($A$)}): 
If $i$ has at least $\B$ clients, open $i$ and disconnect $i$ from the tree by cutting the edge $(i, \sigmaone(i))$ else send its clients to its parent facility. The process is repeated till we reach the root. 

 \begin{lemma}
 \textcolor{red}{
(I think D: Repetition: Let $ i_c$ be the only child, if any,  of the root (/root pair)of a tree. Let $i$ be the parent of $ i_c$ ($i$ is either in $P$ or it is one of $i_{r_1}$ and $i_{r_2}$ in case the root is a root pair).
}
The number of clients collected in the second type of re assignments, at any node $x$  in the subtree rooted at $i_c$, is at most $2\B$.
 \end{lemma}
 
 \begin{proof} 
 \textcolor{violet}{We will show that the number of clients collected at $x$ after Process($x$) is at most $2\B$. For this, note that $x$ receives $< \B$ clients from at most one of it's children. Hence, the claim follows.}
 (to be seen again after finalising the algorithm)
 We will show that the number of clients collected at $i$ after Process($i$) is at most $2\B$. For this, note that if the number of clients collected at both $L_i$ as well as $R_i$ are individually $< \B$, then $R_i$ sends its clients to $L_i$. Thus, $i$ receives clients from at most one of its children in case the child has collected $< \B$ clients. Since all nodes except possibly the root are in $\bar P$, $i$ has at most $\B$ clients of its own. Hence, the claim follows.
 
 \end{proof}


There are two possibilities at the root: either we have a facility $i$ from $P$ or we have a root-pair $<i_{r_1}, i_{r_2}>$. In the first case, we are done as $i$ is already open and has at least $\B$ clients. To handle the second case, we need to do a little more work. So, we define our assignments of third type as follows (see Fig. \ref{type2-3} \textcolor{blue}{($\B$)}): 
($i$) If the total number of clients at   $i_c, i_{r_1}$ and $i_{r_2}$ is at least $\B$ and at most $2\B$ then open the facility with more number of clients from $i_{r_1}$ and $i_{r_2}$, say $i_{r_1}$ and send the clients of $i_c$ and $i_{r_2}$ to $i_{r_1}$.
($ii$) If the total number of clients at $i_c, i_{r_1}$ and $i_{r_2}$ is more than $2\B$  then open both $i_{r_1}$ and $i_{r_2}$, and distribute the clients of $i_c$ so that each one of them gets at least $\B$ clients.
($iii$) If the total number of clients at $i_c, i_{r_1}$ and $i_{r_2}$ is less than $\B$, then let $i$ be the node in $P$ nearest to $\{i_{r_1}, i_{r_2}\}$, then $i$ is already open and has at least $\B$ clients. Send the clients of $i_c, i_{r_1}$ and $i_{r_2}$ to $i$.

($i$) If the total number of clients at the root pair $<i_{r_1},i_{r_2}>$ is at least $\B$ then open the facility with more number of clients, say $i_{r_1}$ and send the clients of $i_{r_2}$ to $i_{r_1}$. %(in our case, we cannot have a scenario in which both have at least \B clients. If $i_2$ is the facility at which the rest of the tree hangs then the number of clients at $i_1$ cannot be more than $\B$.....this is not true in Zoya's case because there a tree hangs at both the ends of the double-edge loop which we have eliminated....Since the number of clients at $i_1$ is less than \B..the number of clients along any edge is still less than \B ....only for our understanding...to be deleted later)..
($ii$) If the total number of clients at the root pair $<i_{r_1},i_{r_2}>$ is less than $\B$, then let $i$ be the node in $P$ nearest to $\{i_{r_1}, i_{r_2}\}$, i.e., $i$ is already open and has at least $\B$ clients. Send the clients of $i_{r_1}$ and $i_{r_2}$ to $i$.
\begin{figure}[t]
	\begin{tabular}{ccc}
		\includegraphics[width=40mm,scale=1.0]{Figures/Type 2 Assignments.jpg}
		&& 
		\includegraphics[width=65mm,scale=1.0]{Figures/Type 3 Assignments.jpg} 	
		\\
		\textbf{(A)}&&\ \ \textbf{(B)}& \ \
	\end{tabular}
	\caption{$\B=4$ (A) Type 2 Assignments: (a) Before assignments. (b) After assignments.
	(B) Type 3 Assignments (i) Total clients at root pair $<i_{r_1},i_{r_2}>$ is at least $\B$: (a) Before assignments. (b) After assignments: $i_{r_2}$ is open.  (ii) Total clients at root pair $<i_{r_1},i_{r_2}>$ is less than $\B$: (a) Before assignments. (b) After assignments: $i_{r_1},i_{r_2}$ are both closed. 
	}
	\label{type2-3}
\end{figure}

%($i$) If both $i_1$ and $i_2$ have at least $\B$ clients, open bot of them ($ii$) if one of them say $i_1$ has at least $\B$ clients but $i_2$ doesn't then open $i_1$ and send the clients of $i_2$ to $i1$ ($iii$) If both of them have clients less than $\B$ but in total they have at least $\B$ clients, open any one of them, say $i_1$ and send the clients of the other to $i_1$.
 
 
% \textcolor{red}{need to see this part again}
 %Next we bound the capacity violation:  Let $\pi_i$ be the number of clients assigned to the facility $i$ after first type of re-assignments. Then as shown earlier, $\pi_i \le \beta \capacityU$. (Reptn:D: Let $ i_c$ be the only child of the root (/root pair). Let $i$ be the parent of $ i_c$. In second and third types of assignments,  we never collect more than $2\B$  \textcolor{red}{additional $2\B$, no?}  clients at any node till we reach $i_c$ \textcolor{blue}{Can we shift this statement to case ii where it is used??}. )
% Now we have the following scenarios: Suppose $ i_c$ has less than $\B$ clients, we have the following cases: ($i$)  the root node $i$ is in $P$ and it gets additional at most $\B$ clients from $i_c$ making a total of at most $\pi_i + \B \le \beta \capacityU + \B \le (\beta + 1) \capacityU$ clients at $i$. ($ii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at least $\B$. Number of clients at $i_{r_1}$ and $i_{r_2}$ are at most $\B$ and $2\B$ respectively. Thus, the number of clients the opened facility gets is at most $3\B \le 3 \capacityU$. ($iii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients less than $\B$. Number of clients at the root pair and their nearest facility in $P$ are at most $\B$ and $\beta \capacityU$ respectively. Thus, the number of clients the opened facility in $P$ gets is at most $\beta \capacityU + \B \le (\beta + 1) \capacityU$. 
 
  Next, we bound the capacity violation: 
 Let $\pi_i$ be the number of clients assigned to the facility $i$ after first type of re-assignments. Then as shown earlier, $\pi_i \le \beta \capacityU$.  Let $i$ be the parent of $ i_c$. In second and third types of assignments,  we never collect  more than $2\B$ clients at any node till we reach $i_c$.
 Now we have the following scenarios: Suppose $ i_c$ has less than $\B$ clients, we have the following cases: ($i$) the root node $i$ is in $P$ and it gets additional at most $\B$ clients from $i_c$ making a total of at most $\pi_i + \B \le \beta \capacityU + \B \le (\beta + 1) \capacityU$ clients at $i$.
 ($ii$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at $i_c, i_{r_1}$ and $i_{r_2}$ is at least $\B$ and at most $2\B$. Thus, the number of clients the opened facility gets is at most $2\B \le 2\capacityU$.
 ($iii$)  the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at $i_c, i_{r_1}$ and $i_{r_2}$ is more than $2\B$.  Note that the total number of clients at these facilities is at most $3\B$ and hence it is possible to distribute them to the two opened facilities $i_{r_1}$ and $i_{r_2}$ so that each of them gets at most $2\B \le 2\capacityU$ clients. ($iv$) the root is a root pair $<i_{r_1}, i_{r_2}>$ with $i = i_{r_2}$ and total number of clients at $i_c, i_{r_1}$ and $i_{r_2}$ is less than $\B$. 
 %Number of clients at $i_c$ and the root pair and, their nearest facility in $P$ are at most $\B$ and $\beta \capacityU$ respectively. 
 Thus, the number of clients the opened facility in $P$ gets is at most $\beta \capacityU + \B \le (\beta + 1) \capacityU$. 
 %The case when $i_c$ has at least $\B$ clients leads to the third scenario above and hence handled.
 
 
 We next bound the connection cost: the cost of first type of re-assignments is \textcolor{olive}{at most the connection cost of $AS_{cap}$.} 
% \textcolor{red}{(or at most?Sapna/rajni) }
 To bound the connection cost of second type, observe that we never send more than $\B$ clients on any edge. 
 %In the second type of assignment, 
 Let a facility $i$ sends its (at most $\B$ clients) to its parent or to its left sibling. Since the facility $i$ was opened in $AS_{cap}$, it pays facility opening cost of $\delta l(i) min \{n_i, \B\} \ge \delta l(i) \alpha \B$. Summing over all $i \in \bar P$ for the second type of re-assignments, we see that the total connection cost in these re-assignments is bounded by 
 \textcolor{red}{
 $3 FCost_{I_{cap}}(AS_{cap})/\alpha \delta$ (Sapna...to be seen)
 } \textcolor{olive}{$\sum_{i \in \bar P} \B l(i) \leq 6FCost_{I_{cap}}(AS_{cap})/\alpha \delta$  where factor 6 comes because sending clients to the left sibling incurs a cost of twice the cost to the node's parent and $FCost_{I_{cap}}(AS_{cap})$ is the facility opening cost of a solution to $I_{cap}$ instance.}
% \textcolor{red}{define FCost}
  %of edge weights being thrice of their original weight during the formation of binary tree.
 %\textcolor{blue}{ \st {where $Cost_f(.)$ is the facility opening cost of a solution to the $I_{cap}$ instance }}


 For the third type of re-assignments, we bound the cost in two parts: ($a$) cost of sending ($< \B$) clients of $i_c$ to it's parent ($b$) Cost of sending ($< \B$) clients collected at the root pair $<i_{r_1}, i_{r_2}>$ to it's nearest facility in $P$. Cost of the first part is bounded by $\B l(i_c)$. The cost of sending ($< \B$) clients by a facility $i$ in the root pair $<i_{r_1}, i_{r_2}>$ is not bounded by $\B l(i)$ (where $l(i) = l(i_{r_1}) = l(i_{r_2})$). We bound the cost as follows: the total number of clients, initially at $i_{r_1}$ and $i_{r_2}$ was $\ge 2 \alpha \B$. However, during re-assignments of type $1$, some of them got reassigned to other facilities. Note that these (other) facilities must have been closed in $AS_{cap}$ and hence do not belong to $\bar P$. Hence, each of these reassignments correspond to an assignment in $AS_{cap}$ whose cost was at least $l(i)$ and a total of at least $(2\alpha  - 1)\B l(i)$. Hence the cost of type $3$ re-assignments is bounded by \textcolor{blue}{$3 CCost_{I_{cap}}(AS_{cap})/ (2\alpha  - 1)$ where $CCost_{I_{cap}}(AS_{cap})$ is the connection cost of $AS_{cap}$ solution.} Hence the total cost of solution $S_1$  is $6\alpha/(2\alpha-1) \textcolor{blue}{Cost_{I_{cap}}(AS_{cap})}$ for $\delta= (2\alpha-1)/6\alpha^2 $. \textcolor{blue}{Why 6 times???}
 

==> NEW Journal version WADS 2021 (LBUBFL)/TriCriteria.tex <==
\section{Computing the Tri-criteria Solution}
\label{tri-criteria}
 %We use a simpler LP-rounding technique to get $(\frac{\ellone-1}{\ellone})$-factor violation in lower bounds and $2$-factor violation in upper bounds at constant factor loss in cost. The technique used is much simpler than Friggstad et al. \cite{friggstad_et_al_LBUFL} because lower bounds are uniform in our case unlike Friggstad et al. that considers non-uniform lower bounds. 
 \textcolor{red}{
 In this section, we give a tri-criteria solution that violates the lower bound by a factor of $\alpha = (1 - \theta)$ and the upper bound by a factor of $\beta = (1 + \theta)$ where $\theta \le 1/2$ is a tune-able parameter.
 }
Instance $I$ of LBUBFL can be formulated as the following integer program (IP):

\label{{unif-CFLP}}
$Minimize ~\mathcal{C}ostLBUBFL(x,y) = \sum_{j \in C}\sum_{i \in F}\dist{i}{j}x_{ij} + \sum_{i \in F}f_iy_i $
\begin{eqnarray}
subject~ to &\sum_{i \in F}{} x_{ij} \geq 1 & \forall ~\singleclient \in C \label{LPFLP_const1}\\ 
%&\sum_{j \in C}{} x_{ij} \leq \capacityU ~ y_i & \forall~ \singlefacility \in F \label{LPFLP_const2}\\ 
& \capacityU y_i \geq \sum_{j \in C}{} x_{ij} \geq \B y_i & \forall~ \singlefacility \in F \label{LPFLP_const3}\\
& x_{ij} \leq y_i & \forall~ \singlefacility \in F , ~\singleclient \in C \label{LPFLP_const4}\\   
& y_i,x_{ij} \in \left\lbrace 0,1 \right\rbrace  \label{LPFLP_const5}
\end{eqnarray}
where  $y_i$ is an indicator variable which is equal to $1$ if facility $i$ is open and is $0$ otherwise. $x_{ij}$ is an indicator variable which is equal to $1$ if client $j$ is served by facility $i$ and is $0$ otherwise.
 Constraints \ref{LPFLP_const1} ensure that all the clients are served. %Constraints \ref{LPFLP_const2} make sure that the total demand assigned to an open facility is no more than its capacity \capacityU. 
 Constraints \ref{LPFLP_const3} make sure that the total demand assigned to an open facility is at least $\B$ and at most $\capacityU$. Constraints \ref{LPFLP_const4} ensure that a client is assigned to a facility only if it is opened. LP-Relaxation  is obtained by allowing the variables to be non-integral.
% $ y_i, x_{ij} \in [0, 1]$. %Call it LP. 
Let $\zeta^{*} = <x^*, y^*>$ be an optimal solution  and $\opt{}$ be its cost.

TBD: In this section, we give a tri-criteria solution that violates the lower bound by a factor of $(\ellone-1)/\ellone$ for a fixed parameter \textcolor{blue}{$\ellone \geq 2$} and the upper bounds by a factor of $2$.

We start by sparsifying the problem instance by removing some clients and distributing their demands to the remaining clients. This is done using clustering technique in the same manner as is done in Grover \etal~\cite{GroverGKP18}: for $j \in C$, let $ \C{j} $ denote the average connection cost paid by $\singleclient$ in $\zeta^*$. 
%i.e., ~$\C{j} = (\sum_{i \in F}{} {x}^*_{ij} \dist{i}{j})/({\sum_{i \in F}{} {x}^*_{ij}})$. 
Further, let \textcolor{blue}{$\ellone \geq 2$} be a fixed parameter and let $\ballofj{j}$ be the ball of facilities within a radius of $\ellone\C{j}$ of $j$.
%~ i.e., \ \ballofj{j}  = \{ \singlefacility \in F \colon \dist{i}{j} \leq \ellone \C{j} \}$.
Then,  $\cardTwo{\ballofj{j}} \ge (1-\frac{1}{\ellone})$ where $\cardTwo{\ballofj{j}}$
%$=  \sum_{i \in \ballofj{j}} y^*_i$ 
denotes the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
The balls 
%The clients 
are processed in the non-decreasing order of their radii dissolving the overlapping balls of larger radii and removing their (client) centers. The process is repeated with the remaining balls. Let $C'$ be the set of  clients remaining at the end of the process. The set of facilities that do not belong to ball of any client in $C'$ are partitioned so as to form clusters around the remaining balls, by assigning them to the cluster of $j'$ where $j'$ is nearest to the facility amongst all $j' \in C'$. %the nearest cluster center.
%Clusters of the remaining facilities are formed around the remaining balls by assigning them to the cluster of the nearest cluster center.
%For a client $j$ at hand, remove all the clients 
%$k : \dist{j}{k} \le 2 \ellone \max \{\C{j}, \C{k}\}$ 
%whose balls overlap with that of $j$ and repeat the process with the remaining clients. Let $C'$ be the set of  clients remaining after all the clients in $C$ have been considered. Clusters, of facilities, are formed around the  clients in $ C'$ by assigning a facility to the cluster of the nearest client in $C'$, i.e. if, for $j' \in C'$, $\bundle{j'}$ denotes the cluster centered at $j'$ then a facility $i$ belongs to $\bundle{j'}$ if and only if $j'$ is the closest client in $C'$ to $i$. Note that $\ballofj{j'} \subseteq \bundle{j'}$.
%
%$\cardTwo{\hat{y}}{\ballofj{j}} \ge (1-\frac{1}{\ellone})(\sum_{i \in F} \hat{x}_{ij}) \geq \frac{1}{2\ellone}$ where $\cardTwo{\hat{y}}{\ballofj{j}} =  \sum_{i \in \ballofj{j}} \hat{y}_i$ denotes the total extent up to which facilities in \ballofj{j} are opened under $\hat{\zeta}$. 
The clients in $C'$ are then called the cluster centers.

\begin{Observation}
Any two cluster centers $j', k'$ in $C'$ satisfy the {\em separation property}: $\dist{j'}{k'} > 2\ellone~max\{ \C{j'},\C{k'}\}$.
\end{Observation}

\begin{lemma}
Let $j' \in \clientset', j \in \clientset, i \in \bundle{j'}$. Then,
\begin{enumerate}
    \item $\dist{i}{j'}  \leq \dist{i}{j} + 2\ellone \C{j}$
    \item $\dist{j}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}  $
\end{enumerate}
\end{lemma}

\begin{proof}
\begin{enumerate}
    \item \textcolor{blue}{Note that, for an arbitrary client $j$,  $\dist{j}{k'} \leq 2\ellone \C{j}$ for some $k' \in \clientset'$. Then we have $\dist{i}{j'} \leq \dist{i}{k'} \leq \dist{i}{j} + \dist{j}{k'} \leq \dist{i}{j} + 2\ellone \C{j}$, where the first inequality follows because $i$ belongs to $\ballofj{j'}$ and not $\ballofj{k'}$.
    \item Thus, 
    %we get the following bound~\cite{GroverGKP18}
%\begin{eqnarray} \label{Cjj'}
$\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}  $
%\end{eqnarray}
    }
\end{enumerate}
 
\end{proof}
 

\begin{figure}
    \centering
    \includegraphics[width=5cm]{Figures/Cjj'.jpg}
    \caption{$\dist{j}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$}
    \label{Cjj'}
\end{figure}

%$\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$ ~\cite{GroverGKP18}.}  

\textcolor{blue}{Next, let $\loadjinc{j}{j'}$ be the extent up to which $j$ was served by the facilities in the cluster of $j'$.}
%Demand of the clients are distributed to various cluster centers: for a client $j$ and a cluster center $j'$, let $\loadjinc{j}{j'}$ be the extent up to which $j$ was served by the facilities in the cluster of $j'$. 
%\textcolor{red}{Then $\loadjinc{j}{j'}$ extent of $j$ is moved to $j'$. The cost of doing so for all the clients is bounded by  $2(\ellone+1)$ $LP_{opt}$: note that  $\dist{j}{k'} \leq 2\ellone \C{j}$ for some $k' \in \clientset'$. Then we have $\dist{i}{j'} \leq \dist{i}{k'} \leq \dist{i}{j} + \dist{j}{k'} \leq \dist{i}{j} + 2\ellone \C{j}$, where the first inequality follows because $i$ belongs to $\ballofj{j'}$ and not $\ballofj{k'}$.  Thus, $\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$ ~\cite{GroverGKP18}.}
Let $d_{j'}= \sum_{j \in \clientset} \loadjinc{j}{j'}$. 
%\sum_{i \in \bundle{j'}}{}  \hat{x}_{ij}.$} %\loadjinc{\hat{\zeta}}{j}{\bundle{j'}}$.
We call a cluster to be $sparse$ if $d_{j'} \le  \capacityU$ and $dense$ otherwise. %\textcolor{blue}{Let $\csparse$ be the set of all sparse clusters and $\cdense$ be the set of all dense clusters.}



%Let $<\hat{x}, \hat{y}>$ be the solution so obtained, i.e., for $ j \in \clientset$, $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$. For $j' \in \crich, i \in \bundle{j'}, j \in \clientset$, $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. 


\textcolor{red}{
\begin{lemma} \label{Sparse}
We can obtain a solution $<\xhat, \yhat>$ such that  exactly one facility $i(j')$ is opened integrally in each sparse cluster centered at $j' \in \clientset'$. The solution violates the lower bound by a factor of $(1 - 1/\ellone)$ and its cost is bounded by
$\sum_{j' \in \clientset'}[\frac{\ellone}{1 - \ellone}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})]$.
\end{lemma}
}



\begin{lemma} \label{Sparse}
For each sparse cluster centered at $j' \in \clientset'$, we can open a facility $i(j')$ integrally and transfer all the assignments in the cluster to it at cost at most
$2 \sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} [\dist{i}{j} + \ellone \C{j}]$.

%the demand $\demandofj{j'}$ can be served from facility $i(j')$ in the cluster $\bundle{j'}$ such that $\sum_{j \in \clientset} \loadjinc{j}{j'} \dist{i(j')}{j}  \leq 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} [\dist{i}{j} + \ellone \C{j}]$ and  $f_{i(j')} \leq 3/2 \sum_{i \in \bundle{j'}} f_i y^*_i $.
\end{lemma}

\begin{proof}
%In a sparse cluster centered at $j'$, we open the cheapest facility, say $i(j')$, in $\ballofj{j'}$ and transfer all the assignments in the cluster onto it.
\textcolor{blue}{ %As specified above, 
Let  $i(j')$ be a cheapest facility in $\ballofj{j'}$. We open $i(j')$ and transfer all the assignments in the cluster onto it (see Figure...). Since $\cardTwo{\ballofj{j'}} \ge (1-\frac{1}{\ellone})$, lower bound is violated at most by $(1-\frac{1}{\ellone})$ and the facility cost is bounded by $\frac{\ellone}{1 - \ellone} \sum_{i \in \bundle{j'}} f_i y^*_i$. To bound the service cost, we will show that $\sum_{j \in \clientset} \loadjinc{j}{j'} \dist{i(j')}{j}  \leq 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})$: 
since $i(j') \in \ballofj{j'}$, we have $\dist{i(j')}{j'} \le \ellone \C{j'}$. 
\{TBD Thus, for an arbitrary client $j \in \clientset$ which was served by a facility $i$ in the cluster of $j'$,\} }
\textcolor{red}{ Thus, for $j \in \clientset$,
we have $\dist{i(j')}{j} \le \dist{j'}{j} + \dist{i(j')}{j'} \le  \dist{j'}{j} + \ellone \C{j'}$. If $\ellone \C{j'} \le \dist{j'}{j}$ then $\dist{i(j')}{j}  \le 2  \dist{j'}{j}  \leq 4 (\dist{i}{j} + \ellone \C{j})$ (for all $i \in \bundle{j'}$ by Lemma 2.1) else $\dist{i(j')}{j}  \le  2 \ellone \C{j'}$.}
%\textcolor{blue}{MOVED IN GLOBAL REGION- DISCUSS} Note that  $\dist{j}{k'} \leq 2\ellone \C{j}$ for some $k' \in \clientset'$. Then we have $\dist{i}{j'} \leq \dist{i}{k'} \leq \dist{i}{j} + \dist{j}{k'} \leq \dist{i}{j} + 2\ellone \C{j}$, where the first inequality follows because $i$ belongs to $\ballofj{j'}$ and not $\ballofj{k'}$.  Thus, $\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$ ~\cite{GroverGKP18}. 
\textcolor{blue}{Thus, in either case $\dist{i(j')}{j} \leq 4 (\dist{i}{j} + \ellone \C{j})$ for all $i \in \bundle{j'}$.}
\textcolor{red}{Substituting $\phi(j, j') = \sum_{i \in \bundle{j'}} x^*_{ij}$ and summing over all $
j' \in \clientset'$ we get the desired claim.}
%Also, since $(1-(1/\ellone)) \ge 1/2$ for $\ellone \ge 2$, we incur a loss of $2$ factor in the facility opening cost.
%Violation in lower bound is at most $(1-(1/\ellone))$; there is no  violation in the capacities as  $d_{j'} \le \capacityU$.
\textcolor{blue}{Discuss else part with Madam}

 \end{proof}
 
%$\le 4\dist{i}{j} + 4 \ellone \C{j} $ else $\dist{i(j')}{j}  \le  2 \ellone \C{j'} \le 4 \ellone \C{j} \le 4\dist{i}{j} + 4 \ellone \C{j}$, where the second inequality in the else part follows because if $\ellone \C{j'} > \dist{j'}{j}$ then $\C{j'} \leq 2\C{j}$ \cite{GroverGKP18}. Also, since the total opening in each cluster is at least $(1-(1/\ellone))$, a loss of factor $\ellone/(\ellone-1) (\leq 2$ for $\ellone \geq 2$) in the facility opening cost is incurred, violation in lower bound is at most $(1-(1/\ellone))$ and  since  $d_{j'} \le \capacityU$ there is no  violation in the capacity.}
   
    
 

    
Next, we consider the dense clusters. To open the facilities integrally in the dense clusters, we solve the following LP for every dense cluster $\bundle{j'}$ centered at $j'$.

($LP_2$): 
\label{dense}
$Minimize ~\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$
\begin{eqnarray}
subject~ to &\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'} \label{denseLP_const1}\\ 
&0 \leq \zofi{i} \leq 1 \label{denseLP_const2}
\end{eqnarray}
   
  % $Minimize $\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$ s.t. $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$ and $\zofi{i} \in [0,1]$. 
   
   
Note that $\zofi{i} = \sum_{j \in C}x_{ij}^*/\capacityU$ is a feasible solution with cost at most $ \sum_{i \in \bundle{j'}} \facilitycost y^*_i + \sum_{i \in \bundle{j'}} \sum_{ j \in C} x^*_{ij} [ \dist{i}{ j} + 2\ellone \C{j} ]$ by claim (1) of Lemma 2.1.

\textcolor{blue}{TBD: facility opening cost at most
$ \sum_{i \in \bundle{j'}} \facilitycost y^*_i$ and service cost
$\sum_{i \in \bundle{j'}} \sum_{ j \in C} x^*_{ij}  \dist{i}{j'} \le \sum_{i \in \bundle{j'}} \sum_{ j \in C} x^*_{ij} [ \dist{i}{ j} + 2\ellone \C{j} ]$. } 

\textcolor{red}{
\begin{lemma} \label{integral_dense}
An integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) by a factor of $(1+1/\ell)$, can be obtained at a loss of factor $(\ell)$ in cost.
\end{lemma}
}


\begin{lemma} \label{integral_dense}
For a fixed $0 < \epsilon < 1$, 
an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) by a factor of $(1+\epsilon)$, can be obtained at a loss of $(1/\epsilon)$ in cost.
%for each dense cluster $\bundle{j'}$ and the demand $\demandofj{j'}$ can be distributed to the opened facilities in the cluster at a loss of $O(1/\epsilon)$ in cost and a loss of $(1+\epsilon)$-factor in constraints (\ref{denseLP_const1}).
\end{lemma}
\begin{proof}
We first obtain an almost integral solution\footnote{A solution is said to be an almost integral solution if it has at most one fractionally opened facility.} $\primezofi{}$ by arranging the facilities opened in $z$, in non-decreasing order of $\facilitycost  + \dist{i}{j'} \capacityU$ and greedily transferring the openings $z$ onto them. %Assignment equivalent to $\capacityU \primezofi{i}$ is allotted to each facility $i \in \bundle{j'}$. 
Clearly,  $\sum_{i \in \bundle{j'}} \primezofi{i} = \sum_{i \in \bundle{j'}} \zofi{i}$. Consider constraint (\ref{denseLP_const1}), $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$. Note that the cost of solution $\primezofi{}$ is no more than that of solution $z$.

%$\capacityU \primezofi{i}$ amount of assignments coming onto the facilities in the cluster....%Each facility $i \in \bundle{j'}$ is assigned demand equivalent to $\capacityU \primezofi{i}$. 

We now convert the almost integral solution $\primezofi{}$ to an integral solution $\hat{z}$. Let $\hat{z} = \primezofi{}$ initially. Let $i'$ be the fractionally opened facility, if any, in $\bundle{j'}$. %Initially, set $\hat{z}_i = \primezofi{i}~ \forall i \in \bundle{j'}$. 
Consider the following cases:


\begin{enumerate}
    \item $\primezofi{i'} < \epsilon$:
    \textcolor{red}{$\primezofi{i'} < 1/\ell$: }close $i'$ in $\hat{z}$, 
   % set $\hat{z}_{i'} = 0$. 
    There must be at least one integrally opened facility, say $i \ne i'$ in $\bundle{j'}$ in $\primezofi{}$, as $\demandofj{j'} \ge \capacityU$. Then, $\demandofj{j'} \leq \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k} + \capacityU  (\primezofi{i} + \primezofi{i'}) \le \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k}  + (1 + \epsilon) \textcolor{red}{(1 + 1/\ell)} \capacityU  \primezofi{i} \le (1 + \epsilon) \textcolor{red}{(1 + 1/\ell)} \capacityU \sum_{k \in \bundle{j'} \setminus \{i'\}} \primezofi{k} = (1 + \epsilon)\textcolor{red}{(1 + 1/\ell)} \capacityU \sum_{k \in \bundle{j'}} \hat{z}_k$. There is no change in cost.

    \item $\primezofi{i'} \geq \epsilon \textcolor{red}{(1/\ell)}$: Open $i'$ integrally at a loss of $1/\epsilon \textcolor{red}{(\ell)}$  in facility opening cost: i.e., $\sum_{i \in \bundle{j'}} f_i \hat{z}_i \le (1/\epsilon) \textcolor{red}{(\ell)} \sum_{i \in \bundle{j'}} f_i \primezofi{i}$.
    %and  no loss in constraint (\ref{denseLP_const1}) and connection cost w.r.t $i'$. 
\end{enumerate}\end{proof}

%Let $\hat{z}$ be the solution so obtained. Then, $(1 + \epsilon) \capacityU \sum_{\singlefacility \in \bundle{j'}} \hat{z}_i \geq \demandofj{j'}$ and $\sum_{i \in \bundle{j'}} f_i \hat{z}_i \le (1/\epsilon) \sum_{i \in \bundle{j'}} f_i \hat{z}_i $.


Next, we define our assignments in the dense clusters. We first distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution.  Clearly $l_i \le (1 + \epsilon) \capacityU$. Let $i \in \bundle{j'}, j \in \clientset$.  Set $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. 



\begin{lemma} \label{Dense}
For a fixed $0<\epsilon< 1/2$, the cost of the solution $<\bar x, \bar y>$ corresponding to a dense cluster centered at $j'$ is bounded by $ (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+ (1/\epsilon))  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} + 2\ellone(1+1/\epsilon) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} $.
%Given the integral solution $\hat{z}$ to $LP_2$ corresponding to a dense cluster centered at $j'$, we can obtain a feasible set of assignments $\bar x$ and distribute $\demandofj{j'}$ to facilities in $\bundle{j'}$ at a loss of ......... 
\end{lemma}

\textcolor{red}{
\begin{proof}
Let $i \in \bundle{j'}, j \in \clientset$. Recall that $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. Consider the cost of the solution:\\ 
$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij}) $\\
$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \dist{i}{j}  \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} (\dist{j}{j'} + \dist{i}{j'})$ (by triangle inequality)\\ 
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )  $ (by definition of $\loadjinc{j}{j'}$, equation (\ref{Cjj'}) and the fact that $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\%(Sapna..I have used multiple things ...pls write them here...)\\
$ \leq  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +  (1+\epsilon) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j} \primezofi{i} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
$\leq max\{(1/\epsilon), (1+\epsilon)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\
$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (for $\epsilon \leq 1/2$)\\
$= (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   (1/\epsilon)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by cost bound of feasible solution $z$)\\
$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   (1/\epsilon)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ellone \C{j}) + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\
$= (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+ (1/\epsilon))  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} + 2\ellone(1+1/\epsilon) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} $ \\
%$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i + \dist{i}{j'} \sum_{j \in \clientset} \bar{x}_{ij}) $\\
%$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
%$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} l_i$\\ 
%$ \leq  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +  (1+\epsilon) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i}$\\
%$\leq max\{(1/\epsilon), (1+\epsilon)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i}$\\
%$= (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i}$ for $\epsilon< 1/2$\\
%$ =  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU  \dist{i}{j'}) z_i$\\
%$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   (1/\epsilon)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij}$\\
%$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} x^*_{ij} [ \dist{i}{ j} + 2\ellone \C{j} ]$.
\end{proof}
}

	%\textcolor{blue}{Choosing $\ellone = O(1/\epsilon)$, the total cost of the tri-criteria solution is $Cost_f(S^t) + Cost_c(S^t) \leq %\frac{\ellone}{\ellone-1} Cost_f(O) + 4Cost_c(O) + O(1/\epsilon)\sum_{j \in \clientset}\C{j} \leq 
	%\max\{2,1/\epsilon\}Cost_f(O) + O(1+\epsilon) Cost_c(O) \leq O(1/\epsilon)Cost(O)$, where $Cost_f(.)$ and $Cost_c(.)$ denote the facility opening cost and connection cost respectively of the particular solution.}








	%\textcolor{blue}{Choosing $\ellone = O(1/\epsilon)$, the total cost of the tri-criteria solution is $Cost_f(S^t) + Cost_c(S^t) \leq %\frac{\ellone}{\ellone-1} Cost_f(O) + 4Cost_c(O) + O(1/\epsilon)\sum_{j \in \clientset}\C{j} \leq 
	%\max\{2,1/\epsilon\}Cost_f(O) + O(1+\epsilon) Cost_c(O) \leq O(1/\epsilon)Cost(O)$, where $Cost_f(.)$ and $Cost_c(.)$ denote the facility opening cost and connection cost respectively of the particular solution.}

\textcolor{magenta}{Summing the cost bound of Lemma (\ref{Sparse}) over all sparse clusters and that of Lemma (\ref{Dense}) over all dense clusters, the total cost of the tri-criteria solution is:}

%Sapna...TBD: 
%$2\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} [\dist{i}{j} + \ellone \C{j}] +  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+ (1/\epsilon))  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} + 2\ellone(1+1/\epsilon) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} $

%Start from here....

$\leq max\{2,1/\epsilon\} \sum_{j' \in \clientset'} \sum_{i \in \bundle{j'}} f_i y^*_i +  max\{4,(2+1/\epsilon)\} \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + \ellone~ max\{4,2(1+1/\epsilon)\} \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \C{j}$

$= (1/\epsilon) \sum_{j' \in \clientset'} \sum_{i \in \bundle{j'}} f_i y^*_i +  (2+1/\epsilon) \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + 2\ellone(1+1/\epsilon) \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\epsilon \leq 1/2$)



%$= max\{2,1/\epsilon\} \sum_{j' \in \clientset'} \sum_{i \in \bundle{j'}} f_i y^*_i +  max\{4,1/\epsilon\} \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + (4+2/\epsilon) \ellone \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \C{j}$

%$=  max\{2,1/\epsilon\} \sum_{j' \in \clientset'} \sum_{i \in \bundle{j'}} f_i y^*_i +  max\{4,1/\epsilon\} \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + (4+2/\epsilon) \ellone \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \C{j}$

Choose $\ellone = floor(1/\epsilon)$ ..sapna use appropriate macro for floor, then the cost of the solution is bounded by $(2\ellone^2 + 3\ellone + 2)LP_{opt}$. For $\epsilon \le 1/2, \ellone \ge 2$. For $\epsilon = 1/2$, the capacity violation is $3/2$ and the approximation ratio is $16$. The capacity violation can be made arbitrarily small at the cost of increase in the approximation ratio.

To obtain integral assignments, we solve a minimum-cost integer flow problem with relaxed lower bounds and increased capacities. Let $S^t$ be the solution so obtained and violations in lower and upper bounds be $\alpha$ and $\beta$ respectively. \textcolor{blue}{Then, $Cost(S^t) \le  (2\ellone^2 + 3\ellone + 2) Cost(O)$, $\alpha = (\ellone-1)/\ellone$ and $\beta= (1+\epsilon)$ where $\ellone = floor(1/\epsilon) \ge 2$ for $\epsilon \leq 1/2$ and $\alpha \ge 1/2$.}
%	\textcolor{red}{	For $\ellone \ge 2, \alpha \ge 1/2$. 	}

	%\textcolor{blue}{	For $\ellone > 2, \alpha \ge 2/3$. 	}
	
		\textcolor{red}{
	Next, using $S^t$, we transform the instance $I$ to an instance $I_{cap}$ of capacitated facility location problem by swapping the roles of clients and facilities. This is done via a series of transformations from instance $I$ to $I_1$, 	$I_1$ to $I_2$ and $I_2$ to $I_{cap}$. The key idea is to create  $B - n_i$ units of demand, where the number $n_i$ of clients served by facility $i$ in $S^t$ is short of the lower bound and create  $n_i - B$ units of supply at locations where $n_i > B$.
	}
	


==> NEW Journal version WADS 2021 (LBUBFL)/TriCriteria_L.tex <==
\section{Computing the Tri-criteria Solution}
\label{tri-criteria}
 %We use a simpler LP-rounding technique to get $(\frac{\ellone-1}{\ellone})$-factor violation in lower bounds and $2$-factor violation in upper bounds at constant factor loss in cost. The technique used is much simpler than Friggstad et al. \cite{friggstad_et_al_LBUFL} because lower bounds are uniform in our case unlike Friggstad et al. that considers non-uniform lower bounds. 

 In this section, we give a tri-criteria solution that violates the lower bound by a factor of  \textcolor{yellow}{$\alpha = 1-1/\ell$}  \textcolor{cyan}{$\alpha > 1/2$} and the upper bound by a factor of  \textcolor{yellow}{$\beta = 1+1/\ell$} \textcolor{cyan}{$\beta = 3/2$.} \textcolor{yellow}{ where $\ell > 2$ is a tune-able parameter.} In particular, we present the following result:
 
 

 \begin{theorem} \label{TricriteriaResult}
 A ($\textcolor{yellow}{(2\ell^2 + 3\ell +2), 1-1/\ell, 1+1/\ell}$) $\textcolor{cyan}{(O(1),1/2, 3/2)}$ -
 approximate solution can be obtained for LBUBFL in polynomial time. \textcolor{yellow}{, where $\ell > 2$ is a tuneable parameter.}
\end{theorem}
 
 
 Instance $I$ of LBUBFL can be formulated as the following integer program (IP):

\label{{unif-CFLP}}
$Minimize ~\mathcal{C}ostLBUBFL(x,y) = \sum_{j \in \clientset}\sum_{i \in \facilityset}\dist{i}{j}x_{ij} + \sum_{i \in \facilityset}f_iy_i $
\begin{eqnarray}
subject~ to &\sum_{i \in \facilityset}{} x_{ij} \geq 1 & \forall ~\singleclient \in \clientset \label{LPFLP_const1}\\ 
%&\sum_{j \in \clientset}{} x_{ij} \leq \capacityU ~ y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const2}\\ 
& \capacityU y_i \geq \sum_{j \in \clientset}{} x_{ij} \geq \B y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const3}\\
& x_{ij} \leq y_i & \forall~ \singlefacility \in \facilityset , ~\singleclient \in \clientset \label{LPFLP_const4}\\   
& y_i,x_{ij} \in \left\lbrace 0,1 \right\rbrace  \label{LPFLP_const5}
\end{eqnarray}
where  $y_i$ is an indicator variable which is equal to $1$ if facility $i$ is open and is $0$ otherwise. $x_{ij}$ is an indicator variable which is equal to $1$ if client $j$ is served by facility $i$ and is $0$ otherwise.
 Constraints \ref{LPFLP_const1} ensure that all the clients are served. %Constraints \ref{LPFLP_const2} make sure that the total demand assigned to an open facility is no more than its capacity \capacityU. 
 Constraints \ref{LPFLP_const3} make sure that the total demand assigned to an open facility is at least $\B$ and at most $\capacityU$. Constraints \ref{LPFLP_const4} ensure that a client is assigned to a facility only if it is opened. LP-Relaxation  is obtained by allowing the variables to be non-integral.
% $ y_i, x_{ij} \in [0, 1]$. %Call it LP. 
Let $\zeta^{*} = <x^*, y^*>$ be an optimal solution  and $\opt{}$ be its cost.


We start by sparsifying the problem instance by removing some clients.
For $j \in \clientset$, let $ \C{j} $ denote the average connection cost paid by $\singleclient$ in $\zeta^*$. 
%i.e., ~$\C{j} = (\sum_{i \in \facilityset}{} {x}^*_{ij} \dist{i}{j})/({\sum_{i \in \facilityset}{} {x}^*_{ij}})$. 
Further, let \textcolor{yellow}{$\ell > 2$ be a tuneable parameter,} $\ballofj{j}$ be the ball of facilities within a radius of \textcolor{yellow}{ $\ellone\C{j}$ } \textcolor{cyan}{$2\C{j}$} of $j$ and $\cardTwo{\ballofj{j}}$
be the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
Then,  \textcolor{olive}{\textcolor{yellow}{$\cardTwo{\ballofj{j}} \ge (1-\frac{1}{\ellone}) > 1/2$.}} \textcolor{cyan}{$\cardTwo{\ballofj{j}} \ge 1/2$.}
%where $\cardTwo{\ballofj{j}}$
%$=  \sum_{i \in \ballofj{j}} y^*_i$ denotes the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
The clients are processed in the non-decreasing order of the radii of their balls, removing the close-by clients with balls of larger radii and dissolving their balls: let $\bar{\clientset} = \clientset$ and $\clientset'$ denote the sparsified set of  clients. Initially $\clientset' = \phi$.
Let $j'$ be a client in $\bar{\clientset}$ with a ball of the smallest radius (breaking the ties arbitrarily). Remove $j'$ from $\bar{\clientset}$ and add it to $\clientset'$. For all $j (\ne j') \in \bar{\clientset}$ with $\dist{j'}{ j} \leq 2\ell \C{j}$, remove $j$ from $\bar{\clientset}$. Repeat the process until $\bar{\clientset} = \phi$. 
Cluster of facilities are formed around the clients in $\clientset'$ by assigning a facility to the cluster of $j' \in \clientset'$ if and only if $j'$ is nearest to the facility amongst all $j' \in \clientset'$, i.e. if $\bundle{j'}$ denotes the cluster centered at $j'$ then, $i$ belongs to $\bundle{j'}$ if and only if $\dist{i}{j'} < \dist{i}{k'}$ for all $k' \textcolor{cyan}{(\ne j')} \in \clientset'$ (assuming that the distances are distinct).
The clients in $C'$ are then called the cluster centers.



\begin{observation}
Any two cluster centers $j', k'$ in $C'$ satisfy the  separation property:
$\dist{j'}{k'} > \textcolor{yellow}{ 2\ellone}  \textcolor{cyan}{4}~max\{ \C{j'},\C{k'}\}$.
\end{observation}


\begin{lemma} \label{distBound}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. Then,
\begin{enumerate}
    \item \label{claim-1}  $\dist{i}{j'}  \leq \dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$
    \item  \label{claim-2} $\dist{j}{j'} \leq 2\dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$
    \item \label{claim-3}  If $\dist{j}{j'} \leq \textcolor{yellow}{ \ellone}\textcolor{cyan}{2} \C{j'}$, then $\C{j'} \le 2\C{j}$
\end{enumerate}
\end{lemma}

\begin{proof}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. 
\begin{enumerate}

    \item Note that, $\dist{j}{k'} \leq \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$ for some $k' \in \clientset'$. Then we have  $\dist{i}{j'} \leq \dist{i}{k'} \leq \dist{i}{j} + \dist{j}{k'} \leq \dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$, where the first inequality follows because $i$ belongs to $\bundle{j'}$ and not $\bundle{k'}$ whenever $k' \ne j'$.  \textcolor{blue}{See Fig: (\ref{Cjj'}).}
    
    
    \item Using triangle inequality, we have   $\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$.
    
     \item Let $j \ne j'$. Note that $\dist{j}{j'} \leq \textcolor{yellow}{ \ellone} \textcolor{cyan}{2} \C{j'}$ $\Rightarrow j \notin \clientset'$. 
     %Further, using contradiction, let's assume 
     Suppose if possible, $\C{j'} > 2\C{j}$. Since $j \notin \cliset', \exists$ some $k'\in \clientset':\dist{j}{k'} \le \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$. Then, $\dist{k'}{j'} \le \dist{k'}{j} + \dist{j}{j'}$  $ \leq \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j} + \textcolor{yellow}{ \ellone} \textcolor{cyan}{2} \C{j'} < \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j'}$. Thus, we arrive at a contradiction to the separation property. Hence, $\C{j'} \le 2\C{j}$.

\end{enumerate} \end{proof}
 

\begin{figure} 
    \centering
    \includegraphics[width=10cm]{Figures/Cjj'.jpg}
    \caption{$\dist{i}{j'}  \leq \dist{i}{j} + 2\ellone \C{j}$}
    \label{Cjj'}
\end{figure}

%$\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$ ~\cite{GroverGKP18}.}  

For $j' \in \clientset', j \in \clientset$, let $\loadjinc{j}{j'}$ be the extent up to which $j$ is served by the facilities in the cluster of $j'$  \textcolor{olive}{under solution $\zeta^*$} and $d_{j'}= \sum_{j \in \clientset} \loadjinc{j}{j'}$.
We call a cluster to be $sparse$ if $d_{j'} \le  \capacityU$ and $dense$ otherwise. Let $\csparse$ and $\cdense$ be the set of cluster centers of sparse  and dense clusters respectively.


%Let $<\hat{x}, \hat{y}>$ be the solution so obtained, i.e., for $ j \in \clientset$, $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$. For $j' \in \crich, i \in \bundle{j'}, j \in \clientset$, $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. 


\begin{lemma} \label{Sparse}
We can obtain a solution $<\hat{x}, \hat{y}>$ such that  exactly one facility $i(j')$ is opened integrally in each sparse cluster centered at $j' \in \clientset'$. The solution violates the lower bound by a factor of \textcolor{yellow}{$(1 - 1/\ellone)$} \textcolor{cyan}{1/2} \textcolor{olive}{such that $\sum_{j' \in \clientset'}\sum_{i \in \bundle{j'}} [f_i \hat{y}_i + \sum_{j \in \clientset}  \hat{x}_{ij} \dist{i}{j}] \leq $}
$\sum_{j' \in \csparse}[\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \textcolor{yellow}{\ellone } \textcolor{cyan}{2}\C{j})] + \sum_{j' \in \cdense} [\sum_{i \in \bundle{j'}} f_i y^*_i + \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$.

%\textcolor{red}{May be we should write the following:$\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \le \sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})]$...will resolve after completing this section}

\end{lemma}

\begin{proof}
%In a sparse cluster centered at $j'$, we open the cheapest facility, say $i(j')$, in $\ballofj{j'}$ and transfer all the assignments in the cluster onto it.
%As specified above, 
For $ j' \in \cdense, i \in \bundle{j'}, j \in \clientset$, set $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. Next,
let $j' \in \csparse$
%$\bundle{j'}$ be a sparse cluster centered at $j'$ 
and $i(j')$ be a cheapest \textcolor{olive}{(lowest facility opening cost)} facility in $\ballofj{j'}$. We open $i(j')$ and transfer all the assignments in the cluster onto it (see Figure (\ref{sparse})). 
%Let $ j \in \clientset$.
i.e. set $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$ and $j \in \clientset$. 
Since $\cardTwo{\ballofj{j'}} \ge \textcolor{yellow}{(1-\frac{1}{\ellone})} \textcolor{cyan}{1/2}$ we have $\sum_{j \in \clientset}{} \hat{x}_{i(j')j} = \demandofj{j'} \ge \textcolor{yellow}{(1-\frac{1}{\ellone})} \textcolor{cyan}{1/2}\B$. Thus, the lower bound is violated at most by $\textcolor{yellow}{(1-\frac{1}{\ellone})} \textcolor{cyan}{1/2}$
and the facility cost is bounded by $\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i y^*_i$.

To bound the service cost, we will show that for $j' \in \csparse, \sum_{j \in \clientset} \loadjinc{j}{j'} \dist{i(j')}{j}  \leq 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})$: 
since $i(j') \in \ballofj{j'}$, we have $\dist{i(j')}{j'} \le  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j'}$. 
Thus, for $j \in \clientset$,
we have $\dist{i(j')}{j} \le \dist{j'}{j} + \dist{i(j')}{j'} \le  \dist{j'}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j'}$. If $ \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j'} \le \dist{j'}{j}$ then $\dist{i(j')}{j}  \le 2  \dist{j'}{j}  \leq 4 (\dist{i}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})$ ($\forall~i \in \bundle{j'}$ by claim (\ref{claim-2}) of Lemma (\ref{distBound})), 
 else $\dist{i(j')}{j}  \leq  \textcolor{yellow}{2\ellone} \textcolor{cyan}{4} \C{j'} \leq  \textcolor{yellow}{4 \ellone} \textcolor{cyan}{8} \C{j}$, where the second inequality in the else part follows by claim (\ref{claim-3}) of Lemma (\ref{distBound}).
Thus, in either case $\dist{i(j')}{j} \leq 4 (\dist{i}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})$ for all $i \in \bundle{j'}$.
Substituting $\phi(j, j') = \sum_{i \in \bundle{j'}} x^*_{ij}$ and summing over all $j \in \clientset$ 
%$j' \in \csparse$ 
we get the desired bound.
Thus, $\sum_{i \in \facilityset} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  \hat{x}_{ij}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \demandofj{j'}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
\le \sum_{j' \in \csparse}[\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})] + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} [ f_i y^*_i + \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$
\end{proof}
 
%$\le 4\dist{i}{j} + 4 \ellone \C{j} $ else $\dist{i(j')}{j}  \le  2 \ellone \C{j'} \le 4 \ellone \C{j} \le 4\dist{i}{j} + 4 \ellone \C{j}$, where the second inequality in the else part follows because if $\ellone \C{j'} > \dist{j'}{j}$ then $\C{j'} \leq 2\C{j}$ \cite{GroverGKP18}. Also, since the total opening in each cluster is at least $(1-(1/\ellone))$, a loss of factor $\ellone/(\ellone-1) (\leq 2$ for $\ellone > 2$) in the facility opening cost is incurred, violation in lower bound is at most $(1-(1/\ellone))$ and  since  $d_{j'} \le \capacityU$ there is no  violation in the capacity.}
   
    \begin{figure} 
    \centering
    \includegraphics[width=10cm]{Figures/sparse.jpg}
    \caption{(A) Cluster $\bundle{j'}$ centered at $j'$. (B) Demand $\demandofj{j'}$ being assigned to facility $i(j') \in \ballofj{j'}$.}
    \label{sparse}
\end{figure}
 

    
%Next, we consider the dense clusters.
To open the facilities integrally in the dense clusters, we solve the following LP for every dense cluster $\bundle{j'}$.
%centered at $j'$.

($LP_1$): 
\label{dense}
$Minimize ~\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$
\begin{eqnarray}
subject~ to &\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'} \label{denseLP_const1}\\ 
&0 \leq \zofi{i} \leq 1 \label{denseLP_const2}
\end{eqnarray}
   
  % $Minimize $\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$ s.t. $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$ and $\zofi{i} \in [0,1]$. 
   
   
Note that for $\zofi{i} = \sum_{j \in \clientset}x_{ij}^*/\capacityU$, we have $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} = \demandofj{j'}$ and $\zofi{i} \le y^*_i$. Thus, $\zofi{}$
is a feasible solution with cost at most $ \sum_{i \in \bundle{j'}} [\facilitycost y^*_i + \sum_{ j \in \clientset} x^*_{ij} ( \dist{i}{j} +   \textcolor{yellow}{2\ellone} \textcolor{cyan}{4} \C{j}) ]$ by claim (\ref{claim-1}) of Lemma (\ref{distBound}).

%\textcolor{blue}{TBD: facility opening cost at most $ \sum_{i \in \bundle{j'}} \facilitycost y^*_i$ and service cost $\sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij}  \dist{i}{j'} \le \sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij} [ \dist{i}{ j} + 2\ellone \C{j} ]$. } 

\begin{lemma} \label{integral_dense}
Given the feasible solution $z$ to $LP_1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) by a factor of \textcolor{yellow}{$(1+1/\ell)$} \textcolor{cyan}{3/2}, can be obtained at a loss of factor $\textcolor{yellow}{\ellone} \textcolor{cyan}{2}$ in cost
i.e. $ \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \hat{z}_{i} \le  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$.
%For a fixed $0 < \epsilon < 1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) by a factor of $(1+\epsilon)$, can be obtained at a loss of $(1/\epsilon)$ in cost.
\end{lemma}

\begin{proof}
\textcolor{green}{
We say that a solution to $LP_1$ is almost integral if it has at most one fractionally opened facility in $\bundle{j'}$.
}
We first obtain an almost integral solution
%\footnote{A solution is said to be an almost integral solution if it has at most one fractionally opened facility.}
$\primezofi{}$ by arranging the facilities opened in $z$, in non-decreasing order of $\facilitycost  + \dist{i}{j'} \capacityU$ and greedily transferring the openings $z$ onto them. 
Then,  $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} = \demandofj{j'}$. %Consider constraint (\ref{denseLP_const1}), $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$.
Note that the cost of solution $\primezofi{}$ is no more than that of solution $z$.


We now convert the almost integral solution $\primezofi{}$ to an integral solution $\hat{z}$. Let $\hat{z} = \primezofi{}$ initially. Let $i'$ be the fractionally opened facility, if any, in $\bundle{j'}$. %Initially, set $\hat{z}_i = \primezofi{i}~ \forall i \in \bundle{j'}$. 
Consider the following cases:


\begin{enumerate}
    %\item $\primezofi{i'} < \epsilon$:
    \item $\primezofi{i'} < \textcolor{yellow}{1/\ell} \textcolor{cyan}{1/2}$: close $i'$ in $\hat{z}$. There must be at least one integrally opened facility, say $i (\ne i') \in \bundle{j'}$ in $\primezofi{}$, as $\demandofj{j'} \ge \capacityU$. Then, $\demandofj{j'} = \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k} + \capacityU  (\primezofi{i} + \primezofi{i'}) \le \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k}  + \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU  \primezofi{i} \le \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU \sum_{k \in \bundle{j'} \setminus \{i'\}} \primezofi{k} = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}  \capacityU \sum_{k \in \bundle{j'}} \hat{z}_k$. There is no increase in cost as we have only (possibly) shut down one of the facilities .
    

    \item $\primezofi{i'} \geq \textcolor{yellow}{1/\ell} \textcolor{cyan}{1/2} $: Open $i'$ integrally at a loss of factor $\textcolor{yellow}{\ell}$ \textcolor{cyan}{2} in facility opening cost i.e., $\sum_{i \in \bundle{j'}} f_i \hat{z}_i \le \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i \primezofi{i}$. 
    \textcolor{cyan}{Also, note that $\capacityU \hat{z}_i \geq 1/2 \B \primezofi{i'}$ ------ CHECK AGAIN.} 
\end{enumerate}\end{proof}

%Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{(1+1/\ell)\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = (1 + 1/\ell) \capacityU \hat{z}_i$ , where the first inequality follows by Lemma (\ref{integral_dense}). 


%\textcolor{cyan}{SAPNA, Revisit the next para later:}

Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{\textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU \hat{z}_i$ , where the first inequality follows by Lemma (\ref{integral_dense}). \textcolor{cyan}{Also, $l_i \geq 1/2 B \hat{z}_i$. -- CHECK AGAIN AND WRITE PROPERLY }


\textcolor{olive}{A solution is said to be an integrally opened solution if all facilities in it are either opened to an extent of $1$ or $0$. We next obtain such a solution to LBUBFL problem.}


\begin{lemma} \label{Dense1}
We can obtain an integrally opened solution $<\bar x, \bar y>$ to LBUBFL problem at a loss of $\textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}$ in upper bounds and $\textcolor{yellow}{(1-1/\ell)} \textcolor{cyan}{(1/2)}$ in lower bounds whose cost is bounded by $\textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)} \textcolor{cyan}{O(1)LP_{opt}}$.
\end{lemma}
\begin{proof}
For $j' \in \csparse$, set $\bar y_i = \hat{y}_i,~\bar{x}_{ij} = \hat{x}_{ij}~\forall i \in \bundle{j'}, j \in \clientset$. \textcolor{yellow}{The violation in lower bound then follows from Lemma (\ref{Sparse})
and, }

\begin{equation}
\label{cost-of-sparse}
\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \bar{y}_i + \sum_{j \in \clientset} \bar{x}_{ij} \dist{i}{j}) \le \sum_{j' \in \csparse}[\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})].
\end{equation}

Next let $j' \in \cdense,~i \in \bundle{j'}, j \in \clientset$. Set $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. 
Consider $ \sum_{j \in \clientset} \bar{x}_{ij} = \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} = l_i \leq   \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \hat{z}_i = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \bar{y}_i$. Thus, the loss in capacities is at most   \textcolor{yellow}{(1+1/\ell)}\textcolor{cyan}{(3/2)}.

\textcolor{cyan}{From Lemma (\ref{Sparse}), the violation in lower bound is $1/2$. Thus, the final violation in lower bound is $ min\{1/2, (1-1/\ell)\} > 1/2$ for $\ell >2$, which implies $\alpha = 1/2$. ---SAPNA,  REVISIT}

Also,\\ 
$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij}) $\\
$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \dist{i}{j}  \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} (\dist{j}{j'} + \dist{i}{j'})$ (by triangle inequality)\\ 
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   
%\sum_{\singlefacility \in \bundle{j'}} 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ (as $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
%$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )  $ (by definition of $\loadjinc{j}{j'}$, claim (\ref{claim-2}) of Lemma (\ref{distBound}) and the fact that $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
$ \leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +    \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{3/2} \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +  
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ (by Lemma (\ref{integral_dense}))\\
%$ \leq  \ell \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +   (1+1/\ell) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
\textcolor{yellow}{$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\}
%$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\ \textcolor{yellow}{(for $\ell > 2$)}\\
%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\ (for $\ell > 2$)\\
$\leq \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (by Lemma (\ref{integral_dense}))\\
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (because $z_i = \sum_{j \in \clientset} x^*_{ij} / \capacityU \leq y^*_i$)\\ 
%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by cost bound of feasible solution $z$.....Sapna..how from this reason?)\\
%\textcolor{red}{
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ellone \C{j}) + \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$  (by claim (\ref{claim-1}) of Lemma (\ref{distBound}))\\
%}
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} +  \textcolor{yellow}{2\ell} \textcolor{cyan}{4} \C{j}) + \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}  (2\dist{i}{j} +  \textcolor{yellow}{2\ell} \textcolor{cyan}{4} \C{j} )$ 
(by definition of $\loadjinc{j}{j'}$ and claims (\ref{claim-1}) and (\ref{claim-2}) of Lemma (\ref{distBound}))\\
$= \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   \textcolor{yellow}{2+\ell} \textcolor{cyan}{4}   \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} +   \textcolor{yellow}{2\ell(1+\ell)} \textcolor{cyan}{12} \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}   \C{j} $ \\

Summing over all $j' \in \cdense$ and adding inequality (\ref{cost-of-sparse}), we get\\
$ \sum_{i \in \facilityset} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij})$\\
$\leq \textcolor{yellow}{max\{\ell, \ell/(\ell-1)\}} \textcolor{cyan}{2} \sum_{i \in \facilityset}  f_i y^*_i + \textcolor{yellow}{ max\{4,(2+\ell)\}} \textcolor{cyan}{4} \sum_{i \in \facilityset}\sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + \textcolor{yellow}{\ellone~ max\{4,2(1+\ell)\}} \textcolor{cyan}{12} \sum_{i \in \facilityset}\sum_{j \in \clientset} x^*_{ij} \C{j}$\\
 \textcolor{yellow}{ $= \sum_{i \in \facilityset}  f_i y^*_i + (2+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + 2\ell(1+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\ell > 2$)}\\
$ \leq \textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)} \textcolor{cyan}{16}LP_{opt}$.
\end{proof}


Theorem~\ref{TricriteriaResult} is obtained by solving a min-cost flow problem with relaxed lower  and upper bounds to obtain the integral assignments.
Let $S^t$ be the solution so obtained. %and violations in lower and upper bounds be denoted by $\alpha$ and $\beta$ respectively.
Then, $Cost_I(S^t) \le \textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)}\textcolor{cyan}{16} Cost_I(O)$,
where $O$ is an optimal solution to $I$, $\textcolor{yellow}{\alpha= (1 - 1/\ellone)} \textcolor{cyan}{\alpha >
1/2}$ and $\textcolor{yellow}{\beta= (1 + 1/\ellone)} \textcolor{cyan}{\beta= 3/2}$.
\textcolor{yellow}{ For $\ell = 2.01$, $\alpha > 1/2$, $\beta < 3/2$ and the approximation ratio is less than $17$. The violations in the lower and the upper bounds can be made arbitrarily close to $0$ at the cost of increase in the approximation ratio.}

%To obtain integral assignments, we solve a minimum-cost integer flow problem with relaxed lower  and upper bounds.



	Next, using $S^t$, we transform the instance $I$ to an instance $I_{cap}$ of capacitated facility location problem by swapping the roles of clients and facilities. This is done via a series of transformations from instance $I$ to $I_1$, 	$I_1$ to $I_2$ and $I_2$ to $I_{cap}$. The key idea is to create  $\B - n_i$ units of demand, where the number $n_i$ of clients served by facility $i$ in $S^t$ is short of the lower bound and create  $n_i - \B$ units of supply at locations where $n_i > \B$.
	
	


==> NEW Journal version WADS 2021 (LBUBFL)/TriCriteria_l=2.tex <==
\section{Computing the Tri-criteria Solution}
\label{tri-criteria}
 %We use a simpler LP-rounding technique to get $(\frac{\ellone-1}{\ellone})$-factor violation in lower bounds and $2$-factor violation in upper bounds at constant factor loss in cost. The technique used is much simpler than Friggstad et al. \cite{friggstad_et_al_LBUFL} because lower bounds are uniform in our case unlike Friggstad et al. that considers non-uniform lower bounds. 

 In this section, we give a tri-criteria solution that violates the lower bound by a factor of  \textcolor{yellow}{$\alpha = 1-1/\ell$}  \textcolor{cyan}{$\alpha > 1/2$} and the upper bound by a factor of  \textcolor{yellow}{$\beta = 1+1/\ell$} \textcolor{cyan}{$\beta = 3/2$.} \textcolor{yellow}{ where $\ell > 2$ is a tune-able parameter.} In particular, we present the following result:
 
 

 \begin{theorem} \label{TricriteriaResult}
 A ($\textcolor{yellow}{(2\ell^2 + 3\ell +2), 1-1/\ell, 1+1/\ell}$) $\textcolor{cyan}{(O(1),1/2, 3/2)}$ -
 approximate solution can be obtained for LBUBFL in polynomial time. \textcolor{yellow}{, where $\ell > 2$ is a tuneable parameter.}
\end{theorem}
 
 
 Instance $I$ of LBUBFL can be formulated as the following integer program (IP):

\label{{unif-CFLP}}
$Minimize ~\mathcal{C}ostLBUBFL(x,y) = \sum_{j \in \clientset}\sum_{i \in \facilityset}\dist{i}{j}x_{ij} + \sum_{i \in \facilityset}f_iy_i $
\begin{eqnarray}
subject~ to &\sum_{i \in \facilityset}{} x_{ij} \geq 1 & \forall ~\singleclient \in \clientset \label{LPFLP_const1}\\ 
%&\sum_{j \in \clientset}{} x_{ij} \leq \capacityU ~ y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const2}\\ 
& \capacityU y_i \geq \sum_{j \in \clientset}{} x_{ij} \geq \B y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const3}\\
& x_{ij} \leq y_i & \forall~ \singlefacility \in \facilityset , ~\singleclient \in \clientset \label{LPFLP_const4}\\   
& y_i,x_{ij} \in \left\lbrace 0,1 \right\rbrace  \label{LPFLP_const5}
\end{eqnarray}
where  $y_i$ is an indicator variable which is equal to $1$ if facility $i$ is open and is $0$ otherwise. $x_{ij}$ is an indicator variable which is equal to $1$ if client $j$ is served by facility $i$ and is $0$ otherwise.
 Constraints \ref{LPFLP_const1} ensure that all the clients are served. %Constraints \ref{LPFLP_const2} make sure that the total demand assigned to an open facility is no more than its capacity \capacityU. 
 Constraints \ref{LPFLP_const3} make sure that the total demand assigned to an open facility is at least $\B$ and at most $\capacityU$. Constraints \ref{LPFLP_const4} ensure that a client is assigned to a facility only if it is opened. LP-Relaxation  is obtained by allowing the variables to be non-integral.
% $ y_i, x_{ij} \in [0, 1]$. %Call it LP. 
Let $\zeta^{*} = <x^*, y^*>$ be an optimal solution  and $\opt{}$ be its cost.


We start by sparsifying the problem instance by removing some clients.
For $j \in \clientset$, let $ \C{j} $ denote the average connection cost paid by $\singleclient$ in $\zeta^*$. 
%i.e., ~$\C{j} = (\sum_{i \in \facilityset}{} {x}^*_{ij} \dist{i}{j})/({\sum_{i \in \facilityset}{} {x}^*_{ij}})$. 
Further, let \textcolor{yellow}{$\ell > 2$ be a tuneable parameter,} $\ballofj{j}$ be the ball of facilities within a radius of \textcolor{yellow}{ $\ellone\C{j}$ } \textcolor{cyan}{$2\C{j}$} of $j$ and $\cardTwo{\ballofj{j}}$
be the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
Then,  \textcolor{olive}{\textcolor{yellow}{$\cardTwo{\ballofj{j}} \ge (1-\frac{1}{\ellone}) > 1/2$.}} \textcolor{cyan}{$\cardTwo{\ballofj{j}} \ge 1/2$.}
%where $\cardTwo{\ballofj{j}}$
%$=  \sum_{i \in \ballofj{j}} y^*_i$ denotes the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
The clients are processed in the non-decreasing order of the radii of their balls, removing the close-by clients with balls of larger radii and dissolving their balls: let $\bar{\clientset} = \clientset$ and $\clientset'$ denote the sparsified set of  clients. Initially $\clientset' = \phi$.
Let $j'$ be a client in $\bar{\clientset}$ with a ball of the smallest radius (breaking the ties arbitrarily). Remove $j'$ from $\bar{\clientset}$ and add it to $\clientset'$. For all $j (\ne j') \in \bar{\clientset}$ with $\dist{j'}{ j} \leq 2\ell \C{j}$, remove $j$ from $\bar{\clientset}$. Repeat the process until $\bar{\clientset} = \phi$. 
Cluster of facilities are formed around the clients in $\clientset'$ by assigning a facility to the cluster of $j' \in \clientset'$ if and only if $j'$ is nearest to the facility amongst all $j' \in \clientset'$, i.e. if $\bundle{j'}$ denotes the cluster centered at $j'$ then, $i$ belongs to $\bundle{j'}$ if and only if $\dist{i}{j'} < \dist{i}{k'}$ for all $k' \textcolor{cyan}{(\ne j')} \in \clientset'$ (assuming that the distances are distinct).
The clients in $C'$ are then called the cluster centers.



\begin{observation}
Any two cluster centers $j', k'$ in $C'$ satisfy the  separation property:
$\dist{j'}{k'} > \textcolor{yellow}{ 2\ellone}  \textcolor{cyan}{4}~max\{ \C{j'},\C{k'}\}$.
\end{observation}


\begin{lemma} \label{distBound}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. Then,
\begin{enumerate}
    \item \label{claim-1}  $\dist{i}{j'}  \leq \dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$
    \item  \label{claim-2} $\dist{j}{j'} \leq 2\dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$
    \item \label{claim-3}  If $\dist{j}{j'} \leq \textcolor{yellow}{ \ellone}\textcolor{cyan}{2} \C{j'}$, then $\C{j'} \le 2\C{j}$
\end{enumerate}
\end{lemma}

\begin{proof}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. 
\begin{enumerate}

    \item Note that, $\dist{j}{k'} \leq \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$ for some $k' \in \clientset'$. Then we have  $\dist{i}{j'} \leq \dist{i}{k'} \leq \dist{i}{j} + \dist{j}{k'} \leq \dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$, where the first inequality follows because $i$ belongs to $\bundle{j'}$ and not $\bundle{k'}$ whenever $k' \ne j'$.  \textcolor{blue}{See Fig: (\ref{Cjj'}).}
    
    
    \item Using triangle inequality, we have   $\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$.
    
     \item Let $j \ne j'$. Note that $\dist{j}{j'} \leq \textcolor{yellow}{ \ellone} \textcolor{cyan}{2} \C{j'}$ $\Rightarrow j \notin \clientset'$. 
     %Further, using contradiction, let's assume 
     Suppose if possible, $\C{j'} > 2\C{j}$. Since $j \notin \cliset', \exists$ some $k'\in \clientset':\dist{j}{k'} \le \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$. Then, $\dist{k'}{j'} \le \dist{k'}{j} + \dist{j}{j'}$  $ \leq \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j} + \textcolor{yellow}{ \ellone} \textcolor{cyan}{2} \C{j'} < \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j'}$. Thus, we arrive at a contradiction to the separation property. Hence, $\C{j'} \le 2\C{j}$.

\end{enumerate} \end{proof}
 

\begin{figure} 
    \centering
    \includegraphics[width=10cm]{Figures/Cjj'.jpg}
    \caption{$\dist{i}{j'}  \leq \dist{i}{j} + 2\ellone \C{j}$}
    \label{Cjj'}
\end{figure}

%$\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$ ~\cite{GroverGKP18}.}  

For $j' \in \clientset', j \in \clientset$, let $\loadjinc{j}{j'}$ be the extent up to which $j$ is served by the facilities in the cluster of $j'$  \textcolor{olive}{under solution $\zeta^*$} and $d_{j'}= \sum_{j \in \clientset} \loadjinc{j}{j'}$.
We call a cluster to be $sparse$ if $d_{j'} \le  \capacityU$ and $dense$ otherwise. Let $\csparse$ and $\cdense$ be the set of cluster centers of sparse  and dense clusters respectively.


%Let $<\hat{x}, \hat{y}>$ be the solution so obtained, i.e., for $ j \in \clientset$, $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$. For $j' \in \crich, i \in \bundle{j'}, j \in \clientset$, $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. 


\begin{lemma} \label{Sparse}
We can obtain a solution $<\hat{x}, \hat{y}>$ such that  exactly one facility $i(j')$ is opened integrally in each sparse cluster centered at $j' \in \clientset'$. The solution violates the lower bound by a factor of \textcolor{yellow}{$(1 - 1/\ellone)$} \textcolor{cyan}{1/2} \textcolor{olive}{such that $\sum_{j' \in \clientset'}\sum_{i \in \bundle{j'}} [f_i \hat{y}_i + \sum_{j \in \clientset}  \hat{x}_{ij} \dist{i}{j}] \leq $}
$\sum_{j' \in \csparse}[\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \textcolor{yellow}{\ellone } \textcolor{cyan}{2}\C{j})] + \sum_{j' \in \cdense} [\sum_{i \in \bundle{j'}} f_i y^*_i + \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$.

%\textcolor{red}{May be we should write the following:$\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \le \sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})]$...will resolve after completing this section}

\end{lemma}

\begin{proof}
%In a sparse cluster centered at $j'$, we open the cheapest facility, say $i(j')$, in $\ballofj{j'}$ and transfer all the assignments in the cluster onto it.
%As specified above, 
For $ j' \in \cdense, i \in \bundle{j'}, j \in \clientset$, set $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. Next,
let $j' \in \csparse$
%$\bundle{j'}$ be a sparse cluster centered at $j'$ 
and $i(j')$ be a cheapest \textcolor{olive}{(lowest facility opening cost)} facility in $\ballofj{j'}$. We open $i(j')$ and transfer all the assignments in the cluster onto it (see Figure (\ref{sparse})). 
%Let $ j \in \clientset$.
i.e. set $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$ and $j \in \clientset$. 
Since $\cardTwo{\ballofj{j'}} \ge \textcolor{yellow}{(1-\frac{1}{\ellone})} \textcolor{cyan}{1/2}$ we have $\sum_{j \in \clientset}{} \hat{x}_{i(j')j} = \demandofj{j'} \ge \textcolor{yellow}{(1-\frac{1}{\ellone})} \textcolor{cyan}{1/2}\B$. Thus, the lower bound is violated at most by $\textcolor{yellow}{(1-\frac{1}{\ellone})} \textcolor{cyan}{1/2}$
and the facility cost is bounded by $\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i y^*_i$.

To bound the service cost, we will show that for $j' \in \csparse, \sum_{j \in \clientset} \loadjinc{j}{j'} \dist{i(j')}{j}  \leq 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})$: 
since $i(j') \in \ballofj{j'}$, we have $\dist{i(j')}{j'} \le  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j'}$. 
Thus, for $j \in \clientset$,
we have $\dist{i(j')}{j} \le \dist{j'}{j} + \dist{i(j')}{j'} \le  \dist{j'}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j'}$. If $ \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j'} \le \dist{j'}{j}$ then $\dist{i(j')}{j}  \le 2  \dist{j'}{j}  \leq 4 (\dist{i}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})$ ($\forall~i \in \bundle{j'}$ by claim (\ref{claim-2}) of Lemma (\ref{distBound})), 
 else $\dist{i(j')}{j}  \leq  \textcolor{yellow}{2\ellone} \textcolor{cyan}{4} \C{j'} \leq  \textcolor{yellow}{4 \ellone} \textcolor{cyan}{8} \C{j}$, where the second inequality in the else part follows by claim (\ref{claim-3}) of Lemma (\ref{distBound}).
Thus, in either case $\dist{i(j')}{j} \leq 4 (\dist{i}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})$ for all $i \in \bundle{j'}$.
Substituting $\phi(j, j') = \sum_{i \in \bundle{j'}} x^*_{ij}$ and summing over all $j \in \clientset$ 
%$j' \in \csparse$ 
we get the desired bound.
Thus, $\sum_{i \in \facilityset} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  \hat{x}_{ij}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \demandofj{j'}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
\le \sum_{j' \in \csparse}[\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})] + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} [ f_i y^*_i + \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$
\end{proof}
 
%$\le 4\dist{i}{j} + 4 \ellone \C{j} $ else $\dist{i(j')}{j}  \le  2 \ellone \C{j'} \le 4 \ellone \C{j} \le 4\dist{i}{j} + 4 \ellone \C{j}$, where the second inequality in the else part follows because if $\ellone \C{j'} > \dist{j'}{j}$ then $\C{j'} \leq 2\C{j}$ \cite{GroverGKP18}. Also, since the total opening in each cluster is at least $(1-(1/\ellone))$, a loss of factor $\ellone/(\ellone-1) (\leq 2$ for $\ellone > 2$) in the facility opening cost is incurred, violation in lower bound is at most $(1-(1/\ellone))$ and  since  $d_{j'} \le \capacityU$ there is no  violation in the capacity.}
   
    \begin{figure} 
    \centering
    \includegraphics[width=10cm]{Figures/sparse.jpg}
    \caption{(A) Cluster $\bundle{j'}$ centered at $j'$. (B) Demand $\demandofj{j'}$ being assigned to facility $i(j') \in \ballofj{j'}$.}
    \label{sparse}
\end{figure}
 

    
%Next, we consider the dense clusters.
To open the facilities integrally in the dense clusters, we solve the following LP for every dense cluster $\bundle{j'}$.
%centered at $j'$.

($LP_1$): 
\label{dense}
$Minimize ~\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$
\begin{eqnarray}
subject~ to &\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'} \label{denseLP_const1}\\
&\textcolor{cyan}{\B \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \leq \demandofj{j'} \label{denseLP_const1-1}}\\ 
&0 \leq \zofi{i} \leq 1 \label{denseLP_const2}
\end{eqnarray}
   
  % $Minimize $\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$ s.t. $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$ and $\zofi{i} \in [0,1]$. 
   
   
Note that for $\zofi{i} = \sum_{j \in \clientset}x_{ij}^*/\capacityU$, we have $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} = \demandofj{j'} \geq \textcolor{cyan}{\B \sum_{\singlefacility \in \bundle{j'}} \zofi{i}}$ and $\zofi{i} \le y^*_i$. Thus, $\zofi{}$
is a feasible solution with cost at most $ \sum_{i \in \bundle{j'}} [\facilitycost y^*_i + \sum_{ j \in \clientset} x^*_{ij} ( \dist{i}{j} +   \textcolor{yellow}{2\ellone} \textcolor{cyan}{4} \C{j}) ]$ by claim (\ref{claim-1}) of Lemma (\ref{distBound}).

%\textcolor{blue}{TBD: facility opening cost at most $ \sum_{i \in \bundle{j'}} \facilitycost y^*_i$ and service cost $\sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij}  \dist{i}{j'} \le \sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij} [ \dist{i}{ j} + 2\ellone \C{j} ]$. } 

\begin{lemma} \label{integral_dense}
Given the feasible solution $z$ to $LP_1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) \textcolor{cyan}{and (\ref{denseLP_const1-1})} by a factor of \textcolor{yellow}{$(1+1/\ell)$} \textcolor{cyan}{$3/2$ and $1/2$ respectively}, can be obtained at a loss of factor $\textcolor{yellow}{\ellone} \textcolor{cyan}{2}$ in cost
i.e. $ \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \hat{z}_{i} \le  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$.
%For a fixed $0 < \epsilon < 1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) by a factor of $(1+\epsilon)$, can be obtained at a loss of $(1/\epsilon)$ in cost.
\end{lemma}

\begin{proof}
\textcolor{green}{
We say that a solution to $LP_1$ is almost integral if it has at most one fractionally opened facility in $\bundle{j'}$.
}
We first obtain an almost integral solution
%\footnote{A solution is said to be an almost integral solution if it has at most one fractionally opened facility.}
$\primezofi{}$ by arranging the facilities opened in $z$, in non-decreasing order of $\facilitycost  + \dist{i}{j'} \capacityU$ and greedily transferring the openings $z$ onto them. 
Then,  $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} = \demandofj{j'}$. %Consider constraint (\ref{denseLP_const1}), $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$.
Note that the cost of solution $\primezofi{}$ is no more than that of solution $z$.


We now convert the almost integral solution $\primezofi{}$ to an integral solution $\hat{z}$. Let $\hat{z} = \primezofi{}$ initially. Let $i'$ be the fractionally opened facility, if any, in $\bundle{j'}$. %Initially, set $\hat{z}_i = \primezofi{i}~ \forall i \in \bundle{j'}$. 
Consider the following cases:


\begin{enumerate}
    %\item $\primezofi{i'} < \epsilon$:
    \item $\primezofi{i'} < \textcolor{yellow}{1/\ell} \textcolor{cyan}{1/2}$: close $i'$ in $\hat{z}$. There must be at least one integrally opened facility, say $i (\ne i') \in \bundle{j'}$ in $\primezofi{}$, as $\demandofj{j'} \ge \capacityU$. Then, $\demandofj{j'} = \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k} + \capacityU  (\primezofi{i} + \primezofi{i'}) \le \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k}  + \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU  \primezofi{i} \le \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU \sum_{k \in \bundle{j'} \setminus \{i'\}} \primezofi{k} = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}  \capacityU \sum_{k \in \bundle{j'}} \hat{z}_k$. There is no increase in cost as we have only (possibly) shut down one of the facilities .
    

    \item $\primezofi{i'} \geq \textcolor{yellow}{1/\ell} \textcolor{cyan}{1/2} $: Open $i'$ integrally at a loss of factor $\textcolor{yellow}{\ell}$ \textcolor{cyan}{2} in facility opening cost i.e., $\sum_{i \in \bundle{j'}} f_i \hat{z}_i \le \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i \primezofi{i}$. 
    %\textcolor{cyan}{Also, note that $\capacityU \hat{z}_i \geq 1/2 \B \primezofi{i'}$ ------ CHECK AGAIN.} 
\end{enumerate}\end{proof}

%Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{(1+1/\ell)\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = (1 + 1/\ell) \capacityU \hat{z}_i$ , where the first inequality follows by Lemma (\ref{integral_dense}). 


%\textcolor{cyan}{SAPNA, Revisit the next para later:}

Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{\textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU \hat{z}_i$ , where the first inequality follows by Lemma (\ref{integral_dense}). \textcolor{cyan}{Also, $l_i  = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \geq \hat{z}_i \frac{\demandofj{j'}}{2\sum_{i \in \bundle{j'}} z'_i} = \hat{z}_i \frac{\demandofj{j'}}{2\sum_{i \in \bundle{j'}} z_i} =  \hat{z}_i \frac{\B \sum_{i \in \bundle{j'}} z_i}{2\sum_{i \in \bundle{j'}} z_i} = 1/2 B \hat{z}_i$, where the first inequality follows because $\sum_{i \in \bundle{j'}} \hat{z}_i \leq 2\sum_{i \in \bundle{j'}} z'_i$.}


\textcolor{olive}{A solution is said to be an integrally opened solution if all facilities in it are either opened to an extent of $1$ or $0$. We next obtain such a solution to LBUBFL problem.}


\begin{lemma} \label{Dense1}
We can obtain an integrally opened solution $<\bar x, \bar y>$ to LBUBFL problem at a loss of $\textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}$ in upper bounds and $\textcolor{yellow}{(1-1/\ell)} \textcolor{cyan}{(1/2)}$ in lower bounds whose cost is bounded by $\textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)} \textcolor{cyan}{O(1)LP_{opt}}$.
\end{lemma}
\begin{proof}
For $j' \in \csparse$, set $\bar y_i = \hat{y}_i,~\bar{x}_{ij} = \hat{x}_{ij}~\forall i \in \bundle{j'}, j \in \clientset$. \textcolor{yellow}{The violation in lower bound then follows from Lemma (\ref{Sparse})
and, }

\begin{equation}
\label{cost-of-sparse}
\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \bar{y}_i + \sum_{j \in \clientset} \bar{x}_{ij} \dist{i}{j}) \le \sum_{j' \in \csparse}[\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})].
\end{equation}

Next let $j' \in \cdense,~i \in \bundle{j'}, j \in \clientset$. Set $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. 
Consider $ \sum_{j \in \clientset} \bar{x}_{ij} = \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} = l_i \leq   \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \hat{z}_i = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \bar{y}_i$. Thus, the loss in capacities is at most   \textcolor{yellow}{(1+1/\ell)}\textcolor{cyan}{(3/2)}.

\textcolor{cyan}{From Lemma (\ref{Sparse}) and the way $\demandofj{j'}$ is distributed for each dense clusters $j'$, the violation in lower bound is $1/2$. Thus, $\alpha > 1/2$.}

Also,\\ 
$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij}) $\\
$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \dist{i}{j}  \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} (\dist{j}{j'} + \dist{i}{j'})$ (by triangle inequality)\\ 
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   
%\sum_{\singlefacility \in \bundle{j'}} 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ (as $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
%$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )  $ (by definition of $\loadjinc{j}{j'}$, claim (\ref{claim-2}) of Lemma (\ref{distBound}) and the fact that $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
$ \leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +    \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{3/2} \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +  
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ (by Lemma (\ref{integral_dense}))\\
%$ \leq  \ell \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +   (1+1/\ell) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
\textcolor{yellow}{$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\}
%$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\ \textcolor{yellow}{(for $\ell > 2$)}\\
%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\ (for $\ell > 2$)\\
$\leq \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (by Lemma (\ref{integral_dense}))\\
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (because $z_i = \sum_{j \in \clientset} x^*_{ij} / \capacityU \leq y^*_i$)\\ 
%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by cost bound of feasible solution $z$.....Sapna..how from this reason?)\\
%\textcolor{red}{
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ellone \C{j}) + \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$  (by claim (\ref{claim-1}) of Lemma (\ref{distBound}))\\
%}
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} +  \textcolor{yellow}{2\ell} \textcolor{cyan}{4} \C{j}) + \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}  (2\dist{i}{j} +  \textcolor{yellow}{2\ell} \textcolor{cyan}{4} \C{j} )$ 
(by definition of $\loadjinc{j}{j'}$ and claims (\ref{claim-1}) and (\ref{claim-2}) of Lemma (\ref{distBound}))\\
$= \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   \textcolor{yellow}{2+\ell} \textcolor{cyan}{4}   \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} +   \textcolor{yellow}{2\ell(1+\ell)} \textcolor{cyan}{12} \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}   \C{j} $ \\

Summing over all $j' \in \cdense$ and adding inequality (\ref{cost-of-sparse}), we get\\
$ \sum_{i \in \facilityset} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij})$\\
$\leq \textcolor{yellow}{max\{\ell, \ell/(\ell-1)\}} \textcolor{cyan}{2} \sum_{i \in \facilityset}  f_i y^*_i + \textcolor{yellow}{ max\{4,(2+\ell)\}} \textcolor{cyan}{4} \sum_{i \in \facilityset}\sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + \textcolor{yellow}{\ellone~ max\{4,2(1+\ell)\}} \textcolor{cyan}{12} \sum_{i \in \facilityset}\sum_{j \in \clientset} x^*_{ij} \C{j}$\\
 \textcolor{yellow}{ $= \sum_{i \in \facilityset}  f_i y^*_i + (2+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + 2\ell(1+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\ell > 2$)}\\
$ \leq \textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)} \textcolor{cyan}{16}LP_{opt}$.
\end{proof}


Theorem~\ref{TricriteriaResult} is obtained by solving a min-cost flow problem with relaxed lower  and upper bounds to obtain the integral assignments.
Let $S^t$ be the solution so obtained. %and violations in lower and upper bounds be denoted by $\alpha$ and $\beta$ respectively.
Then, $Cost_I(S^t) \le \textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)}\textcolor{cyan}{16} Cost_I(O)$,
where $O$ is an optimal solution to $I$, $\textcolor{yellow}{\alpha= (1 - 1/\ellone)} \textcolor{cyan}{\alpha >
1/2}$ and $\textcolor{yellow}{\beta= (1 + 1/\ellone)} \textcolor{cyan}{\beta= 3/2}$.
\textcolor{yellow}{ For $\ell = 2.01$, $\alpha > 1/2$, $\beta < 3/2$ and the approximation ratio is less than $17$. The violations in the lower and the upper bounds can be made arbitrarily close to $0$ at the cost of increase in the approximation ratio.}

%To obtain integral assignments, we solve a minimum-cost integer flow problem with relaxed lower  and upper bounds.



	Next, using $S^t$, we transform the instance $I$ to an instance $I_{cap}$ of capacitated facility location problem by swapping the roles of clients and facilities. This is done via a series of transformations from instance $I$ to $I_1$, 	$I_1$ to $I_2$ and $I_2$ to $I_{cap}$. The key idea is to create  $\B - n_i$ units of demand, where the number $n_i$ of clients served by facility $i$ in $S^t$ is short of the lower bound and create  $n_i - \B$ units of supply at locations where $n_i > \B$.
	
	


==> NEW Journal version WADS 2021 (LBUBFL)/TriCriteria_l_1By2.tex <==
\section{Computing the Tri-criteria Solution}
\label{tri-criteria}
 %We use a simpler LP-rounding technique to get $(\frac{\ellone-1}{\ellone})$-factor violation in lower bounds and $2$-factor violation in upper bounds at constant factor loss in cost. The technique used is much simpler than Friggstad et al. \cite{friggstad_et_al_LBUFL} because lower bounds are uniform in our case unlike Friggstad et al. that considers non-uniform lower bounds. 

 In this section, we give a tri-criteria solution that violates the lower bound by a factor of \textcolor{yellow}{$\alpha = (1 - \frac{1}{\ell})$} \textcolor{cyan}{$\alpha > 1/2$} and the upper bound by a factor of \textcolor{cyan}{$\beta = 3/2$.} \textcolor{yellow}{$\beta = (1 + \frac{1}{\ell})$ where $\ell > 2$ is a tune-able parameter.} In particular, we present the following result:
 
 

 \begin{theorem} \label{TricriteriaResult}
 A \textcolor{yellow}{$( 2\ell^2+ 3\ell+2 ,  (1 - \frac{1}{\ell}) ,  (1 + \frac{1}{\ell}))$} \textcolor{cyan}{$(O(1),1/2,3/2)$} -
 approximate solution can be obtained for LBUBFL in polynomial time. \textcolor{yellow}{, where $\ell > 2$ is a tuneable parameter.}
\end{theorem}
 
 
 Instance $I$ of LBUBFL can be formulated as the following integer program (IP):

\label{{unif-CFLP}}
$Minimize ~\mathcal{C}ostLBUBFL(x,y) = \sum_{j \in \clientset}\sum_{i \in \facilityset}\dist{i}{j}x_{ij} + \sum_{i \in \facilityset}f_iy_i $
\begin{eqnarray}
subject~ to &\sum_{i \in \facilityset}{} x_{ij} \geq 1 & \forall ~\singleclient \in \clientset \label{LPFLP_const1}\\ 
%&\sum_{j \in \clientset}{} x_{ij} \leq \capacityU ~ y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const2}\\ 
& \capacityU y_i \geq \sum_{j \in \clientset}{} x_{ij} \geq \B y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const3}\\
& x_{ij} \leq y_i & \forall~ \singlefacility \in \facilityset , ~\singleclient \in \clientset \label{LPFLP_const4}\\   
& y_i,x_{ij} \in \left\lbrace 0,1 \right\rbrace  \label{LPFLP_const5}
\end{eqnarray}
where  $y_i$ is an indicator variable which is equal to $1$ if facility $i$ is open and is $0$ otherwise. $x_{ij}$ is an indicator variable which is equal to $1$ if client $j$ is served by facility $i$ and is $0$ otherwise.
 Constraints \ref{LPFLP_const1} ensure that all the clients are served. %Constraints \ref{LPFLP_const2} make sure that the total demand assigned to an open facility is no more than its capacity \capacityU. 
 Constraints \ref{LPFLP_const3} make sure that the total demand assigned to an open facility is at least $\B$ and at most $\capacityU$. Constraints \ref{LPFLP_const4} ensure that a client is assigned to a facility only if it is opened. LP-Relaxation  is obtained by allowing the variables to be non-integral.
% $ y_i, x_{ij} \in [0, 1]$. %Call it LP. 
Let $\zeta^{*} = <x^*, y^*>$ be an optimal solution  and $\opt{}$ be its cost.

%TBD: In this section, we give a tri-criteria solution that violates the lower bound by a factor of $(\ellone-1)/\ellone$ for a fixed parameter \textcolor{blue}{$\ellone > 2$} and the upper bounds by a factor of $2$.

We start by sparsifying the problem instance by removing some clients.
For $j \in \clientset$, let $ \C{j} $ denote the average connection cost paid by $\singleclient$ in $\zeta^*$. 
%i.e., ~$\C{j} = (\sum_{i \in \facilityset}{} {x}^*_{ij} \dist{i}{j})/({\sum_{i \in \facilityset}{} {x}^*_{ij}})$. 
Further, let $\ell > 2$ be a tuneable parameter, $\ballofj{j}$ be the ball of facilities within a radius of $\ellone\C{j}$ of $j$ and $\cardTwo{\ballofj{j}}$
%$=  \sum_{i \in \ballofj{j}} y^*_i$ 
be the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
%~ i.e., \ \ballofj{j}  = \{ \singlefacility \in \facilityset \colon \dist{i}{j} \leq \ellone \C{j} \}$.
Then,  \textcolor{olive}{$\cardTwo{\ballofj{j}} \ge (1-\frac{1}{\ellone}) > 1/2$.}
%where $\cardTwo{\ballofj{j}}$
%$=  \sum_{i \in \ballofj{j}} y^*_i$ denotes the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
The clients are processed in the non-decreasing order of the radii of their balls, removing the close-by clients with balls of larger radii and dissolving their balls: let $\bar{\clientset} = \clientset$ and $\clientset'$ denote the sparsified set of  clients. Initially $\clientset' = \phi$.
Let $j'$ be a client in $\bar{\clientset}$ with a ball of the smallest radius (breaking the ties arbitrarily). Remove $j'$ from $\bar{\clientset}$ and add it to $\clientset'$. For all $j (\ne j') \in \bar{\clientset}$ with $\dist{j'}{ j} \leq 2\ell \C{j}$, remove $j$ from $\bar{\clientset}$. Repeat the process until $\bar{\clientset} = \phi$. 
Cluster of facilities are formed around the clients in $\clientset'$ by assigning a facility to the cluster of $j' \in \clientset'$ if and only if $j'$ is nearest to the facility amongst all $j' \in \clientset'$, i.e. if $\bundle{j'}$ denotes the cluster centered at $j'$ then, $i$ belongs to $\bundle{j'}$ if and only if $\dist{i}{j'} < \dist{i}{k'}$ for all $k' \in \clientset'$ (assuming that the distances are distinct).
The clients in $C'$ are then called the cluster centers.



\begin{observation}
Any two cluster centers $j', k'$ in $C'$ satisfy the  separation property: $\dist{j'}{k'} > 2\ellone~max\{ \C{j'},\C{k'}\}$.
\end{observation}

\begin{lemma} \label{distBound}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. Then,
\begin{enumerate}
    \item \label{claim-1} $\dist{i}{j'}  \leq \dist{i}{j} + 2\ellone \C{j}$
    \item \label{claim-2} $\dist{j}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$
    \item \label{claim-3} If $\dist{j}{j'} \leq \ell \C{j'}$, then $\C{j'} \le 2\C{j}$.
\end{enumerate}
\end{lemma}

\begin{proof}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. 
\begin{enumerate}

    \item Note that, $\dist{j}{k'} \leq 2\ellone \C{j}$ for some $k' \in \clientset'$. Then we have $\dist{i}{j'} \leq \dist{i}{k'} \leq \dist{i}{j} + \dist{j}{k'} \leq \dist{i}{j} + 2\ellone \C{j}$, where the first inequality follows because $i$ belongs to $\bundle{j'}$ and not $\bundle{k'}$ whenever $k' \ne j'$.  \textcolor{blue}{See Fig: (\ref{Cjj'}).}
    
    
    \item Using triangle inequality, we have $\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$.
     \item Let $j \ne j'$. Note that  $\dist{j}{j'} \leq \ell \C{j'} \Rightarrow j \notin \clientset'$. 
     %Further, using contradiction, let's assume 
     Suppose if possible, $\C{j'} > 2\C{j}$. Since $j \notin \cliset', \exists$ some $k'\in \clientset':\dist{j}{k'} \le 2 \ell \C{j}$. Then, $\dist{k'}{j'} \le \dist{k'}{j} + \dist{j}{j'}$ $ \leq 2 \ell \C{j} + \ell \C{j'} < 2\ell \C{j'}$. Thus, we arrive at a contradiction to the separation property. Hence, $\C{j'} \le 2\C{j}$.
\end{enumerate} \end{proof}
 

\begin{figure} 
    \centering
    \includegraphics[width=10cm]{Figures/Cjj'.jpg}
    \caption{$\dist{i}{j'}  \leq \dist{i}{j} + 2\ellone \C{j}$}
    \label{Cjj'}
\end{figure}

%$\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$ ~\cite{GroverGKP18}.}  

For $j' \in \clientset', j \in \clientset$, let $\loadjinc{j}{j'}$ be the extent up to which $j$ is served by the facilities in the cluster of $j'$  \textcolor{olive}{under solution $\zeta^*$} and $d_{j'}= \sum_{j \in \clientset} \loadjinc{j}{j'}$.
We call a cluster to be $sparse$ if $d_{j'} \le  \capacityU$ and $dense$ otherwise. Let $\csparse$ and $\cdense$ be the set of cluster centers of sparse  and dense clusters respectively.


%Let $<\hat{x}, \hat{y}>$ be the solution so obtained, i.e., for $ j \in \clientset$, $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$. For $j' \in \crich, i \in \bundle{j'}, j \in \clientset$, $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. 


\begin{lemma} \label{Sparse}
We can obtain a solution $<\hat{x}, \hat{y}>$ such that  exactly one facility $i(j')$ is opened integrally in each sparse cluster centered at $j' \in \clientset'$. The solution violates the lower bound by a factor of $(1 - 1/\ellone)$ \textcolor{olive}{such that $\sum_{j' \in \clientset'}\sum_{i \in \bundle{j'}} [f_i \hat{y}_i + \sum_{j \in \clientset}  \hat{x}_{ij} \dist{i}{j}] \leq $}
$\sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})] + \sum_{j' \in \cdense} [\sum_{i \in \bundle{j'}} f_i y^*_i + \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$.

%\textcolor{red}{May be we should write the following:$\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \le \sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})]$...will resolve after completing this section}

\end{lemma}

\begin{proof}
%In a sparse cluster centered at $j'$, we open the cheapest facility, say $i(j')$, in $\ballofj{j'}$ and transfer all the assignments in the cluster onto it.
%As specified above, 
For $ j' \in \cdense, i \in \bundle{j'}, j \in \clientset$, set $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. Next,
let $j' \in \csparse$
%$\bundle{j'}$ be a sparse cluster centered at $j'$ 
and $i(j')$ be a cheapest \textcolor{olive}{(lowest facility opening cost)} facility in $\ballofj{j'}$. We open $i(j')$ and transfer all the assignments in the cluster onto it (see Figure (\ref{sparse})). 
%Let $ j \in \clientset$.
i.e. set $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$ and $j \in \clientset$. 
Since $\cardTwo{\ballofj{j'}} \ge (1-\frac{1}{\ellone})$ we have $\sum_{j \in \clientset}{} \hat{x}_{i(j')j} = \demandofj{j'} \ge (1-\frac{1}{\ellone})\B$. Thus, the lower bound is violated at most by $(1-\frac{1}{\ellone})$
and the facility cost is bounded by $\frac{\ellone}{\ellone - 1} \sum_{i \in \bundle{j'}} f_i y^*_i$.

To bound the service cost, we will show that for $j' \in \csparse, \sum_{j \in \clientset} \loadjinc{j}{j'} \dist{i(j')}{j}  \leq 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})$: 
since $i(j') \in \ballofj{j'}$, we have $\dist{i(j')}{j'} \le \ellone \C{j'}$. 
Thus, for $j \in \clientset$,
we have $\dist{i(j')}{j} \le \dist{j'}{j} + \dist{i(j')}{j'} \le  \dist{j'}{j} + \ellone \C{j'}$. If $\ellone \C{j'} \le \dist{j'}{j}$ then $\dist{i(j')}{j}  \le 2  \dist{j'}{j}  \leq 4 (\dist{i}{j} + \ellone \C{j})$ ($\forall~i \in \bundle{j'}$ by claim (\ref{claim-2}) of Lemma (\ref{distBound})), 
 else $\dist{i(j')}{j}  \leq 2 \ell \C{j'} \leq 4 \ellone \C{j}$, where the second inequality in the else part follows by claim (\ref{claim-3}) of Lemma (\ref{distBound}).
Thus, in either case $\dist{i(j')}{j} \leq 4 (\dist{i}{j} + \ellone \C{j})$ for all $i \in \bundle{j'}$.
Substituting $\phi(j, j') = \sum_{i \in \bundle{j'}} x^*_{ij}$ and summing over all $j \in \clientset$ 
%$j' \in \csparse$ 
we get the desired bound.
Thus, $\sum_{i \in \facilityset} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  \hat{x}_{ij}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \demandofj{j'}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
\le \sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})] + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} [ f_i y^*_i + \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$
\end{proof}
 
%$\le 4\dist{i}{j} + 4 \ellone \C{j} $ else $\dist{i(j')}{j}  \le  2 \ellone \C{j'} \le 4 \ellone \C{j} \le 4\dist{i}{j} + 4 \ellone \C{j}$, where the second inequality in the else part follows because if $\ellone \C{j'} > \dist{j'}{j}$ then $\C{j'} \leq 2\C{j}$ \cite{GroverGKP18}. Also, since the total opening in each cluster is at least $(1-(1/\ellone))$, a loss of factor $\ellone/(\ellone-1) (\leq 2$ for $\ellone > 2$) in the facility opening cost is incurred, violation in lower bound is at most $(1-(1/\ellone))$ and  since  $d_{j'} \le \capacityU$ there is no  violation in the capacity.}
   
    \begin{figure} 
    \centering
    \includegraphics[width=10cm]{Figures/sparse.jpg}
    \caption{(A) Cluster $\bundle{j'}$ centered at $j'$. (B) Demand $\demandofj{j'}$ being assigned to facility $i(j') \in \ballofj{j'}$.}
    \label{sparse}
\end{figure}
 
To open the facilities integrally in the dense clusters, we solve the following LP for every dense cluster $\bundle{j'}$.
%centered at $j'$.

($LP_1$): 
\label{dense}
$Minimize ~\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$
\begin{eqnarray}
subject~ to &\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'} \label{denseLP_const1}\\
&\textcolor{cyan}{\B \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \leq \demandofj{j'} \label{denseLP_const1-1}}\\ 
&0 \leq \zofi{i} \leq 1 \label{denseLP_const2}
\end{eqnarray}
   
  % $Minimize $\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$ s.t. $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$ and $\zofi{i} \in [0,1]$. 
   
   
Note that for $\zofi{i} = \sum_{j \in \clientset}x_{ij}^*/\capacityU$, we have $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} = \demandofj{j'} \geq \textcolor{cyan}{\B \sum_{\singlefacility \in \bundle{j'}} \zofi{i}}$ and $\zofi{i} \le y^*_i$. Thus, $\zofi{}$
is a feasible solution with cost at most $ \sum_{i \in \bundle{j'}} [\facilitycost y^*_i + \sum_{ j \in \clientset} x^*_{ij} ( \dist{i}{j} +  2\ellone \C{j}) ]$ by claim (\ref{claim-1}) of Lemma (\ref{distBound}).

%\textcolor{blue}{TBD: facility opening cost at most $ \sum_{i \in \bundle{j'}} \facilitycost y^*_i$ and service cost $\sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij}  \dist{i}{j'} \le \sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij} [ \dist{i}{ j} + 2\ellone \C{j} ]$. } 

\begin{lemma} \label{integral_dense}
Given the feasible solution $z$ to $LP_1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) \textcolor{cyan}{and (\ref{denseLP_const1-1})} by a factor of \textcolor{yellow}{$(1+1/\ell)$} \textcolor{cyan}{$3/2$ and $1/2$ respectively}, can be obtained at a loss of factor $\textcolor{yellow}{\ellone} \textcolor{cyan}{2}$ in cost
i.e. $ \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \hat{z}_{i} \le  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$.
%For a fixed $0 < \epsilon < 1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) by a factor of $(1+\epsilon)$, can be obtained at a loss of $(1/\epsilon)$ in cost.
\end{lemma}

\begin{proof}
\textcolor{green}{
We say that a solution to $LP_1$ is almost integral if it has at most one fractionally opened facility in $\bundle{j'}$.
}
We first obtain an almost integral solution
%\footnote{A solution is said to be an almost integral solution if it has at most one fractionally opened facility.}
$\primezofi{}$ by arranging the facilities opened in $z$, in non-decreasing order of $\facilitycost  + \dist{i}{j'} \capacityU$ and greedily transferring the openings $z$ onto them. 
Then,  $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} = \demandofj{j'}$. %Consider constraint (\ref{denseLP_const1}), $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$.
Note that the cost of solution $\primezofi{}$ is no more than that of solution $z$.


We now convert the almost integral solution $\primezofi{}$ to an integral solution $\hat{z}$. Let $\hat{z} = \primezofi{}$ initially. Let $i'$ be the fractionally opened facility, if any, in $\bundle{j'}$. %Initially, set $\hat{z}_i = \primezofi{i}~ \forall i \in \bundle{j'}$. 
Consider the following cases:


\begin{enumerate}
    %\item $\primezofi{i'} < \epsilon$:
    \item $\primezofi{i'} \textcolor{yellow}{ < 1/\ell} \textcolor{cyan}{ \leq 1/2}$: close $i'$ in $\hat{z}$. There must be at least one integrally opened facility, say $i (\ne i') \in \bundle{j'}$ in $\primezofi{}$, as $\demandofj{j'} \ge \capacityU$. Then, $\demandofj{j'} = \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k} + \capacityU  (\primezofi{i} + \primezofi{i'}) \le \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k}  + \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU  \primezofi{i} \le \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU \sum_{k \in \bundle{j'} \setminus \{i'\}} \primezofi{k} = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}  \capacityU \sum_{k \in \bundle{j'}} \hat{z}_k$. There is no increase in cost as we have only (possibly) shut down one of the facilities .
    

    \item $\primezofi{i'} \textcolor{yellow}{ \geq 1/\ell} \textcolor{cyan}{> 1/2} $: Open $i'$ integrally at a loss of factor $\textcolor{yellow}{\ell}$ \textcolor{cyan}{2} in facility opening cost i.e., $\sum_{i \in \bundle{j'}} f_i \hat{z}_i \le \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i \primezofi{i}$ \textcolor{cyan}{and $1/2$ factor in lower bound, i.e., $\demandofj{j'} \geq \B \sum_{k \in \bundle{j'}} \primezofi{k} \geq \B/2  \sum_{k \in \bundle{j'}} \hat{z}_{k}$,  where the second inequality follows because $\sum_{i \in \bundle{j'}} \hat{z}_i \leq 2\sum_{i \in \bundle{j'}} z'_i$.}
\end{enumerate}\end{proof}

%Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{(1+1/\ell)\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = (1 + 1/\ell) \capacityU \hat{z}_i$ , where the first inequality follows by Lemma (\ref{integral_dense}). 


%\textcolor{cyan}{SAPNA, Revisit the next para later:}

Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{\textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU \hat{z}_i$ , where the first inequality follows by Lemma (\ref{integral_dense}). \textcolor{cyan}{Also, $l_i  = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \geq \hat{z}_i \frac{\demandofj{j'}}{2\sum_{i \in \bundle{j'}} z'_i} = \hat{z}_i \frac{\demandofj{j'}}{2\sum_{i \in \bundle{j'}} z_i} =  \hat{z}_i \frac{\B \sum_{i \in \bundle{j'}} z_i}{2\sum_{i \in \bundle{j'}} z_i} = 1/2 B \hat{z}_i$, where the first inequality follows because $\sum_{i \in \bundle{j'}} \hat{z}_i \leq 2\sum_{i \in \bundle{j'}} z'_i$.}


    

\textcolor{olive}{A solution is said to be an integrally opened solution if all facilities in it are either opened to an extent of $1$ or $0$. We next obtain such a solution to LBUBFL problem.}



\begin{lemma} \label{Dense1}
We can obtain an integrally opened solution $<\bar x, \bar y>$ to LBUBFL problem at a loss of \textcolor{yellow}{($1+1/\ell$)} \textcolor{cyan}{$3/2$} in upper bounds and \textcolor{yellow}{$(1-1/\ell)$} \textcolor{cyan}{$1/2$}  in lower bounds whose cost is bounded by $(10\ellone + 4)LP_{opt}$.
\end{lemma}

\begin{proof}
For $j' \in \csparse$, set $\bar y_i = \hat{y}_i,~\bar{x}_{ij} = \hat{x}_{ij}~\forall i \in \bundle{j'}, j \in \clientset$. \textcolor{yellow}{The violation in lower bound then follows from Lemma (\ref{Sparse})
and, }

\begin{equation}
\label{cost-of-sparse}
\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \bar{y}_i + \sum_{j \in \clientset} \bar{x}_{ij} \dist{i}{j}) \le \sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})].
\end{equation}



Next let $j' \in \cdense,~i \in \bundle{j'}, j \in \clientset$. Set $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. 
Consider $ \sum_{j \in \clientset} \bar{x}_{ij} = \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} = l_i \leq   \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \hat{z}_i = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \bar{y}_i$. Thus, the loss in capacities is at most   \textcolor{yellow}{(1+1/\ell)}\textcolor{cyan}{(3/2).}

\textcolor{cyan}{From Lemma (\ref{Sparse}) and (\ref{integral_dense}), the violation in lower bound is $min\{1-1\ell,1/2\} > 1/2$ for $\ell>2$. Thus, $\alpha > 1/2$.}



Also,\\ 
$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij}) $\\
$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \dist{i}{j}  \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} (\dist{j}{j'} + \dist{i}{j'})$ (by triangle inequality)\\ 
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   
%\sum_{\singlefacility \in \bundle{j'}} 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ (as $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
%$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )  $ (by definition of $\loadjinc{j}{j'}$, claim (\ref{claim-2}) of Lemma (\ref{distBound}) and the fact that $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
$ \leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +    \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{3/2} \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +  
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ (by Lemma (\ref{integral_dense}))\\
%$ \leq  \ell \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +   (1+1/\ell) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
\textcolor{yellow}{$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\}
%$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\ \textcolor{yellow}{(for $\ell > 2$)}\\
%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\ (for $\ell > 2$)\\
$\leq \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (by Lemma (\ref{integral_dense}))\\
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (because $z_i = \sum_{j \in \clientset} x^*_{ij} / \capacityU \leq y^*_i$)\\ 
%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by cost bound of feasible solution $z$.....Sapna..how from this reason?)\\
%\textcolor{red}{
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ellone \C{j}) + \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$  (by claim (\ref{claim-1}) of Lemma (\ref{distBound}))\\
%}
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ell \C{j}) + \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}  (2\dist{i}{j} + 2\ell\C{j} )$ 
(by definition of $\loadjinc{j}{j'}$ and claims (\ref{claim-1}) and (\ref{claim-2}) of Lemma (\ref{distBound}))\\
$= \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   \textcolor{yellow}{2+\ell} \textcolor{cyan}{4}   \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} +   \textcolor{yellow}{2\ell(1+\ell)} \textcolor{cyan}{6\ell} \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}   \C{j} $ \\

Summing over all $j' \in \cdense$ and adding inequality (\ref{cost-of-sparse}), we get\\
$ \sum_{i \in \facilityset} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij})$\\
$\leq max\{2, \ell/(\ell-1)\} \sum_{i \in \facilityset}  f_i y^*_i + \textcolor{yellow}{ max\{4,(2+\ell)\}} \textcolor{cyan}{4} \sum_{i \in \facilityset}\sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + \textcolor{yellow}{\ellone~ max\{4,2(1+\ell)\}} \textcolor{cyan}{10 \ell} \sum_{i \in \facilityset}\sum_{j \in \clientset} x^*_{ij} \C{j}$\\
 \textcolor{yellow}{ $= \sum_{i \in \facilityset}  f_i y^*_i + (2+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + 2\ell(1+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\ell > 2$)}\\
  \textcolor{cyan}{$ \leq 2 \sum_{i \in \facilityset}  f_i y^*_i + 4\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + 10\ell \sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\ell > 2$)}\\
$ \leq \textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)}
\textcolor{cyan}{(10 \ell+4)}LP_{opt}$.
\end{proof}


Theorem~\ref{TricriteriaResult} is obtained by solving a min-cost flow problem with relaxed lower  and upper bounds to obtain the integral assignments.
Let $S^t$ be the solution so obtained. %and violations in lower and upper bounds be denoted by $\alpha$ and $\beta$ respectively.
Then, $Cost_I(S^t) \le \textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)} \textcolor{cyan}{(10\ell+4)}Cost_I(O)$,
where $O$ is an optimal solution to $I$, $\textcolor{yellow}{\alpha= (1 - 1/\ellone)} \textcolor{cyan}{\alpha >
1/2}$ and $\textcolor{yellow}{\beta= (1 + 1/\ellone)} \textcolor{cyan}{\beta= 3/2}$. \textcolor{cyan}{ Fix $\ell = 2.01$, we get an approximation ratio of less than $16.5$.}
\textcolor{yellow}{ For $\ell = 2.01$, $\alpha > 1/2$, $\beta < 3/2$ and the approximation ratio is less than $17$. The violations in the lower and the upper bounds can be made arbitrarily close to $0$ at the cost of increase in the approximation ratio.}

%To obtain integral assignments, we solve a minimum-cost integer flow problem with relaxed lower  and upper bounds.



	Next, using $S^t$, we transform the instance $I$ to an instance $I_{cap}$ of capacitated facility location problem by swapping the roles of clients and facilities. This is done via a series of transformations from instance $I$ to $I_1$, 	$I_1$ to $I_2$ and $I_2$ to $I_{cap}$. The key idea is to create  $\B - n_i$ units of demand, where the number $n_i$ of clients served by facility $i$ in $S^t$ is short of the lower bound and create  $n_i - \B$ units of supply at locations where $n_i > \B$.
	


==> NEW Journal version WADS 2021 (LBUBFL)/TriCriteria_l_1Minus1Byl.tex <==
\section{Computing the Tri-criteria Solution}
\label{tri-criteria}
 %We use a simpler LP-rounding technique to get $(\frac{\ellone-1}{\ellone})$-factor violation in lower bounds and $2$-factor violation in upper bounds at constant factor loss in cost. The technique used is much simpler than Friggstad et al. \cite{friggstad_et_al_LBUFL} because lower bounds are uniform in our case unlike Friggstad et al. that considers non-uniform lower bounds. 

 In this section, we first give a tri-criteria solution that violates the lower bound by a factor of $\alpha = (1 - \frac{1}{\ell})$ %\textcolor{cyan}{$\alpha > 1/2$}
 and the upper bound by a factor of $\beta = (2 - \frac{1}{\ell})$, where $\ell \ge 2$ is a tune-able parameter. 
 %\textcolor{red}{The result can be of independent interest. We then give a tri-criteria solution that violates the lower bound by a factor of $\alpha > 1/2$ \textcolor{cyan}{$\alpha > 1/2$}
 %and the upper bound by a factor of $\beta = 3/2$. Note that the second result follows nearly but not exactly from the first. We use the latter to obtain our bounds of Theorem~\ref{?} }
 This is one of the two major contributions of our work.
 In particular, we present the following results:
 
 

 \begin{theorem} \label{TricriteriaResult}
 An $((1 - \frac{1}{\ell}),(2 - \frac{1}{\ell}),(10\ell+4))$-
 approximate solution can be obtained for LBUBFL in polynomial time, where $\ell \ge 2$ is a tuneable parameter.
\end{theorem}
 
 % \begin{theorem} \label{TricriteriaResult}
 %An \textcolor{red}{$(O(1),> 1/2,3/2)$ -
 %approximate solution can be obtained for LBUBFL in polynomial time.}
%\end{theorem}
 
 Instance $I$ of LBUBFL can be formulated as the following integer program (IP):

\label{{unif-CFLP}}
$Minimize ~\mathcal{C}ostLBUBFL(x,y) = \sum_{j \in \clientset}\sum_{i \in \facilityset}\dist{i}{j}x_{ij} + \sum_{i \in \facilityset}f_iy_i $
\begin{eqnarray}
subject~ to &\sum_{i \in \facilityset}{} x_{ij} \geq 1 & \forall ~\singleclient \in \clientset \label{LPFLP_const1}\\ 
%&\sum_{j \in \clientset}{} x_{ij} \leq \capacityU ~ y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const2}\\ 
& \capacityU y_i \geq \sum_{j \in \clientset}{} x_{ij} \geq \B y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const3}\\
& x_{ij} \leq y_i & \forall~ \singlefacility \in \facilityset , ~\singleclient \in \clientset \label{LPFLP_const4}\\   
& y_i,x_{ij} \in \left\lbrace 0,1 \right\rbrace  \label{LPFLP_const5}
\end{eqnarray}
where  $y_i$ is an indicator variable which is equal to $1$ if facility $i$ is open and is $0$ otherwise. $x_{ij}$ is an indicator variable which is equal to $1$ if client $j$ is served by facility $i$ and is $0$ otherwise. Constraints \ref{LPFLP_const1} ensure that every client is served. %Constraints \ref{LPFLP_const2} make sure that the total demand assigned to an open facility is no more than its capacity \capacityU. 
 Constraints \ref{LPFLP_const3} make sure that the total demand assigned to an open facility is at least $\B$ and at most $\capacityU$. Constraints \ref{LPFLP_const4} ensure that a client is assigned to a facility only if it is opened. LP-Relaxation  is obtained by allowing the variables to be non-integral.
% $ y_i, x_{ij} \in [0, 1]$. %Call it LP. 
Let $\zeta^{*} = <x^*, y^*>$ be an optimal solution to the LP-relaxation and $\opt{}$ be its cost.

%TBD: In this section, we give a tri-criteria solution that violates the lower bound by a factor of $(\ellone-1)/\ellone$ for a fixed parameter \textcolor{blue}{$\ellone > 2$} and the upper bounds by a factor of $2$.

We start by sparsifying the problem instance by removing some clients.
For $j \in \clientset$, let $ \C{j}= \sum_{i \in \facilityset} x^*_{ij} \dist{i}{j}$ denote the average connection cost paid by $\singleclient$ in $\zeta^*$. 
%i.e., ~$\C{j} = (\sum_{i \in \facilityset}{} {x}^*_{ij} \dist{i}{j})/({\sum_{i \in \facilityset}{} {x}^*_{ij}})$. 
Further, let $\ell \ge 2$ be a tuneable parameter, $\ballofj{j}$ be the ball of facilities within a radius of $\ellone\C{j}$ of $j$ and $\cardTwo{\ballofj{j}}$ be the total extent up to which facilities are opened in $\ballofj{j}$ under solution $\zeta^*$ , i.e.,  $\cardTwo{\ballofj{j}} = \sum_{i \in \ballofj{j}} y^*_i $.
%~ i.e., \ \ballofj{j}  = \{ \singlefacility \in \facilityset \colon \dist{i}{j} \leq \ellone \C{j} \}$.
Then, $\cardTwo{\ballofj{j}} \ge (1-\frac{1}{\ellone}) \ge 1/2$.
%where $\cardTwo{\ballofj{j}}$
%$=  \sum_{i \in \ballofj{j}} y^*_i$ denotes the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
The clients are processed in the non-decreasing order of the radii of their balls, removing the close-by clients with balls of larger radii and dissolving their balls: let $\bar{\clientset} = \clientset$ and $\clientset'$ denote the sparsified set of  clients. Initially $\clientset' = \phi$.
Let $j'$ be a client in $\bar{\clientset}$ with a ball of the smallest radius (breaking the ties arbitrarily). Remove $j'$ from $\bar{\clientset}$ and add it to $\clientset'$. For all $j (\ne j') \in \bar{\clientset}$ with $\dist{j'}{ j} \leq 2\ell \C{j}$, remove $j$ from $\bar{\clientset}$. Repeat the process until $\bar{\clientset} = \phi$. 
Cluster of facilities are formed around the clients in $\clientset'$ by assigning a facility to the cluster of $j' \in \clientset'$ if and only if $j'$ is nearest to the facility amongst all $j' \in \clientset'$, i.e. if $\bundle{j'}$ denotes the cluster centered at $j'$ then, $i$ belongs to $\bundle{j'}$ if and only if $\dist{i}{j'} < \dist{i}{k'}$ for all $k'(\ne j') \in \clientset'$ (assuming that the distances are distinct).
The clients in $C'$ are then called the cluster centers.



\begin{observation}
Any two cluster centers $j', k'$ in $C'$ satisfy the  separation property: $\dist{j'}{k'} > 2\ellone~max\{ \C{j'},\C{k'}\}$.
\end{observation}

\begin{lemma} \label{distBound}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. Then,
\begin{enumerate}
    \item \label{claim-1} $\dist{i}{j'}  \leq \dist{i}{j} + 2\ellone \C{j}$
    \item \label{claim-2} $\dist{j}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$
    \item \label{claim-3} If $\dist{j}{j'} \leq \ell \C{j'}$, then $\C{j'} \le 2\C{j}$.
\end{enumerate}
\end{lemma}

\begin{proof}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. 
\begin{enumerate}

    \item Note that, $\dist{j}{k'} \leq 2\ellone \C{j}$ for some $k' \in \clientset'$. Then we have $\dist{i}{j'} \leq \dist{i}{k'} \leq \dist{i}{j} + \dist{j}{k'} \leq \dist{i}{j} + 2\ellone \C{j}$, where the first inequality follows because $i$ belongs to $\bundle{j'}$ and not $\bundle{k'}$ whenever $k' \ne j'$.  See Fig: (\ref{Cjj}).
    
    
    \item Using triangle inequality, we have $\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$.
     \item Let $j \ne j'$. Note that  $\dist{j}{j'} \leq \ell \C{j'} \Rightarrow j \notin \clientset'$. 
     %Further, using contradiction, let's assume 
     Suppose if possible, $\C{j'} > 2\C{j}$. Since $j \notin \cliset', \exists$ some $k'\in \clientset':\dist{j}{k'} \le 2 \ell \C{j}$. Then, $\dist{k'}{j'} \le \dist{k'}{j} + \dist{j}{j'}$ $ \leq 2 \ell \C{j} + \ell \C{j'} < 2\ell \C{j'}$. Thus, we arrive at a contradiction to the separation property. Hence, $\C{j'} \le 2\C{j}$.
\end{enumerate} \end{proof}
 

\begin{figure} 
    \centering
    \includegraphics[width=10cm]{ Cjj.jpg}
    \caption{$\dist{i}{j'}  \leq \dist{i}{j} + 2\ellone \C{j}$}
    \label{Cjj}
\end{figure}

%$\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$ ~\cite{GroverGKP18}.}  

For $j' \in \clientset', j \in \clientset$, let $\loadjinc{j}{j'}$ be the extent up to which $j$ is served by the facilities in the cluster of $j'$ under solution $\zeta^*$ and $d_{j'}= \sum_{j \in \clientset} \loadjinc{j}{j'}$.
We call a cluster to be $sparse$ if $d_{j'} \le  \capacityU$ and $dense$ otherwise. Let $\csparse$ and $\cdense$ be the set of cluster centers of sparse  and dense clusters respectively.


%Let $<\hat{x}, \hat{y}>$ be the solution so obtained, i.e., for $ j \in \clientset$, $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$. For $j' \in \crich, i \in \bundle{j'}, j \in \clientset$, $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. 


\begin{lemma} \label{Sparse}
We can obtain a solution $<\hat{x}, \hat{y}>$ such that  exactly one facility $i(j')$ is opened integrally in each sparse cluster centered at $j' \in \clientset'$. The solution violates the lower bound by a factor of $(1 - 1/\ellone)$ and $\sum_{j' \in \clientset'}\sum_{i \in \bundle{j'}} [f_i \hat{y}_i + \sum_{j \in \clientset}  \hat{x}_{ij} \dist{i}{j}] \leq $
$\sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})] + \sum_{j' \in \cdense} [\sum_{i \in \bundle{j'}} f_i y^*_i + \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$.

%\textcolor{red}{May be we should write the following:$\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \le \sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})]$...will resolve after completing this section}

\end{lemma}

\begin{proof}
%In a sparse cluster centered at $j'$, we open the cheapest facility, say $i(j')$, in $\ballofj{j'}$ and transfer all the assignments in the cluster onto it.
%As specified above, 
For $ j' \in \cdense, i \in \bundle{j'}, j \in \clientset$, set $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. Next,
let $j' \in \csparse$
%$\bundle{j'}$ be a sparse cluster centered at $j'$ 
and $i(j')$ be a cheapest (lowest facility opening cost) facility in $\ballofj{j'}$. We open $i(j')$ and transfer all the assignments in the cluster onto it (see Figure (\ref{sparse})),
%Let $ j \in \clientset$.
i.e. set $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$ and $j \in \clientset$. 
Since $\cardTwo{\ballofj{j'}} \ge (1-\frac{1}{\ellone})$ we have $\sum_{j \in \clientset}{} \hat{x}_{i(j')j} = \demandofj{j'} \ge (1-\frac{1}{\ellone})\B$.
%\textcolor{red}{
%(Theorem 2.1) and $> (1/2) \B$ for $\ell > 2$ (Theorem 2.2).}
Thus, the lower bound is violated at most by $(1-\frac{1}{\ellone})$ %....\textcolor{red}{i guess will have to delete this}
and the facility cost is bounded by $\frac{\ellone}{\ellone - 1} \sum_{i \in \bundle{j'}} f_i y^*_i$.

To bound the service cost, we will show that for $j' \in \csparse, \sum_{j \in \clientset} \loadjinc{j}{j'} \dist{i(j')}{j}  \leq 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})$: 
since $i(j') \in \ballofj{j'}$, we have $\dist{i(j')}{j'} \le \ellone \C{j'}$. 
Thus, for $j \in \clientset$,
we have $\dist{i(j')}{j} \le \dist{j'}{j} + \dist{i(j')}{j'} \le  \dist{j'}{j} + \ellone \C{j'}$. If $\ellone \C{j'} \le \dist{j'}{j}$ then $\dist{i(j')}{j}  \le 2  \dist{j'}{j}  \leq 4 (\dist{i}{j} + \ellone \C{j})$ ($\forall~i \in \bundle{j'}$ by claim (\ref{claim-2}) of Lemma (\ref{distBound})), 
 else $\dist{i(j')}{j}  \leq 2 \ell \C{j'} \leq 4 \ellone \C{j}$, where the second inequality in the else part follows by claim (\ref{claim-3}) of Lemma (\ref{distBound}).
Thus, in either case $\dist{i(j')}{j} \leq 4 (\dist{i}{j} + \ellone \C{j})$ for all $i \in \bundle{j'}$.
Substituting $\phi(j, j') = \sum_{i \in \bundle{j'}} x^*_{ij}$ and summing over all $j \in \clientset$ 
%$j' \in \csparse$ 
we get the desired bound.
Thus, $\sum_{i \in \facilityset} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  \hat{x}_{ij}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \demandofj{j'}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
\le \sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})] + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} [ f_i y^*_i + \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$
\end{proof}
 
%$\le 4\dist{i}{j} + 4 \ellone \C{j} $ else $\dist{i(j')}{j}  \le  2 \ellone \C{j'} \le 4 \ellone \C{j} \le 4\dist{i}{j} + 4 \ellone \C{j}$, where the second inequality in the else part follows because if $\ellone \C{j'} > \dist{j'}{j}$ then $\C{j'} \leq 2\C{j}$ \cite{GroverGKP18}. Also, since the total opening in each cluster is at least $(1-(1/\ellone))$, a loss of factor $\ellone/(\ellone-1) (\leq 2$ for $\ellone > 2$) in the facility opening cost is incurred, violation in lower bound is at most $(1-(1/\ellone))$ and  since  $d_{j'} \le \capacityU$ there is no  violation in the capacity.}
   
    \begin{figure} 
    \centering
    \includegraphics[width=10cm]{ sparse.jpg}
    \caption{(A) Cluster $\bundle{j'}$ centered at $j'$. (B) Demand $\demandofj{j'}$ being assigned to facility $i(j') \in \ballofj{j'}$.}
    \label{sparse}
\end{figure}
 
To open the facilities integrally in the dense clusters, we consider the following LP for every dense cluster $\bundle{j'}$.
%centered at $j'$.

($LP_1$): 
\label{dense}
$Minimize ~\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$
\begin{eqnarray}
subject~ to &\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'} \label{denseLP_const1}\\
&\B \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \leq \demandofj{j'} \label{denseLP_const1-1}\\ 
&0 \leq \zofi{i} \leq 1 \label{denseLP_const2}
\end{eqnarray}
   
  % $Minimize $\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$ s.t. $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$ and $\zofi{i} \in [0,1]$. 
   
   
Note that for $\zofi{i} = \sum_{j \in \clientset}x_{ij}^*/\capacityU$, we have $\demandofj{j'} = \capacityU \sum_{\singlefacility \in   \bundle{j'}} \zofi{i} \geq \B \sum_{\singlefacility \in \bundle{j'}} \zofi{i}$ and $\zofi{i} \le y^*_i$. Thus, $z$
is a feasible solution with cost at most $ \sum_{i \in \bundle{j'}} [\facilitycost y^*_i + \sum_{ j \in \clientset} x^*_{ij} ( \dist{i}{j} +  2\ellone \C{j}) ]$ by claim (\ref{claim-1}) of Lemma (\ref{distBound}).

%\textcolor{blue}{TBD: facility opening cost at most $ \sum_{i \in \bundle{j'}} \facilitycost y^*_i$ and service cost $\sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij}  \dist{i}{j'} \le \sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij} [ \dist{i}{ j} + 2\ellone \C{j} ]$. } 

\begin{lemma} \label{integral_dense}
Given the feasible solution $z$ to $LP_1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) and (\ref{denseLP_const1-1}) by a factor of %\textcolor{magenta}{$(1+1/\ell)$} 
$(2-1/\ell)$ 
%($3/2$ for Theorem 2.2) 
and $(1-1/\ell)$ 
%($> 1/2$ for Theorem 2.2) 
respectively, can be obtained at a loss of factor $\ell/(\ell-1)$ in cost
i.e. $ \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \hat{z}_{i} \le \ell/(\ell-1) \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$.
%For a fixed $0 < \epsilon < 1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) by a factor of $(1+\epsilon)$, can be obtained at a loss of $(1/\epsilon)$ in cost.
\end{lemma}

\begin{proof}

We say that a solution to $LP_1$ is almost integral if it has at most one fractionally opened facility in $\bundle{j'}$.
We first obtain an almost integral solution
%\footnote{A solution is said to be an almost integral solution if it has at most one fractionally opened facility.}
$\primezofi{}$ by arranging the facilities opened in $z$, in non-decreasing order of $\facilitycost  + \dist{i}{j'} \capacityU$ and greedily transferring the openings $z$ onto them. 
Then,  $\B \sum_{i \in \bundle{j'}} \primezofi{i} \leq \capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} = \demandofj{j'}$. %Consider constraint (\ref{denseLP_const1}), $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$.
Note that the cost of solution $\primezofi{}$ is no more than that of solution $z$.


We now convert the almost integral solution $\primezofi{}$ to an integral solution $\hat{z}$. Let $\hat{z} = \primezofi{}$ initially. Let $i'$ be the fractionally opened facility, if any, in $\bundle{j'}$. %Initially, set $\hat{z}_i = \primezofi{i}~ \forall i \in \bundle{j'}$. 
Consider the following cases:


\begin{enumerate}
    %\item $\primezofi{i'} < \epsilon$:
    \item $\primezofi{i'} \leq 1-1/\ell$ 
    %( $1/2$ for Theorem 2.2)
    : close $i'$ in $\hat{z}$. There must be at least one integrally opened facility, say $i (\ne i') \in \bundle{j'}$ in $\primezofi{}$, as $\demandofj{j'} \ge \capacityU$. Then, $\demandofj{j'} = \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k} + \capacityU  (\primezofi{i} + \primezofi{i'}) \le \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k}  + %\textcolor{magenta}{(1+1/\ell)} 
    (2-1/\ell) \capacityU  \primezofi{i} \le %\textcolor{magenta}{(1+1/\ell)} 
    (2-1/\ell) \capacityU \sum_{k \in \bundle{j'} \setminus \{i'\}} \primezofi{k} = %\textcolor{magenta}{(1+1/\ell)} 
    (2-1/\ell) \capacityU \sum_{k \in \bundle{j'}} \hat{z}_k$. There is no increase in cost as we have only (possibly) shut down one of the facilities. Also, $\demandofj{j'} \geq \B \sum_{i \in \bundle{j'}} \primezofi{i} > \B \sum_{i \in \bundle{j'}} \hat{z}_{i}$ as $\sum_{i \in \bundle{j'}} \primezofi{i} > \sum_{i \in \bundle{j'}} \hat{z}_{i}$.
    

    \item $\primezofi{i'} %\textcolor{magenta}{ \geq 1/\ell} 
    > 1-1/\ell$ %($1/2$ for Theorem 2.2)
    : Open $i'$ integrally at a loss of factor %$\textcolor{magenta}{\ell}$ 
    $(\ell/\ell-1)$ in facility opening cost i.e., $\sum_{i \in \bundle{j'}} f_i \hat{z}_i \le %\textcolor{magenta}{\ell} 
    (\ell/\ell-1) \sum_{i \in \bundle{j'}} f_i \primezofi{i}$ and $(1-1/\ell)$ factor in lower bound, i.e., $\demandofj{j'} \geq \B \sum_{k \in \bundle{j'}} \primezofi{k} \geq \B \frac{\ell-1}{\ell} \sum_{k \in \bundle{j'}} \hat{z}_{k}$,  where the second inequality follows because $\sum_{i \in \bundle{j'}} \hat{z}_i \leq \frac{\ell}{\ell-1}\sum_{i \in \bundle{j'}} z'_i$. Also,  $\demandofj{j'} = \capacityU \sum_{i \in \bundle{j'}} \primezofi{i} < \capacityU \sum_{i \in \bundle{j'}} \hat{z}_{i}$ as $\sum_{i \in \bundle{j'}} \primezofi{i} < \sum_{i \in \bundle{j'}} \hat{z}_{i}$.
\end{enumerate}\end{proof}

%Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{(1+1/\ell)\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = (1 + 1/\ell) \capacityU \hat{z}_i$ , where the first inequality follows by Lemma (\ref{integral_dense}). 


%\textcolor{cyan}{SAPNA, Revisit the next para later:}

%\textcolor{red}{
%Replace $1 - 1/\ell$ by $1/2$ in Lemma 2.6 to obtain the result for Theorem 2.2.
%}
Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{%\textcolor{magenta}{(1+1/\ell)} 
(2-1/\ell)\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = %\textcolor{magenta}{(1+1/\ell)} 
(2-1/\ell) \capacityU \hat{z}_i$, where the first inequality follows by Lemma (\ref{integral_dense}). Also, $l_i  = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \geq \hat{z}_i \frac{\demandofj{j'}}{\frac{\ell}{\ell-1}\sum_{i \in \bundle{j'}} z'_i} = \hat{z}_i \frac{\demandofj{j'}}{\frac{\ell}{\ell-1}\sum_{i \in \bundle{j'}} z_i} \geq  \hat{z}_i \frac{\B \sum_{i \in \bundle{j'}} z_i}{\frac{\ell}{\ell-1}\sum_{i \in \bundle{j'}} z_i} = \frac{\ell-1}{\ell} \B \hat{z}_i$, where the first inequality follows because $\sum_{i \in \bundle{j'}} \hat{z}_i \leq \frac{\ell}{\ell-1}\sum_{i \in \bundle{j'}} z'_i$.

A solution is said to be an integrally opened solution if all facilities in it are opened to an extent of either $1$ or $0$. We next obtain such a solution to LBUBFL problem.

\begin{lemma} \label{Dense1}
We can obtain an integrally opened solution $<\bar x, \bar y>$ to LBUBFL problem at a loss of %\textcolor{magenta}{($1+1/\ell$)} 
$(2-1/\ell)$ in upper bounds and $(1-1/\ell)$ in lower bounds whose cost is bounded by %\textcolor{magenta}{$(2\ellone^2 + 3\ellone + 2)$} 
$(10\ellone + 4)LP_{opt}$.
\end{lemma}

\begin{proof}
For $j' \in \csparse$, set $\bar y_i = \hat{y}_i,~\bar{x}_{ij} = \hat{x}_{ij}~\forall i \in \bundle{j'}, j \in \clientset$. The violation in lower bound and the following cost bound then follows from Lemma (\ref{Sparse}).

\begin{equation}
\label{cost-of-sparse}
\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \bar{y}_i + \sum_{j \in \clientset} \bar{x}_{ij} \dist{i}{j}) \le \sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})].
\end{equation}



Next let $j' \in \cdense,~i \in \bundle{j'}, j \in \clientset$. Set $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. %\textcolor{cyan}{The violation in lower bound then follows from Lemma (\ref{Sparse}) and (\ref{integral_dense}).}
Consider $ \sum_{j \in \clientset} \bar{x}_{ij} = \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} = l_i \leq   %\textcolor{magenta}{(1+1/\ell)} 
(2-1/\ell)\capacityU \hat{z}_i = %\textcolor{magenta}{(1+1/\ell)} 
(2-1/\ell)\capacityU \bar{y}_i$. Also, $\sum_{j \in \clientset} \bar{x}_{ij} = l_i \geq   
(1-1/\ell)\B \hat{z}_i = (1-1/\ell)\B \bar{y}_i $. Thus, the loss in upper bound and lower bound is at most %\textcolor{magenta}{($1+1/\ell$)}
$(2-1/\ell)$ and $(1-1/\ell)$ respectively.

%\textcolor{cyan}{From Lemma (\ref{Sparse}) and (\ref{integral_dense}), the violation in lower bound is $min\{1-1\ell,1/2\} > 1/2$ for $\ell>2$. Thus, $\alpha > 1/2$.}



Also,\\ 
$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij}) $\\
$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \dist{i}{j}  \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} (\dist{j}{j'} + \dist{i}{j'})$ (by triangle inequality)\\ 
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   
%\sum_{\singlefacility \in \bundle{j'}} 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ (as $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
%$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )  $ (by definition of $\loadjinc{j}{j'}$, claim (\ref{claim-2}) of Lemma (\ref{distBound}) and the fact that $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
$ \leq  %\textcolor{magenta}{\ell} 
\ell/(\ell-1) \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +    %\textcolor{magenta}{(1+1/\ell)} 
(2-1/\ell) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +  
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ \\ %(by Lemma (\ref{integral_dense}))\\
%$ \leq  \ell \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +   (1+1/\ell) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
%\textcolor{magenta}{$\leq max\{\ell, (1+1/\ell)\}$} 
$\leq  max\{\ell/(\ell-1), (2-1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\
%$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\
$\leq  %\textcolor{magenta}{\ell} 
2  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\ %\textcolor{magenta}{(for $\ell > 2$)}\\

%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\ (for $\ell > 2$)\\
$\leq %\textcolor{magenta}{\ell} 
2  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (by Lemma (\ref{integral_dense}))\\
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
$\leq  %\textcolor{magenta}{\ell} 
2 \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   
%\textcolor{magenta}{\ell} 
2  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (because $z_i = \sum_{j \in \clientset} x^*_{ij} / \capacityU \leq y^*_i$)\\ 
%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by cost bound of feasible solution $z$.....Sapna..how from this reason?)\\
%\textcolor{red}{
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ellone \C{j}) + \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$  (by claim (\ref{claim-1}) of Lemma (\ref{distBound}))\\
%}
$\leq  %\textcolor{magenta}{\ell} 
2  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  %\textcolor{magenta}{\ell} 
2 \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ell \C{j}) + \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}  (2\dist{i}{j} + 2\ell\C{j} )$ 
(by definition of $\loadjinc{j}{j'}$ and claims (\ref{claim-1}) and (\ref{claim-2}) of Lemma (\ref{distBound}))\\
$= %\textcolor{magenta}{\ell} 
2  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   %\textcolor{magenta}{2+\ell} 
4   \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} +   %\textcolor{magenta}{2\ell(1+\ell)} 
6\ell \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}   \C{j} $ \\

Summing over all $j' \in \cdense$ and adding inequality (\ref{cost-of-sparse}), we get\\
$ \sum_{i \in \facilityset} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij})$\\
$\leq max\{2, \ell/(\ell-1)\} \sum_{i \in \facilityset}  f_i y^*_i + %\textcolor{magenta}{ max\{4,(2+\ell)\}} 
4 \sum_{i \in \facilityset}\sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + %\textcolor{magenta}{\ellone~ max\{4,2(1+\ell)\}} 
10 \ell \sum_{i \in \facilityset}\sum_{j \in \clientset} x^*_{ij} \C{j}$\\
% \textcolor{magenta}{ $= \sum_{i \in \facilityset}  f_i y^*_i + (2+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + 2\ell(1+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\ell > 2$)}\\
  
$ \leq 2 \sum_{i \in \facilityset}  f_i y^*_i + 4\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + 10\ell \sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\ell \geq 2$)\\
$ \leq %\textcolor{magenta}{(2\ellone^2 + 3\ellone + 2)}
(10 \ell+4)LP_{opt}$.
\end{proof}


Theorem~\ref{TricriteriaResult} is obtained by solving a min-cost flow problem with relaxed lower  and upper bounds to obtain the integral assignments.

%\textcolor{red}{To obtain Theorem 2.2 we make the following minor modifications: In sparse clusters, we choose $\ell > 2$ so that we get $\alpha > 1/2$. In the dense clusters, we make the following modifications while converting an almost integral solution to an integral solution in the proof of Lemma 2.6: close $i'$ in $\hat z$ if $\primezofi{i'} \le 1/2$ and distribute the assignment coming onto it to the other opened facilities in the cluster at a loss of $3/2$ in the upper bound else open $i'$. Claimed bounds can be shown to hold in the same way.}

%\textcolor{cyan}{ For $\ell = 2.01$, we get an approximation ratio of less than $25$.}
For $\ell = 2.01$, we get $\alpha > 1/2$, $\beta$  slightly more than $3/2$ and the approximation ratio less than $25$. $\beta$ can be reduced to $3/2$ by a slight modification in obtaining an integral solution $\hat z$ from an almost integral solution $\primezofi{}$ in Lemma~(\ref{integral_dense}): instead of comparing $\primezofi{i'}$ with $(1 - 1/\ell)$, we compare it with $1/2$.
%The violations in the lower and the upper bounds can be made arbitrarily close to $0$ at the cost of increase in the approximation ratio.

Let $S^t$ be the solution so obtained with $\alpha > 1/2$, $\beta = 3/2$ . %and violations in lower and upper bounds be denoted by $\alpha$ and $\beta$ respectively.
Then, $Cost_I(S^t) \le %\textcolor{magenta}{(2\ellone^2 + 3\ellone + 2)}
O(1)Cost_I(O)$,
where $O$ is an optimal solution to $I$. %., $\textcolor{cyan}{\alpha= (1 - 1/\ellone)} %\textcolor{cyan}{\alpha >1/2}$ and $\textcolor{magenta}{\beta= (1 + 1/\ellone)} \textcolor{cyan}{\beta= (2-1/\ell)}$. 
%To obtain integral assignments, we solve a minimum-cost integer flow problem with relaxed lower  and upper bounds.
%
	Next, using $S^t$, we transform the instance $I$ to an instance $I_{cap}$ of capacitated facility location problem by swapping the roles of clients and facilities. This is done via a series of transformations from instance $I$ to $I_1$, 	$I_1$ to $I_2$ and $I_2$ to $I_{cap}$. The key idea is to create  $\B - n_i$ units of demand, where the number $n_i$ of clients served by facility $i$ in $S^t$ is short of the lower bound and create  $n_i - \B$ units of supply at locations where $n_i > \B$.
	


==> NEW Journal version WADS 2021 (LBUBFL)/abstract.tex <==
\begin{abstract}
With growing emphasis on e-commerce marketplace platforms where we have a central platform mediating between the seller and the buyer, it becomes important to keep a check on the availability and profitability of the central store. A store serving too less clients can be non-profitable and a store getting too many orders can lead to bad service to the customers which can be detrimental for the business.
In this paper, we study the facility location problem(FL) with upper and lower bounds on the number of clients an open facility serves. 
Constant factor approximations are known for the restricted variants of the problem with only the upper bounds or only the lower bounds. The only work that deals with bounds on both the sides violates both the bounds \cite{friggstad_et_al_LBUFL}.
In this paper, we present the first (constant factor) approximation for the problem violating the upper bound by a factor of 
%\textcolor{magenta}{$(2 + \epsilon)$}
$(5/2)$ without violating the lower bounds when both the lower and the upper bounds are uniform.  
We first give a tri-criteria (constant factor) approximation violating both the upper and the lower bounds and 
then get rid of violation in lower bounds by transforming the problem instance to an instance of capacitated facility location problem. %\textcolor{red}{Binary facility trees are used to check the violations in the upper bounds.} 
%\textcolor{cyan}{Facility trees are constructed to get rid of the violations in the lower bounds.}

%\keywords{ Facility Location  \and Lower Bounds \and Upper Bounds \and Approximation.}
\end{abstract}

==> NEW Journal version WADS 2021 (LBUBFL)/macro_AP.tex <==
% % % % Problem Instances % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
\newcommand{\UKMPI}{(\clientset, ~\facilityset,~\textit{c},~\textit{f},~\capacity, ~\budget)}			% % % sapna
\newcommand{\InstanceUKMP}{(\clientset, ~\facilityset,~\textit{c},~\textit{f},~\capacity, ~\budget)}	% % % aditya

\newcommand{\UkFLPI}{(\clientset,~\facilityset,~\textit{c},~\textit{f},~\capacity,~k)}					% % % sapna
\newcommand{\InstanceUKFLP}{(\clientset,~\facilityset,~\textit{c},~\textit{f},~\capacity,~k)}			% % % aditya
\newcommand{\UFLPI}{(\clientset,~\facilityset,~\textit{c},~\textit{f},~\capacity)}	

\newcommand{\starinst}[5]{\mathcal{#1}_{#2}(#2,~#3,~#4,~#5)}	

\newcommand{\starinstflp}[4]{\mathcal{#1}_#2(#2,~#3,~#4)}												% % % sapna
\newcommand{\InstanceSTAR}[5]{\mathcal{#1}_#2(#2,~#3,~#4,~#5)}											% % % aditya

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %


% % % % % % % %  maths and fancy stuff % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %

\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}			% % % aditya (not used)

\newcommand{\thetajjp}[2]{\theta({#1},{#2})}

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %



% % % % Problem Name  % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
\newcommand{\LPUKMP}{\textbf{LP(UKMP)}}			% % % sapna

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %




% % % % Sets, Constants and related stuff % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\newcommand{\facilityset}{\mathcal{F}}	
\newcommand{\facilitysetone}{\mathcal{F}^1}	
\newcommand{\facilitysettwo}{\mathcal{F}^2}		% % % sapna
\newcommand{\facset}{\mathcal{F}}				% % % aditya
\newcommand{\opfacset}{\mathcal{A}}	
\newcommand{\opfacsettwo}{\mathcal{A}^2}	
\newcommand{\temp}{\mathcal{T}}	

\newcommand{\clientset}{\mathcal{C}}			% % % sapna
\newcommand{\cliset}{\mathcal{C}}				% % % aditya

\newcommand{\si}[1]{\mathcal{S}_#1}				% % % sapna
\newcommand{\sset}[1]{\mathcal{S}_#1}			% % % aditya

\newcommand{\budget}{\mathcal{B}}
\newcommand{\budgetone}{\mathcal{B}^1}
\newcommand{\budgettwo}{\mathcal{B}^2}				% % % sapna
\newcommand{\budgetset}[1]{\mathcal{B}_{#1}}

\newcommand{\capacity}{\textit{u}}				% % % sapna
\newcommand{\capacityU}{\mathcal{U}}				% % % aditya

\newcommand{\crich}{\mathcal{C}_D}				% % % sapna		Dense Clusters
\newcommand{\cpoor}{\mathcal{C}_S}				% % % sapna		Sparse Clusters
\newcommand{\cdense}{\mathcal{C}_D}				% % % aditya
\newcommand{\csparse}{\mathcal{C}_S}
\newcommand{\csparseprime}{\mathcal{C}'_S}
\newcommand{\csparsetilde}{\mathcal{\tilde{C}}_S}
\newcommand{\csparsegroup}[1]{\mathcal{C}_{S,#1}}
\newcommand{\facilitysetgroup}[1]{\mathcal{F}_{#1}}
\newcommand{\csone}{\mathcal{C}_S^1}		
\newcommand{\cstwo}{\mathcal{C}_S^2}
\newcommand{\cdone}{\mathcal{C}_D^1}	% % % sapna

			% % % aditya
\newcommand{\cdensegood}{\mathcal{C}^D_{Good}}	% % % aditya
\newcommand{\cdensebad}{\mathcal{C}^D_{Bad}}	% % % aditya
\newcommand{\cminusl}{\mathcal{\tilde{C}}}	
\newcommand{\csparseminusl}{\mathcal{\tilde{C}_S}}

\newcommand{\cdensegoodname}{\textit{Good Dense}}	% % % aditya
\newcommand{\cdensebadname}{\textit{Bad Dense}}		% % % aditya
\newcommand{\csparsename}{\textit{Sparse}}
\newcommand{\cdensename}{\textit{Dense}}

\newcommand{\csparseplusbad}{\overline{\mathcal{C}}}		% % % aditya
\newcommand{\leafnodes}{\mathcal{L}}		% % % sapna

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 





% % % % Balls and Clusters and related stuff  % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %

\newcommand{\ballofj}[1]{\textit{$\mathcal{B}( #1 $)}} 	% % % sapna
\newcommand{\ball}[1]{\textit{ball($ #1 $)}} 		% % % aditya

\newcommand{\C}[1]{\hat{C_{#1}}}					% % % sapna
\newcommand{\hatofC}[1]{\hat{C_{#1}}}				% % % aditya
\newcommand{\hatof}[2]{\hat{{#1}_{#2}}}				% % % aditya

\newcommand{\bundle}[1]{\mathcal{N}_{#1}}			% % % sapna
\newcommand{\neighbor}[1]{\mathcal{N}_{#1}}
\newcommand{\p}[1]{\mathcal{N}_{#1}}
			% % % aditya
\newcommand{\nnew}[1]{\mathcal{N}'_{#1}}

\newcommand{\R}[1]{\mathcal{R}_{#1}}					% % % aditya
\newcommand{\Njincbar}[1]{\delta({#1})}				% % % aditya
\newcommand{\T}[1]{\tau({#1})}
\newcommand{\Tp}[1]{\mathcal{T}'({#1})}
\newcommand{\TC}{\mathcal{TC}}

\newcommand{\cen}[1]{G_{#1}}
\newcommand{\sj}[1]{\mathcal{S}_{#1}}
\newcommand{\s}{\mathcal{S}}	
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %





% % % %  distance, costs and related stuff  % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
\newcommand{\dist}[2]{c(#1,~#2)}
\newcommand{\dists}[2]{c_{s}(#1,~#2)}					% % % sapna

\newcommand{\facilitycost}{\textit{$ f_i $}}		% % % sapna
\newcommand{\faccosti}{\textit{$ f_i $}}			% % % aditya
\newcommand{\faccost}[1]{\textit{$ f_#1 $}}			% % % aditya

\newcommand{\A}[2]{\mathcal{A}_{\rho^*}(#1,{#2})}						% % % aditya

\newcommand{\x}[3]{x_{#1}(#2,#3)}					% % % sapna
\newcommand{\X}[2]{x_{#1#2}}						% % % aditya
\newcommand{\Xstar}[2]{x^*_{#1#2}}					% % % aditya

\newcommand{\bard}[1]{{d_{#1}}}			% % % aditya

\newcommand{\hatofbjc}[1]{\hat{b}^c_{#1}}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}	

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %






% % % % Summations % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
\newcommand{\sumlimits}[2]{\displaystyle\sum\limits_{#1}^{#2}}												% % % aditya
\newcommand{\unionlimits}[2]{\displaystyle\bigcup\limits_{#1}^{#2}}

\newcommand{\sumofx}[1]{\sum_{#1 \in \clientset} x_{i#1}}													% % % sapna
\newcommand{\sumxoverclients}[2]{\displaystyle\sum\limits_{#2 \in \clientset} x_{#1#2}}						% % % aditya

\newcommand{\sumxioverclients}[1]{\displaystyle\sum\limits_{#1 \in \clientset} x_{i#1}}						% % % aditya
\newcommand{\sumofvaronf}[2]{\sum_{i \in \facilityset'} #1_{#2j}}											% % % sapna

\newcommand{\sumap}[1]{\sum_{#1}{}} % % %aditya

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %



\newcommand{\price}[1]{b^c_{#1}}
\newcommand{\pricef}[1]{b^f_{#1}}
\newcommand{\budgett}[1]{b_{#1}}

\newcommand{\load}[1]{l_{#1}}


\newcommand{\mass}[2]{size(#1,#2)}
%\newcommand{\mass}[1]{size(#1,#2)}
\newcommand{\Load}[1]{load(#1)}
\newcommand{\massofbundle}[3]{\sum_{#1 \in #2}{} #3_#1}
\newcommand{\FC}[1]{\sum_{\singlefacility \in \facilityset} \facilitycost  #1_i}
\newcommand{\FCofbundle}[3]{\sum_{#1 \in #2} f_#1 #3_#1}
\newcommand{\CC}[1]{\sum_{\singlefacility \in \facilityset} \sum_{j \in \clientset} \dist{i}{j} #1_{ij}}
\newcommand{\CCa}{\sum_{i,j} \demandofj{j} \dist{i}{j}}

\newcommand{\CCofBundle}[1]{\sum_{i \in \facilityset} \dist{#1}{j} x^*_{#1j}}
\newcommand{\kmed}{\textit{k}}     

\newcommand{\singleclient}{\textit{j}}
\newcommand{\singlefacility}{\textit{i}}
\newcommand{\demand}[1]{\tilde{l_{#1}}}
\newcommand{\hatofdemand}[1]{\hat{l_{#1}}}
\newcommand{\zofi}[1]{z_#1}
\newcommand{\hatzofi}[1]{\hat{z}_#1}
\newcommand{\primezofi}[1]{z'_{#1}}
\newcommand{\tildezofi}[1]{\tilde{z}_#1}
%\newcommand{\g}[2]{g_{#1}{#2}}


% client set bundle is the modifed macro
\newcommand{\clientsetbundle}[1]{\mathcal{C}^{#1}}
\newcommand{\radiusballofj}{\dist{i}{j} \leq 2 \C{j} }
% NEw Macros - Dipti -09/03/2016
\newcommand{\demandofj}[1]{\textit{$ d_{#1} $}}
\newcommand{\neighbourhood}[1]{\mathbb{N}(#1)}
\newcommand{\shtree}{\cal{F}}
\newcommand{\BCtree}{\hat{\cal{F}}}
\newcommand{\CCLPtwo}[1]{\sum_{i \in \facilityset',j \in \clientsetbundle{'}} \demandofj{j} \dist{i}{j}  #1_{ij}}
\newcommand{\priceofcorf}[2]{b_{#1}^{#2}}
\newcommand{\hatofy}[1]{\hat{y_#1}}
\newcommand{\hatofx}[2]{\hat{x}_{#1#2}}
\newcommand{\barofclientsetbundle}{\bar{\mathcal{C}}}

\newcommand{\obj}[1]{\mathcal{C}ostKM(#1)} 
\newcommand{\objflp}[1]{\mathcal{C}ostkFLP_{sp}(#1)} 
\newcommand{\objflpSD}[1]{\mathcal{C}ostkFLP(#1)} 

\newcommand{\Costone}[1]{Cost^1(#1)}
\newcommand{\Costtwo}[1]{Cost^2(#1)}
\newcommand{\cost}[2]{Cost_{#1}(#2)} 
\newcommand{\sigmabar}{\bar{\sigma}}
\newcommand{\sigmahat}{\hat{\sigma}}
\newcommand{\costsingle}[1]{Cost(#1)}
\newcommand{\costjprimeinc}[3]{Cost_{#1}(#2,~#3)}
\newcommand{\loadjinc}[2]{\phi(#1,~#2)}

\newcommand{\costFLPThree}[3]{Cost_{#1}(#2,~#3)}
\newcommand{\costtwo}[2]{Cost(#1,~#2)}
\newcommand{\costthree}[3]{Cost_{#1}(#2,~#3)}
\newcommand{\costFLPFour}[4]{Cost_{#1}(#2,~#3,~#4)}
\newcommand{\cardTwo}[1]{Y^*(#1)}
\newcommand{\totalcost}[2]{Cost(#1,~#2)}
% new macros-19042016-21:11
\newcommand{\etal}{\textit{et al}.}
\newcommand{\ie}{\textit{i}.\textit{e}.}
\newcommand{\eg}{\textit{e}.\textit{g}.}
\newcommand{\Cost}[1]{Cost(#1)}


%BY Sapna 16042017
\newcommand{\soner}[1]{s^1_{#1}}
\newcommand{\stwor}[1]{s^2_{#1}}
\newcommand{\Soner}[1]{S^1_{#1}}
\newcommand{\Stwor}[1]{S^2_{#1}}

%By neelima begins
\newcommand{\mcone}[1]{G^1_{#1}}
\newcommand{\mctwo}[1]{G^2_{#1}}
\newcommand{\denser}[1]{j_{d_{#1}}}
\newcommand{\dense}{j_d}
\newcommand{\sparseoner}[1]{j_{s1_{#1}}}
\newcommand{\sparseone}{j_{s}}
\newcommand{\sparsetwor}[1]{j_{s2_{#1}}}
\newcommand{\sparsetwo}{j_{s2}}
\newcommand{\That}[1]{\hat{\tau}({#1})}
\newcommand{\muj}[1]{\mu({#1})}
\newcommand{\resj}[1]{res({#1})}
\newcommand{\floordjbyu}[1]{\lfloor{d_{#1}/u}\rfloor}
% by neelima ends

\newcommand{\tauhat}[1]{\hat{\tau}({#1})}


%by sapna 30-07-17
\newcommand{\sone}{S_1}
\newcommand{\stwo}{S_2}
\newcommand{\sthree}{S_3}
\newcommand{\Gralpha}{G_{r_\alpha}}
\newcommand{\Grbeta}{G_{r_\beta}}


%10 July 2018
\newcommand{\sigmaone}{\psi}
\newcommand{\sr}[1]{s_{#1}}
\newcommand{\Sr}[1]{S_{#1}}

%rd
\newcommand{\B}{\mathcal{B}}

%rajni
\newcommand{\clirem}{\mathcal{C}_r}
\newcommand{\clipen}{\mathcal{C}_p}
\newcommand{\cliout}{\mathcal{C}_o}
\newcommand{\opt}[1]{LP_{opt}}
\newcommand{\lp}[1]{LP_{#1}}
\newcommand{\scost}{Cost_s}
\newcommand{\pcost}{Cost_p}
\newcommand{\fcost}{Cost_f}

\newcommand{\MC}{Meta-Cluster }
\newcommand{\MCs}{Meta-Clusters }

%NG 14 Feb 2021
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{definition}[theorem]{Definition}
\newcommand{\rhobar}{\bar\rho}
\newcommand{\cone}{y}

%ng April 2021
\newcommand{\ellone}{\ell}

\newcommand{\rootpair}{<r_1, r_2>}

==> NEW Journal version WADS 2021 (LBUBFL)/temp.tex <==
\begin{comment}
\textcolor{blue}{
\begin{proof}
Let $i \in \bundle{j'}, j \in \clientset$. Recall that $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. Consider the cost of the solution:\\ 
$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij}) $\\
$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \dist{i}{j}  \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} (\dist{j}{j'} + \dist{i}{j'})$ (by triangle inequality)\\ 
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ell \C{j} + \dist{i}{j'})  $ (by definition of $\loadjinc{j}{j'}$)\\ 
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  2 \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \C{j} +$\\
$\sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \dist{i}{j'} $\\
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  2  \sum_{j \in \clientset} \sum_{i' \in \bundle{j'}} x^*_{i'j}   \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \C{j} + \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} $ (because $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i + \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j} $\\
$ \leq  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +  (1+\epsilon) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j} \primezofi{i} +  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j}$ (by Lemma (\ref{integral_dense}))\\
$\leq max\{(1/\epsilon), (1+\epsilon)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} ++  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j}$\\
$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j}$ (for $\epsilon< 1/2$)\\
$= (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j}$ (by Lemma (\ref{integral_dense}))\\
$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   (1/\epsilon)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} +  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j}$ (by cost bound of feasible solution $z$)\\
$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   (1/\epsilon)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ell \C{j}) +  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j}$\\
$= (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+ (1/\epsilon))  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} + 2\ell(1+1/\epsilon) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} $ \\
%$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i + \dist{i}{j'} \sum_{j \in \clientset} \bar{x}_{ij}) $\\
%$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
%$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} l_i$\\ 
%$ \leq  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +  (1+\epsilon) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i}$\\
%$\leq max\{(1/\epsilon), (1+\epsilon)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i}$\\
%$= (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i}$ for $\epsilon< 1/2$\\
%$ =  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU  \dist{i}{j'}) z_i$\\
%$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   (1/\epsilon)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij}$\\
%$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} x^*_{ij} [ \dist{i}{ j} + 2\ell \C{j} ]$.
\end{proof}
}
	\end{comment}
	
	
	\begin{lemma}
TBD: We can obtain an integrally opened solution $<\tilde x, \tilde y>$ to LBUBFL problem such that the sum of facility opening costs and the cost of assignment to the opened facilities is bounded by $(2\ellone^2 + 3\ellone + 2)LP_{opt}$. The solution violates the lower bound by a factor of $(1 - 1/\ellone)$  and upper bound by a factor of $(1 + 1/\ellone)$.
\end{lemma}
\begin{proof}
%For a sparse cluster $\bundle{j'}$ centered at $j'$, set $\tilde y_i=\hat{y}_i$ and $\tilde x_{ij} = \hat{x}_{ij}~\forall i \in \bundle{j'}, j \in \clientset$. If  $\bundle{j'}$ is a dense cluster centered at $j'$, then 
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. Set $\tilde y_i=\bar{y}_i$ and $\tilde x_{ij} = \bar{x}_{ij}$. The violation in lower and upper bound follows from Lemma (\ref{Sparse}) and  Lemma (\ref{Dense}) respectively.
Summing the cost bound of Lemma (\ref{Sparse}) over all sparse clusters and that of Lemma (\ref{Dense}) over all dense clusters, the total cost of the tri-criteria solution is:\\
%\textcolor{magenta}{Summing the cost bound of Lemma (\ref{Sparse}) over all sparse clusters and that of Lemma (\ref{Dense}) over all dense clusters, the total cost of the tri-criteria solution is: SApna...will have to see the language...I have already summed in Lemma  2.3 I guess...should have the same format in Lemma 2.7 ..and make change in the language here accordingly....will see tomorrow}
$\leq max\{\ell, \ell/(\ell-1)\} \sum_{j' \in \clientset'} \sum_{i \in \bundle{j'}} f_i y^*_i +  max\{4,(2+\ell)\} \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + \ellone~ max\{4,2(1+\ell)\} \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \C{j}$\\
$= (\ell) \sum_{j' \in \clientset'} \sum_{i \in \bundle{j'}} f_i y^*_i +  (2+\ell) \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} $\\
$+ 2\ell(1+\ell) \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\ell \geq 2$)\\
$ \leq (2\ellone^2 + 3\ellone + 2)LP_{opt}$.

%\textcolor{green}{ $ \le (2\ellone^2 + 3\ellone + 2)LP_{opt}$ ...Sapna..verify this..is it ok?}

%TBD: Choose $\ellone = \floor{1/\epsilon}$, then the cost of the solution is bounded by $(2\ellone ^2 + 3\ellone + 2)LP_{opt}$. For $\epsilon \le 1/2, \ellone \ge 2$. 
\end{proof}


\begin{lemma} \label{Dense}
We can obtain an integrally opened solution $<\bar x, \bar y>$ at a loss of ($1+1/\ell$) in upper bounds and ($1-1/\ell$) in lower bounds, such that the sum of facility opening costs and the cost of assignment to the opened facilities in dense clusters is bounded by\\
 $ \sum_{j' \in \cdense} \left[ \ellone \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+ \ellone)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} + 2\ellone (1 + \ellone) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} \right]$ and that in sparse clusters is bounded from Lemma (\ref{Sparse}).
%For a fixed $0<\epsilon< 1/2$, the cost of the solution $<\bar x, \bar y>$ corresponding to a dense cluster centered at $j'$ is bounded by $ (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+ (1/\epsilon))  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} + 2\ellone(1+1/\epsilon) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} $.
\end{lemma}

\begin{proof}
Let $\bundle{j'}$ is a sparse cluster centered at $j'$, then set $\bar y_i = \hat{y}_i,~\bar{x}_{ij} = \hat{x}_{ij}~\forall i \in \bundle{j'}, j \in \clientset$. The violation in lower bound and cost bound for sparse clusters then follows directly from Lemma (\ref{Sparse}). %Next, let $\bundle{j'}$ be dense cluster centered at $j'$.  
Let $j' \in \cdense,~i \in \bundle{j'}, j \in \clientset$. Set $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. 
Consider $ \sum_{j \in \clientset} \bar{x}_{ij} = \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} = l_i \leq (1+1/\ell)\capacityU =  (1+1/\ell)\capacityU \hat{z}_i = (1+1/\ell)\capacityU \bar{y}_i$. Thus, the loss in capacities is at most ($1+1/\ell$).
Consider the cost of the solution:\\ 
$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij}) $\\
$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \dist{i}{j}  \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} (\dist{j}{j'} + \dist{i}{j'})$ (by triangle inequality)\\ 
\textcolor{red}{
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'}) $ (as $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
}
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )  $ (by definition of $\loadjinc{j}{j'}$, claim (\ref{claim-2}) of Lemma (\ref{distBound}) and the fact that $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
\textcolor{red}{$ \leq  \ell \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +   (1+1/\ell) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j} \primezofi{i} +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'}) $ (by Lemma (\ref{integral_dense}))\\}
$ \leq  \ell \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +   (1+1/\ell) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j} \primezofi{i} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
\textcolor{red}{
$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$ \\
}
$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\
\textcolor{red}{
$\leq \ell \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +   \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$ \\ (for $\ell \geq 2$)\\
}
$\leq \ell \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\ (for $\ell \geq 2$)\\
\textcolor{red}{
$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$ (by Lemma (\ref{integral_dense}))\\
}
$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
\textcolor{red}{
$\leq \ell \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$ \\
}
$\leq \ell \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by cost bound of feasible solution $z$.....Sapna..how from this reason?)\\
%\textcolor{red}{
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ellone \C{j}) + \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$  (by claim (\ref{claim-1}) of Lemma (\ref{distBound}))\\
%}
$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ellone \C{j}) + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \textcolor{red}{ 
(by definition of $\loadjinc{j}{j'}$ and claims (\ref{claim-1}) and (\ref{claim-2}) of Lemma (\ref{distBound}))
}\\
$=\ell  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+\ell)   \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} +  2\ell(1+\ell) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} $ \\

\end{proof}


==> TriCriteria.tex <==
\section{Computing the Tri-criteria Solution}
\label{tri-criteria}
 %We use a simpler LP-rounding technique to get $(\frac{\ellone-1}{\ellone})$-factor violation in lower bounds and $2$-factor violation in upper bounds at constant factor loss in cost. The technique used is much simpler than Friggstad et al. \cite{friggstad_et_al_LBUFL} because lower bounds are uniform in our case unlike Friggstad et al. that considers non-uniform lower bounds. 
 \textcolor{red}{
 In this section, we give a tri-criteria solution that violates the lower bound by a factor of $\alpha = (1 - \theta)$ and the upper bound by a factor of $\beta = (1 + \theta)$ where $\theta \le 1/2$ is a tune-able parameter.
 }
Instance $I$ of LBUBFL can be formulated as the following integer program (IP):

\label{{unif-CFLP}}
$Minimize ~\mathcal{C}ostLBUBFL(x,y) = \sum_{j \in C}\sum_{i \in F}\dist{i}{j}x_{ij} + \sum_{i \in F}f_iy_i $
\begin{eqnarray}
subject~ to &\sum_{i \in F}{} x_{ij} \geq 1 & \forall ~\singleclient \in C \label{LPFLP_const1}\\ 
%&\sum_{j \in C}{} x_{ij} \leq \capacityU ~ y_i & \forall~ \singlefacility \in F \label{LPFLP_const2}\\ 
& \capacityU y_i \geq \sum_{j \in C}{} x_{ij} \geq \B y_i & \forall~ \singlefacility \in F \label{LPFLP_const3}\\
& x_{ij} \leq y_i & \forall~ \singlefacility \in F , ~\singleclient \in C \label{LPFLP_const4}\\   
& y_i,x_{ij} \in \left\lbrace 0,1 \right\rbrace  \label{LPFLP_const5}
\end{eqnarray}
where  $y_i$ is an indicator variable which is equal to $1$ if facility $i$ is open and is $0$ otherwise. $x_{ij}$ is an indicator variable which is equal to $1$ if client $j$ is served by facility $i$ and is $0$ otherwise.
 Constraints \ref{LPFLP_const1} ensure that all the clients are served. %Constraints \ref{LPFLP_const2} make sure that the total demand assigned to an open facility is no more than its capacity \capacityU. 
 Constraints \ref{LPFLP_const3} make sure that the total demand assigned to an open facility is at least $\B$ and at most $\capacityU$. Constraints \ref{LPFLP_const4} ensure that a client is assigned to a facility only if it is opened. LP-Relaxation  is obtained by allowing the variables to be non-integral.
% $ y_i, x_{ij} \in [0, 1]$. %Call it LP. 
Let $\zeta^{*} = <x^*, y^*>$ be an optimal solution  and $\opt{}$ be its cost.

TBD: In this section, we give a tri-criteria solution that violates the lower bound by a factor of $(\ellone-1)/\ellone$ for a fixed parameter \textcolor{blue}{$\ellone \geq 2$} and the upper bounds by a factor of $2$.

We start by sparsifying the problem instance by removing some clients and distributing their demands to the remaining clients. This is done using clustering technique in the same manner as is done in Grover \etal~\cite{GroverGKP18}: for $j \in C$, let $ \C{j} $ denote the average connection cost paid by $\singleclient$ in $\zeta^*$. 
%i.e., ~$\C{j} = (\sum_{i \in F}{} {x}^*_{ij} \dist{i}{j})/({\sum_{i \in F}{} {x}^*_{ij}})$. 
Further, let \textcolor{blue}{$\ellone \geq 2$} be a fixed parameter and let $\ballofj{j}$ be the ball of facilities within a radius of $\ellone\C{j}$ of $j$.
%~ i.e., \ \ballofj{j}  = \{ \singlefacility \in F \colon \dist{i}{j} \leq \ellone \C{j} \}$.
Then,  $\cardTwo{\ballofj{j}} \ge (1-\frac{1}{\ellone})$ where $\cardTwo{\ballofj{j}}$
%$=  \sum_{i \in \ballofj{j}} y^*_i$ 
denotes the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
The balls 
%The clients 
are processed in the non-decreasing order of their radii dissolving the overlapping balls of larger radii and removing their (client) centers. The process is repeated with the remaining balls. Let $C'$ be the set of  clients remaining at the end of the process. The set of facilities that do not belong to ball of any client in $C'$ are partitioned so as to form clusters around the remaining balls, by assigning them to the cluster of $j'$ where $j'$ is nearest to the facility amongst all $j' \in C'$. %the nearest cluster center.
%Clusters of the remaining facilities are formed around the remaining balls by assigning them to the cluster of the nearest cluster center.
%For a client $j$ at hand, remove all the clients 
%$k : \dist{j}{k} \le 2 \ellone \max \{\C{j}, \C{k}\}$ 
%whose balls overlap with that of $j$ and repeat the process with the remaining clients. Let $C'$ be the set of  clients remaining after all the clients in $C$ have been considered. Clusters, of facilities, are formed around the  clients in $ C'$ by assigning a facility to the cluster of the nearest client in $C'$, i.e. if, for $j' \in C'$, $\bundle{j'}$ denotes the cluster centered at $j'$ then a facility $i$ belongs to $\bundle{j'}$ if and only if $j'$ is the closest client in $C'$ to $i$. Note that $\ballofj{j'} \subseteq \bundle{j'}$.
%
%$\cardTwo{\hat{y}}{\ballofj{j}} \ge (1-\frac{1}{\ellone})(\sum_{i \in F} \hat{x}_{ij}) \geq \frac{1}{2\ellone}$ where $\cardTwo{\hat{y}}{\ballofj{j}} =  \sum_{i \in \ballofj{j}} \hat{y}_i$ denotes the total extent up to which facilities in \ballofj{j} are opened under $\hat{\zeta}$. 
The clients in $C'$ are then called the cluster centers.

\begin{Observation}
Any two cluster centers $j', k'$ in $C'$ satisfy the {\em separation property}: $\dist{j'}{k'} > 2\ellone~max\{ \C{j'},\C{k'}\}$.
\end{Observation}

\begin{lemma}
Let $j' \in \clientset', j \in \clientset, i \in \bundle{j'}$. Then,
\begin{enumerate}
    \item $\dist{i}{j'}  \leq \dist{i}{j} + 2\ellone \C{j}$
    \item $\dist{j}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}  $
\end{enumerate}
\end{lemma}

\begin{proof}
\begin{enumerate}
    \item \textcolor{blue}{Note that, for an arbitrary client $j$,  $\dist{j}{k'} \leq 2\ellone \C{j}$ for some $k' \in \clientset'$. Then we have $\dist{i}{j'} \leq \dist{i}{k'} \leq \dist{i}{j} + \dist{j}{k'} \leq \dist{i}{j} + 2\ellone \C{j}$, where the first inequality follows because $i$ belongs to $\ballofj{j'}$ and not $\ballofj{k'}$.
    \item Thus, 
    %we get the following bound~\cite{GroverGKP18}
%\begin{eqnarray} \label{Cjj'}
$\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}  $
%\end{eqnarray}
    }
\end{enumerate}
 
\end{proof}
 

\begin{figure}
    \centering
    \includegraphics[width=5cm]{Figures/Cjj'.jpg}
    \caption{$\dist{j}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$}
    \label{Cjj'}
\end{figure}

%$\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$ ~\cite{GroverGKP18}.}  

\textcolor{blue}{Next, let $\loadjinc{j}{j'}$ be the extent up to which $j$ was served by the facilities in the cluster of $j'$.}
%Demand of the clients are distributed to various cluster centers: for a client $j$ and a cluster center $j'$, let $\loadjinc{j}{j'}$ be the extent up to which $j$ was served by the facilities in the cluster of $j'$. 
%\textcolor{red}{Then $\loadjinc{j}{j'}$ extent of $j$ is moved to $j'$. The cost of doing so for all the clients is bounded by  $2(\ellone+1)$ $LP_{opt}$: note that  $\dist{j}{k'} \leq 2\ellone \C{j}$ for some $k' \in \clientset'$. Then we have $\dist{i}{j'} \leq \dist{i}{k'} \leq \dist{i}{j} + \dist{j}{k'} \leq \dist{i}{j} + 2\ellone \C{j}$, where the first inequality follows because $i$ belongs to $\ballofj{j'}$ and not $\ballofj{k'}$.  Thus, $\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$ ~\cite{GroverGKP18}.}
Let $d_{j'}= \sum_{j \in \clientset} \loadjinc{j}{j'}$. 
%\sum_{i \in \bundle{j'}}{}  \hat{x}_{ij}.$} %\loadjinc{\hat{\zeta}}{j}{\bundle{j'}}$.
We call a cluster to be $sparse$ if $d_{j'} \le  \capacityU$ and $dense$ otherwise. %\textcolor{blue}{Let $\csparse$ be the set of all sparse clusters and $\cdense$ be the set of all dense clusters.}



%Let $<\hat{x}, \hat{y}>$ be the solution so obtained, i.e., for $ j \in \clientset$, $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$. For $j' \in \crich, i \in \bundle{j'}, j \in \clientset$, $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. 


\textcolor{red}{
\begin{lemma} \label{Sparse}
We can obtain a solution $<\xhat, \yhat>$ such that  exactly one facility $i(j')$ is opened integrally in each sparse cluster centered at $j' \in \clientset'$. The solution violates the lower bound by a factor of $(1 - 1/\ellone)$ and its cost is bounded by
$\sum_{j' \in \clientset'}[\frac{\ellone}{1 - \ellone}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})]$.
\end{lemma}
}



\begin{lemma} \label{Sparse}
For each sparse cluster centered at $j' \in \clientset'$, we can open a facility $i(j')$ integrally and transfer all the assignments in the cluster to it at cost at most
$2 \sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} [\dist{i}{j} + \ellone \C{j}]$.

%the demand $\demandofj{j'}$ can be served from facility $i(j')$ in the cluster $\bundle{j'}$ such that $\sum_{j \in \clientset} \loadjinc{j}{j'} \dist{i(j')}{j}  \leq 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} [\dist{i}{j} + \ellone \C{j}]$ and  $f_{i(j')} \leq 3/2 \sum_{i \in \bundle{j'}} f_i y^*_i $.
\end{lemma}

\begin{proof}
%In a sparse cluster centered at $j'$, we open the cheapest facility, say $i(j')$, in $\ballofj{j'}$ and transfer all the assignments in the cluster onto it.
\textcolor{blue}{ %As specified above, 
Let  $i(j')$ be a cheapest facility in $\ballofj{j'}$. We open $i(j')$ and transfer all the assignments in the cluster onto it (see Figure...). Since $\cardTwo{\ballofj{j'}} \ge (1-\frac{1}{\ellone})$, lower bound is violated at most by $(1-\frac{1}{\ellone})$ and the facility cost is bounded by $\frac{\ellone}{1 - \ellone} \sum_{i \in \bundle{j'}} f_i y^*_i$. To bound the service cost, we will show that $\sum_{j \in \clientset} \loadjinc{j}{j'} \dist{i(j')}{j}  \leq 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})$: 
since $i(j') \in \ballofj{j'}$, we have $\dist{i(j')}{j'} \le \ellone \C{j'}$. 
\{TBD Thus, for an arbitrary client $j \in \clientset$ which was served by a facility $i$ in the cluster of $j'$,\} }
\textcolor{red}{ Thus, for $j \in \clientset$,
we have $\dist{i(j')}{j} \le \dist{j'}{j} + \dist{i(j')}{j'} \le  \dist{j'}{j} + \ellone \C{j'}$. If $\ellone \C{j'} \le \dist{j'}{j}$ then $\dist{i(j')}{j}  \le 2  \dist{j'}{j}  \leq 4 (\dist{i}{j} + \ellone \C{j})$ (for all $i \in \bundle{j'}$ by Lemma 2.1) else $\dist{i(j')}{j}  \le  2 \ellone \C{j'}$.}
%\textcolor{blue}{MOVED IN GLOBAL REGION- DISCUSS} Note that  $\dist{j}{k'} \leq 2\ellone \C{j}$ for some $k' \in \clientset'$. Then we have $\dist{i}{j'} \leq \dist{i}{k'} \leq \dist{i}{j} + \dist{j}{k'} \leq \dist{i}{j} + 2\ellone \C{j}$, where the first inequality follows because $i$ belongs to $\ballofj{j'}$ and not $\ballofj{k'}$.  Thus, $\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$ ~\cite{GroverGKP18}. 
\textcolor{blue}{Thus, in either case $\dist{i(j')}{j} \leq 4 (\dist{i}{j} + \ellone \C{j})$ for all $i \in \bundle{j'}$.}
\textcolor{red}{Substituting $\phi(j, j') = \sum_{i \in \bundle{j'}} x^*_{ij}$ and summing over all $
j' \in \clientset'$ we get the desired claim.}
%Also, since $(1-(1/\ellone)) \ge 1/2$ for $\ellone \ge 2$, we incur a loss of $2$ factor in the facility opening cost.
%Violation in lower bound is at most $(1-(1/\ellone))$; there is no  violation in the capacities as  $d_{j'} \le \capacityU$.
\textcolor{blue}{Discuss else part with Madam}

 \end{proof}
 
%$\le 4\dist{i}{j} + 4 \ellone \C{j} $ else $\dist{i(j')}{j}  \le  2 \ellone \C{j'} \le 4 \ellone \C{j} \le 4\dist{i}{j} + 4 \ellone \C{j}$, where the second inequality in the else part follows because if $\ellone \C{j'} > \dist{j'}{j}$ then $\C{j'} \leq 2\C{j}$ \cite{GroverGKP18}. Also, since the total opening in each cluster is at least $(1-(1/\ellone))$, a loss of factor $\ellone/(\ellone-1) (\leq 2$ for $\ellone \geq 2$) in the facility opening cost is incurred, violation in lower bound is at most $(1-(1/\ellone))$ and  since  $d_{j'} \le \capacityU$ there is no  violation in the capacity.}
   
    
 

    
Next, we consider the dense clusters. To open the facilities integrally in the dense clusters, we solve the following LP for every dense cluster $\bundle{j'}$ centered at $j'$.

($LP_2$): 
\label{dense}
$Minimize ~\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$
\begin{eqnarray}
subject~ to &\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'} \label{denseLP_const1}\\ 
&0 \leq \zofi{i} \leq 1 \label{denseLP_const2}
\end{eqnarray}
   
  % $Minimize $\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$ s.t. $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$ and $\zofi{i} \in [0,1]$. 
   
   
Note that $\zofi{i} = \sum_{j \in C}x_{ij}^*/\capacityU$ is a feasible solution with cost at most $ \sum_{i \in \bundle{j'}} \facilitycost y^*_i + \sum_{i \in \bundle{j'}} \sum_{ j \in C} x^*_{ij} [ \dist{i}{ j} + 2\ellone \C{j} ]$ by claim (1) of Lemma 2.1.

\textcolor{blue}{TBD: facility opening cost at most
$ \sum_{i \in \bundle{j'}} \facilitycost y^*_i$ and service cost
$\sum_{i \in \bundle{j'}} \sum_{ j \in C} x^*_{ij}  \dist{i}{j'} \le \sum_{i \in \bundle{j'}} \sum_{ j \in C} x^*_{ij} [ \dist{i}{ j} + 2\ellone \C{j} ]$. } 

\textcolor{red}{
\begin{lemma} \label{integral_dense}
An integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) by a factor of $(1+1/\ell)$, can be obtained at a loss of factor $(\ell)$ in cost.
\end{lemma}
}


\begin{lemma} \label{integral_dense}
For a fixed $0 < \epsilon < 1$, 
an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) by a factor of $(1+\epsilon)$, can be obtained at a loss of $(1/\epsilon)$ in cost.
%for each dense cluster $\bundle{j'}$ and the demand $\demandofj{j'}$ can be distributed to the opened facilities in the cluster at a loss of $O(1/\epsilon)$ in cost and a loss of $(1+\epsilon)$-factor in constraints (\ref{denseLP_const1}).
\end{lemma}
\begin{proof}
We first obtain an almost integral solution\footnote{A solution is said to be an almost integral solution if it has at most one fractionally opened facility.} $\primezofi{}$ by arranging the facilities opened in $z$, in non-decreasing order of $\facilitycost  + \dist{i}{j'} \capacityU$ and greedily transferring the openings $z$ onto them. %Assignment equivalent to $\capacityU \primezofi{i}$ is allotted to each facility $i \in \bundle{j'}$. 
Clearly,  $\sum_{i \in \bundle{j'}} \primezofi{i} = \sum_{i \in \bundle{j'}} \zofi{i}$. Consider constraint (\ref{denseLP_const1}), $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$. Note that the cost of solution $\primezofi{}$ is no more than that of solution $z$.

%$\capacityU \primezofi{i}$ amount of assignments coming onto the facilities in the cluster....%Each facility $i \in \bundle{j'}$ is assigned demand equivalent to $\capacityU \primezofi{i}$. 

We now convert the almost integral solution $\primezofi{}$ to an integral solution $\hat{z}$. Let $\hat{z} = \primezofi{}$ initially. Let $i'$ be the fractionally opened facility, if any, in $\bundle{j'}$. %Initially, set $\hat{z}_i = \primezofi{i}~ \forall i \in \bundle{j'}$. 
Consider the following cases:


\begin{enumerate}
    \item $\primezofi{i'} < \epsilon$:
    \textcolor{red}{$\primezofi{i'} < 1/\ell$: }close $i'$ in $\hat{z}$, 
   % set $\hat{z}_{i'} = 0$. 
    There must be at least one integrally opened facility, say $i \ne i'$ in $\bundle{j'}$ in $\primezofi{}$, as $\demandofj{j'} \ge \capacityU$. Then, $\demandofj{j'} \leq \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k} + \capacityU  (\primezofi{i} + \primezofi{i'}) \le \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k}  + (1 + \epsilon) \textcolor{red}{(1 + 1/\ell)} \capacityU  \primezofi{i} \le (1 + \epsilon) \textcolor{red}{(1 + 1/\ell)} \capacityU \sum_{k \in \bundle{j'} \setminus \{i'\}} \primezofi{k} = (1 + \epsilon)\textcolor{red}{(1 + 1/\ell)} \capacityU \sum_{k \in \bundle{j'}} \hat{z}_k$. There is no change in cost.

    \item $\primezofi{i'} \geq \epsilon \textcolor{red}{(1/\ell)}$: Open $i'$ integrally at a loss of $1/\epsilon \textcolor{red}{(\ell)}$  in facility opening cost: i.e., $\sum_{i \in \bundle{j'}} f_i \hat{z}_i \le (1/\epsilon) \textcolor{red}{(\ell)} \sum_{i \in \bundle{j'}} f_i \primezofi{i}$.
    %and  no loss in constraint (\ref{denseLP_const1}) and connection cost w.r.t $i'$. 
\end{enumerate}\end{proof}

%Let $\hat{z}$ be the solution so obtained. Then, $(1 + \epsilon) \capacityU \sum_{\singlefacility \in \bundle{j'}} \hat{z}_i \geq \demandofj{j'}$ and $\sum_{i \in \bundle{j'}} f_i \hat{z}_i \le (1/\epsilon) \sum_{i \in \bundle{j'}} f_i \hat{z}_i $.


Next, we define our assignments in the dense clusters. We first distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution.  Clearly $l_i \le (1 + \epsilon) \capacityU$. Let $i \in \bundle{j'}, j \in \clientset$.  Set $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. 



\begin{lemma} \label{Dense}
For a fixed $0<\epsilon< 1/2$, the cost of the solution $<\bar x, \bar y>$ corresponding to a dense cluster centered at $j'$ is bounded by $ (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+ (1/\epsilon))  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} + 2\ellone(1+1/\epsilon) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} $.
%Given the integral solution $\hat{z}$ to $LP_2$ corresponding to a dense cluster centered at $j'$, we can obtain a feasible set of assignments $\bar x$ and distribute $\demandofj{j'}$ to facilities in $\bundle{j'}$ at a loss of ......... 
\end{lemma}

\textcolor{red}{
\begin{proof}
Let $i \in \bundle{j'}, j \in \clientset$. Recall that $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. Consider the cost of the solution:\\ 
$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij}) $\\
$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \dist{i}{j}  \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} (\dist{j}{j'} + \dist{i}{j'})$ (by triangle inequality)\\ 
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )  $ (by definition of $\loadjinc{j}{j'}$, equation (\ref{Cjj'}) and the fact that $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\%(Sapna..I have used multiple things ...pls write them here...)\\
$ \leq  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +  (1+\epsilon) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j} \primezofi{i} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
$\leq max\{(1/\epsilon), (1+\epsilon)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\
$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (for $\epsilon \leq 1/2$)\\
$= (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   (1/\epsilon)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by cost bound of feasible solution $z$)\\
$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   (1/\epsilon)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ellone \C{j}) + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\
$= (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+ (1/\epsilon))  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} + 2\ellone(1+1/\epsilon) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} $ \\
%$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i + \dist{i}{j'} \sum_{j \in \clientset} \bar{x}_{ij}) $\\
%$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
%$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} l_i$\\ 
%$ \leq  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +  (1+\epsilon) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i}$\\
%$\leq max\{(1/\epsilon), (1+\epsilon)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i}$\\
%$= (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i}$ for $\epsilon< 1/2$\\
%$ =  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU  \dist{i}{j'}) z_i$\\
%$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   (1/\epsilon)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij}$\\
%$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} x^*_{ij} [ \dist{i}{ j} + 2\ellone \C{j} ]$.
\end{proof}
}

	%\textcolor{blue}{Choosing $\ellone = O(1/\epsilon)$, the total cost of the tri-criteria solution is $Cost_f(S^t) + Cost_c(S^t) \leq %\frac{\ellone}{\ellone-1} Cost_f(O) + 4Cost_c(O) + O(1/\epsilon)\sum_{j \in \clientset}\C{j} \leq 
	%\max\{2,1/\epsilon\}Cost_f(O) + O(1+\epsilon) Cost_c(O) \leq O(1/\epsilon)Cost(O)$, where $Cost_f(.)$ and $Cost_c(.)$ denote the facility opening cost and connection cost respectively of the particular solution.}








	%\textcolor{blue}{Choosing $\ellone = O(1/\epsilon)$, the total cost of the tri-criteria solution is $Cost_f(S^t) + Cost_c(S^t) \leq %\frac{\ellone}{\ellone-1} Cost_f(O) + 4Cost_c(O) + O(1/\epsilon)\sum_{j \in \clientset}\C{j} \leq 
	%\max\{2,1/\epsilon\}Cost_f(O) + O(1+\epsilon) Cost_c(O) \leq O(1/\epsilon)Cost(O)$, where $Cost_f(.)$ and $Cost_c(.)$ denote the facility opening cost and connection cost respectively of the particular solution.}

\textcolor{magenta}{Summing the cost bound of Lemma (\ref{Sparse}) over all sparse clusters and that of Lemma (\ref{Dense}) over all dense clusters, the total cost of the tri-criteria solution is:}

%Sapna...TBD: 
%$2\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} [\dist{i}{j} + \ellone \C{j}] +  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+ (1/\epsilon))  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} + 2\ellone(1+1/\epsilon) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} $

%Start from here....

$\leq max\{2,1/\epsilon\} \sum_{j' \in \clientset'} \sum_{i \in \bundle{j'}} f_i y^*_i +  max\{4,(2+1/\epsilon)\} \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + \ellone~ max\{4,2(1+1/\epsilon)\} \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \C{j}$

$= (1/\epsilon) \sum_{j' \in \clientset'} \sum_{i \in \bundle{j'}} f_i y^*_i +  (2+1/\epsilon) \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + 2\ellone(1+1/\epsilon) \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\epsilon \leq 1/2$)



%$= max\{2,1/\epsilon\} \sum_{j' \in \clientset'} \sum_{i \in \bundle{j'}} f_i y^*_i +  max\{4,1/\epsilon\} \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + (4+2/\epsilon) \ellone \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \C{j}$

%$=  max\{2,1/\epsilon\} \sum_{j' \in \clientset'} \sum_{i \in \bundle{j'}} f_i y^*_i +  max\{4,1/\epsilon\} \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + (4+2/\epsilon) \ellone \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \C{j}$

Choose $\ellone = floor(1/\epsilon)$ ..sapna use appropriate macro for floor, then the cost of the solution is bounded by $(2\ellone^2 + 3\ellone + 2)LP_{opt}$. For $\epsilon \le 1/2, \ellone \ge 2$. For $\epsilon = 1/2$, the capacity violation is $3/2$ and the approximation ratio is $16$. The capacity violation can be made arbitrarily small at the cost of increase in the approximation ratio.

To obtain integral assignments, we solve a minimum-cost integer flow problem with relaxed lower bounds and increased capacities. Let $S^t$ be the solution so obtained and violations in lower and upper bounds be $\alpha$ and $\beta$ respectively. \textcolor{blue}{Then, $Cost(S^t) \le  (2\ellone^2 + 3\ellone + 2) Cost(O)$, $\alpha = (\ellone-1)/\ellone$ and $\beta= (1+\epsilon)$ where $\ellone = floor(1/\epsilon) \ge 2$ for $\epsilon \leq 1/2$ and $\alpha \ge 1/2$.}
%	\textcolor{red}{	For $\ellone \ge 2, \alpha \ge 1/2$. 	}

	%\textcolor{blue}{	For $\ellone > 2, \alpha \ge 2/3$. 	}
	
		\textcolor{red}{
	Next, using $S^t$, we transform the instance $I$ to an instance $I_{cap}$ of capacitated facility location problem by swapping the roles of clients and facilities. This is done via a series of transformations from instance $I$ to $I_1$, 	$I_1$ to $I_2$ and $I_2$ to $I_{cap}$. The key idea is to create  $B - n_i$ units of demand, where the number $n_i$ of clients served by facility $i$ in $S^t$ is short of the lower bound and create  $n_i - B$ units of supply at locations where $n_i > B$.
	}
	


==> TriCriteria_L.tex <==
\section{Computing the Tri-criteria Solution}
\label{tri-criteria}
 %We use a simpler LP-rounding technique to get $(\frac{\ellone-1}{\ellone})$-factor violation in lower bounds and $2$-factor violation in upper bounds at constant factor loss in cost. The technique used is much simpler than Friggstad et al. \cite{friggstad_et_al_LBUFL} because lower bounds are uniform in our case unlike Friggstad et al. that considers non-uniform lower bounds. 

 In this section, we give a tri-criteria solution that violates the lower bound by a factor of  \textcolor{yellow}{$\alpha = 1-1/\ell$}  \textcolor{cyan}{$\alpha > 1/2$} and the upper bound by a factor of  \textcolor{yellow}{$\beta = 1+1/\ell$} \textcolor{cyan}{$\beta = 3/2$.} \textcolor{yellow}{ where $\ell > 2$ is a tune-able parameter.} In particular, we present the following result:
 
 

 \begin{theorem} \label{TricriteriaResult}
 A ($\textcolor{yellow}{(2\ell^2 + 3\ell +2), 1-1/\ell, 1+1/\ell}$) $\textcolor{cyan}{(O(1),1/2, 3/2)}$ -
 approximate solution can be obtained for LBUBFL in polynomial time. \textcolor{yellow}{, where $\ell > 2$ is a tuneable parameter.}
\end{theorem}
 
 
 Instance $I$ of LBUBFL can be formulated as the following integer program (IP):

\label{{unif-CFLP}}
$Minimize ~\mathcal{C}ostLBUBFL(x,y) = \sum_{j \in \clientset}\sum_{i \in \facilityset}\dist{i}{j}x_{ij} + \sum_{i \in \facilityset}f_iy_i $
\begin{eqnarray}
subject~ to &\sum_{i \in \facilityset}{} x_{ij} \geq 1 & \forall ~\singleclient \in \clientset \label{LPFLP_const1}\\ 
%&\sum_{j \in \clientset}{} x_{ij} \leq \capacityU ~ y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const2}\\ 
& \capacityU y_i \geq \sum_{j \in \clientset}{} x_{ij} \geq \B y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const3}\\
& x_{ij} \leq y_i & \forall~ \singlefacility \in \facilityset , ~\singleclient \in \clientset \label{LPFLP_const4}\\   
& y_i,x_{ij} \in \left\lbrace 0,1 \right\rbrace  \label{LPFLP_const5}
\end{eqnarray}
where  $y_i$ is an indicator variable which is equal to $1$ if facility $i$ is open and is $0$ otherwise. $x_{ij}$ is an indicator variable which is equal to $1$ if client $j$ is served by facility $i$ and is $0$ otherwise.
 Constraints \ref{LPFLP_const1} ensure that all the clients are served. %Constraints \ref{LPFLP_const2} make sure that the total demand assigned to an open facility is no more than its capacity \capacityU. 
 Constraints \ref{LPFLP_const3} make sure that the total demand assigned to an open facility is at least $\B$ and at most $\capacityU$. Constraints \ref{LPFLP_const4} ensure that a client is assigned to a facility only if it is opened. LP-Relaxation  is obtained by allowing the variables to be non-integral.
% $ y_i, x_{ij} \in [0, 1]$. %Call it LP. 
Let $\zeta^{*} = <x^*, y^*>$ be an optimal solution  and $\opt{}$ be its cost.


We start by sparsifying the problem instance by removing some clients.
For $j \in \clientset$, let $ \C{j} $ denote the average connection cost paid by $\singleclient$ in $\zeta^*$. 
%i.e., ~$\C{j} = (\sum_{i \in \facilityset}{} {x}^*_{ij} \dist{i}{j})/({\sum_{i \in \facilityset}{} {x}^*_{ij}})$. 
Further, let \textcolor{yellow}{$\ell > 2$ be a tuneable parameter,} $\ballofj{j}$ be the ball of facilities within a radius of \textcolor{yellow}{ $\ellone\C{j}$ } \textcolor{cyan}{$2\C{j}$} of $j$ and $\cardTwo{\ballofj{j}}$
be the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
Then,  \textcolor{olive}{\textcolor{yellow}{$\cardTwo{\ballofj{j}} \ge (1-\frac{1}{\ellone}) > 1/2$.}} \textcolor{cyan}{$\cardTwo{\ballofj{j}} \ge 1/2$.}
%where $\cardTwo{\ballofj{j}}$
%$=  \sum_{i \in \ballofj{j}} y^*_i$ denotes the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
The clients are processed in the non-decreasing order of the radii of their balls, removing the close-by clients with balls of larger radii and dissolving their balls: let $\bar{\clientset} = \clientset$ and $\clientset'$ denote the sparsified set of  clients. Initially $\clientset' = \phi$.
Let $j'$ be a client in $\bar{\clientset}$ with a ball of the smallest radius (breaking the ties arbitrarily). Remove $j'$ from $\bar{\clientset}$ and add it to $\clientset'$. For all $j (\ne j') \in \bar{\clientset}$ with $\dist{j'}{ j} \leq 2\ell \C{j}$, remove $j$ from $\bar{\clientset}$. Repeat the process until $\bar{\clientset} = \phi$. 
Cluster of facilities are formed around the clients in $\clientset'$ by assigning a facility to the cluster of $j' \in \clientset'$ if and only if $j'$ is nearest to the facility amongst all $j' \in \clientset'$, i.e. if $\bundle{j'}$ denotes the cluster centered at $j'$ then, $i$ belongs to $\bundle{j'}$ if and only if $\dist{i}{j'} < \dist{i}{k'}$ for all $k' \textcolor{cyan}{(\ne j')} \in \clientset'$ (assuming that the distances are distinct).
The clients in $C'$ are then called the cluster centers.



\begin{observation}
Any two cluster centers $j', k'$ in $C'$ satisfy the  separation property:
$\dist{j'}{k'} > \textcolor{yellow}{ 2\ellone}  \textcolor{cyan}{4}~max\{ \C{j'},\C{k'}\}$.
\end{observation}


\begin{lemma} \label{distBound}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. Then,
\begin{enumerate}
    \item \label{claim-1}  $\dist{i}{j'}  \leq \dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$
    \item  \label{claim-2} $\dist{j}{j'} \leq 2\dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$
    \item \label{claim-3}  If $\dist{j}{j'} \leq \textcolor{yellow}{ \ellone}\textcolor{cyan}{2} \C{j'}$, then $\C{j'} \le 2\C{j}$
\end{enumerate}
\end{lemma}

\begin{proof}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. 
\begin{enumerate}

    \item Note that, $\dist{j}{k'} \leq \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$ for some $k' \in \clientset'$. Then we have  $\dist{i}{j'} \leq \dist{i}{k'} \leq \dist{i}{j} + \dist{j}{k'} \leq \dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$, where the first inequality follows because $i$ belongs to $\bundle{j'}$ and not $\bundle{k'}$ whenever $k' \ne j'$.  \textcolor{blue}{See Fig: (\ref{Cjj'}).}
    
    
    \item Using triangle inequality, we have   $\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$.
    
     \item Let $j \ne j'$. Note that $\dist{j}{j'} \leq \textcolor{yellow}{ \ellone} \textcolor{cyan}{2} \C{j'}$ $\Rightarrow j \notin \clientset'$. 
     %Further, using contradiction, let's assume 
     Suppose if possible, $\C{j'} > 2\C{j}$. Since $j \notin \cliset', \exists$ some $k'\in \clientset':\dist{j}{k'} \le \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$. Then, $\dist{k'}{j'} \le \dist{k'}{j} + \dist{j}{j'}$  $ \leq \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j} + \textcolor{yellow}{ \ellone} \textcolor{cyan}{2} \C{j'} < \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j'}$. Thus, we arrive at a contradiction to the separation property. Hence, $\C{j'} \le 2\C{j}$.

\end{enumerate} \end{proof}
 

\begin{figure} 
    \centering
    \includegraphics[width=10cm]{Figures/Cjj'.jpg}
    \caption{$\dist{i}{j'}  \leq \dist{i}{j} + 2\ellone \C{j}$}
    \label{Cjj'}
\end{figure}

%$\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$ ~\cite{GroverGKP18}.}  

For $j' \in \clientset', j \in \clientset$, let $\loadjinc{j}{j'}$ be the extent up to which $j$ is served by the facilities in the cluster of $j'$  \textcolor{olive}{under solution $\zeta^*$} and $d_{j'}= \sum_{j \in \clientset} \loadjinc{j}{j'}$.
We call a cluster to be $sparse$ if $d_{j'} \le  \capacityU$ and $dense$ otherwise. Let $\csparse$ and $\cdense$ be the set of cluster centers of sparse  and dense clusters respectively.


%Let $<\hat{x}, \hat{y}>$ be the solution so obtained, i.e., for $ j \in \clientset$, $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$. For $j' \in \crich, i \in \bundle{j'}, j \in \clientset$, $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. 


\begin{lemma} \label{Sparse}
We can obtain a solution $<\hat{x}, \hat{y}>$ such that  exactly one facility $i(j')$ is opened integrally in each sparse cluster centered at $j' \in \clientset'$. The solution violates the lower bound by a factor of \textcolor{yellow}{$(1 - 1/\ellone)$} \textcolor{cyan}{1/2} \textcolor{olive}{such that $\sum_{j' \in \clientset'}\sum_{i \in \bundle{j'}} [f_i \hat{y}_i + \sum_{j \in \clientset}  \hat{x}_{ij} \dist{i}{j}] \leq $}
$\sum_{j' \in \csparse}[\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \textcolor{yellow}{\ellone } \textcolor{cyan}{2}\C{j})] + \sum_{j' \in \cdense} [\sum_{i \in \bundle{j'}} f_i y^*_i + \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$.

%\textcolor{red}{May be we should write the following:$\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \le \sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})]$...will resolve after completing this section}

\end{lemma}

\begin{proof}
%In a sparse cluster centered at $j'$, we open the cheapest facility, say $i(j')$, in $\ballofj{j'}$ and transfer all the assignments in the cluster onto it.
%As specified above, 
For $ j' \in \cdense, i \in \bundle{j'}, j \in \clientset$, set $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. Next,
let $j' \in \csparse$
%$\bundle{j'}$ be a sparse cluster centered at $j'$ 
and $i(j')$ be a cheapest \textcolor{olive}{(lowest facility opening cost)} facility in $\ballofj{j'}$. We open $i(j')$ and transfer all the assignments in the cluster onto it (see Figure (\ref{sparse})). 
%Let $ j \in \clientset$.
i.e. set $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$ and $j \in \clientset$. 
Since $\cardTwo{\ballofj{j'}} \ge \textcolor{yellow}{(1-\frac{1}{\ellone})} \textcolor{cyan}{1/2}$ we have $\sum_{j \in \clientset}{} \hat{x}_{i(j')j} = \demandofj{j'} \ge \textcolor{yellow}{(1-\frac{1}{\ellone})} \textcolor{cyan}{1/2}\B$. Thus, the lower bound is violated at most by $\textcolor{yellow}{(1-\frac{1}{\ellone})} \textcolor{cyan}{1/2}$
and the facility cost is bounded by $\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i y^*_i$.

To bound the service cost, we will show that for $j' \in \csparse, \sum_{j \in \clientset} \loadjinc{j}{j'} \dist{i(j')}{j}  \leq 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})$: 
since $i(j') \in \ballofj{j'}$, we have $\dist{i(j')}{j'} \le  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j'}$. 
Thus, for $j \in \clientset$,
we have $\dist{i(j')}{j} \le \dist{j'}{j} + \dist{i(j')}{j'} \le  \dist{j'}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j'}$. If $ \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j'} \le \dist{j'}{j}$ then $\dist{i(j')}{j}  \le 2  \dist{j'}{j}  \leq 4 (\dist{i}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})$ ($\forall~i \in \bundle{j'}$ by claim (\ref{claim-2}) of Lemma (\ref{distBound})), 
 else $\dist{i(j')}{j}  \leq  \textcolor{yellow}{2\ellone} \textcolor{cyan}{4} \C{j'} \leq  \textcolor{yellow}{4 \ellone} \textcolor{cyan}{8} \C{j}$, where the second inequality in the else part follows by claim (\ref{claim-3}) of Lemma (\ref{distBound}).
Thus, in either case $\dist{i(j')}{j} \leq 4 (\dist{i}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})$ for all $i \in \bundle{j'}$.
Substituting $\phi(j, j') = \sum_{i \in \bundle{j'}} x^*_{ij}$ and summing over all $j \in \clientset$ 
%$j' \in \csparse$ 
we get the desired bound.
Thus, $\sum_{i \in \facilityset} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  \hat{x}_{ij}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \demandofj{j'}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
\le \sum_{j' \in \csparse}[\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})] + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} [ f_i y^*_i + \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$
\end{proof}
 
%$\le 4\dist{i}{j} + 4 \ellone \C{j} $ else $\dist{i(j')}{j}  \le  2 \ellone \C{j'} \le 4 \ellone \C{j} \le 4\dist{i}{j} + 4 \ellone \C{j}$, where the second inequality in the else part follows because if $\ellone \C{j'} > \dist{j'}{j}$ then $\C{j'} \leq 2\C{j}$ \cite{GroverGKP18}. Also, since the total opening in each cluster is at least $(1-(1/\ellone))$, a loss of factor $\ellone/(\ellone-1) (\leq 2$ for $\ellone > 2$) in the facility opening cost is incurred, violation in lower bound is at most $(1-(1/\ellone))$ and  since  $d_{j'} \le \capacityU$ there is no  violation in the capacity.}
   
    \begin{figure} 
    \centering
    \includegraphics[width=10cm]{Figures/sparse.jpg}
    \caption{(A) Cluster $\bundle{j'}$ centered at $j'$. (B) Demand $\demandofj{j'}$ being assigned to facility $i(j') \in \ballofj{j'}$.}
    \label{sparse}
\end{figure}
 

    
%Next, we consider the dense clusters.
To open the facilities integrally in the dense clusters, we solve the following LP for every dense cluster $\bundle{j'}$.
%centered at $j'$.

($LP_1$): 
\label{dense}
$Minimize ~\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$
\begin{eqnarray}
subject~ to &\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'} \label{denseLP_const1}\\ 
&0 \leq \zofi{i} \leq 1 \label{denseLP_const2}
\end{eqnarray}
   
  % $Minimize $\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$ s.t. $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$ and $\zofi{i} \in [0,1]$. 
   
   
Note that for $\zofi{i} = \sum_{j \in \clientset}x_{ij}^*/\capacityU$, we have $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} = \demandofj{j'}$ and $\zofi{i} \le y^*_i$. Thus, $\zofi{}$
is a feasible solution with cost at most $ \sum_{i \in \bundle{j'}} [\facilitycost y^*_i + \sum_{ j \in \clientset} x^*_{ij} ( \dist{i}{j} +   \textcolor{yellow}{2\ellone} \textcolor{cyan}{4} \C{j}) ]$ by claim (\ref{claim-1}) of Lemma (\ref{distBound}).

%\textcolor{blue}{TBD: facility opening cost at most $ \sum_{i \in \bundle{j'}} \facilitycost y^*_i$ and service cost $\sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij}  \dist{i}{j'} \le \sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij} [ \dist{i}{ j} + 2\ellone \C{j} ]$. } 

\begin{lemma} \label{integral_dense}
Given the feasible solution $z$ to $LP_1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) by a factor of \textcolor{yellow}{$(1+1/\ell)$} \textcolor{cyan}{3/2}, can be obtained at a loss of factor $\textcolor{yellow}{\ellone} \textcolor{cyan}{2}$ in cost
i.e. $ \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \hat{z}_{i} \le  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$.
%For a fixed $0 < \epsilon < 1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) by a factor of $(1+\epsilon)$, can be obtained at a loss of $(1/\epsilon)$ in cost.
\end{lemma}

\begin{proof}
\textcolor{green}{
We say that a solution to $LP_1$ is almost integral if it has at most one fractionally opened facility in $\bundle{j'}$.
}
We first obtain an almost integral solution
%\footnote{A solution is said to be an almost integral solution if it has at most one fractionally opened facility.}
$\primezofi{}$ by arranging the facilities opened in $z$, in non-decreasing order of $\facilitycost  + \dist{i}{j'} \capacityU$ and greedily transferring the openings $z$ onto them. 
Then,  $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} = \demandofj{j'}$. %Consider constraint (\ref{denseLP_const1}), $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$.
Note that the cost of solution $\primezofi{}$ is no more than that of solution $z$.


We now convert the almost integral solution $\primezofi{}$ to an integral solution $\hat{z}$. Let $\hat{z} = \primezofi{}$ initially. Let $i'$ be the fractionally opened facility, if any, in $\bundle{j'}$. %Initially, set $\hat{z}_i = \primezofi{i}~ \forall i \in \bundle{j'}$. 
Consider the following cases:


\begin{enumerate}
    %\item $\primezofi{i'} < \epsilon$:
    \item $\primezofi{i'} < \textcolor{yellow}{1/\ell} \textcolor{cyan}{1/2}$: close $i'$ in $\hat{z}$. There must be at least one integrally opened facility, say $i (\ne i') \in \bundle{j'}$ in $\primezofi{}$, as $\demandofj{j'} \ge \capacityU$. Then, $\demandofj{j'} = \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k} + \capacityU  (\primezofi{i} + \primezofi{i'}) \le \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k}  + \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU  \primezofi{i} \le \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU \sum_{k \in \bundle{j'} \setminus \{i'\}} \primezofi{k} = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}  \capacityU \sum_{k \in \bundle{j'}} \hat{z}_k$. There is no increase in cost as we have only (possibly) shut down one of the facilities .
    

    \item $\primezofi{i'} \geq \textcolor{yellow}{1/\ell} \textcolor{cyan}{1/2} $: Open $i'$ integrally at a loss of factor $\textcolor{yellow}{\ell}$ \textcolor{cyan}{2} in facility opening cost i.e., $\sum_{i \in \bundle{j'}} f_i \hat{z}_i \le \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i \primezofi{i}$. 
    \textcolor{cyan}{Also, note that $\capacityU \hat{z}_i \geq 1/2 \B \primezofi{i'}$ ------ CHECK AGAIN.} 
\end{enumerate}\end{proof}

%Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{(1+1/\ell)\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = (1 + 1/\ell) \capacityU \hat{z}_i$ , where the first inequality follows by Lemma (\ref{integral_dense}). 


%\textcolor{cyan}{SAPNA, Revisit the next para later:}

Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{\textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU \hat{z}_i$ , where the first inequality follows by Lemma (\ref{integral_dense}). \textcolor{cyan}{Also, $l_i \geq 1/2 B \hat{z}_i$. -- CHECK AGAIN AND WRITE PROPERLY }


\textcolor{olive}{A solution is said to be an integrally opened solution if all facilities in it are either opened to an extent of $1$ or $0$. We next obtain such a solution to LBUBFL problem.}


\begin{lemma} \label{Dense1}
We can obtain an integrally opened solution $<\bar x, \bar y>$ to LBUBFL problem at a loss of $\textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}$ in upper bounds and $\textcolor{yellow}{(1-1/\ell)} \textcolor{cyan}{(1/2)}$ in lower bounds whose cost is bounded by $\textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)} \textcolor{cyan}{O(1)LP_{opt}}$.
\end{lemma}
\begin{proof}
For $j' \in \csparse$, set $\bar y_i = \hat{y}_i,~\bar{x}_{ij} = \hat{x}_{ij}~\forall i \in \bundle{j'}, j \in \clientset$. \textcolor{yellow}{The violation in lower bound then follows from Lemma (\ref{Sparse})
and, }

\begin{equation}
\label{cost-of-sparse}
\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \bar{y}_i + \sum_{j \in \clientset} \bar{x}_{ij} \dist{i}{j}) \le \sum_{j' \in \csparse}[\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})].
\end{equation}

Next let $j' \in \cdense,~i \in \bundle{j'}, j \in \clientset$. Set $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. 
Consider $ \sum_{j \in \clientset} \bar{x}_{ij} = \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} = l_i \leq   \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \hat{z}_i = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \bar{y}_i$. Thus, the loss in capacities is at most   \textcolor{yellow}{(1+1/\ell)}\textcolor{cyan}{(3/2)}.

\textcolor{cyan}{From Lemma (\ref{Sparse}), the violation in lower bound is $1/2$. Thus, the final violation in lower bound is $ min\{1/2, (1-1/\ell)\} > 1/2$ for $\ell >2$, which implies $\alpha = 1/2$. ---SAPNA,  REVISIT}

Also,\\ 
$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij}) $\\
$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \dist{i}{j}  \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} (\dist{j}{j'} + \dist{i}{j'})$ (by triangle inequality)\\ 
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   
%\sum_{\singlefacility \in \bundle{j'}} 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ (as $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
%$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )  $ (by definition of $\loadjinc{j}{j'}$, claim (\ref{claim-2}) of Lemma (\ref{distBound}) and the fact that $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
$ \leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +    \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{3/2} \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +  
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ (by Lemma (\ref{integral_dense}))\\
%$ \leq  \ell \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +   (1+1/\ell) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
\textcolor{yellow}{$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\}
%$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\ \textcolor{yellow}{(for $\ell > 2$)}\\
%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\ (for $\ell > 2$)\\
$\leq \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (by Lemma (\ref{integral_dense}))\\
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (because $z_i = \sum_{j \in \clientset} x^*_{ij} / \capacityU \leq y^*_i$)\\ 
%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by cost bound of feasible solution $z$.....Sapna..how from this reason?)\\
%\textcolor{red}{
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ellone \C{j}) + \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$  (by claim (\ref{claim-1}) of Lemma (\ref{distBound}))\\
%}
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} +  \textcolor{yellow}{2\ell} \textcolor{cyan}{4} \C{j}) + \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}  (2\dist{i}{j} +  \textcolor{yellow}{2\ell} \textcolor{cyan}{4} \C{j} )$ 
(by definition of $\loadjinc{j}{j'}$ and claims (\ref{claim-1}) and (\ref{claim-2}) of Lemma (\ref{distBound}))\\
$= \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   \textcolor{yellow}{2+\ell} \textcolor{cyan}{4}   \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} +   \textcolor{yellow}{2\ell(1+\ell)} \textcolor{cyan}{12} \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}   \C{j} $ \\

Summing over all $j' \in \cdense$ and adding inequality (\ref{cost-of-sparse}), we get\\
$ \sum_{i \in \facilityset} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij})$\\
$\leq \textcolor{yellow}{max\{\ell, \ell/(\ell-1)\}} \textcolor{cyan}{2} \sum_{i \in \facilityset}  f_i y^*_i + \textcolor{yellow}{ max\{4,(2+\ell)\}} \textcolor{cyan}{4} \sum_{i \in \facilityset}\sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + \textcolor{yellow}{\ellone~ max\{4,2(1+\ell)\}} \textcolor{cyan}{12} \sum_{i \in \facilityset}\sum_{j \in \clientset} x^*_{ij} \C{j}$\\
 \textcolor{yellow}{ $= \sum_{i \in \facilityset}  f_i y^*_i + (2+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + 2\ell(1+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\ell > 2$)}\\
$ \leq \textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)} \textcolor{cyan}{16}LP_{opt}$.
\end{proof}


Theorem~\ref{TricriteriaResult} is obtained by solving a min-cost flow problem with relaxed lower  and upper bounds to obtain the integral assignments.
Let $S^t$ be the solution so obtained. %and violations in lower and upper bounds be denoted by $\alpha$ and $\beta$ respectively.
Then, $Cost_I(S^t) \le \textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)}\textcolor{cyan}{16} Cost_I(O)$,
where $O$ is an optimal solution to $I$, $\textcolor{yellow}{\alpha= (1 - 1/\ellone)} \textcolor{cyan}{\alpha >
1/2}$ and $\textcolor{yellow}{\beta= (1 + 1/\ellone)} \textcolor{cyan}{\beta= 3/2}$.
\textcolor{yellow}{ For $\ell = 2.01$, $\alpha > 1/2$, $\beta < 3/2$ and the approximation ratio is less than $17$. The violations in the lower and the upper bounds can be made arbitrarily close to $0$ at the cost of increase in the approximation ratio.}

%To obtain integral assignments, we solve a minimum-cost integer flow problem with relaxed lower  and upper bounds.



	Next, using $S^t$, we transform the instance $I$ to an instance $I_{cap}$ of capacitated facility location problem by swapping the roles of clients and facilities. This is done via a series of transformations from instance $I$ to $I_1$, 	$I_1$ to $I_2$ and $I_2$ to $I_{cap}$. The key idea is to create  $\B - n_i$ units of demand, where the number $n_i$ of clients served by facility $i$ in $S^t$ is short of the lower bound and create  $n_i - \B$ units of supply at locations where $n_i > \B$.
	
	


==> TriCriteria_l=2.tex <==
\section{Computing the Tri-criteria Solution}
\label{tri-criteria}
 %We use a simpler LP-rounding technique to get $(\frac{\ellone-1}{\ellone})$-factor violation in lower bounds and $2$-factor violation in upper bounds at constant factor loss in cost. The technique used is much simpler than Friggstad et al. \cite{friggstad_et_al_LBUFL} because lower bounds are uniform in our case unlike Friggstad et al. that considers non-uniform lower bounds. 

 In this section, we give a tri-criteria solution that violates the lower bound by a factor of  \textcolor{yellow}{$\alpha = 1-1/\ell$}  \textcolor{cyan}{$\alpha > 1/2$} and the upper bound by a factor of  \textcolor{yellow}{$\beta = 1+1/\ell$} \textcolor{cyan}{$\beta = 3/2$.} \textcolor{yellow}{ where $\ell > 2$ is a tune-able parameter.} In particular, we present the following result:
 
 

 \begin{theorem} \label{TricriteriaResult}
 A ($\textcolor{yellow}{(2\ell^2 + 3\ell +2), 1-1/\ell, 1+1/\ell}$) $\textcolor{cyan}{(O(1),1/2, 3/2)}$ -
 approximate solution can be obtained for LBUBFL in polynomial time. \textcolor{yellow}{, where $\ell > 2$ is a tuneable parameter.}
\end{theorem}
 
 
 Instance $I$ of LBUBFL can be formulated as the following integer program (IP):

\label{{unif-CFLP}}
$Minimize ~\mathcal{C}ostLBUBFL(x,y) = \sum_{j \in \clientset}\sum_{i \in \facilityset}\dist{i}{j}x_{ij} + \sum_{i \in \facilityset}f_iy_i $
\begin{eqnarray}
subject~ to &\sum_{i \in \facilityset}{} x_{ij} \geq 1 & \forall ~\singleclient \in \clientset \label{LPFLP_const1}\\ 
%&\sum_{j \in \clientset}{} x_{ij} \leq \capacityU ~ y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const2}\\ 
& \capacityU y_i \geq \sum_{j \in \clientset}{} x_{ij} \geq \B y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const3}\\
& x_{ij} \leq y_i & \forall~ \singlefacility \in \facilityset , ~\singleclient \in \clientset \label{LPFLP_const4}\\   
& y_i,x_{ij} \in \left\lbrace 0,1 \right\rbrace  \label{LPFLP_const5}
\end{eqnarray}
where  $y_i$ is an indicator variable which is equal to $1$ if facility $i$ is open and is $0$ otherwise. $x_{ij}$ is an indicator variable which is equal to $1$ if client $j$ is served by facility $i$ and is $0$ otherwise.
 Constraints \ref{LPFLP_const1} ensure that all the clients are served. %Constraints \ref{LPFLP_const2} make sure that the total demand assigned to an open facility is no more than its capacity \capacityU. 
 Constraints \ref{LPFLP_const3} make sure that the total demand assigned to an open facility is at least $\B$ and at most $\capacityU$. Constraints \ref{LPFLP_const4} ensure that a client is assigned to a facility only if it is opened. LP-Relaxation  is obtained by allowing the variables to be non-integral.
% $ y_i, x_{ij} \in [0, 1]$. %Call it LP. 
Let $\zeta^{*} = <x^*, y^*>$ be an optimal solution  and $\opt{}$ be its cost.


We start by sparsifying the problem instance by removing some clients.
For $j \in \clientset$, let $ \C{j} $ denote the average connection cost paid by $\singleclient$ in $\zeta^*$. 
%i.e., ~$\C{j} = (\sum_{i \in \facilityset}{} {x}^*_{ij} \dist{i}{j})/({\sum_{i \in \facilityset}{} {x}^*_{ij}})$. 
Further, let \textcolor{yellow}{$\ell > 2$ be a tuneable parameter,} $\ballofj{j}$ be the ball of facilities within a radius of \textcolor{yellow}{ $\ellone\C{j}$ } \textcolor{cyan}{$2\C{j}$} of $j$ and $\cardTwo{\ballofj{j}}$
be the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
Then,  \textcolor{olive}{\textcolor{yellow}{$\cardTwo{\ballofj{j}} \ge (1-\frac{1}{\ellone}) > 1/2$.}} \textcolor{cyan}{$\cardTwo{\ballofj{j}} \ge 1/2$.}
%where $\cardTwo{\ballofj{j}}$
%$=  \sum_{i \in \ballofj{j}} y^*_i$ denotes the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
The clients are processed in the non-decreasing order of the radii of their balls, removing the close-by clients with balls of larger radii and dissolving their balls: let $\bar{\clientset} = \clientset$ and $\clientset'$ denote the sparsified set of  clients. Initially $\clientset' = \phi$.
Let $j'$ be a client in $\bar{\clientset}$ with a ball of the smallest radius (breaking the ties arbitrarily). Remove $j'$ from $\bar{\clientset}$ and add it to $\clientset'$. For all $j (\ne j') \in \bar{\clientset}$ with $\dist{j'}{ j} \leq 2\ell \C{j}$, remove $j$ from $\bar{\clientset}$. Repeat the process until $\bar{\clientset} = \phi$. 
Cluster of facilities are formed around the clients in $\clientset'$ by assigning a facility to the cluster of $j' \in \clientset'$ if and only if $j'$ is nearest to the facility amongst all $j' \in \clientset'$, i.e. if $\bundle{j'}$ denotes the cluster centered at $j'$ then, $i$ belongs to $\bundle{j'}$ if and only if $\dist{i}{j'} < \dist{i}{k'}$ for all $k' \textcolor{cyan}{(\ne j')} \in \clientset'$ (assuming that the distances are distinct).
The clients in $C'$ are then called the cluster centers.



\begin{observation}
Any two cluster centers $j', k'$ in $C'$ satisfy the  separation property:
$\dist{j'}{k'} > \textcolor{yellow}{ 2\ellone}  \textcolor{cyan}{4}~max\{ \C{j'},\C{k'}\}$.
\end{observation}


\begin{lemma} \label{distBound}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. Then,
\begin{enumerate}
    \item \label{claim-1}  $\dist{i}{j'}  \leq \dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$
    \item  \label{claim-2} $\dist{j}{j'} \leq 2\dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$
    \item \label{claim-3}  If $\dist{j}{j'} \leq \textcolor{yellow}{ \ellone}\textcolor{cyan}{2} \C{j'}$, then $\C{j'} \le 2\C{j}$
\end{enumerate}
\end{lemma}

\begin{proof}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. 
\begin{enumerate}

    \item Note that, $\dist{j}{k'} \leq \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$ for some $k' \in \clientset'$. Then we have  $\dist{i}{j'} \leq \dist{i}{k'} \leq \dist{i}{j} + \dist{j}{k'} \leq \dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$, where the first inequality follows because $i$ belongs to $\bundle{j'}$ and not $\bundle{k'}$ whenever $k' \ne j'$.  \textcolor{blue}{See Fig: (\ref{Cjj'}).}
    
    
    \item Using triangle inequality, we have   $\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$.
    
     \item Let $j \ne j'$. Note that $\dist{j}{j'} \leq \textcolor{yellow}{ \ellone} \textcolor{cyan}{2} \C{j'}$ $\Rightarrow j \notin \clientset'$. 
     %Further, using contradiction, let's assume 
     Suppose if possible, $\C{j'} > 2\C{j}$. Since $j \notin \cliset', \exists$ some $k'\in \clientset':\dist{j}{k'} \le \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j}$. Then, $\dist{k'}{j'} \le \dist{k'}{j} + \dist{j}{j'}$  $ \leq \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j} + \textcolor{yellow}{ \ellone} \textcolor{cyan}{2} \C{j'} < \textcolor{yellow}{ 2\ellone} \textcolor{cyan}{4} \C{j'}$. Thus, we arrive at a contradiction to the separation property. Hence, $\C{j'} \le 2\C{j}$.

\end{enumerate} \end{proof}
 

\begin{figure} 
    \centering
    \includegraphics[width=10cm]{Figures/Cjj'.jpg}
    \caption{$\dist{i}{j'}  \leq \dist{i}{j} + 2\ellone \C{j}$}
    \label{Cjj'}
\end{figure}

%$\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$ ~\cite{GroverGKP18}.}  

For $j' \in \clientset', j \in \clientset$, let $\loadjinc{j}{j'}$ be the extent up to which $j$ is served by the facilities in the cluster of $j'$  \textcolor{olive}{under solution $\zeta^*$} and $d_{j'}= \sum_{j \in \clientset} \loadjinc{j}{j'}$.
We call a cluster to be $sparse$ if $d_{j'} \le  \capacityU$ and $dense$ otherwise. Let $\csparse$ and $\cdense$ be the set of cluster centers of sparse  and dense clusters respectively.


%Let $<\hat{x}, \hat{y}>$ be the solution so obtained, i.e., for $ j \in \clientset$, $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$. For $j' \in \crich, i \in \bundle{j'}, j \in \clientset$, $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. 


\begin{lemma} \label{Sparse}
We can obtain a solution $<\hat{x}, \hat{y}>$ such that  exactly one facility $i(j')$ is opened integrally in each sparse cluster centered at $j' \in \clientset'$. The solution violates the lower bound by a factor of \textcolor{yellow}{$(1 - 1/\ellone)$} \textcolor{cyan}{1/2} \textcolor{olive}{such that $\sum_{j' \in \clientset'}\sum_{i \in \bundle{j'}} [f_i \hat{y}_i + \sum_{j \in \clientset}  \hat{x}_{ij} \dist{i}{j}] \leq $}
$\sum_{j' \in \csparse}[\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \textcolor{yellow}{\ellone } \textcolor{cyan}{2}\C{j})] + \sum_{j' \in \cdense} [\sum_{i \in \bundle{j'}} f_i y^*_i + \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$.

%\textcolor{red}{May be we should write the following:$\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \le \sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})]$...will resolve after completing this section}

\end{lemma}

\begin{proof}
%In a sparse cluster centered at $j'$, we open the cheapest facility, say $i(j')$, in $\ballofj{j'}$ and transfer all the assignments in the cluster onto it.
%As specified above, 
For $ j' \in \cdense, i \in \bundle{j'}, j \in \clientset$, set $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. Next,
let $j' \in \csparse$
%$\bundle{j'}$ be a sparse cluster centered at $j'$ 
and $i(j')$ be a cheapest \textcolor{olive}{(lowest facility opening cost)} facility in $\ballofj{j'}$. We open $i(j')$ and transfer all the assignments in the cluster onto it (see Figure (\ref{sparse})). 
%Let $ j \in \clientset$.
i.e. set $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$ and $j \in \clientset$. 
Since $\cardTwo{\ballofj{j'}} \ge \textcolor{yellow}{(1-\frac{1}{\ellone})} \textcolor{cyan}{1/2}$ we have $\sum_{j \in \clientset}{} \hat{x}_{i(j')j} = \demandofj{j'} \ge \textcolor{yellow}{(1-\frac{1}{\ellone})} \textcolor{cyan}{1/2}\B$. Thus, the lower bound is violated at most by $\textcolor{yellow}{(1-\frac{1}{\ellone})} \textcolor{cyan}{1/2}$
and the facility cost is bounded by $\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i y^*_i$.

To bound the service cost, we will show that for $j' \in \csparse, \sum_{j \in \clientset} \loadjinc{j}{j'} \dist{i(j')}{j}  \leq 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})$: 
since $i(j') \in \ballofj{j'}$, we have $\dist{i(j')}{j'} \le  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j'}$. 
Thus, for $j \in \clientset$,
we have $\dist{i(j')}{j} \le \dist{j'}{j} + \dist{i(j')}{j'} \le  \dist{j'}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j'}$. If $ \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j'} \le \dist{j'}{j}$ then $\dist{i(j')}{j}  \le 2  \dist{j'}{j}  \leq 4 (\dist{i}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})$ ($\forall~i \in \bundle{j'}$ by claim (\ref{claim-2}) of Lemma (\ref{distBound})), 
 else $\dist{i(j')}{j}  \leq  \textcolor{yellow}{2\ellone} \textcolor{cyan}{4} \C{j'} \leq  \textcolor{yellow}{4 \ellone} \textcolor{cyan}{8} \C{j}$, where the second inequality in the else part follows by claim (\ref{claim-3}) of Lemma (\ref{distBound}).
Thus, in either case $\dist{i(j')}{j} \leq 4 (\dist{i}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})$ for all $i \in \bundle{j'}$.
Substituting $\phi(j, j') = \sum_{i \in \bundle{j'}} x^*_{ij}$ and summing over all $j \in \clientset$ 
%$j' \in \csparse$ 
we get the desired bound.
Thus, $\sum_{i \in \facilityset} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  \hat{x}_{ij}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \demandofj{j'}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
\le \sum_{j' \in \csparse}[\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} +  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})] + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} [ f_i y^*_i + \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$
\end{proof}
 
%$\le 4\dist{i}{j} + 4 \ellone \C{j} $ else $\dist{i(j')}{j}  \le  2 \ellone \C{j'} \le 4 \ellone \C{j} \le 4\dist{i}{j} + 4 \ellone \C{j}$, where the second inequality in the else part follows because if $\ellone \C{j'} > \dist{j'}{j}$ then $\C{j'} \leq 2\C{j}$ \cite{GroverGKP18}. Also, since the total opening in each cluster is at least $(1-(1/\ellone))$, a loss of factor $\ellone/(\ellone-1) (\leq 2$ for $\ellone > 2$) in the facility opening cost is incurred, violation in lower bound is at most $(1-(1/\ellone))$ and  since  $d_{j'} \le \capacityU$ there is no  violation in the capacity.}
   
    \begin{figure} 
    \centering
    \includegraphics[width=10cm]{Figures/sparse.jpg}
    \caption{(A) Cluster $\bundle{j'}$ centered at $j'$. (B) Demand $\demandofj{j'}$ being assigned to facility $i(j') \in \ballofj{j'}$.}
    \label{sparse}
\end{figure}
 

    
%Next, we consider the dense clusters.
To open the facilities integrally in the dense clusters, we solve the following LP for every dense cluster $\bundle{j'}$.
%centered at $j'$.

($LP_1$): 
\label{dense}
$Minimize ~\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$
\begin{eqnarray}
subject~ to &\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'} \label{denseLP_const1}\\
&\textcolor{cyan}{\B \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \leq \demandofj{j'} \label{denseLP_const1-1}}\\ 
&0 \leq \zofi{i} \leq 1 \label{denseLP_const2}
\end{eqnarray}
   
  % $Minimize $\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$ s.t. $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$ and $\zofi{i} \in [0,1]$. 
   
   
Note that for $\zofi{i} = \sum_{j \in \clientset}x_{ij}^*/\capacityU$, we have $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} = \demandofj{j'} \geq \textcolor{cyan}{\B \sum_{\singlefacility \in \bundle{j'}} \zofi{i}}$ and $\zofi{i} \le y^*_i$. Thus, $\zofi{}$
is a feasible solution with cost at most $ \sum_{i \in \bundle{j'}} [\facilitycost y^*_i + \sum_{ j \in \clientset} x^*_{ij} ( \dist{i}{j} +   \textcolor{yellow}{2\ellone} \textcolor{cyan}{4} \C{j}) ]$ by claim (\ref{claim-1}) of Lemma (\ref{distBound}).

%\textcolor{blue}{TBD: facility opening cost at most $ \sum_{i \in \bundle{j'}} \facilitycost y^*_i$ and service cost $\sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij}  \dist{i}{j'} \le \sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij} [ \dist{i}{ j} + 2\ellone \C{j} ]$. } 

\begin{lemma} \label{integral_dense}
Given the feasible solution $z$ to $LP_1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) \textcolor{cyan}{and (\ref{denseLP_const1-1})} by a factor of \textcolor{yellow}{$(1+1/\ell)$} \textcolor{cyan}{$3/2$ and $1/2$ respectively}, can be obtained at a loss of factor $\textcolor{yellow}{\ellone} \textcolor{cyan}{2}$ in cost
i.e. $ \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \hat{z}_{i} \le  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$.
%For a fixed $0 < \epsilon < 1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) by a factor of $(1+\epsilon)$, can be obtained at a loss of $(1/\epsilon)$ in cost.
\end{lemma}

\begin{proof}
\textcolor{green}{
We say that a solution to $LP_1$ is almost integral if it has at most one fractionally opened facility in $\bundle{j'}$.
}
We first obtain an almost integral solution
%\footnote{A solution is said to be an almost integral solution if it has at most one fractionally opened facility.}
$\primezofi{}$ by arranging the facilities opened in $z$, in non-decreasing order of $\facilitycost  + \dist{i}{j'} \capacityU$ and greedily transferring the openings $z$ onto them. 
Then,  $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} = \demandofj{j'}$. %Consider constraint (\ref{denseLP_const1}), $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$.
Note that the cost of solution $\primezofi{}$ is no more than that of solution $z$.


We now convert the almost integral solution $\primezofi{}$ to an integral solution $\hat{z}$. Let $\hat{z} = \primezofi{}$ initially. Let $i'$ be the fractionally opened facility, if any, in $\bundle{j'}$. %Initially, set $\hat{z}_i = \primezofi{i}~ \forall i \in \bundle{j'}$. 
Consider the following cases:


\begin{enumerate}
    %\item $\primezofi{i'} < \epsilon$:
    \item $\primezofi{i'} < \textcolor{yellow}{1/\ell} \textcolor{cyan}{1/2}$: close $i'$ in $\hat{z}$. There must be at least one integrally opened facility, say $i (\ne i') \in \bundle{j'}$ in $\primezofi{}$, as $\demandofj{j'} \ge \capacityU$. Then, $\demandofj{j'} = \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k} + \capacityU  (\primezofi{i} + \primezofi{i'}) \le \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k}  + \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU  \primezofi{i} \le \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU \sum_{k \in \bundle{j'} \setminus \{i'\}} \primezofi{k} = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}  \capacityU \sum_{k \in \bundle{j'}} \hat{z}_k$. There is no increase in cost as we have only (possibly) shut down one of the facilities .
    

    \item $\primezofi{i'} \geq \textcolor{yellow}{1/\ell} \textcolor{cyan}{1/2} $: Open $i'$ integrally at a loss of factor $\textcolor{yellow}{\ell}$ \textcolor{cyan}{2} in facility opening cost i.e., $\sum_{i \in \bundle{j'}} f_i \hat{z}_i \le \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i \primezofi{i}$. 
    %\textcolor{cyan}{Also, note that $\capacityU \hat{z}_i \geq 1/2 \B \primezofi{i'}$ ------ CHECK AGAIN.} 
\end{enumerate}\end{proof}

%Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{(1+1/\ell)\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = (1 + 1/\ell) \capacityU \hat{z}_i$ , where the first inequality follows by Lemma (\ref{integral_dense}). 


%\textcolor{cyan}{SAPNA, Revisit the next para later:}

Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{\textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU \hat{z}_i$ , where the first inequality follows by Lemma (\ref{integral_dense}). \textcolor{cyan}{Also, $l_i  = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \geq \hat{z}_i \frac{\demandofj{j'}}{2\sum_{i \in \bundle{j'}} z'_i} = \hat{z}_i \frac{\demandofj{j'}}{2\sum_{i \in \bundle{j'}} z_i} =  \hat{z}_i \frac{\B \sum_{i \in \bundle{j'}} z_i}{2\sum_{i \in \bundle{j'}} z_i} = 1/2 B \hat{z}_i$, where the first inequality follows because $\sum_{i \in \bundle{j'}} \hat{z}_i \leq 2\sum_{i \in \bundle{j'}} z'_i$.}


\textcolor{olive}{A solution is said to be an integrally opened solution if all facilities in it are either opened to an extent of $1$ or $0$. We next obtain such a solution to LBUBFL problem.}


\begin{lemma} \label{Dense1}
We can obtain an integrally opened solution $<\bar x, \bar y>$ to LBUBFL problem at a loss of $\textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}$ in upper bounds and $\textcolor{yellow}{(1-1/\ell)} \textcolor{cyan}{(1/2)}$ in lower bounds whose cost is bounded by $\textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)} \textcolor{cyan}{O(1)LP_{opt}}$.
\end{lemma}
\begin{proof}
For $j' \in \csparse$, set $\bar y_i = \hat{y}_i,~\bar{x}_{ij} = \hat{x}_{ij}~\forall i \in \bundle{j'}, j \in \clientset$. \textcolor{yellow}{The violation in lower bound then follows from Lemma (\ref{Sparse})
and, }

\begin{equation}
\label{cost-of-sparse}
\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \bar{y}_i + \sum_{j \in \clientset} \bar{x}_{ij} \dist{i}{j}) \le \sum_{j' \in \csparse}[\textcolor{yellow}{\frac{\ellone}{\ellone - 1}} \textcolor{cyan}{2}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \C{j})].
\end{equation}

Next let $j' \in \cdense,~i \in \bundle{j'}, j \in \clientset$. Set $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. 
Consider $ \sum_{j \in \clientset} \bar{x}_{ij} = \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} = l_i \leq   \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \hat{z}_i = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \bar{y}_i$. Thus, the loss in capacities is at most   \textcolor{yellow}{(1+1/\ell)}\textcolor{cyan}{(3/2)}.

\textcolor{cyan}{From Lemma (\ref{Sparse}) and the way $\demandofj{j'}$ is distributed for each dense clusters $j'$, the violation in lower bound is $1/2$. Thus, $\alpha > 1/2$.}

Also,\\ 
$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij}) $\\
$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \dist{i}{j}  \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} (\dist{j}{j'} + \dist{i}{j'})$ (by triangle inequality)\\ 
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   
%\sum_{\singlefacility \in \bundle{j'}} 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ (as $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
%$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )  $ (by definition of $\loadjinc{j}{j'}$, claim (\ref{claim-2}) of Lemma (\ref{distBound}) and the fact that $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
$ \leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +    \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{3/2} \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +  
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ (by Lemma (\ref{integral_dense}))\\
%$ \leq  \ell \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +   (1+1/\ell) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
\textcolor{yellow}{$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\}
%$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\ \textcolor{yellow}{(for $\ell > 2$)}\\
%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\ (for $\ell > 2$)\\
$\leq \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (by Lemma (\ref{integral_dense}))\\
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (because $z_i = \sum_{j \in \clientset} x^*_{ij} / \capacityU \leq y^*_i$)\\ 
%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by cost bound of feasible solution $z$.....Sapna..how from this reason?)\\
%\textcolor{red}{
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ellone \C{j}) + \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$  (by claim (\ref{claim-1}) of Lemma (\ref{distBound}))\\
%}
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} +  \textcolor{yellow}{2\ell} \textcolor{cyan}{4} \C{j}) + \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}  (2\dist{i}{j} +  \textcolor{yellow}{2\ell} \textcolor{cyan}{4} \C{j} )$ 
(by definition of $\loadjinc{j}{j'}$ and claims (\ref{claim-1}) and (\ref{claim-2}) of Lemma (\ref{distBound}))\\
$= \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   \textcolor{yellow}{2+\ell} \textcolor{cyan}{4}   \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} +   \textcolor{yellow}{2\ell(1+\ell)} \textcolor{cyan}{12} \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}   \C{j} $ \\

Summing over all $j' \in \cdense$ and adding inequality (\ref{cost-of-sparse}), we get\\
$ \sum_{i \in \facilityset} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij})$\\
$\leq \textcolor{yellow}{max\{\ell, \ell/(\ell-1)\}} \textcolor{cyan}{2} \sum_{i \in \facilityset}  f_i y^*_i + \textcolor{yellow}{ max\{4,(2+\ell)\}} \textcolor{cyan}{4} \sum_{i \in \facilityset}\sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + \textcolor{yellow}{\ellone~ max\{4,2(1+\ell)\}} \textcolor{cyan}{12} \sum_{i \in \facilityset}\sum_{j \in \clientset} x^*_{ij} \C{j}$\\
 \textcolor{yellow}{ $= \sum_{i \in \facilityset}  f_i y^*_i + (2+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + 2\ell(1+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\ell > 2$)}\\
$ \leq \textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)} \textcolor{cyan}{16}LP_{opt}$.
\end{proof}


Theorem~\ref{TricriteriaResult} is obtained by solving a min-cost flow problem with relaxed lower  and upper bounds to obtain the integral assignments.
Let $S^t$ be the solution so obtained. %and violations in lower and upper bounds be denoted by $\alpha$ and $\beta$ respectively.
Then, $Cost_I(S^t) \le \textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)}\textcolor{cyan}{16} Cost_I(O)$,
where $O$ is an optimal solution to $I$, $\textcolor{yellow}{\alpha= (1 - 1/\ellone)} \textcolor{cyan}{\alpha >
1/2}$ and $\textcolor{yellow}{\beta= (1 + 1/\ellone)} \textcolor{cyan}{\beta= 3/2}$.
\textcolor{yellow}{ For $\ell = 2.01$, $\alpha > 1/2$, $\beta < 3/2$ and the approximation ratio is less than $17$. The violations in the lower and the upper bounds can be made arbitrarily close to $0$ at the cost of increase in the approximation ratio.}

%To obtain integral assignments, we solve a minimum-cost integer flow problem with relaxed lower  and upper bounds.



	Next, using $S^t$, we transform the instance $I$ to an instance $I_{cap}$ of capacitated facility location problem by swapping the roles of clients and facilities. This is done via a series of transformations from instance $I$ to $I_1$, 	$I_1$ to $I_2$ and $I_2$ to $I_{cap}$. The key idea is to create  $\B - n_i$ units of demand, where the number $n_i$ of clients served by facility $i$ in $S^t$ is short of the lower bound and create  $n_i - \B$ units of supply at locations where $n_i > \B$.
	
	


==> TriCriteria_l_1By2.tex <==
\section{Computing the Tri-criteria Solution}
\label{tri-criteria}
 %We use a simpler LP-rounding technique to get $(\frac{\ellone-1}{\ellone})$-factor violation in lower bounds and $2$-factor violation in upper bounds at constant factor loss in cost. The technique used is much simpler than Friggstad et al. \cite{friggstad_et_al_LBUFL} because lower bounds are uniform in our case unlike Friggstad et al. that considers non-uniform lower bounds. 

 In this section, we give a tri-criteria solution that violates the lower bound by a factor of \textcolor{yellow}{$\alpha = (1 - \frac{1}{\ell})$} \textcolor{cyan}{$\alpha > 1/2$} and the upper bound by a factor of \textcolor{cyan}{$\beta = 3/2$.} \textcolor{yellow}{$\beta = (1 + \frac{1}{\ell})$ where $\ell > 2$ is a tune-able parameter.} In particular, we present the following result:
 
 

 \begin{theorem} \label{TricriteriaResult}
 A \textcolor{yellow}{$( 2\ell^2+ 3\ell+2 ,  (1 - \frac{1}{\ell}) ,  (1 + \frac{1}{\ell}))$} \textcolor{cyan}{$(O(1),1/2,3/2)$} -
 approximate solution can be obtained for LBUBFL in polynomial time. \textcolor{yellow}{, where $\ell > 2$ is a tuneable parameter.}
\end{theorem}
 
 
 Instance $I$ of LBUBFL can be formulated as the following integer program (IP):

\label{{unif-CFLP}}
$Minimize ~\mathcal{C}ostLBUBFL(x,y) = \sum_{j \in \clientset}\sum_{i \in \facilityset}\dist{i}{j}x_{ij} + \sum_{i \in \facilityset}f_iy_i $
\begin{eqnarray}
subject~ to &\sum_{i \in \facilityset}{} x_{ij} \geq 1 & \forall ~\singleclient \in \clientset \label{LPFLP_const1}\\ 
%&\sum_{j \in \clientset}{} x_{ij} \leq \capacityU ~ y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const2}\\ 
& \capacityU y_i \geq \sum_{j \in \clientset}{} x_{ij} \geq \B y_i & \forall~ \singlefacility \in \facilityset \label{LPFLP_const3}\\
& x_{ij} \leq y_i & \forall~ \singlefacility \in \facilityset , ~\singleclient \in \clientset \label{LPFLP_const4}\\   
& y_i,x_{ij} \in \left\lbrace 0,1 \right\rbrace  \label{LPFLP_const5}
\end{eqnarray}
where  $y_i$ is an indicator variable which is equal to $1$ if facility $i$ is open and is $0$ otherwise. $x_{ij}$ is an indicator variable which is equal to $1$ if client $j$ is served by facility $i$ and is $0$ otherwise.
 Constraints \ref{LPFLP_const1} ensure that all the clients are served. %Constraints \ref{LPFLP_const2} make sure that the total demand assigned to an open facility is no more than its capacity \capacityU. 
 Constraints \ref{LPFLP_const3} make sure that the total demand assigned to an open facility is at least $\B$ and at most $\capacityU$. Constraints \ref{LPFLP_const4} ensure that a client is assigned to a facility only if it is opened. LP-Relaxation  is obtained by allowing the variables to be non-integral.
% $ y_i, x_{ij} \in [0, 1]$. %Call it LP. 
Let $\zeta^{*} = <x^*, y^*>$ be an optimal solution  and $\opt{}$ be its cost.

%TBD: In this section, we give a tri-criteria solution that violates the lower bound by a factor of $(\ellone-1)/\ellone$ for a fixed parameter \textcolor{blue}{$\ellone > 2$} and the upper bounds by a factor of $2$.

We start by sparsifying the problem instance by removing some clients.
For $j \in \clientset$, let $ \C{j} $ denote the average connection cost paid by $\singleclient$ in $\zeta^*$. 
%i.e., ~$\C{j} = (\sum_{i \in \facilityset}{} {x}^*_{ij} \dist{i}{j})/({\sum_{i \in \facilityset}{} {x}^*_{ij}})$. 
Further, let $\ell > 2$ be a tuneable parameter, $\ballofj{j}$ be the ball of facilities within a radius of $\ellone\C{j}$ of $j$ and $\cardTwo{\ballofj{j}}$
%$=  \sum_{i \in \ballofj{j}} y^*_i$ 
be the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
%~ i.e., \ \ballofj{j}  = \{ \singlefacility \in \facilityset \colon \dist{i}{j} \leq \ellone \C{j} \}$.
Then,  \textcolor{olive}{$\cardTwo{\ballofj{j}} \ge (1-\frac{1}{\ellone}) > 1/2$.}
%where $\cardTwo{\ballofj{j}}$
%$=  \sum_{i \in \ballofj{j}} y^*_i$ denotes the total extent up to which facilities are opened in \ballofj{j} under solution $\zeta^*$.
The clients are processed in the non-decreasing order of the radii of their balls, removing the close-by clients with balls of larger radii and dissolving their balls: let $\bar{\clientset} = \clientset$ and $\clientset'$ denote the sparsified set of  clients. Initially $\clientset' = \phi$.
Let $j'$ be a client in $\bar{\clientset}$ with a ball of the smallest radius (breaking the ties arbitrarily). Remove $j'$ from $\bar{\clientset}$ and add it to $\clientset'$. For all $j (\ne j') \in \bar{\clientset}$ with $\dist{j'}{ j} \leq 2\ell \C{j}$, remove $j$ from $\bar{\clientset}$. Repeat the process until $\bar{\clientset} = \phi$. 
Cluster of facilities are formed around the clients in $\clientset'$ by assigning a facility to the cluster of $j' \in \clientset'$ if and only if $j'$ is nearest to the facility amongst all $j' \in \clientset'$, i.e. if $\bundle{j'}$ denotes the cluster centered at $j'$ then, $i$ belongs to $\bundle{j'}$ if and only if $\dist{i}{j'} < \dist{i}{k'}$ for all $k' \in \clientset'$ (assuming that the distances are distinct).
The clients in $C'$ are then called the cluster centers.



\begin{observation}
Any two cluster centers $j', k'$ in $C'$ satisfy the  separation property: $\dist{j'}{k'} > 2\ellone~max\{ \C{j'},\C{k'}\}$.
\end{observation}

\begin{lemma} \label{distBound}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. Then,
\begin{enumerate}
    \item \label{claim-1} $\dist{i}{j'}  \leq \dist{i}{j} + 2\ellone \C{j}$
    \item \label{claim-2} $\dist{j}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$
    \item \label{claim-3} If $\dist{j}{j'} \leq \ell \C{j'}$, then $\C{j'} \le 2\C{j}$.
\end{enumerate}
\end{lemma}

\begin{proof}
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. 
\begin{enumerate}

    \item Note that, $\dist{j}{k'} \leq 2\ellone \C{j}$ for some $k' \in \clientset'$. Then we have $\dist{i}{j'} \leq \dist{i}{k'} \leq \dist{i}{j} + \dist{j}{k'} \leq \dist{i}{j} + 2\ellone \C{j}$, where the first inequality follows because $i$ belongs to $\bundle{j'}$ and not $\bundle{k'}$ whenever $k' \ne j'$.  \textcolor{blue}{See Fig: (\ref{Cjj'}).}
    
    
    \item Using triangle inequality, we have $\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$.
     \item Let $j \ne j'$. Note that  $\dist{j}{j'} \leq \ell \C{j'} \Rightarrow j \notin \clientset'$. 
     %Further, using contradiction, let's assume 
     Suppose if possible, $\C{j'} > 2\C{j}$. Since $j \notin \cliset', \exists$ some $k'\in \clientset':\dist{j}{k'} \le 2 \ell \C{j}$. Then, $\dist{k'}{j'} \le \dist{k'}{j} + \dist{j}{j'}$ $ \leq 2 \ell \C{j} + \ell \C{j'} < 2\ell \C{j'}$. Thus, we arrive at a contradiction to the separation property. Hence, $\C{j'} \le 2\C{j}$.
\end{enumerate} \end{proof}
 

\begin{figure} 
    \centering
    \includegraphics[width=10cm]{Figures/Cjj'.jpg}
    \caption{$\dist{i}{j'}  \leq \dist{i}{j} + 2\ellone \C{j}$}
    \label{Cjj'}
\end{figure}

%$\dist{j}{j'} \leq \dist{i}{j} + \dist{i}{j'} \leq 2\dist{i}{j} + 2\ellone \C{j}$ ~\cite{GroverGKP18}.}  

For $j' \in \clientset', j \in \clientset$, let $\loadjinc{j}{j'}$ be the extent up to which $j$ is served by the facilities in the cluster of $j'$  \textcolor{olive}{under solution $\zeta^*$} and $d_{j'}= \sum_{j \in \clientset} \loadjinc{j}{j'}$.
We call a cluster to be $sparse$ if $d_{j'} \le  \capacityU$ and $dense$ otherwise. Let $\csparse$ and $\cdense$ be the set of cluster centers of sparse  and dense clusters respectively.


%Let $<\hat{x}, \hat{y}>$ be the solution so obtained, i.e., for $ j \in \clientset$, $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$. For $j' \in \crich, i \in \bundle{j'}, j \in \clientset$, $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. 


\begin{lemma} \label{Sparse}
We can obtain a solution $<\hat{x}, \hat{y}>$ such that  exactly one facility $i(j')$ is opened integrally in each sparse cluster centered at $j' \in \clientset'$. The solution violates the lower bound by a factor of $(1 - 1/\ellone)$ \textcolor{olive}{such that $\sum_{j' \in \clientset'}\sum_{i \in \bundle{j'}} [f_i \hat{y}_i + \sum_{j \in \clientset}  \hat{x}_{ij} \dist{i}{j}] \leq $}
$\sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})] + \sum_{j' \in \cdense} [\sum_{i \in \bundle{j'}} f_i y^*_i + \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$.

%\textcolor{red}{May be we should write the following:$\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \le \sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})]$...will resolve after completing this section}

\end{lemma}

\begin{proof}
%In a sparse cluster centered at $j'$, we open the cheapest facility, say $i(j')$, in $\ballofj{j'}$ and transfer all the assignments in the cluster onto it.
%As specified above, 
For $ j' \in \cdense, i \in \bundle{j'}, j \in \clientset$, set $\hat{y}_i = y^*_i,  \hat{x}_{ij} = x^*_{ij}$. Next,
let $j' \in \csparse$
%$\bundle{j'}$ be a sparse cluster centered at $j'$ 
and $i(j')$ be a cheapest \textcolor{olive}{(lowest facility opening cost)} facility in $\ballofj{j'}$. We open $i(j')$ and transfer all the assignments in the cluster onto it (see Figure (\ref{sparse})). 
%Let $ j \in \clientset$.
i.e. set $\hat{y}_{i(j')}=1, \hat{x}_{i(j')j} = \sum_{i \in \bundle{j'}}x^*_{ij}$, and $ \hat{y}_i =0$, $\hat{x}_{ij} =0$ for $i \in \bundle{j'} \setminus \{i(j')\}$ and $j \in \clientset$. 
Since $\cardTwo{\ballofj{j'}} \ge (1-\frac{1}{\ellone})$ we have $\sum_{j \in \clientset}{} \hat{x}_{i(j')j} = \demandofj{j'} \ge (1-\frac{1}{\ellone})\B$. Thus, the lower bound is violated at most by $(1-\frac{1}{\ellone})$
and the facility cost is bounded by $\frac{\ellone}{\ellone - 1} \sum_{i \in \bundle{j'}} f_i y^*_i$.

To bound the service cost, we will show that for $j' \in \csparse, \sum_{j \in \clientset} \loadjinc{j}{j'} \dist{i(j')}{j}  \leq 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})$: 
since $i(j') \in \ballofj{j'}$, we have $\dist{i(j')}{j'} \le \ellone \C{j'}$. 
Thus, for $j \in \clientset$,
we have $\dist{i(j')}{j} \le \dist{j'}{j} + \dist{i(j')}{j'} \le  \dist{j'}{j} + \ellone \C{j'}$. If $\ellone \C{j'} \le \dist{j'}{j}$ then $\dist{i(j')}{j}  \le 2  \dist{j'}{j}  \leq 4 (\dist{i}{j} + \ellone \C{j})$ ($\forall~i \in \bundle{j'}$ by claim (\ref{claim-2}) of Lemma (\ref{distBound})), 
 else $\dist{i(j')}{j}  \leq 2 \ell \C{j'} \leq 4 \ellone \C{j}$, where the second inequality in the else part follows by claim (\ref{claim-3}) of Lemma (\ref{distBound}).
Thus, in either case $\dist{i(j')}{j} \leq 4 (\dist{i}{j} + \ellone \C{j})$ for all $i \in \bundle{j'}$.
Substituting $\phi(j, j') = \sum_{i \in \bundle{j'}} x^*_{ij}$ and summing over all $j \in \clientset$ 
%$j' \in \csparse$ 
we get the desired bound.
Thus, $\sum_{i \in \facilityset} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  \hat{x}_{ij}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
%= \sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} f_i \hat{y}_i + \sum_{j' \in \csparse} \demandofj{j'}  \dist{i(j')}{j}  + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} (f_i \hat{y}_i + \sum_{j \in \clientset} \hat{x}_{ij} \dist{i}{j} ) \\
\le \sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})] + \sum_{j' \in \cdense} \sum_{i \in \bundle{j'}} [ f_i y^*_i + \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j}]$
\end{proof}
 
%$\le 4\dist{i}{j} + 4 \ellone \C{j} $ else $\dist{i(j')}{j}  \le  2 \ellone \C{j'} \le 4 \ellone \C{j} \le 4\dist{i}{j} + 4 \ellone \C{j}$, where the second inequality in the else part follows because if $\ellone \C{j'} > \dist{j'}{j}$ then $\C{j'} \leq 2\C{j}$ \cite{GroverGKP18}. Also, since the total opening in each cluster is at least $(1-(1/\ellone))$, a loss of factor $\ellone/(\ellone-1) (\leq 2$ for $\ellone > 2$) in the facility opening cost is incurred, violation in lower bound is at most $(1-(1/\ellone))$ and  since  $d_{j'} \le \capacityU$ there is no  violation in the capacity.}
   
    \begin{figure} 
    \centering
    \includegraphics[width=10cm]{Figures/sparse.jpg}
    \caption{(A) Cluster $\bundle{j'}$ centered at $j'$. (B) Demand $\demandofj{j'}$ being assigned to facility $i(j') \in \ballofj{j'}$.}
    \label{sparse}
\end{figure}
 
To open the facilities integrally in the dense clusters, we solve the following LP for every dense cluster $\bundle{j'}$.
%centered at $j'$.

($LP_1$): 
\label{dense}
$Minimize ~\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$
\begin{eqnarray}
subject~ to &\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'} \label{denseLP_const1}\\
&\textcolor{cyan}{\B \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \leq \demandofj{j'} \label{denseLP_const1-1}}\\ 
&0 \leq \zofi{i} \leq 1 \label{denseLP_const2}
\end{eqnarray}
   
  % $Minimize $\sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$ s.t. $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$ and $\zofi{i} \in [0,1]$. 
   
   
Note that for $\zofi{i} = \sum_{j \in \clientset}x_{ij}^*/\capacityU$, we have $\capacityU \sum_{\singlefacility \in \bundle{j'}} \zofi{i} = \demandofj{j'} \geq \textcolor{cyan}{\B \sum_{\singlefacility \in \bundle{j'}} \zofi{i}}$ and $\zofi{i} \le y^*_i$. Thus, $\zofi{}$
is a feasible solution with cost at most $ \sum_{i \in \bundle{j'}} [\facilitycost y^*_i + \sum_{ j \in \clientset} x^*_{ij} ( \dist{i}{j} +  2\ellone \C{j}) ]$ by claim (\ref{claim-1}) of Lemma (\ref{distBound}).

%\textcolor{blue}{TBD: facility opening cost at most $ \sum_{i \in \bundle{j'}} \facilitycost y^*_i$ and service cost $\sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij}  \dist{i}{j'} \le \sum_{i \in \bundle{j'}} \sum_{ j \in \clientset} x^*_{ij} [ \dist{i}{ j} + 2\ellone \C{j} ]$. } 

\begin{lemma} \label{integral_dense}
Given the feasible solution $z$ to $LP_1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) \textcolor{cyan}{and (\ref{denseLP_const1-1})} by a factor of \textcolor{yellow}{$(1+1/\ell)$} \textcolor{cyan}{$3/2$ and $1/2$ respectively}, can be obtained at a loss of factor $\textcolor{yellow}{\ellone} \textcolor{cyan}{2}$ in cost
i.e. $ \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \hat{z}_{i} \le  \textcolor{yellow}{\ellone} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU \dist{i}{j'}) \zofi{i}$.
%For a fixed $0 < \epsilon < 1$, an integral solution $\hat{z}$, that violates constraint (\ref{denseLP_const1}) by a factor of $(1+\epsilon)$, can be obtained at a loss of $(1/\epsilon)$ in cost.
\end{lemma}

\begin{proof}
\textcolor{green}{
We say that a solution to $LP_1$ is almost integral if it has at most one fractionally opened facility in $\bundle{j'}$.
}
We first obtain an almost integral solution
%\footnote{A solution is said to be an almost integral solution if it has at most one fractionally opened facility.}
$\primezofi{}$ by arranging the facilities opened in $z$, in non-decreasing order of $\facilitycost  + \dist{i}{j'} \capacityU$ and greedily transferring the openings $z$ onto them. 
Then,  $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} = \demandofj{j'}$. %Consider constraint (\ref{denseLP_const1}), $\capacityU \sum_{i \in \bundle{j'}} \primezofi{i} = \capacityU \sum_{i \in \bundle{j'}} \zofi{i} \geq \demandofj{j'}$.
Note that the cost of solution $\primezofi{}$ is no more than that of solution $z$.


We now convert the almost integral solution $\primezofi{}$ to an integral solution $\hat{z}$. Let $\hat{z} = \primezofi{}$ initially. Let $i'$ be the fractionally opened facility, if any, in $\bundle{j'}$. %Initially, set $\hat{z}_i = \primezofi{i}~ \forall i \in \bundle{j'}$. 
Consider the following cases:


\begin{enumerate}
    %\item $\primezofi{i'} < \epsilon$:
    \item $\primezofi{i'} \textcolor{yellow}{ < 1/\ell} \textcolor{cyan}{ \leq 1/2}$: close $i'$ in $\hat{z}$. There must be at least one integrally opened facility, say $i (\ne i') \in \bundle{j'}$ in $\primezofi{}$, as $\demandofj{j'} \ge \capacityU$. Then, $\demandofj{j'} = \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k} + \capacityU  (\primezofi{i} + \primezofi{i'}) \le \capacityU \sum_{k \in \bundle{j'} \setminus \{i, i'\}} \primezofi{k}  + \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU  \primezofi{i} \le \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU \sum_{k \in \bundle{j'} \setminus \{i'\}} \primezofi{k} = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}  \capacityU \sum_{k \in \bundle{j'}} \hat{z}_k$. There is no increase in cost as we have only (possibly) shut down one of the facilities .
    

    \item $\primezofi{i'} \textcolor{yellow}{ \geq 1/\ell} \textcolor{cyan}{> 1/2} $: Open $i'$ integrally at a loss of factor $\textcolor{yellow}{\ell}$ \textcolor{cyan}{2} in facility opening cost i.e., $\sum_{i \in \bundle{j'}} f_i \hat{z}_i \le \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{i \in \bundle{j'}} f_i \primezofi{i}$ \textcolor{cyan}{and $1/2$ factor in lower bound, i.e., $\demandofj{j'} \geq \B \sum_{k \in \bundle{j'}} \primezofi{k} \geq \B/2  \sum_{k \in \bundle{j'}} \hat{z}_{k}$,  where the second inequality follows because $\sum_{i \in \bundle{j'}} \hat{z}_i \leq 2\sum_{i \in \bundle{j'}} z'_i$.}
\end{enumerate}\end{proof}

%Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{(1+1/\ell)\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = (1 + 1/\ell) \capacityU \hat{z}_i$ , where the first inequality follows by Lemma (\ref{integral_dense}). 


%\textcolor{cyan}{SAPNA, Revisit the next para later:}

Next, we define our assignments, possibly fractional, in the dense clusters. For $j' \in \cdense$, we distribute $d_{j'}$ equally to the facilities opened in $ \hat{z}$. Let $l_i$ be the amount assigned to  facility $i$ under this distribution. Then, $l_i = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \leq \hat{z}_i \frac{\textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \sum_{i \in \bundle{j'}} \hat{z}_i}{\sum_{i \in \bundle{j'}} \hat{z}_i } = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)} \capacityU \hat{z}_i$ , where the first inequality follows by Lemma (\ref{integral_dense}). \textcolor{cyan}{Also, $l_i  = \hat{z}_i \frac{\demandofj{j'}}{\sum_{i \in \bundle{j'}} \hat{z}_i} \geq \hat{z}_i \frac{\demandofj{j'}}{2\sum_{i \in \bundle{j'}} z'_i} = \hat{z}_i \frac{\demandofj{j'}}{2\sum_{i \in \bundle{j'}} z_i} =  \hat{z}_i \frac{\B \sum_{i \in \bundle{j'}} z_i}{2\sum_{i \in \bundle{j'}} z_i} = 1/2 B \hat{z}_i$, where the first inequality follows because $\sum_{i \in \bundle{j'}} \hat{z}_i \leq 2\sum_{i \in \bundle{j'}} z'_i$.}


    

\textcolor{olive}{A solution is said to be an integrally opened solution if all facilities in it are either opened to an extent of $1$ or $0$. We next obtain such a solution to LBUBFL problem.}



\begin{lemma} \label{Dense1}
We can obtain an integrally opened solution $<\bar x, \bar y>$ to LBUBFL problem at a loss of \textcolor{yellow}{($1+1/\ell$)} \textcolor{cyan}{$3/2$} in upper bounds and \textcolor{yellow}{$(1-1/\ell)$} \textcolor{cyan}{$1/2$}  in lower bounds whose cost is bounded by $(10\ellone + 4)LP_{opt}$.
\end{lemma}

\begin{proof}
For $j' \in \csparse$, set $\bar y_i = \hat{y}_i,~\bar{x}_{ij} = \hat{x}_{ij}~\forall i \in \bundle{j'}, j \in \clientset$. \textcolor{yellow}{The violation in lower bound then follows from Lemma (\ref{Sparse})
and, }

\begin{equation}
\label{cost-of-sparse}
\sum_{j' \in \csparse} \sum_{i \in \bundle{j'}} (f_i \bar{y}_i + \sum_{j \in \clientset} \bar{x}_{ij} \dist{i}{j}) \le \sum_{j' \in \csparse}[\frac{\ellone}{\ellone - 1}\sum_{i \in \bundle{j'}} f_i y^*_i + 4 \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{j} + \ellone \C{j})].
\end{equation}



Next let $j' \in \cdense,~i \in \bundle{j'}, j \in \clientset$. Set $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. 
Consider $ \sum_{j \in \clientset} \bar{x}_{ij} = \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} = l_i \leq   \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \hat{z}_i = \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{(3/2)}\capacityU \bar{y}_i$. Thus, the loss in capacities is at most   \textcolor{yellow}{(1+1/\ell)}\textcolor{cyan}{(3/2).}

\textcolor{cyan}{From Lemma (\ref{Sparse}) and (\ref{integral_dense}), the violation in lower bound is $min\{1-1\ell,1/2\} > 1/2$ for $\ell>2$. Thus, $\alpha > 1/2$.}



Also,\\ 
$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij}) $\\
$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \dist{i}{j}  \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} (\dist{j}{j'} + \dist{i}{j'})$ (by triangle inequality)\\ 
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   
%\sum_{\singlefacility \in \bundle{j'}} 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ (as $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
%$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )  $ (by definition of $\loadjinc{j}{j'}$, claim (\ref{claim-2}) of Lemma (\ref{distBound}) and the fact that $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
$ \leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +    \textcolor{yellow}{(1+1/\ell)} \textcolor{cyan}{3/2} \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +  
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'} $ (by Lemma (\ref{integral_dense}))\\
%$ \leq  \ell \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +   (1+1/\ell) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
\textcolor{yellow}{$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + 
\sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\}
%$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ \\ \textcolor{yellow}{(for $\ell > 2$)}\\
%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\ (for $\ell > 2$)\\
$\leq \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (by Lemma (\ref{integral_dense}))\\
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \loadjinc{j}{j'} \dist{j}{j'}$ (because $z_i = \sum_{j \in \clientset} x^*_{ij} / \capacityU \leq y^*_i$)\\ 
%$\leq \ell \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by cost bound of feasible solution $z$.....Sapna..how from this reason?)\\
%\textcolor{red}{
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ellone \C{j}) + \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$  (by claim (\ref{claim-1}) of Lemma (\ref{distBound}))\\
%}
$\leq  \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \textcolor{yellow}{\ell} \textcolor{cyan}{2} \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ell \C{j}) + \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}  (2\dist{i}{j} + 2\ell\C{j} )$ 
(by definition of $\loadjinc{j}{j'}$ and claims (\ref{claim-1}) and (\ref{claim-2}) of Lemma (\ref{distBound}))\\
$= \textcolor{yellow}{\ell} \textcolor{cyan}{2}  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   \textcolor{yellow}{2+\ell} \textcolor{cyan}{4}   \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} +   \textcolor{yellow}{2\ell(1+\ell)} \textcolor{cyan}{6\ell} \sum_{j \in \clientset}  \sum_{i \in \bundle{j'}} x^*_{ij}   \C{j} $ \\

Summing over all $j' \in \cdense$ and adding inequality (\ref{cost-of-sparse}), we get\\
$ \sum_{i \in \facilityset} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij})$\\
$\leq max\{2, \ell/(\ell-1)\} \sum_{i \in \facilityset}  f_i y^*_i + \textcolor{yellow}{ max\{4,(2+\ell)\}} \textcolor{cyan}{4} \sum_{i \in \facilityset}\sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + \textcolor{yellow}{\ellone~ max\{4,2(1+\ell)\}} \textcolor{cyan}{10 \ell} \sum_{i \in \facilityset}\sum_{j \in \clientset} x^*_{ij} \C{j}$\\
 \textcolor{yellow}{ $= \sum_{i \in \facilityset}  f_i y^*_i + (2+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + 2\ell(1+\ell)\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\ell > 2$)}\\
  \textcolor{cyan}{$ \leq 2 \sum_{i \in \facilityset}  f_i y^*_i + 4\sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + 10\ell \sum_{i \in \facilityset}  \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\ell > 2$)}\\
$ \leq \textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)}
\textcolor{cyan}{(10 \ell+4)}LP_{opt}$.
\end{proof}


Theorem~\ref{TricriteriaResult} is obtained by solving a min-cost flow problem with relaxed lower  and upper bounds to obtain the integral assignments.
Let $S^t$ be the solution so obtained. %and violations in lower and upper bounds be denoted by $\alpha$ and $\beta$ respectively.
Then, $Cost_I(S^t) \le \textcolor{yellow}{(2\ellone^2 + 3\ellone + 2)} \textcolor{cyan}{(10\ell+4)}Cost_I(O)$,
where $O$ is an optimal solution to $I$, $\textcolor{yellow}{\alpha= (1 - 1/\ellone)} \textcolor{cyan}{\alpha >
1/2}$ and $\textcolor{yellow}{\beta= (1 + 1/\ellone)} \textcolor{cyan}{\beta= 3/2}$. \textcolor{cyan}{ Fix $\ell = 2.01$, we get an approximation ratio of less than $16.5$.}
\textcolor{yellow}{ For $\ell = 2.01$, $\alpha > 1/2$, $\beta < 3/2$ and the approximation ratio is less than $17$. The violations in the lower and the upper bounds can be made arbitrarily close to $0$ at the cost of increase in the approximation ratio.}

%To obtain integral assignments, we solve a minimum-cost integer flow problem with relaxed lower  and upper bounds.



	Next, using $S^t$, we transform the instance $I$ to an instance $I_{cap}$ of capacitated facility location problem by swapping the roles of clients and facilities. This is done via a series of transformations from instance $I$ to $I_1$, 	$I_1$ to $I_2$ and $I_2$ to $I_{cap}$. The key idea is to create  $\B - n_i$ units of demand, where the number $n_i$ of clients served by facility $i$ in $S^t$ is short of the lower bound and create  $n_i - \B$ units of supply at locations where $n_i > \B$.
	


==> temp.tex <==
\begin{comment}
\textcolor{blue}{
\begin{proof}
Let $i \in \bundle{j'}, j \in \clientset$. Recall that $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. Consider the cost of the solution:\\ 
$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij}) $\\
$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \dist{i}{j}  \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} (\dist{j}{j'} + \dist{i}{j'})$ (by triangle inequality)\\ 
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ell \C{j} + \dist{i}{j'})  $ (by definition of $\loadjinc{j}{j'}$)\\ 
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  2 \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \C{j} +$\\
$\sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \dist{i}{j'} $\\
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  2  \sum_{j \in \clientset} \sum_{i' \in \bundle{j'}} x^*_{i'j}   \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \C{j} + \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} $ (because $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i + \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j} $\\
$ \leq  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +  (1+\epsilon) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j} \primezofi{i} +  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j}$ (by Lemma (\ref{integral_dense}))\\
$\leq max\{(1/\epsilon), (1+\epsilon)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} ++  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j}$\\
$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j}$ (for $\epsilon< 1/2$)\\
$= (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j}$ (by Lemma (\ref{integral_dense}))\\
$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   (1/\epsilon)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} +  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j}$ (by cost bound of feasible solution $z$)\\
$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   (1/\epsilon)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ell \C{j}) +  2  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  \dist{i'}{j} + 2\ell   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j} \C{j}$\\
$= (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+ (1/\epsilon))  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} + 2\ell(1+1/\epsilon) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} $ \\
%$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i + \dist{i}{j'} \sum_{j \in \clientset} \bar{x}_{ij}) $\\
%$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
%$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} l_i$\\ 
%$ \leq  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +  (1+\epsilon) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j'} \primezofi{i}$\\
%$\leq max\{(1/\epsilon), (1+\epsilon)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i}$\\
%$= (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i}$ for $\epsilon< 1/2$\\
%$ =  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} (f_i +\capacityU  \dist{i}{j'}) z_i$\\
%$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +   (1/\epsilon)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij}$\\
%$\leq (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} x^*_{ij} [ \dist{i}{ j} + 2\ell \C{j} ]$.
\end{proof}
}
	\end{comment}
	
	
	\begin{lemma}
TBD: We can obtain an integrally opened solution $<\tilde x, \tilde y>$ to LBUBFL problem such that the sum of facility opening costs and the cost of assignment to the opened facilities is bounded by $(2\ellone^2 + 3\ellone + 2)LP_{opt}$. The solution violates the lower bound by a factor of $(1 - 1/\ellone)$  and upper bound by a factor of $(1 + 1/\ellone)$.
\end{lemma}
\begin{proof}
%For a sparse cluster $\bundle{j'}$ centered at $j'$, set $\tilde y_i=\hat{y}_i$ and $\tilde x_{ij} = \hat{x}_{ij}~\forall i \in \bundle{j'}, j \in \clientset$. If  $\bundle{j'}$ is a dense cluster centered at $j'$, then 
Let $j' \in \clientset',~i \in \bundle{j'},~j \in \clientset$. Set $\tilde y_i=\bar{y}_i$ and $\tilde x_{ij} = \bar{x}_{ij}$. The violation in lower and upper bound follows from Lemma (\ref{Sparse}) and  Lemma (\ref{Dense}) respectively.
Summing the cost bound of Lemma (\ref{Sparse}) over all sparse clusters and that of Lemma (\ref{Dense}) over all dense clusters, the total cost of the tri-criteria solution is:\\
%\textcolor{magenta}{Summing the cost bound of Lemma (\ref{Sparse}) over all sparse clusters and that of Lemma (\ref{Dense}) over all dense clusters, the total cost of the tri-criteria solution is: SApna...will have to see the language...I have already summed in Lemma  2.3 I guess...should have the same format in Lemma 2.7 ..and make change in the language here accordingly....will see tomorrow}
$\leq max\{\ell, \ell/(\ell-1)\} \sum_{j' \in \clientset'} \sum_{i \in \bundle{j'}} f_i y^*_i +  max\{4,(2+\ell)\} \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} + \ellone~ max\{4,2(1+\ell)\} \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \C{j}$\\
$= (\ell) \sum_{j' \in \clientset'} \sum_{i \in \bundle{j'}} f_i y^*_i +  (2+\ell) \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{j} $\\
$+ 2\ell(1+\ell) \sum_{j' \in \clientset'}  \sum_{i \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \C{j}$ (for $\ell \geq 2$)\\
$ \leq (2\ellone^2 + 3\ellone + 2)LP_{opt}$.

%\textcolor{green}{ $ \le (2\ellone^2 + 3\ellone + 2)LP_{opt}$ ...Sapna..verify this..is it ok?}

%TBD: Choose $\ellone = \floor{1/\epsilon}$, then the cost of the solution is bounded by $(2\ellone ^2 + 3\ellone + 2)LP_{opt}$. For $\epsilon \le 1/2, \ellone \ge 2$. 
\end{proof}


\begin{lemma} \label{Dense}
We can obtain an integrally opened solution $<\bar x, \bar y>$ at a loss of ($1+1/\ell$) in upper bounds and ($1-1/\ell$) in lower bounds, such that the sum of facility opening costs and the cost of assignment to the opened facilities in dense clusters is bounded by\\
 $ \sum_{j' \in \cdense} \left[ \ellone \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+ \ellone)  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} + 2\ellone (1 + \ellone) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} \right]$ and that in sparse clusters is bounded from Lemma (\ref{Sparse}).
%For a fixed $0<\epsilon< 1/2$, the cost of the solution $<\bar x, \bar y>$ corresponding to a dense cluster centered at $j'$ is bounded by $ (1/\epsilon) \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+ (1/\epsilon))  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} + 2\ellone(1+1/\epsilon) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} $.
\end{lemma}

\begin{proof}
Let $\bundle{j'}$ is a sparse cluster centered at $j'$, then set $\bar y_i = \hat{y}_i,~\bar{x}_{ij} = \hat{x}_{ij}~\forall i \in \bundle{j'}, j \in \clientset$. The violation in lower bound and cost bound for sparse clusters then follows directly from Lemma (\ref{Sparse}). %Next, let $\bundle{j'}$ be dense cluster centered at $j'$.  
Let $j' \in \cdense,~i \in \bundle{j'}, j \in \clientset$. Set $\bar y_i = \hat{z}_i,~\bar{x}_{ij} = \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$. 
Consider $ \sum_{j \in \clientset} \bar{x}_{ij} = \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} = l_i \leq (1+1/\ell)\capacityU =  (1+1/\ell)\capacityU \hat{z}_i = (1+1/\ell)\capacityU \bar{y}_i$. Thus, the loss in capacities is at most ($1+1/\ell$).
Consider the cost of the solution:\\ 
$\sum_{\singlefacility \in \bundle{j'}} (f_i \bar{y}_i +  \sum_{j \in \clientset} \dist{i}{j} \bar{x}_{ij}) $\\
$= \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \dist{i}{j}  \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'}$\\
$ \leq \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset} \frac{l_i}{\demandofj{j'}} \loadjinc{j}{j'} (\dist{j}{j'} + \dist{i}{j'})$ (by triangle inequality)\\ 
\textcolor{red}{
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'}) $ (as $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
}
$ = \sum_{\singlefacility \in \bundle{j'}} f_i \hat{z}_i +  \sum_{\singlefacility \in \bundle{j'}}  l_i \dist{i}{j'} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )  $ (by definition of $\loadjinc{j}{j'}$, claim (\ref{claim-2}) of Lemma (\ref{distBound}) and the fact that $ \sum_{\singlefacility \in \bundle{j'}} l_i = \sum_{j \in \clientset} \loadjinc{j}{j'}  = \demandofj{j'}$)\\
\textcolor{red}{$ \leq  \ell \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +   (1+1/\ell) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j} \primezofi{i} +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'}) $ (by Lemma (\ref{integral_dense}))\\}
$ \leq  \ell \sum_{\singlefacility \in \bundle{j'}} f_i \primezofi{i} +   (1+1/\ell) \capacityU \sum_{\singlefacility \in \bundle{j'}} \dist{i}{j} \primezofi{i} +   \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
\textcolor{red}{
$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$ \\
}
$\leq max\{\ell, (1+1/\ell)\} \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\
\textcolor{red}{
$\leq \ell \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +   \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$ \\ (for $\ell \geq 2$)\\
}
$\leq \ell \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} )\primezofi{i} +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \\ (for $\ell \geq 2$)\\
\textcolor{red}{
$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$ (by Lemma (\ref{integral_dense}))\\
}
$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} (f_i  +  \capacityU \dist{i}{j'} ) z_i +  \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by Lemma (\ref{integral_dense}))\\
\textcolor{red}{
$\leq \ell \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$ \\
}
$\leq \ell \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell  \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset} \dist{i}{j'} x^*_{ij} + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ (by cost bound of feasible solution $z$.....Sapna..how from this reason?)\\
%\textcolor{red}{
%$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ellone \C{j}) + \sum_{\singlefacility \in \bundle{j'}}  \sum_{j \in \clientset}  \loadjinc{j}{j'} (\dist{j}{j'})$  (by claim (\ref{claim-1}) of Lemma (\ref{distBound}))\\
%}
$\leq \ell  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  \ell \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} (\dist{i}{ j} + 2\ellone \C{j}) + \sum_{j \in \clientset}  \sum_{i' \in \bundle{j'}} x^*_{i'j}  (2\dist{i'}{j} + 2\ellone \C{j} )$ \textcolor{red}{ 
(by definition of $\loadjinc{j}{j'}$ and claims (\ref{claim-1}) and (\ref{claim-2}) of Lemma (\ref{distBound}))
}\\
$=\ell  \sum_{\singlefacility \in \bundle{j'}} f_i y^*_i  +  (2+\ell)   \sum_{\singlefacility \in \bundle{j'}} \sum_{j \in \clientset}  x^*_{ij} \dist{i}{ j} +  2\ell(1+\ell) \sum_{j \in \clientset}  \loadjinc{j}{j'}  \C{j} $ \\

\end{proof}

